Direct-Write Digital Holography. Development and research of a hologram printer

Chapter 1 gives a brief history of the field of holography along with an overview of this thesis. A more detailed description of holography is provided in Chapter 2 along with a discussion of digital holography. Chapter 3 examines the design of a one-step monochromatic hologram printer capable producing white-light viewable transmission holograms created with the aid of an LCOS display system and printed in a dot-matrix sequence. The lens system employed includes a microlens array and an afocal relay telescope which are both quantitatively examined in order to maximise the contrast, diffraction efficiency and depth of view of the final hologram image. A brief overview of speckle reduction techniques and their applicability to pulsed digital holography is presented along with experimental results of the use of a microlens array to reduce speckle effects. Chapter 4 presents an analysis of the unwanted side effects of the angular intensity distribution of a hologram pixel, using a case study for analysis. Chapter 5 examines methods for increasing both the printing speed and resolution of the hologram printer. Chapter 6 describes the analysis and design of a temperature-energy feedback system to correct for pulsed laser instabilities arising from mode beating due to temperature variations. Chapter 7 provides a conclusion to the work and discusses possible future developments.

==> acknowledgements.tex <==

I would first like to thank the people who made this project possible:  My university supervisors Professor Chris Chatwin and Dr. Rupert Young for their help and encouragement; and my work supervisor Dr. David Brotherton-Ratcliffe and the staff at Geola Technologies for allowing me to break much of their valuable equipment over the three years of employment.  I would also like to make a special mention to Doug Ollivier for his permission for the use of his 3D futuristic-tank model.

\bigskip

A special thanks goes out to my brother, Ian Kevin Tapsell, who spent many days and nights working with me in the dark room handling the chemicals and processing the holograms with expert ease.

\bigskip

I would also like to acknowledge the support of a EPSRC fellowship.  This work was funded by the UK's leading funding agency - the Engineering and Physical Sciences Research Council.  Without this opportunity, I never would have delved into the world of physics and engineering.

\bigskip

Finally, my warmest appreciation goes to my darling wife Saki Tapsell, who looked after me at every step of the way. Without her, none of this would have been possible.


==> acronyms.tex <==
\newpage
\makeatletter
\chapter*{List of Acronyms\@mkboth {LIST OF ACRONYMS}{LIST OF ACRONYMS}}
\makeatother
%\chapter*{List of Acronyms}
\begin{acronym}
\acro{SLM}{Spacial Light Modulator}. A device that spatially modulates a beam of light.
\acro{EASLM}{Electrically Addressed Spacial Light Modulator}. A SLM display that is electrically (as opposed to optically) controlled, typically by a computer.
\acro{LCD}{Liquid Crystal Display}. In this usage, a transmissive EASLM display that spatially modulates the beam intensity.
\acro{LCOS}{Liquid Crystal On Silicon}. A reflective EASLM display that spatially modulates the beam phase.  Used in conjunction with a polariser to modulate the intensity.
\acro{NDYAG}[Nd:YAG]{Neodymium Doped Yttrium Aluminum Garnet}. A lasing material used in near-infrared lasers.
\acro{VSYNC}{Vertical Synchronization}.  Matching a display (such as an SLM) refresh rate.
\acro{CW}{Continuous Wave}. A laser beam that is continuous, rather than pulsed.
\acro{3D}{Three-Dimensional}. A three dimensional object or image.
\acro{2D}{Two-Dimensional}. A two dimensional image, without depth.  Such as a photograph.
\acro{2.5D}{2.5 Dimensional}. An image with, typically, horizontal but not vertical parallax.
\acro{CCD}{Charge-coupled device}. A device that enables electric charges to be transported through successive capacitors controlled by a clock signal. Used mainly for sensors that capture and record light.
\acro{DTC}{Digital Temperature Controller}.  The name we gave to the PCB that heats and measures the temperature of a component.
\acro{PCB}{Printed Circuit Board}. A board for supporting, mounting and connecting electronic components.
\acro{PID}{\textbf{P}roportional \textbf{I}ntegral \textbf{D}erivative}. A standard algorithm to change an output in response to an input.
\acro{ID}{identification number}. Assigned unique number for identification.
\acro{USB}{Universal Serial Bus}. A serial bus standard for communication between devices.
\acro{PC}{Personal Computer}.
\acro{A-D}{Analogue-Digital}.
\acro{EIA}{Electronics Industry Alliance}. A trade organization for electronics manufacturers in the United States.
\acro{DPI}{Dots Per Inch}.  The number of dots (pixels) per linear inch.
\acro{RGB}{Red Green Blue}.  Three additive primary colors.
\acro{IO}[I/O]{Input/Output}.  Input and output data streams.
\acro{OS}{Operating System}.   The software that manages the computer's hardware resources.
\acro{NDF}{Neutral Density Filter}.  A darkened piece of glass used to decrease the energy of a laser beam.
\end{acronym}
\newpage

==> dedication.tex <==
\thispagestyle{empty} 
\newenvironment{dedication}
  {\cleardoublepage \thispagestyle{empty} \vspace*{\stretch{1}} \begin{center} \em}
  {\end{center} \vspace*{\stretch{3}} \clearpage}
\begin{dedication}
To my wife, Saki.
\end{dedication}


==> formulas_used.tex <==

(Page numbers indicate the first use of the variable)

\section*{Hologram printer components}\label{sec:printercomponents}
The components in the hologram printer are labelled uniquely throughout the thesis.  See Appendix~\ref{chap:hologramprinterdiagrams} for full page schematic labelled diagrams.
\begin{center}
% use packages: array
\begin{longtable}{ll}
L1 & Lens between microlens array and LCOS. \\ 
L2 & First compound lens in relay telescope to image LCOS to plane I2 \\ 
L3 & Second compound lens in relay telescope to image LCOS to plane I2 \\ 
L4 & Objective compound lens, to image the Fourier plane of I2 onto I3 \\ 
L5 & First lens in afocal telescope in object beam to magnify the beam \\
L6 & Second lens in afocal telescope in object beam to magnify the beam \\
L7 & Acts with lens L8 to image I4 to I3 \\
L8 & Acts with lens L7 to image I4 to I3 \\
L9 & Acts with lens L10 to image aperture to image I4 \\
L10 & Acts with lens L9 to image aperture to image I4 \\
LCOS & LCOS display system \\ 
I1 & Real focal image plane inside relay telescope \\ 
I2 & Real focal image plane inside relay telescope \\ 
I3 & Real holopixel plane.  Fourier transform of LCOS \\
I4 & Real image plane of aperture \\
I5 & Focal plane of L10 and L9 - aperture placed here to clean beam \\
A & Microlens array \\ 
a & Optical distance from microlens array to lens L1 \\ 
b & Optical distance from lens L1 to LCOS, via mirror and cube polariser \\ 
c & Optical distance from LCOS to lens L2 via split beam polariser \\ 
d & Optical distance from lens L2 to image plane I1 \\ 
e & Optical distance from image plane I1 to lens L3 \\ 
f & Optical distance from lens L3 to image plane I2 \\ 
g & Optical distance from image plane I2 to lens L4 \\ 
h & Optical distance from lens L4 to image plane I3 \\ 
j & Optical distance from image plane I3 to lens L7 \\ 
k & Optical distance from between lenses L7 and L8 \\ 
m & Optical distance from lens L8 to image plane I4 \\ 
n & Optical distance from image plane I4 to lens L9 \\ 
y & Width of aperture on microlens array A \\ 
z & Distance between aperture and microlens array \\ 
Laser & Laser mounted on breadboard
\end{longtable}
\end{center}



\section*{Equation reference}
\subsection*{Sensitivity analysis}
Provides a measure of the sensitivity of a function with respect to one of its
input variables. A value of $<<1$ means the output of the function is very insensitive to changes in the variable.  A value of $>>1$ means that the output of the function is very sensitive to changes in the variable.
\begin{equation}
\text{Relative sensitivity of $f$ w.r.t. $x$} =\frac{x}{f}\cdot {\frac{\partial f}{\partial x}}
\end{equation}
\subsection*{Lens equations}
The thin lens formula in air is:
\begin{equation}
\frac{1}{S_1}+\frac{1}{S_2}=\frac{1}{f}
\end{equation}
Where  $S_1$  is the distance between an object plane and a thin
lens with focal length $f$ and
$S_2$ is the distance between the thin
lens and the image plane.

For two thin lenses with focal lengths $f_1$ and $f_2$ respectively, separated
by an optical distance of $f_1+f_2$ , the final convergence
of the beam is not altered (making it afocal), but the width
of the beam is magnified by a factor $M$ of:
\begin{equation}
M=-\frac{f_1}{f_2}
\end{equation}

Small angle approximation for paraxial rays:
\begin{equation}
\sin(\theta) \approx \theta 
\end{equation}

\subsection*{Matrix method for lens system analysis}\label{sec:matrixmethod}
The matrix method for lens system analysis works on the basis that a thin-lens system can be described with a matrix, $\vec{M}$.  The input vector, $\vec{v}_\text{input}$, is modified by the matrix to produce the output vector, $\vec{v}_\text{final}$ as so:
\begin{align}
\vec{v}_\text{final} &= \vec{M}\cdot \vec{v}_\text{input}\\
\intertext{Vector for light ray at height $r$ and travelling at angle $\theta$ from the horizontal (From \citet[pages 120-130]{IntroOptics}):}
\vec{v}&=\left(r, \theta\right)^T\\
\intertext{Transfer matrix for ray travelling distance $b$ in constant medium:}
\vec{M}&=\left(\begin{matrix}1&b\\0&1\end{matrix}\right)\\
\intertext{Lens matrix for ray travelling through a thin-lens with focus $f$:}
\vec{M}&=\left(\begin{matrix}1&0\\-\dfrac{1}{f}&1\end{matrix}\right)\\
\intertext{Matrix for surface with initial index of refraction $n_1$, final index of refraction $n_2$ and curvature $R$:}
\vec{M}&= \begin{pmatrix}1 & 0 \\ \frac{n_1-n_2}{R\cdot n_2} & \frac{n_1}{n_2}\end{pmatrix}
\end{align}


==> pgfplots.code.tex <==
%--------------------------------------------
%
% Package pgfplots
%
% Provides a user-friendly interface to create function plots (normal
% plots, semi-logplots and double-logplots).
% 
% It is based on Till Tantau's PGF package.
%
% Copyright 2007/2008 by Christian Feuersänger.
%
% This program is free software: you can redistribute it and/or modify
% it under the terms of the GNU General Public License as published by
% the Free Software Foundation, either version 3 of the License, or
% (at your option) any later version.
% 
% This program is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
% GNU General Public License for more details.
% 
% You should have received a copy of the GNU General Public License
% along with this program.  If not, see <http://www.gnu.org/licenses/>.
%
%--------------------------------------------

\input pgfplotsutil.code.tex
\input pgfplotsoldpgfsupp_loader.code.tex
\input pgfplots.stackedplots.code.tex

\usetikzlibrary{decorations,decorations.pathmorphing,decorations.pathreplacing}

% FIXME: reduce number of variables!

\newif\ifpgfplots@xislinear
\newif\ifpgfplots@yislinear
\newcount\pgfplots@numplots
\newdimen\pgfplots@xcoordminTEX
\newdimen\pgfplots@xcoordmaxTEX
\newdimen\pgfplots@ycoordminTEX
\newdimen\pgfplots@ycoordmaxTEX
\newif\ifpgfplots@warn@for@filter@discards
\newif\ifpgfplots@isuniformtick
\newif\ifpgfplots@clip@limits
\newif\ifpgfplots@enlargelimits
\newif\ifpgfplots@enlargelimits@rel@thresh
\newif\ifpgfplots@enlargelimits@auto
\newif\ifpgfplots@tickshow
\newif\ifpgfplots@xminorticks
\newif\ifpgfplots@xmajorticks
\newif\ifpgfplots@yminorticks
\newif\ifpgfplots@ymajorticks
\newif\ifpgfplots@xminorgrids
\newif\ifpgfplots@xmajorgrids
\newif\ifpgfplots@yminorgrids
\newif\ifpgfplots@ymajorgrids
\newif\ifpgfplots@clip@marker@paths
\newif\ifpgfplots@axis@on@top
\newif\ifpgfplots@separate@axis@lines
\newif\ifpgfplots@scaled@ticks@x
\newif\ifpgfplots@scaled@ticks@y
\newif\ifpgfplots@identify@log@minor@tick@pos
\newif\ifpgfplots@disablelogfilter
\newif\ifpgfplots@disabledatascaling
\newif\ifpgfplots@hide@x
\newif\ifpgfplots@hide@y
\newif\ifpgfplots@is@old@list@format
\newif\ifpgfplots@errorbars@enabled
\newif\ifpgfplots@scale@only@axis
\newif\ifpgfplots@xticklabel@interval
\newif\ifpgfplots@yticklabel@interval
\newif\ifpgfplots@stacked@x
\newif\ifpgfplots@stackedmode
\newif\ifpgfplots@stacked@reverse
\newif\ifpgfplots@stacked@plus
\newif\ifpgfplots@plot@file@skipfirst
\let\pgfnodepartimagebox=\pgfnodeparttextbox

\newif\ifpgfplots@collect@firstplot@astick

\def\pgfplots@errorbars@xdirection{0}% pre-init, see below
\def\pgfplots@errorbars@ydirection{0}%

\def\axisdefaultwidth{240pt}
\def\axisdefaultheight{207pt}




% Creates a named plot cycle list.
%
% #1:  the name of the final list. Can be used in 'cycle list name'
% #2:  the list entries. You can use either a comma-separated list or
%      a '\\'-terminated list. The latter case also requires '\\'
%      AFTER the last entry.
\def\pgfcreateplotcyclelist#1#2{\pgfplots@assign@list#1{#2}}

\pgfcreateplotcyclelist{\blackwhiteplotspeclist}{%
	every mark/.append style={fill=gray},mark=*\\%
	every mark/.append style={fill=gray},mark=square*\\%
	every mark/.append style={fill=gray},mark=otimes*\\%
	mark=star\\%
	every mark/.append style={fill=gray},mark=diamond*\\%
	densely dashed,every mark/.append style={solid,fill=gray},mark=*\\%
	densely dashed,every mark/.append style={solid,fill=gray},mark=square*\\%
	densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
	densely dashed,every mark/.append style={solid},mark=star\\%
	densely dashed,every mark/.append style={solid,fill=gray},mark=diamond*\\%
}
\pgfcreateplotcyclelist{\coloredplotspeclist}{%
	blue,every mark/.append style={fill=blue!80!black},mark=*\\%
	red,every mark/.append style={fill=red!80!black},mark=square*\\%
	brown!60!black,every mark/.append style={fill=brown!80!black},mark=otimes*\\%
	black,mark=star\\%
	blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
	red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
	brown!60!black,densely dashed,every mark/.append style={solid,fill=brown!80!black},mark=square*\\%
	black,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
	blue,densely dashed,mark=star,every mark/.append style=solid\\%
	red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*\\%
}

\def\pgfplotsset#{\pgfqkeys{/pgfplots}}

\def\pgfplotsdeprecatedstylecheck#1{%
	\pgfkeysifdefined{#1/.@cmd}{%
		\begingroup
		\edef\pgfkeyscurrentkey{#1}%
		\pgfkeyssplitpath
		\pgfplots@warning{Loading deprecated style option 
			\pgfkeyscurrentpath/\pgfkeyscurrentname.  
			Please replace '\string\tikzstyle{\pgfkeyscurrentname}' 
			with '\string\pgfplotsset{\pgfkeyscurrentname/.style={}}'
			(or '\string\pgfplotsset{\pgfkeyscurrentname/.append style={}}').}%
		\endgroup
		\pgfkeysvalueof{#1/.@cmd}\pgfeov
	}{}%
}%

\pgfkeys{%
	/pgfplots/search path for tikz/.unknown/.code={%
		\let\searchname=\pgfkeyscurrentname%
		\pgfkeysalso{%
			/tikz/\searchname/.try=#1,
			/pgfplots/\searchname/.lastretry=#1
		}%
	},%
	/pgfplots/.is family,
	/pgfplots/scale/.is family,
	/pgfplots/legend/.is family,
	/pgfplots/tick/.is family,
	/pgfplots/axis/.is family,
	/pgfplots/descriptions/.is family,
	/pgfplots/style commands/.is family,
	/pgfplots/naming commands/.is family,
	/pgfplots/error bars/.is family,
	/pgfplots/every axis/.style={},
	/pgfplots/every axis/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every axis}},
	/pgfplots/every axis/.belongs to family=/pgfplots/style commands,
	/pgfplots/every semilogx axis/.style={},
	/pgfplots/every semilogx axis/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every semilogx axis}},
	/pgfplots/every semilogx axis/.belongs to family=/pgfplots/style commands,
	/pgfplots/every semilogy axis/.style={},
	/pgfplots/every semilogy axis/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every semilogy axis}},
	/pgfplots/every semilogy axis/.belongs to family=/pgfplots/style commands,
	/pgfplots/every loglog axis/.style={},
	/pgfplots/every loglog axis/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every loglog axis}},
	/pgfplots/every loglog axis/.belongs to family=/pgfplots/style commands,
	/pgfplots/every linear axis/.style={},
	/pgfplots/every linear axis/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every linear axis}},
	/pgfplots/every linear axis/.belongs to family=/pgfplots/style commands,
	/pgfplots/every axis plot/.style={},
	/pgfplots/every axis plot/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every axis plot}},
	/pgfplots/every axis plot/.belongs to family=/pgfplots/style commands,
	/pgfplots/every axis plot post/.style={},
	/pgfplots/every axis plot post/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every axis plot}},
	/pgfplots/every axis label/.style={},
	/pgfplots/every axis label/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every axis label}},
	/pgfplots/every axis label/.belongs to family=/pgfplots/style commands,
	/pgfplots/every axis x label/.style={at={(0.5,0)},below,yshift=-15pt},
	/pgfplots/every axis x label/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every axis x label}},
	/pgfplots/every axis x label/.belongs to family=/pgfplots/style commands,
	/pgfplots/every axis y label/.style={at={(0,0.5)},xshift=-35pt,rotate=90},
	/pgfplots/every axis y label/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every axis y label}},
	/pgfplots/every axis y label/.belongs to family=/pgfplots/style commands,
	/pgfplots/every axis title/.style={at={(0.5,1)},above,yshift=6pt},
	/pgfplots/every axis title/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every axis title}},
	/pgfplots/every axis title/.belongs to family=/pgfplots/style commands,
	/pgfplots/every tick/.style={very thin,gray},
	/pgfplots/every tick/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every tick}},
	/pgfplots/every tick/.belongs to family=/pgfplots/style commands,
	/pgfplots/every inner x axis line/.style={},
	/pgfplots/every inner y axis line/.style={},
	/pgfplots/every outer x axis line/.style={},
	/pgfplots/every outer y axis line/.style={},
	/pgfplots/x axis line style/.style={
		/pgfplots/every outer x axis line/.append style={#1},
		/pgfplots/every inner x axis line/.append style={#1},
	},
	/pgfplots/y axis line style/.style={
		/pgfplots/every outer y axis line/.append style={#1},
		/pgfplots/every inner y axis line/.append style={#1},
	},
	/pgfplots/outer axis line style/.style={
		/pgfplots/every outer x axis line/.append style={#1},
		/pgfplots/every outer y axis line/.append style={#1}%
	},
	/pgfplots/inner axis line style/.style={
		/pgfplots/every inner x axis line/.append style={#1},
		/pgfplots/every inner y axis line/.append style={#1}%
	},
	/pgfplots/axis line style/.style={
		/pgfplots/inner axis line style={#1},
		/pgfplots/outer axis line style={#1}%
	},
	/pgfplots/separate axis lines/.is if=pgfplots@separate@axis@lines,
	/pgfplots/separate axis lines/.default=true,
	/pgfplots/every minor tick/.style={},
	/pgfplots/every minor tick/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every minor tick}},
	/pgfplots/every minor tick/.belongs to family=/pgfplots/style commands,
	/pgfplots/every major tick/.style={},
	/pgfplots/every major tick/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every major tick}},
	/pgfplots/every major tick/.belongs to family=/pgfplots/style commands,
	/pgfplots/every x tick/.style={},
	/pgfplots/every x tick/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every x tick}},
	/pgfplots/every x tick/.belongs to family=/pgfplots/style commands,
	/pgfplots/every minor x tick/.style={},
	/pgfplots/every minor x tick/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every minor x tick}},
	/pgfplots/every minor x tick/.belongs to family=/pgfplots/style commands,
	/pgfplots/every major x tick/.style={},
	/pgfplots/every major x tick/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every major x tick}},
	/pgfplots/every major x tick/.belongs to family=/pgfplots/style commands,
	/pgfplots/every y tick/.style={},
	/pgfplots/every y tick/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every y tick}},
	/pgfplots/every y tick/.belongs to family=/pgfplots/style commands,
	/pgfplots/every minor y tick/.style={},
	/pgfplots/every minor y tick/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every minor y tick}},
	/pgfplots/every minor y tick/.belongs to family=/pgfplots/style commands,
	/pgfplots/every major y tick/.style={},
	/pgfplots/every major y tick/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every major y tick}},
	/pgfplots/every major y tick/.belongs to family=/pgfplots/style commands,
	%/pgfplots/every axis grid/.style={help lines},
	/pgfplots/every axis grid/.style={thin,black!25},
	/pgfplots/every axis grid/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every axis grid}},
	/pgfplots/every axis grid/.belongs to family=/pgfplots/style commands,
	/pgfplots/every minor grid/.style={},
	/pgfplots/every minor grid/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every minor grid}},
	/pgfplots/every minor grid/.belongs to family=/pgfplots/style commands,
	/pgfplots/every major grid/.style={},
	/pgfplots/every major grid/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every major grid}},
	/pgfplots/every major grid/.belongs to family=/pgfplots/style commands,
	/pgfplots/every axis x grid/.style={},
	/pgfplots/every axis x grid/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every axis x grid}},
	/pgfplots/every axis x grid/.belongs to family=/pgfplots/style commands,
	/pgfplots/every minor x grid/.style={},
	/pgfplots/every minor x grid/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every minor x grid}},
	/pgfplots/every minor x grid/.belongs to family=/pgfplots/style commands,
	/pgfplots/every major x grid/.style={},
	/pgfplots/every major x grid/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every major x grid}},
	/pgfplots/every major x grid/.belongs to family=/pgfplots/style commands,
	/pgfplots/every axis y grid/.style={},
	/pgfplots/every axis y grid/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every axis y grid}},
	/pgfplots/every axis y grid/.belongs to family=/pgfplots/style commands,
	/pgfplots/every minor y grid/.style={},
	/pgfplots/every minor y grid/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every minor y grid}},
	/pgfplots/every minor y grid/.belongs to family=/pgfplots/style commands,
	/pgfplots/every major y grid/.style={},
	/pgfplots/every major y grid/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every major y grid}},
	/pgfplots/every major y grid/.belongs to family=/pgfplots/style commands,
	/pgfplots/every tick label/.style={},
	/pgfplots/every tick label/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every tick label}},
	/pgfplots/every tick label/.belongs to family=/pgfplots/style commands,
	/pgfplots/every x tick label/.style={},
	/pgfplots/every x tick label/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every x tick label}},
	/pgfplots/every x tick label/.belongs to family=/pgfplots/style commands,
	/pgfplots/every extra x tick/.style={
		/pgfplots/log identify minor tick positions=true,
	},
	/pgfplots/every extra x tick/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every extra x tick}},
	/pgfplots/every extra x tick/.belongs to family=/pgfplots/style commands,
	/pgfplots/extra x tick style/.belongs to family=/pgfplots/style commands,
	/pgfplots/extra x tick style/.code={%
		\pgfkeysalso{/pgfplots/every extra x tick/.append style={#1}}%
	},
	/pgfplots/every x tick scale label/.style={at={(1,0)},yshift=-2em,left,inner sep=0pt},
	/pgfplots/every x tick scale label/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every x tick scale label}},
	/pgfplots/every x tick scale label/.belongs to family=/pgfplots/style commands,
	/pgfplots/every y tick label/.style={},
	/pgfplots/every y tick label/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every y tick label}},
	/pgfplots/every y tick label/.belongs to family=/pgfplots/style commands,
	/pgfplots/every extra y tick/.style={
		/pgfplots/log identify minor tick positions=true,
	},
	/pgfplots/every extra y tick/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every extra y tick}},
	/pgfplots/every extra y tick/.belongs to family=/pgfplots/style commands,
	/pgfplots/extra y tick style/.belongs to family=/pgfplots/style commands,
	/pgfplots/extra y tick style/.code={%
		\pgfkeysalso{/pgfplots/every extra y tick/.append style={#1}}%
	},
	/pgfplots/every y tick scale label/.style={at={(0,1)},above right,inner sep=0pt,yshift=0.3em},
	/pgfplots/every y tick scale label/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every y tick scale label}},
	/pgfplots/every y tick scale label/.belongs to family=/pgfplots/style commands,
	/pgfplots/every axis legend/.style={%
		cells={anchor=center},
		inner xsep=3pt,inner ysep=2pt,nodes={inner sep=2pt,text depth=0.15em},
		anchor=north east,%
		shape=rectangle,%
		fill=white,%
		draw=black,
		at={(0.98,0.98)},
	},
	/pgfplots/every axis legend/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every axis legend}},
	/pgfplots/every axis legend/.belongs to family=/pgfplots/style commands,
% tick options:
	/pgfplots/xticklabel/.store in=	\pgfplots@xticklabel,
	/pgfplots/xticklabel/.belongs to family=/pgfplots/tick,
	/pgfplots/xticklabel=,
	/pgfplots/xticklabels/.belongs to family=/pgfplots/tick,
	/pgfplots/xticklabels/.code={%
		\pgfplots@foreach@to@list{#1}\to\pgfplots@xticklabels
		\let\pgfplots@xticklabel=\pgfplots@user@ticklabel@list@x
	},
	/pgfplots/yticklabels/.belongs to family=/pgfplots/tick,
	/pgfplots/yticklabels/.code={%
		\pgfplots@foreach@to@list{#1}\to\pgfplots@yticklabels
		\let\pgfplots@yticklabel=\pgfplots@user@ticklabel@list@y
	},
	/pgfplots/yticklabel/.store in=	\pgfplots@yticklabel,
	/pgfplots/yticklabel/.belongs to family=/pgfplots/tick,
	/pgfplots/yticklabel=,
	/pgfplots/x tick label as interval/.is if=pgfplots@xticklabel@interval,
	/pgfplots/x tick label as interval/.default=true,
	/pgfplots/x tick label as interval/.belongs to family=/pgfplots/tick,
	/pgfplots/y tick label as interval/.is if=pgfplots@yticklabel@interval,
	/pgfplots/y tick label as interval/.default=true,
	/pgfplots/y tick label as interval/.belongs to family=/pgfplots/tick,
	/pgfplots/extra x tick label/.store in=	\pgfplots@extra@xticklabel,
	/pgfplots/extra x tick label/.belongs to family=/pgfplots/tick,
	/pgfplots/extra x tick label=,
	/pgfplots/extra x tick labels/.belongs to family=/pgfplots/tick,
	/pgfplots/extra x tick labels/.code={%
		\pgfplots@foreach@to@list{#1}\to\pgfplots@extra@xticklabels
		\let\pgfplots@extra@xticklabel=\pgfplots@user@extra@ticklabel@list@x
	},
	/pgfplots/extra y tick labels/.code={%
		\pgfplots@foreach@to@list{#1}\to\pgfplots@extra@yticklabels
		\let\pgfplots@extra@yticklabel=\pgfplots@user@extra@ticklabel@list@y
	},
	/pgfplots/xtick/.store in=			\pgfplots@xtick,
	/pgfplots/xtick/.belongs to family=/pgfplots/tick,
	/pgfplots/xtick=,
	/pgfplots/extra x ticks/.store in=\pgfplots@extra@xtick,
	/pgfplots/extra x ticks/.belongs to family=/pgfplots/tick,
	/pgfplots/extra x ticks=,
	/pgfplots/xtickten/.store in=		\pgfplots@xtickten,
	/pgfplots/xtickten/.belongs to family=/pgfplots/tick,
	/pgfplots/xtickten=,
	/pgfplots/extra y tick label/.store in=	\pgfplots@extra@yticklabel,
	/pgfplots/extra y tick label/.belongs to family=/pgfplots/tick,
	/pgfplots/extra y tick label=,
	/pgfplots/ytick/.store in=			\pgfplots@ytick,
	/pgfplots/ytick/.belongs to family=/pgfplots/tick,
	/pgfplots/ytick=,
	/pgfplots/extra y ticks/.store in=\pgfplots@extra@ytick,
	/pgfplots/extra y ticks/.belongs to family=/pgfplots/tick,
	/pgfplots/extra y ticks=,
	/pgfplots/ytickten/.store in=		\pgfplots@ytickten,
	/pgfplots/ytickten/.belongs to family=/pgfplots/tick,
	/pgfplots/ytickten=,
	/pgfplots/tick scale label code/.code={$\cdot 10^{#1}$},
	/pgfplots/tick scale label code/.belongs to family=/pgfplots/tick,
	/pgfplots/scaled x ticks/.is if=pgfplots@scaled@ticks@x,
	/pgfplots/scaled x ticks/.belongs to family=/pgfplots/tick,
	/pgfplots/scaled x ticks=true,
	/pgfplots/scaled y ticks/.is if=pgfplots@scaled@ticks@y,
	/pgfplots/scaled y ticks/.belongs to family=/pgfplots/tick,
	/pgfplots/scaled y ticks=true,
	/pgfplots/scaled ticks/.style={%
		/pgfplots/scaled x ticks=#1,
		/pgfplots/scaled y ticks=#1},
	/pgfplots/scale ticks above exponent/.store in=	\pgfplots@scale@ticks@above@exponent,
	/pgfplots/scale ticks above exponent/.belongs to family=/pgfplots/tick,
	/pgfplots/scale ticks above exponent=3,
	/pgfplots/scale ticks below exponent/.store in=	\pgfplots@scale@ticks@below@exponent,
	/pgfplots/scale ticks below exponent/.belongs to family=/pgfplots/tick,
	/pgfplots/scale ticks below exponent=-1,
	/pgfplots/subtickwidth/.store in=	\pgfplots@subtickwidth,
	/pgfplots/subtickwidth/.belongs to family=/pgfplots/tick,
	/pgfplots/subtickwidth=0.1cm,
	/pgfplots/tickwidth/.store in=		\pgfplots@tickwidth,
	/pgfplots/tickwidth/.belongs to family=/pgfplots/tick,
	/pgfplots/tickwidth=0.15cm,
	/pgfplots/minor x tick num/.initial=0,
	/pgfplots/minor x tick num/.belongs to family=/pgfplots/tick,
	/pgfplots/minor y tick num/.initial=0,
	/pgfplots/minor y tick num/.belongs to family=/pgfplots/tick,
	/pgfplots/minor tick num/.style={/pgfplots/minor x tick num=#1,/pgfplots/minor y tick num=#1},
	/pgfplots/minor tick num/.belongs to family=/pgfplots/tick,
	/pgfplots/minor tick length/.estore in=\pgfplots@subtickwidth,
	/pgfplots/minor tick length/.belongs to family=/pgfplots/tick,
	/pgfplots/major tick length/.estore in=\pgfplots@tickwidth,
	/pgfplots/major tick length/.belongs to family=/pgfplots/tick,
	/pgfplots/max space between ticks/.estore in=\axisdefaulttickwidth,
	/pgfplots/max space between ticks/.belongs to family=/pgfplots/tick,
	/pgfplots/max space between ticks=35,% the maximum space between adjacent ticks (in pt, but don't specify the unit 'pt')
	/pgfplots/try min ticks/.estore in=			\axisdefaulttryminticks,
	/pgfplots/try min ticks/.belongs to family=/pgfplots/tick,
	/pgfplots/try min ticks=4,
	/pgfplots/try min ticks log/.estore in=			\pgfplots@default@try@minticks@log,
	/pgfplots/try min ticks log/.belongs to family=/pgfplots/tick,
	/pgfplots/try min ticks log=3,
	/pgfplots/log plot exponent style/.style={/pgf/number format/fixed,/pgf/number format/precision=2},
	/pgfplots/log plot exponent style/.belongs to family=/pgfplots/tick,
	/pgfplots/log identify minor tick positions/.is if=pgfplots@identify@log@minor@tick@pos,
	/pgfplots/log identify minor tick positions/.belongs to family=/pgfplots/tick,
	/pgfplots/log identify minor tick positions=false,
	/pgfplots/log number format code/.code={{%
		\pgfmathlogtologten@{#1}%
		\ifpgfplots@identify@log@minor@tick@pos
			\expandafter\pgfplots@is@log@tick@a@minor@tick@pos\pgfmathresult\relax%
		\else
			\pgfplots@log@tick@isminor@tick@posfalse
		\fi
		\ifpgfplots@log@tick@isminor@tick@pos
			\pgfmathprintnumber[sci]{\pgfmathresult}%
		\else
			\pgfkeysalso{/pgfplots/log plot exponent style,/pgfplots/log base 10 number format code=\pgfmathresult}%
		\fi
	}},
	/pgfplots/log number format code/.belongs to family=/pgfplots/tick,
	/pgfplots/log base 10 number format code/.code={$10^{\pgfmathprintnumber{#1}}$},
	/pgfplots/log base 10 number format code/.belongs to family=/pgfplots/tick,
% sets \pgfplots@[xy]tickposnum to
	/pgfplots/xtick pos/.is choice,
	/pgfplots/xtick pos/.belongs to family=/pgfplots/tick,
	/pgfplots/xtick pos/left/.code	={\def\pgfplots@xtickposnum{1}},
	/pgfplots/xtick pos/left/.belongs to family=/pgfplots/tick,
	/pgfplots/xtick pos/right/.code	={\def\pgfplots@xtickposnum{3}},
	/pgfplots/xtick pos/right/.belongs to family=/pgfplots/tick,
	/pgfplots/xtick pos/both/.code	={\def\pgfplots@xtickposnum{0}},
	/pgfplots/xtick pos/both/.belongs to family=/pgfplots/tick,
	/pgfplots/xtick pos=both,
	/pgfplots/ytick pos/.is choice,
	/pgfplots/ytick pos/.belongs to family=/pgfplots/tick,
	/pgfplots/ytick pos/left/.code	={\def\pgfplots@ytickposnum{1}},
	/pgfplots/ytick pos/left/.belongs to family=/pgfplots/tick,
	/pgfplots/ytick pos/right/.code	={\def\pgfplots@ytickposnum{3}},
	/pgfplots/ytick pos/right/.belongs to family=/pgfplots/tick,
	/pgfplots/ytick pos/both/.code	={\def\pgfplots@ytickposnum{0}},
	/pgfplots/ytick pos/both/.belongs to family=/pgfplots/tick,
	/pgfplots/ytick pos/top/.style={/pgfplots/ytick pos/right},
	/pgfplots/ytick pos/bottom/.style={/pgfplots/ytick pos/left},
	/pgfplots/ytick pos=both,
	/pgfplots/tickpos/.style={/pgfplots/xtick pos={#1},/pgfplots/ytick pos={#1}},
	/pgfplots/tickpos/.belongs to family=/pgfplots/tick,
% sets the tick LABEL position, \pgfplots@[xy]ticklabelposnum
	/pgfplots/xticklabel pos/.is choice,
	/pgfplots/xticklabel pos/.belongs to family=/pgfplots/tick,
	/pgfplots/xticklabel pos/default/.code	={\def\pgfplots@xticklabelposnum{0}},
	/pgfplots/xticklabel pos/default/.belongs to family=/pgfplots/tick,
	/pgfplots/xticklabel pos/left/.code	={\def\pgfplots@xticklabelposnum{1}},
	/pgfplots/xticklabel pos/left/.belongs to family=/pgfplots/tick,
	/pgfplots/xticklabel pos/right/.code	={\def\pgfplots@xticklabelposnum{3}},
	/pgfplots/xticklabel pos/right/.belongs to family=/pgfplots/tick,
	/pgfplots/xticklabel pos=default,
	/pgfplots/yticklabel pos/.is choice,
	/pgfplots/yticklabel pos/.belongs to family=/pgfplots/tick,
	/pgfplots/yticklabel pos/default/.code	={\def\pgfplots@yticklabelposnum{0}},
	/pgfplots/yticklabel pos/default/.belongs to family=/pgfplots/tick,
	/pgfplots/yticklabel pos/left/.code	={\def\pgfplots@yticklabelposnum{1}},
	/pgfplots/yticklabel pos/left/.belongs to family=/pgfplots/tick,
	/pgfplots/yticklabel pos/right/.code	={\def\pgfplots@yticklabelposnum{3}},
	/pgfplots/yticklabel pos/right/.belongs to family=/pgfplots/tick,
	/pgfplots/yticklabel pos/top/.style={/pgfplots/yticklabel pos/right},
	/pgfplots/yticklabel pos/bottom/.style={/pgfplots/yticklabel pos/left},
	/pgfplots/yticklabel pos=default,
	/pgfplots/ticklabelpos/.style={/pgfplots/xticklabel pos={#1},/pgfplots/yticklabel pos={#1}},
% sets \pgfplots@{x,y}tickalignnum to
% inside=0
% outside=1
% center=2
	/pgfplots/xtick align/.is choice,
	/pgfplots/xtick align/.belongs to family=/pgfplots/tick,
	/pgfplots/xtick align/inside/.code	={\def\pgfplots@xtickalignnum{0}},
	/pgfplots/xtick align/inside/.belongs to family=/pgfplots/tick,
	/pgfplots/xtick align/outside/.code	={\def\pgfplots@xtickalignnum{1}},
	/pgfplots/xtick align/outside/.belongs to family=/pgfplots/tick,
	/pgfplots/xtick align/center/.code	={\def\pgfplots@xtickalignnum{2}},
	/pgfplots/xtick align/center/.belongs to family=/pgfplots/tick,
	/pgfplots/xtick align=inside,
	/pgfplots/ytick align/.is choice,
	/pgfplots/ytick align/.belongs to family=/pgfplots/tick,
	/pgfplots/ytick align/inside/.code	={\def\pgfplots@ytickalignnum{0}},
	/pgfplots/ytick align/inside/.belongs to family=/pgfplots/tick,
	/pgfplots/ytick align/outside/.code	={\def\pgfplots@ytickalignnum{1}},
	/pgfplots/ytick align/outside/.belongs to family=/pgfplots/tick,
	/pgfplots/ytick align/center/.code	={\def\pgfplots@ytickalignnum{2}},
	/pgfplots/ytick align/center/.belongs to family=/pgfplots/tick,
	/pgfplots/ytick align=inside,
	/pgfplots/tick align/.belongs to family=/pgfplots/tick,
	/pgfplots/tick align/.style={%
		/pgfplots/xtick align=#1,
		/pgfplots/ytick align=#1,
	},%
% 'axis' options:
	/pgfplots/anchor/.belongs to family=/pgfplots,
	/pgfplots/anchor/.store in=			\pgfplots@anchorname,
	/pgfplots/anchor=south west,
% tick options:
	/pgfplots/ticks/.is choice,
	/pgfplots/ticks/.belongs to family=/pgfplots/tick,
	/pgfplots/ticks/none/.belongs to family=/pgfplots/tick,
	/pgfplots/ticks/none/.code={%
		\pgfplots@xminorticksfalse
		\pgfplots@yminorticksfalse
		\pgfplots@xmajorticksfalse
		\pgfplots@ymajorticksfalse
	},
	/pgfplots/ticks/major/.belongs to family=/pgfplots/tick,
	/pgfplots/ticks/major/.code={%
		\pgfplots@xminorticksfalse
		\pgfplots@yminorticksfalse
		\pgfplots@xmajortickstrue
		\pgfplots@ymajortickstrue
	},
	/pgfplots/ticks/minor/.belongs to family=/pgfplots/tick,
	/pgfplots/ticks/minor/.code={%
		\pgfplots@xminortickstrue
		\pgfplots@yminortickstrue
		\pgfplots@xmajorticksfalse
		\pgfplots@ymajorticksfalse
	},
	/pgfplots/ticks/both/.belongs to family=/pgfplots/tick,
	/pgfplots/ticks/both/.code={%
		\pgfplots@xminortickstrue
		\pgfplots@yminortickstrue
		\pgfplots@xmajortickstrue
		\pgfplots@ymajortickstrue
	},
	/pgfplots/ticks=both,
	/pgfplots/grid/.is choice,
	/pgfplots/grid/.belongs to family=/pgfplots/tick,
	/pgfplots/grid/none/.belongs to family=/pgfplots/tick,
	/pgfplots/grid/none/.code={%
		\pgfplots@xminorgridsfalse
		\pgfplots@yminorgridsfalse
		\pgfplots@xmajorgridsfalse
		\pgfplots@ymajorgridsfalse
	},
	/pgfplots/grid/major/.belongs to family=/pgfplots/tick,
	/pgfplots/grid/major/.code={%
		\pgfplots@xminorgridsfalse
		\pgfplots@yminorgridsfalse
		\pgfplots@xmajorgridstrue
		\pgfplots@ymajorgridstrue
	},
	/pgfplots/grid/minor/.belongs to family=/pgfplots/tick,
	/pgfplots/grid/minor/.code={%
		\pgfplots@xminorgridstrue
		\pgfplots@yminorgridstrue
		\pgfplots@xmajorgridsfalse
		\pgfplots@ymajorgridsfalse
	},
	/pgfplots/grid/both/.belongs to family=/pgfplots/tick,
	/pgfplots/grid/both/.code={%
		\pgfplots@xminorgridstrue
		\pgfplots@yminorgridstrue
		\pgfplots@xmajorgridstrue
		\pgfplots@ymajorgridstrue
	},
	/pgfplots/grid=none,
	/pgfplots/grid/.default=major,
	/pgfplots/xminorticks/.is if=pgfplots@xminorticks,
	/pgfplots/xminorticks/.default=true,
	/pgfplots/xminorticks/.belongs to family=/pgfplots/tick,
	/pgfplots/xmajorticks/.is if=pgfplots@xmajorticks,
	/pgfplots/xmajorticks/.default=true,
	/pgfplots/xmajorticks/.belongs to family=/pgfplots/tick,
	/pgfplots/yminorticks/.is if=pgfplots@yminorticks,
	/pgfplots/yminorticks/.default=true,
	/pgfplots/yminorticks/.belongs to family=/pgfplots/tick,
	/pgfplots/ymajorticks/.is if=pgfplots@ymajorticks,
	/pgfplots/ymajorticks/.default=true,
	/pgfplots/ymajorticks/.belongs to family=/pgfplots/tick,
	/pgfplots/xminorgrids/.is if=pgfplots@xminorgrids,
	/pgfplots/xminorgrids/.default=true,
	/pgfplots/xminorgrids/.belongs to family=/pgfplots/tick,
	/pgfplots/xmajorgrids/.is if=pgfplots@xmajorgrids,
	/pgfplots/xmajorgrids/.default=true,
	/pgfplots/xmajorgrids/.belongs to family=/pgfplots/tick,
	/pgfplots/yminorgrids/.is if=pgfplots@yminorgrids,
	/pgfplots/yminorgrids/.default=true,
	/pgfplots/yminorgrids/.belongs to family=/pgfplots/tick,
	/pgfplots/ymajorgrids/.is if=pgfplots@ymajorgrids,
	/pgfplots/ymajorgrids/.default=true,
	/pgfplots/ymajorgrids/.belongs to family=/pgfplots/tick,
% legend options:
	/pgfplots/legend entries/.initial={},
	/pgfplots/legend entries/.belongs to family=/pgfplots/legend,
	/pgfplots/legend columns/.store in=\pgfplots@legend@columns,
	/pgfplots/legend columns/.belongs to family=/pgfplots/legend,
	/pgfplots/legend columns=1,
	/pgfplots/legend plot pos/.is choice,
	/pgfplots/legend plot pos/.belongs to family=/pgfplots/legend,
	/pgfplots/legend plot pos/left/.code=	{\def\pgfplots@legend@plot@pos{0}},
	/pgfplots/legend plot pos/left/.belongs to family=/pgfplots/legend,
	/pgfplots/legend plot pos/right/.code=	{\def\pgfplots@legend@plot@pos{1}},
	/pgfplots/legend plot pos/right/.belongs to family=/pgfplots/legend,
	/pgfplots/legend plot pos/none/.code=	{\def\pgfplots@legend@plot@pos{2}},
	/pgfplots/legend plot pos/none/.belongs to family=/pgfplots/legend,
	/pgfplots/legend plot pos=left,
	/pgfplots/legend image code/.code={%
		\draw[#1,mark repeat=2,mark phase=2] 
			plot coordinates {
				(0cm,0cm) 
				(0.3cm,0cm)
				(0.6cm,0cm)%
			};%
	},
	/pgfplots/legend image code/.belongs to family=/pgfplots/legend,
% axis description options:
	/pgfplots/title/.initial=,
	/pgfplots/title/.belongs to family=/pgfplots/descriptions,
	/pgfplots/xlabel/.initial=,
	/pgfplots/xlabel/.belongs to family=/pgfplots/descriptions,
	/pgfplots/ylabel/.initial=,
	/pgfplots/ylabel/.belongs to family=/pgfplots/descriptions,
	/pgfplots/before end axis/.code=,
	/pgfplots/after end axis/.code=,
	/pgfplots/extra description/.code=,
	/pgfplots/extra description/.belongs to family=/pgfplots/descriptions,
% axis options:
	/pgfplots/at/.code={%
		\pgfplots@assert@tikzinternal@exists{tikz@scan@one@point}%
		\tikz@scan@one@point\pgfplots@set@at#1},
	/pgfplots/at/.belongs to family=/pgfplots,
	/pgfplots/clip limits/.is if=pgfplots@clip@limits,
	/pgfplots/clip limits/.default=true,
	/pgfplots/clip limits=true,
	/pgfplots/clip limits/.belongs to family=/pgfplots,
	/pgfplots/xmin/.belongs to family=/pgfplots,
	/pgfplots/xmin/.initial=,
	/pgfplots/xmax/.belongs to family=/pgfplots,
	/pgfplots/xmax/.initial=,
	/pgfplots/ymin/.belongs to family=/pgfplots,
	/pgfplots/ymin/.initial=,
	/pgfplots/ymax/.belongs to family=/pgfplots,
	/pgfplots/ymax/.initial=,
	/pgfplots/stack plots/.is choice,
	/pgfplots/stack plots/.belongs to family=/pgfplots,
	/pgfplots/stack plots/x/.code={\pgfplots@stacked@xtrue\pgfplots@stackedmodetrue},
	/pgfplots/stack plots/x/.belongs to family=/pgfplots,
	/pgfplots/stack plots/y/.code={\pgfplots@stacked@xfalse\pgfplots@stackedmodetrue},
	/pgfplots/stack plots/y/.belongs to family=/pgfplots,
	/pgfplots/stack plots/false/.code={\pgfplots@stackedmodefalse},
	/pgfplots/stack plots/false/.belongs to family=/pgfplots,
	/pgfplots/stack plots=false,
	/pgfplots/reverse stacked plots/.is if=pgfplots@stacked@reverse,
	/pgfplots/reverse stacked plots/.belongs to family=/pgfplots,
	/pgfplots/reverse stacked plots/.default=true,
	/pgfplots/reverse stacked plots=true,
	/pgfplots/stack dir/.is choice,
	/pgfplots/stack dir/.belongs to family=/pgfplots,
	/pgfplots/stack dir/plus/.code={\pgfplots@stacked@plustrue},
	/pgfplots/stack dir/plus/.belongs to family=/pgfplots,
	/pgfplots/stack dir/minus/.code={\pgfplots@stacked@plusfalse},
	/pgfplots/stack dir/minus/.belongs to family=/pgfplots,
	/pgfplots/stack dir=plus,
	/pgfplots/filter discard warning/.is if=pgfplots@warn@for@filter@discards,
	/pgfplots/filter discard warning=true,
	/pgfplots/x filter/.code={},
	/pgfplots/x filter/.belongs to family=/pgfplots,
	/pgfplots/y filter/.code={},
	/pgfplots/y filter/.belongs to family=/pgfplots,
	/pgfplots/skip coords between index/.style 2 args={%
		/pgfplots/x filter/.append code={%
			\ifnum\coordindex<#1\relax
			\else
				\ifnum\coordindex<#2\relax
					\let\pgfmathresult=\pgfutil@empty
				\fi
			\fi}
	},
	/pgfplots/xfilter/.initial=,% DEPRECATED
	/pgfplots/xfilter/.belongs to family=/pgfplots,
	/pgfplots/yfilter/.initial=,% DEPRECATED
	/pgfplots/yfilter/.belongs to family=/pgfplots,
	/pgfplots/width/.store in=		\pgfplots@width,
	/pgfplots/width/.belongs to family=/pgfplots,
	/pgfplots/width=,
	/pgfplots/height/.store in=	\pgfplots@height,
	/pgfplots/height/.belongs to family=/pgfplots,
	/pgfplots/height=,
	/pgfplots/execute at begin plot/.store in=\pgfplots@execute@at@begin@plot,
	/pgfplots/execute at begin plot/.belongs to family=/pgfplots,
	/pgfplots/execute at begin plot=,
	/pgfplots/execute at end plot/.store in=		\pgfplots@execute@at@end@plot,
	/pgfplots/execute at end plot/.belongs to family=/pgfplots,
	/pgfplots/execute at end plot=,
	/pgfplots/enlarge x limits/.initial=auto,
	/pgfplots/enlarge x limits/.default=true,
	/pgfplots/enlarge y limits/.initial=auto,
	/pgfplots/enlarge y limits/.default=true,
	/pgfplots/enlargelimits/.style={%
		/pgfplots/enlarge x limits=#1,%
		/pgfplots/enlarge y limits=#1,%
	},%
	/pgfplots/enlargelimits/.default=true,
	/pgfplots/x/.store in=		\pgfplots@x,
	/pgfplots/x/.belongs to family=/pgfplots,
	/pgfplots/x=,% is implicitly set by 'width' and/or '\axisdefaultwidth'
	/pgfplots/y/.store in=		\pgfplots@y,
	/pgfplots/y/.belongs to family=/pgfplots,
	/pgfplots/y=,% is implicitly set by 'width' and/or '\axisdefaultwidth'
	/pgfplots/cycle list/.code={\pgfplots@assign@list\autoplotspeclist{#1}},
	/pgfplots/cycle list/.belongs to family=/pgfplots,
	/pgfplots/cycle list name/.code={\let\autoplotspeclist=#1\relax},
	/pgfplots/cycle list name/.belongs to family=/pgfplots,
	/pgfplots/cycle list name=\coloredplotspeclist,
	/pgfplots/legend style/.belongs to family=/pgfplots/style commands,
	/pgfplots/legend style/.code={%
		\pgfkeysalso{/pgfplots/every axis legend/.append style={#1}}%
	},
	/pgfplots/label style/.belongs to family=/pgfplots/style commands,
	/pgfplots/label style/.code={%
		\pgfkeysalso{/pgfplots/every axis label/.append style={#1}}%
	},%
	/pgfplots/x label style/.belongs to family=/pgfplots/style commands,
	/pgfplots/x label style/.code={%
		\pgfkeysalso{/pgfplots/every axis x label/.append style={#1}}%
	},
	/pgfplots/y label style/.belongs to family=/pgfplots/style commands,
	/pgfplots/y label style/.code={%
		\pgfkeysalso{/pgfplots/every axis y label/.append style={#1}}%
	},
	/pgfplots/title style/.belongs to family=/pgfplots/style commands,
	/pgfplots/title style/.code={%
		\pgfkeysalso{/pgfplots/every axis title/.append style={#1}}%
	},
	/pgfplots/tick label style/.belongs to family=/pgfplots/style commands,
	/pgfplots/tick label style/.code={%
		\pgfkeysalso{/pgfplots/every tick label/.append style={#1}}%
	},
	/pgfplots/x tick label style/.belongs to family=/pgfplots/style commands,
	/pgfplots/x tick label style/.code={%
		\pgfkeysalso{/pgfplots/every x tick label/.append style={#1}}%
	},
	/pgfplots/y tick label style/.belongs to family=/pgfplots/style commands,
	/pgfplots/y tick label style/.code={%
		\pgfkeysalso{/pgfplots/every y tick label/.append style={#1}}%
	},
	/pgfplots/x tick scale label style/.belongs to family=/pgfplots/style commands,
	/pgfplots/x tick scale label style/.code={%
		\pgfkeysalso{/pgfplots/every x scale tick label/.append style={#1}}%
	},
	/pgfplots/y tick scale label style/.belongs to family=/pgfplots/style commands,
	/pgfplots/y tick scale label style/.code={%
		\pgfkeysalso{/pgfplots/every y scale tick label/.append style={#1}}%
	},
	/pgfplots/tick style/.belongs to family=/pgfplots/style commands,
	/pgfplots/tick style/.code={%
		\pgfkeysalso{/pgfplots/every tick/.append style={#1}}%
	},
	/pgfplots/minor tick style/.belongs to family=/pgfplots/style commands,
	/pgfplots/minor tick style/.code={%
		\pgfkeysalso{/pgfplots/every minor tick/.append style={#1}}%
	},
	/pgfplots/major tick style/.belongs to family=/pgfplots/style commands,
	/pgfplots/major tick style/.code={%
		\pgfkeysalso{/pgfplots/every major tick/.append style={#1}}%
	},
	/pgfplots/x tick style/.belongs to family=/pgfplots/style commands,
	/pgfplots/x tick style/.code={%
		\pgfkeysalso{/pgfplots/every x tick/.append style={#1}}%
	},
	/pgfplots/minor x tick style/.belongs to family=/pgfplots/style commands,
	/pgfplots/minor x tick style/.code={%
		\pgfkeysalso{/pgfplots/every minor x tick/.append style={#1}}%
	},
	/pgfplots/major x tick style/.belongs to family=/pgfplots/style commands,
	/pgfplots/major x tick style/.code={%
		\pgfkeysalso{/pgfplots/every major x tick/.append style={#1}}%
	},
	/pgfplots/y tick style/.belongs to family=/pgfplots/style commands,
	/pgfplots/y tick style/.code={%
		\pgfkeysalso{/pgfplots/every y tick/.append style={#1}}%
	},
	/pgfplots/minor y tick style/.belongs to family=/pgfplots/style commands,
	/pgfplots/minor y tick style/.code={%
		\pgfkeysalso{/pgfplots/every minor y tick/.append style={#1}}%
	},
	/pgfplots/major y tick style/.belongs to family=/pgfplots/style commands,
	/pgfplots/major y tick style/.code={%
		\pgfkeysalso{/pgfplots/every major y tick/.append style={#1}}%
	},
	/pgfplots/grid style/.belongs to family=/pgfplots/style commands,
	/pgfplots/grid style/.code={%
		\pgfkeysalso{/pgfplots/every axis grid/.append style={#1}}%
	},
	/pgfplots/minor grid style/.belongs to family=/pgfplots/style commands,
	/pgfplots/minor grid style/.code={%
		\pgfkeysalso{/pgfplots/every minor grid/.append style={#1}}%
	},
	/pgfplots/major grid style/.belongs to family=/pgfplots/style commands,
	/pgfplots/major grid style/.code={%
		\pgfkeysalso{/pgfplots/every major grid/.append style={#1}}%
	},
	/pgfplots/x grid style/.belongs to family=/pgfplots/style commands,
	/pgfplots/x grid style/.code={%
		\pgfkeysalso{/pgfplots/every axis x grid/.append style={#1}}%
	},
	/pgfplots/minor x grid style/.belongs to family=/pgfplots/style commands,
	/pgfplots/minor x grid style/.code={%
		\pgfkeysalso{/pgfplots/every minor x grid/.append style={#1}}%
	},
	/pgfplots/major x grid style/.belongs to family=/pgfplots/style commands,
	/pgfplots/major x grid style/.code={%
		\pgfkeysalso{/pgfplots/every major x grid/.append style={#1}}%
	},
	/pgfplots/y grid style/.belongs to family=/pgfplots/style commands,
	/pgfplots/y grid style/.code={%
		\pgfkeysalso{/pgfplots/every axis y grid/.append style={#1}}%
	},
	/pgfplots/minor y grid style/.belongs to family=/pgfplots/style commands,
	/pgfplots/minor y grid style/.code={%
		\pgfkeysalso{/pgfplots/every minor y grid/.append style={#1}}%
	},
	/pgfplots/major y grid style/.belongs to family=/pgfplots/style commands,
	/pgfplots/major y grid style/.code={%
		\pgfkeysalso{/pgfplots/every major y grid/.append style={#1}}%
	},
	/pgfplots/disablelogfilter/.is if=pgfplots@disablelogfilter,
	/pgfplots/disablelogfilter/.default=true,
	/pgfplots/disablelogfilter/.belongs to family=/pgfplots,
	/pgfplots/disablelogfilter=false,
	/pgfplots/disabledatascaling/.is if=pgfplots@disabledatascaling,
	/pgfplots/disabledatascaling/.default=true,
	/pgfplots/disabledatascaling/.belongs to family=/pgfplots,
	/pgfplots/disabledatascaling=false,
	/pgfplots/hide x axis/.is if=pgfplots@hide@x,
	/pgfplots/hide x axis/.default=true,
	/pgfplots/hide x axis=false,
	/pgfplots/hide y axis/.is if=pgfplots@hide@y,
	/pgfplots/hide y axis/.default=true,
	/pgfplots/hide y axis=false,
	/pgfplots/hide axis/.style={%
		/pgfplots/hide x axis=#1,
		/pgfplots/hide y axis=#1,
	},
	/pgfplots/hide axis/.default=true,
	/pgfplots/every non boxed x axis/.style={%
		xtick align=center,
		enlarge x limits=false,
		x axis line style={-stealth}
	},
	/pgfplots/every non boxed y axis/.style={%
		ytick align=center,
		enlarge y limits=false,
		y axis line style={-stealth}
	},
	/pgfplots/every boxed x axis/.style={},
	/pgfplots/every boxed y axis/.style={},
%	/pgfplots/hide axis/.belongs to family=/pgfplots,
% sets \pgfplots@xaxislinesnum to
% box=0
% bottom=1
% middle=2 ( aliased with center )
% top=3
	/pgfplots/axis x line*/.is choice,
	/pgfplots/axis x line*/box/.code	={\def\pgfplots@xaxislinesnum{0}\def\pgfplots@xtickposnum{0}},
	/pgfplots/axis x line*/bottom/.code	={\def\pgfplots@xaxislinesnum{1}\def\pgfplots@xtickposnum{1}},
	/pgfplots/axis x line*/middle/.code	={\def\pgfplots@xaxislinesnum{2}\def\pgfplots@xtickposnum{2}},
	/pgfplots/axis x line*/center/.style	={/pgfplots/axis x line*/middle},
	/pgfplots/axis x line*/top/.code	={\def\pgfplots@xaxislinesnum{3}\def\pgfplots@xtickposnum{3}},
	/pgfplots/axis x line*/none/.code	={\def\pgfplots@xaxislinesnum{4}\def\pgfplots@xtickposnum{4}},
	/pgfplots/axis x line*=box,
	%
	/pgfplots/axis x line/.is choice,
	/pgfplots/axis x line/box/.style	={
		/pgfplots/axis x line*/box,
		/pgfplots/every boxed x axis
	},
	/pgfplots/axis x line/bottom/.style	={
		/pgfplots/axis x line*/bottom,
		/pgfplots/every non boxed x axis
	},
	/pgfplots/axis x line/middle/.code	={%
		\ifnum\pgfplots@yaxislinesnum=3 % if 'axis y line==right' then
			\pgfkeysalso{/pgfplots/every axis x label/.style={at={(current axis.left of origin)},anchor=south west}}%
		\else
			\pgfkeysalso{/pgfplots/every axis x label/.style={at={(current axis.right of origin)},anchor=south east}}%
		\fi
		\pgfkeysalso{/pgfplots/axis x line*/middle,
			/pgfplots/every non boxed x axis}%
	},
	/pgfplots/axis x line/center/.style	={/pgfplots/axis x line/middle},
	/pgfplots/axis x line/top/.code	={
		\ifnum\pgfplots@yaxislinesnum=2 % if 'axis y line==center' then
			\pgfkeysalso{
				/pgfplots/every axis y label/.style={at={(current axis.below origin)},anchor=south west}}%
		\fi
		\pgfkeysalso{%
			/pgfplots/axis x line*/top,
			/pgfplots/every axis x label/.style={at={(0.5,1)},anchor=south,yshift=15pt},
			/pgfplots/every non boxed x axis}%
	},
	/pgfplots/axis x line/none/.style	={axis x line*/none,hide x axis},
% sets \pgfplots@yaxislinesnum to
% box=0
% left=1
% center=2 ( aliased with middle )
% right=3
	/pgfplots/axis y line*/.is choice,
	/pgfplots/axis y line*/box/.code	={\def\pgfplots@yaxislinesnum{0}\def\pgfplots@ytickposnum{0}},
	/pgfplots/axis y line*/left/.code	={\def\pgfplots@yaxislinesnum{1}\def\pgfplots@ytickposnum{1}},
	/pgfplots/axis y line*/center/.code	={\def\pgfplots@yaxislinesnum{2}\def\pgfplots@ytickposnum{2}},
	/pgfplots/axis y line*/middle/.style	={/pgfplots/axis y line*/center},
	/pgfplots/axis y line*/right/.code	={\def\pgfplots@yaxislinesnum{3}\def\pgfplots@ytickposnum{3}},
	/pgfplots/axis y line*/none/.code	={\def\pgfplots@yaxislinesnum{4}\def\pgfplots@ytickposnum{4}},
	/pgfplots/axis y line*=box,
	%
	/pgfplots/axis y line/.is choice,
	/pgfplots/axis y line/box/.style	={
		/pgfplots/axis y line*/box,
		/pgfplots/every boxed y axis
	},
	/pgfplots/axis y line/left/.style	={
		/pgfplots/axis y line*/left,
		/pgfplots/every non boxed y axis
	},
	/pgfplots/axis y line/center/.code	={
		\ifnum\pgfplots@xaxislinesnum=3 % if 'axis x line==top' then
			\pgfkeysalso{%
				/pgfplots/every axis y label/.style={at={(current axis.below origin)},anchor=south west}}%
		\else
			\pgfkeysalso{%
				/pgfplots/every axis y label/.style={at={(current axis.above origin)},anchor=north west}}%
		\fi
		\pgfkeysalso{%
			/pgfplots/axis y line*/center,
			/pgfplots/every non boxed y axis}%
	},
	/pgfplots/axis y line/middle/.style	={/pgfplots/axis y line/center},
	/pgfplots/axis y line/right/.code	={%
		\ifnum\pgfplots@xaxislinesnum=2
			\pgfkeysalso{every axis x label/.style={at={(current axis.left of origin)},anchor=south west}}%
		\fi
		\pgfkeysalso{
			axis y line*/right,
			%every axis y label/.style={at={(1,1)},anchor=north west,xshift=15pt},
			every axis y label/.style={at={(1,0.5)},xshift=33pt,rotate=90},
			/pgfplots/every non boxed y axis
		}%
	},%
	/pgfplots/axis y line/none/.style	={axis y line*/none,hide y axis},
% set \pgfplots@xaxisdiscontnum
% none = 0
% crunch = 1
% open = 2
	/pgfplots/axis x discontinuity/.is choice,
	/pgfplots/axis x discontinuity/.belongs to family=/pgfplots, %/axis,
	/pgfplots/axis x discontinuity/none/.code	={\def\pgfplots@xaxisdiscontnum{0}},
	/pgfplots/axis x discontinuity/none/.belongs to family=/pgfplots, %/axis,
	/pgfplots/axis x discontinuity/crunch/.code	={\def\pgfplots@xaxisdiscontnum{1}},
	/pgfplots/axis x discontinuity/crunch/.belongs to family=/pgfplots, %/axis,
	/pgfplots/axis x discontinuity/parallel/.code	={\def\pgfplots@xaxisdiscontnum{2}},
	/pgfplots/axis x discontinuity/parallel/.belongs to family=/pgfplots, %/axis,
	/pgfplots/axis x discontinuity=none,
% set \pgfplots@yaxisdiscontnum
% none = 0
% crunch = 1
% open = 2
	/pgfplots/axis y discontinuity/.is choice,
	/pgfplots/axis y discontinuity/.belongs to family=/pgfplots, %/axis,
	/pgfplots/axis y discontinuity/none/.code	={\def\pgfplots@yaxisdiscontnum{0}},
	/pgfplots/axis y discontinuity/none/.belongs to family=/pgfplots, %/axis,
	/pgfplots/axis y discontinuity/crunch/.code	={\def\pgfplots@yaxisdiscontnum{1}},
	/pgfplots/axis y discontinuity/crunch/.belongs to family=/pgfplots, %/axis,
	/pgfplots/axis y discontinuity/parallel/.code	={\def\pgfplots@yaxisdiscontnum{2}},
	/pgfplots/axis y discontinuity/parallel/.belongs to family=/pgfplots, %/axis,
	/pgfplots/axis y discontinuity=none,
	/pgfplots/scale only axis/.is if=pgfplots@scale@only@axis,
	/pgfplots/scale only axis/.default=true,
	/pgfplots/scale only axis/.belongs to family=/pgfplots,
	/pgfplots/scale only axis=false,
% sets \pgfplots@xislinear to
% normal=true
% log=false
	/pgfplots/xmode/.is choice,
	/pgfplots/xmode/.belongs to family=/pgfplots/scale,
	/pgfplots/xmode/normal/.code={\pgfplots@xislineartrue},
	/pgfplots/xmode/normal/.belongs to family=/pgfplots/scale,
	/pgfplots/xmode/linear/.code={\pgfplots@xislineartrue},
	/pgfplots/xmode/linear/.belongs to family=/pgfplots/scale,
	/pgfplots/xmode/log/.code={\pgfplots@xislinearfalse},
	/pgfplots/xmode/log/.belongs to family=/pgfplots/scale,
	/pgfplots/xmode=linear,
	/pgfplots/ymode/.is choice,
	/pgfplots/ymode/.belongs to family=/pgfplots/scale,
	/pgfplots/ymode/normal/.code={\pgfplots@yislineartrue},
	/pgfplots/ymode/normal/.belongs to family=/pgfplots/scale,
	/pgfplots/ymode/linear/.code={\pgfplots@yislineartrue},
	/pgfplots/ymode/linear/.belongs to family=/pgfplots/scale,
	/pgfplots/ymode/log/.code={\pgfplots@yislinearfalse},
	/pgfplots/ymode/log/.belongs to family=/pgfplots/scale,
	/pgfplots/ymode=linear,
	/pgfplots/error bars/x fixed/.code=				\def\pgfplots@errorbars@xfixed{#1}\def\pgfplots@errorbars@xmode{0},
	/pgfplots/error bars/x fixed relative/.code=		\def\pgfplots@errorbars@xrel{#1}\def\pgfplots@errorbars@xmode{1},
	/pgfplots/error bars/x explicit/.code=			\def\pgfplots@errorbars@xmode{2},
	/pgfplots/error bars/x explicit relative/.code=	\def\pgfplots@errorbars@xmode{3},
	/pgfplots/error bars/x fixed relative=0,
	/pgfplots/error bars/x fixed=0,
	/pgfplots/error bars/y fixed/.code=				\def\pgfplots@errorbars@yfixed{#1}\def\pgfplots@errorbars@ymode{0},
	/pgfplots/error bars/y fixed relative/.code=		\def\pgfplots@errorbars@yrel{#1}\def\pgfplots@errorbars@ymode{1},
	/pgfplots/error bars/y explicit/.code=			\def\pgfplots@errorbars@ymode{2},
	/pgfplots/error bars/y explicit relative/.code=	\def\pgfplots@errorbars@ymode{3},
	/pgfplots/error bars/y fixed relative=0,
	/pgfplots/error bars/y fixed=0,
	/pgfplots/error bars/x dir/.is choice,
	/pgfplots/error bars/x dir/none/.code={%
		\def\pgfplots@errorbars@xdirection{0}%
		\ifnum\pgfplots@errorbars@ydirection=0
			\pgfplots@errorbars@enabledfalse
		\fi
	},
	/pgfplots/error bars/x dir/plus/.code=				\def\pgfplots@errorbars@xdirection{1}\pgfplots@errorbars@enabledtrue,
	/pgfplots/error bars/x dir/minus/.code=				\def\pgfplots@errorbars@xdirection{2}\pgfplots@errorbars@enabledtrue,
	/pgfplots/error bars/x dir/both/.code=				\def\pgfplots@errorbars@xdirection{3}\pgfplots@errorbars@enabledtrue,
	/pgfplots/error bars/x dir=none,
	/pgfplots/error bars/y dir/.is choice,
	/pgfplots/error bars/y dir/none/.code={%
		\def\pgfplots@errorbars@ydirection{0}%
		\ifnum\pgfplots@errorbars@xdirection=0
			\pgfplots@errorbars@enabledfalse
		\fi
	},
	/pgfplots/error bars/y dir/plus/.code=				\def\pgfplots@errorbars@ydirection{1}\pgfplots@errorbars@enabledtrue,
	/pgfplots/error bars/y dir/minus/.code=				\def\pgfplots@errorbars@ydirection{2}\pgfplots@errorbars@enabledtrue,
	/pgfplots/error bars/y dir/both/.code=				\def\pgfplots@errorbars@ydirection{3}\pgfplots@errorbars@enabledtrue,
	/pgfplots/error bars/y dir=none,
	/pgfplots/error bars/error mark/.initial={-},
	/pgfplots/error bars/error mark options/.initial={rotate=90},
	/pgfplots/error bars/error bar style/.code={%
		\pgfkeysalso{/pgfplots/every error bar/.append style={#1}}%
	},
	/pgfplots/every error bar/.style={thin},
	/pgfplots/every error bar/.append code={\pgfplotsdeprecatedstylecheck{/tikz/every error bar}},
	/pgfplots/error bars/draw error bar/.code 2 args={%
%\message{/pgfplots/error bars/draw error bar:  working with '#1' -- '#2'.}%
		\pgfkeysgetvalue{/pgfplots/error bars/error mark}{\pgfplotserrorbarsmark}%
		\pgfkeysgetvalue{/pgfplots/error bars/error mark options}{\pgfplotserrorbarsmarkopts}%
		\draw #1 -- #2 node[pos=1,sloped,allow upside down] {%
			\expandafter\tikz\expandafter[\pgfplotserrorbarsmarkopts]{%
				\expandafter\pgfuseplotmark\expandafter{\pgfplotserrorbarsmark}%
				\pgfusepath{stroke}}%
		};
	},
	/pgfplots/bar cycle list/.style={/pgfplots/cycle list={%
		{blue,fill=blue!30!white,mark=none},%
		{red,fill=red!30!white,mark=none},%
		{brown!60!black,fill=brown!30!white,mark=none},%
		{black,fill=gray,mark=none},%
		}
	},
	/pgfplots/area cycle list/.style={bar cycle list},
	/pgfplots/area legend/.style={%
		/pgfplots/legend image code/.code={%
			\draw[##1] (0cm,-0.1cm) rectangle (0.6cm,0.1cm);
		}%
	},
	/pgfplots/area style/.style={%
		area cycle list,
		area legend,
		axis on top,
	},
	/pgfplots/ybar/.style={
		bar cycle list,
		xtick align=outside,
		/pgfplots/legend image code/.code={\draw[##1,bar width=3pt,yshift=-0.2em,bar shift=0pt] plot coordinates {(0cm,0.8em) (2*\pgfplotbarwidth,0.6em)};},
		/pgf/bar shift={%
				% total width = n*w + (n-1)*skip
				% -> subtract half for centering
				-0.5*(\numplots*\pgfplotbarwidth + (\numplots-1)*#1)  + 
				% the '0.5*w' is for centering
				(.5+\plotnum)*\pgfplotbarwidth + \plotnum*#1},%
		/tikz/ybar,
	},
	/pgfplots/ybar/.default=2pt,
	/pgfplots/ybar/.belongs to family=/pgfplots,
	/pgfplots/xbar/.style={
		bar cycle list,
		ytick align=outside,
		/pgfplots/legend image code/.code={\draw[##1,bar width=3pt,yshift=-0.2em,bar shift=0pt] plot coordinates {(0cm,0.8em) (2*\pgfplotbarwidth,0.6em)};},
		/pgf/bar shift={%
				% total width = n*w + (n-1)*skip
				% -> subtract half for centering
				-0.5*(\numplots*\pgfplotbarwidth + (\numplots-1)*#1)  + 
				% the '0.5*w' is for centering
				(.5+\plotnum)*\pgfplotbarwidth + \plotnum*#1},%
		/tikz/xbar,
	},
	/pgfplots/xbar/.default=2pt,
	/pgfplots/xbar/.belongs to family=/pgfplots,
	/pgfplots/ybar interval/.style={%
		bar cycle list,
		x tick label as interval,
		xmajorgrids,
		xtick align=outside,
	%	xtick=data,
		/pgfplots/legend image code/.code={\draw[##1,yshift=-0.2em,bar interval width=0.7,bar interval shift=0.5] plot coordinates {(0cm,0.8em) (5pt,0.6em) (10pt,0.6em)};},
		bar interval width={#1/\numplots},
		bar interval shift={(\plotnum+0.5)/\numplots},
		/tikz/ybar interval,
	},
	/pgfplots/ybar interval/.default=1,
	/pgfplots/ybar interval/.belongs to family=/pgfplots,
	/pgfplots/xbar interval/.style={%
		bar cycle list,
		y tick label as interval,
	%	ytick=data,
		ymajorgrids,
		ytick align=outside,
		/pgfplots/legend image code/.code={\draw[##1,yshift=-0.2em,bar interval width=0.7,bar interval shift=0.5] plot coordinates {(0cm,0.8em) (5pt,0.6em) (10pt,0.6em)};},
		bar interval width={#1/\numplots},
		bar interval shift={(\plotnum+0.5)/\numplots},
		/tikz/xbar interval,
	},
	/pgfplots/xbar interval/.default=1,
	/pgfplots/xbar interval/.belongs to family=/pgfplots,
	/pgfplots/xbar stacked/.style={
		bar cycle list,
		stack plots=x,
		stack dir=#1,
		/tikz/xbar,
	},
	/pgfplots/xbar stacked/.default=plus,
	/pgfplots/xbar stacked/.belongs to family=/pgfplots,
	/pgfplots/ybar stacked/.style={
		bar cycle list,
		stack plots=y,
		stack dir=#1,
		/tikz/ybar,
	},
	/pgfplots/ybar stacked/.default=plus,
	/pgfplots/ybar stacked/.belongs to family=/pgfplots,
	/pgfplots/xbar interval stacked/.style={
		bar cycle list,
		stack plots=x,
		stack dir=#1,
		/tikz/xbar interval,
	},
	/pgfplots/xbar interval stacked/.default=plus,
	/pgfplots/xbar interval stacked/.belongs to family=/pgfplots,
	/pgfplots/ybar interval stacked/.style={
		bar cycle list,
		stack plots=y,
		stack dir=#1,
		/tikz/ybar interval,
	},
	/pgfplots/ybar interval stacked/.default=plus,
	/pgfplots/ybar interval stacked/.belongs to family=/pgfplots,
	/pgfplots/yticklabel interval boundaries/.style={%
		y tick label as interval,
		yticklabel={$\pgfmathprintnumber{\tick}$ -- $\pgfmathprintnumber{\nexttick}$}
	},
	/pgfplots/xticklabel interval boundaries/.style={%
		x tick label as interval,
		xticklabel={$\pgfmathprintnumber{\tick}$ -- $\pgfmathprintnumber{\nexttick}$}
	},
	/pgfplots/plot file/skip first/.is if=pgfplots@plot@file@skipfirst,
	/pgfplots/plot file/skip first/.default=true,
	/pgfplots/clip marker paths/.is if=pgfplots@clip@marker@paths,
	/pgfplots/clip marker paths/.default=true,
	/pgfplots/axis on top/.is if=pgfplots@axis@on@top,
	/pgfplots/axis on top/.default=true,
	/pgfplots/every crossref picture/.style={%
		baseline,yshift=0.3em
	},
	/pgfplots/x coord trafo/.code={},
	/pgfplots/x coord inv trafo/.code={},
	/pgfplots/y coord trafo/.code={},
	/pgfplots/y coord inv trafo/.code={},
}

{
\pgfkeysdef{/pgfplots/empty command key}{}%
\pgfkeysgetvalue{/pgfplots/empty command key/.@cmd}\pgfplots@loc@TMPa
\global\let\pgfplots@empty@command@key=\pgfplots@loc@TMPa
}

\def\pgfplots@cmdkey@alias#1=#2;{%
	\pgfkeysgetvalue{/pgfplots/#2/.@cmd}\pgfplots@glob@TMPa
	\pgfkeyslet{/pgfplots/#1/.@cmd}\pgfplots@glob@TMPa
}%
\pgfplots@cmdkey@alias xlabel style=x label style;
\pgfplots@cmdkey@alias ylabel style=y label style;
\pgfplots@cmdkey@alias xticklabel style=x tick label style;
\pgfplots@cmdkey@alias yticklabel style=y tick label style;
%\pgfplots@cmdkey@alias xtick scale label style=x tick scale label style;
%\pgfplots@cmdkey@alias ytick scale label style=y tick scale label style;
\pgfplots@cmdkey@alias xtick style=x tick style;
\pgfplots@cmdkey@alias ytick style=y tick style;

\newif\ifpgfplots@log@tick@isminor@tick@pos
% Checks whether the tick position given as #1.#2=log10(T) belongs to
% T=i*10^j with an integer i>1.
%
% If T=i*10^j,  \ifpgfplots@log@tick@isminor@tick@pos will be set to true and
% \pgfmathresult will contain T.
%
% Otherwise, \ifpgfplots@log@tick@isminor@tick@pos will be set to false and
% pgfmathresult to #1.#2
%
% Arguments:
% #1.#2  the value log10(T)
%
% Implementation:  
% if T = i*10^j,  log10(T) = log10(i) + j.
% That means if log10(T) in \Z,  we have T = 10^j. If not, we need to
% check wether i is an integer. Please note that log10(i) < 1.
%
% Further note: log(T) < 0 <=>  j<0.
% In case j<0, we have 
%   #1.#2 = j + log(i) 
%         = - ( -j - log(i) ) 
%         = - ( -j - 1  + (1-log(i)) )
%         = #1 '.' #2 [ up to the '0.'
% that means #1 = j-1  and #2 = 1-log(i).
\def\pgfplots@is@log@tick@a@minor@tick@pos#1.#2\relax{%
	\pgfmathapproxequalto@{#1.#2}{#1.0}%
	\ifpgfmathcomparison
		% in MOST cases, this here will be true:
		\pgfplots@log@tick@isminor@tick@posfalse
		\def\pgfmathresult{#1.#2}%
	\else
		% I guess this won't happen too often. In fact, it's a very
		% special case.
		\begingroup
		\c@pgf@counta=#1\relax
		\ifnum\c@pgf@counta<0
			\advance\c@pgf@counta by-1
			\pgfmathsubtract@{1}{0.#2}%
			\expandafter\pgfplots@is@log@tick@a@minor@tick@pos@IDENTIFY@LOGi\pgfmathresult\relax
			\ifpgfplots@log@tick@isminor@tick@pos
				\aftergroup\pgfplots@log@tick@isminor@tick@postrue
				\edef\pgfmathresult{\pgfmathresult e\the\c@pgf@counta}%
			\else
			\aftergroup\pgfplots@log@tick@isminor@tick@posfalse
				\def\pgfmathresult{#1.#2}%
			\fi
		\else
			\pgfplots@is@log@tick@a@minor@tick@pos@IDENTIFY@LOGi0.#2\relax
			\ifpgfplots@log@tick@isminor@tick@pos
				\aftergroup\pgfplots@log@tick@isminor@tick@postrue
				\edef\pgfmathresult{\pgfmathresult e\the\c@pgf@counta}%
			\else
				\aftergroup\pgfplots@log@tick@isminor@tick@posfalse
				\def\pgfmathresult{#1.#2}%
			\fi
		\fi
		\pgfmath@smuggleone\pgfmathresult
		\endgroup
	\fi
}

% expects a positive number.
\def\pgfplots@is@log@tick@a@minor@tick@pos@IDENTIFY@LOGi0.#1\relax{%
	\pgfplots@log@tick@isminor@tick@postrue
	\pgfmathapproxequalto@{0.#1}{0.3010299956639}%
	\ifpgfmathcomparison
		\def\pgfmathresult{2}%
	\else
		\pgfmathapproxequalto@{0.#1}{0.4771212547196}%
		\ifpgfmathcomparison
			\def\pgfmathresult{3}%
		\else
			\pgfmathapproxequalto@{0.#1}{0.6020599913279}%
			\ifpgfmathcomparison
				\def\pgfmathresult{4}%
			\else
				\pgfmathapproxequalto@{0.#1}{0.698970004}%
				\ifpgfmathcomparison
					\def\pgfmathresult{5}%
				\else
					\pgfmathapproxequalto@{0.#1}{0.7781512503}%
					\ifpgfmathcomparison
						\def\pgfmathresult{6}%
					\else
						\pgfmathapproxequalto@{0.#1}{0.8450980400}%
						\ifpgfmathcomparison
							\def\pgfmathresult{7}%
						\else
							\pgfmathapproxequalto@{0.#1}{0.9030899869}%
							\ifpgfmathcomparison
								\def\pgfmathresult{8}%
							\else
								\pgfmathapproxequalto@{0.#1}{0.954242509439}%
								\ifpgfmathcomparison
									\def\pgfmathresult{9}%
								\else
									\pgfplots@log@tick@isminor@tick@posfalse
								\fi
							\fi
						\fi
					\fi
				\fi
			\fi
		\fi
	\fi
}


\def\pgfplots@set@at#1{\def\pgfplots@at{#1}}%



% converts a comma-separated list (PGF foreach)  to my internal list
% structure.
\long\def\pgfplots@foreach@to@list#1\to#2{%
	\global\pgfplotslistnewempty\pgfplots@glob@TMPa
	\begingroup
	\foreach \pgfplots@i in {#1} {%
		\expandafter\pgfplotslistpushbackglobal\pgfplots@i\to\pgfplots@glob@TMPa
	}%
	\endgroup
	\pgfplotslistcopy\pgfplots@glob@TMPa\to#2\relax
}

% Several tick options:
\long\def\axispreset#1{%
	\pgfplotsset{every axis/.append style={#1}}%
}
\long\def\legendpreset#1{%
	\pgfplots@error{Sorry, legendpreset is now deprecated, along with the legend options text width and font. Legends are now TikZ-matrizes which provide better alignment and can be placed horizontally. See the manual for details.}%
}

% Checks whether we need to create a separate 'tick scale label',
% a node with ' * 10^3' on the side of the axis:
%
% PRECONDITION:
%    Axis limits for #1 are given. I need their values before any data
%    scale transformation has been applied.
%    If  
%    	\pgfplots@#1min@unscaled@as@float 
%    and
%    	\pgfplots@#1max@unscaled@as@float 
%    exist; I will use these macros.
%    Otherwise, I will use \pgfplots@#1min and \pgfplots@#1max;
%    assuming that no data scale transformation is active.
%    FIXME : does that need further attention?
\def\pgfplots@init@scaled@tick@for#1{%
	\begingroup
	% the \pgfplots@xmin@unscaled@as@float  is set just before the data
	% scale transformation is initialised.
	%
	% The variables are empty if there is no datascale transformation.
	\expandafter\let\expandafter\pgfplots@cur@min@unscaled\csname pgfplots@#1min@unscaled@as@float\endcsname
	\expandafter\let\expandafter\pgfplots@cur@max@unscaled\csname pgfplots@#1max@unscaled@as@float\endcsname
	%
	\ifx\pgfplots@cur@min@unscaled\pgfutil@empty
		\edef\pgfplots@loc@TMPa{\csname pgfplots@#1min\endcsname}%
		\expandafter\pgfmathfloatparsenumber\expandafter{\pgfplots@loc@TMPa}%
		\let\pgfplots@cur@min@unscaled=\pgfmathresult
		\edef\pgfplots@loc@TMPa{\csname pgfplots@#1max\endcsname}%
		\expandafter\pgfmathfloatparsenumber\expandafter{\pgfplots@loc@TMPa}%
		\let\pgfplots@cur@max@unscaled=\pgfmathresult
	\fi
	%
	\expandafter\pgfmathfloat@decompose@E\pgfplots@cur@min@unscaled\relax\pgfmathfloat@a@E
	\expandafter\pgfmathfloat@decompose@E\pgfplots@cur@max@unscaled\relax\pgfmathfloat@b@E
	\ifnum\pgfmathfloat@b@E<\pgfmathfloat@a@E
		\pgfmathfloat@b@E=\pgfmathfloat@a@E
	\fi
	\xdef\pgfplots@glob@TMPa{\pgfplots@scale@ticks@above@exponent}%
	\expandafter\ifnum\pgfplots@glob@TMPa<\pgfmathfloat@b@E
		% ok, scale it:
		\multiply\pgfmathfloat@b@E by-1
		\xdef\pgfplots@glob@TMPa{\the\pgfmathfloat@b@E}%
	\else
		\xdef\pgfplots@glob@TMPa{\pgfplots@scale@ticks@below@exponent}%
		\expandafter\ifnum\pgfplots@glob@TMPa>\pgfmathfloat@b@E
			% ok, scale it:
			\multiply\pgfmathfloat@b@E by-1
			\xdef\pgfplots@glob@TMPa{\the\pgfmathfloat@b@E}%
		\else
			% no scaling necessary:
			\xdef\pgfplots@glob@TMPa{0}%
		\fi
	\fi
	\endgroup
	\expandafter\let\csname pgfplots@tick@scale@#1\endcsname=\pgfplots@glob@TMPa%
}

% x-axis tick labels for #1th tick
% #1: the axis (x or y)
% #2: the value
% #3,#4: coordinates for tikz
% #5: ticknumber
\def\pgfplots@show@ticklabel#1#2(#3,#4)#5{{%
	\csname ifpgfplots@#1ticklabel@interval\endcsname
		\pgfmathparse{#3}%
		\edef\pgfplots@show@ticklabel@coord@x@new{\pgfmathresult pt}%
		\pgfmathparse{#4}%
		\edef\pgfplots@show@ticklabel@coord@y@new{\pgfmathresult pt}%
		%
		\pgfplots@show@ticklabel@{#1}{#2}%
		\let\nexttick=\tick
		\ifx\pgfplots@show@ticklabel@LASTTICK\pgfutil@empty
			% its the first call. Simply remember arguments and wait
			% for interval boundary before proceeding.
		\else
			% acquire options of first interval boundary:
			\pgfplots@show@ticklabel@LASTTICK
			% compute new node position:
			\pgfmathparse{0.5*(\csname pgfplots@show@ticklabel@coord@#1\endcsname + \csname pgfplots@show@ticklabel@coord@#1@new\endcsname)}%
			\expandafter\edef\csname pgfplots@show@ticklabel@coord@#1\endcsname{\pgfmathresult pt}%
			\let\ticknum=\pgfplots@show@ticklabel@num\relax%
			\let\tick=\pgfplots@show@ticklabel@tick%
			\edef\pgfplots@loc@TMPa{at (\pgfplots@show@ticklabel@coord@x,\pgfplots@show@ticklabel@coord@y)}%
			\expandafter\node\pgfplots@loc@TMPa
				{\csname pgfplots@#1ticklabel\endcsname};%
		\fi
		\xdef\pgfplots@show@ticklabel@LASTTICK{%
			\noexpand\def\noexpand\pgfplots@show@ticklabel@tick{\nexttick}%
			\noexpand\def\noexpand\pgfplots@show@ticklabel@coord@x{\pgfplots@show@ticklabel@coord@x@new}%
			\noexpand\def\noexpand\pgfplots@show@ticklabel@coord@y{\pgfplots@show@ticklabel@coord@y@new}%
			\noexpand\edef\noexpand\pgfplots@show@ticklabel@num{#5}%
		}%
	\else
		\let\ticknum=#5\relax%
		\pgfplots@show@ticklabel@{#1}{#2}%
		\node at (#3,#4) {\csname pgfplots@#1ticklabel\endcsname};%
	\fi
}}

% Defines \tick by applying any necessary math to the (possibly
% transformed) tick value #2.
%
% #1: axis (x or y)
% #2: tick value.
\def\pgfplots@show@ticklabel@#1#2{%
	\csname ifpgfplots@apply@datatrafo@#1\endcsname
		\csname pgfplots@inverse@datascaletrafo@#1\endcsname{#2}%
		\pgfplots@if{pgfplots@scaled@ticks@#1}{%
			\expandafter\pgfmathfloatshift@\expandafter{\pgfmathresult}{\csname pgfplots@tick@scale@#1\endcsname}%
		}\relax
		% .. and this here provides \tick as fixed point repr:
		\expandafter\pgfmathfloattofixed\expandafter{\pgfmathresult}%
		\let\tick=\pgfmathresult
	\else
		\edef\tick{#2}%
		\pgfplots@if{pgfplots@#1islinear}{%
			\pgfplots@if{pgfplots@scaled@ticks@#1}{%
				\pgfmathfloatparsenumber{#2}%
				\expandafter\pgfmathfloatshift@\expandafter{\pgfmathresult}{\csname pgfplots@tick@scale@#1\endcsname}%
				\expandafter\pgfmathfloattofixed\expandafter{\pgfmathresult}%
				\let\tick=\pgfmathresult
			}{}%
		}{}%
	\fi
	\pgfkeysgetvalue{/pgfplots/#1 coord inv trafo/.@cmd}\pgfplots@loc@TMPa
	\ifx\pgfplots@loc@TMPa\pgfplots@empty@command@key
	\else
		\let\pgfmathresult=\tick%
		\expandafter\pgfplots@loc@TMPa\expandafter{\tick}\pgfeov
		\let\tick=\pgfmathresult
	\fi
}%

\def\pgfplots@user@ticklabel@list@x{%
	\pgfplotslistselectorempty\ticknum\of\pgfplots@xticklabels\to\tick
	\tick
}
\def\pgfplots@user@ticklabel@list@y{%
	\pgfplotslistselectorempty\ticknum\of\pgfplots@yticklabels\to\tick
	\tick
}
\def\pgfplots@user@extra@ticklabel@list@x{%
	\pgfplotslistselectorempty\ticknum\of\pgfplots@extra@xticklabels\to\tick
	\tick
}
\def\pgfplots@user@extra@ticklabel@list@y{%
	\pgfplotslistselectorempty\ticknum\of\pgfplots@extra@yticklabels\to\tick
	\tick
}


% #1 axis (x or y)
% #2 the label
\def\pgfplots@show@label#1#2{%
	\node 
		[/pgfplots/every axis label,%
		/pgfplots/every axis #1 label]
	{#2};
}

\def\pgfplots@show@title#1{%
	\node%
		[/pgfplots/every axis title]
		{#1};
}

% Check if a label does not cross the x-axis
\def\pgfplots@ytick@check@tickshow{%
	\pgfplots@tickshowtrue
	\ifnum\pgfplots@yaxislinesnum=2\relax
		\ifcase\pgfplots@xaxislinesnum\relax
			\ifdim\pgfplots@tmpa=\pgfplots@ycoordminTEX\relax
				\pgfplots@tickshowfalse
			\fi
			\ifdim\pgfplots@tmpa=\pgfplots@ycoordmaxTEX\relax
				\pgfplots@tickshowfalse
			\fi
		\or
			\ifdim\pgfplots@tmpa=\pgfplots@ycoordminTEX\relax
				\pgfplots@tickshowfalse
			\fi
		\or
			\ifdim\pgfplots@tmpa=\pgfplots@ZERO@y\relax
				\pgfplots@tickshowfalse
			\fi
		\or
			\ifdim\pgfplots@tmpa=\pgfplots@ycoordmaxTEX\relax
				\pgfplots@tickshowfalse
			\fi
		\fi
	\fi
}

% Fills the macros
%   \pgfplots@tick@beg@a \pgfplots@tick@end@a
%   \pgfplots@tick@beg@b \pgfplots@tick@end@b
% with coordinates such that 
%   (\pgfplots@tick@beg@a,\pgfplots@tmpa) -- (\pgfplots@tick@end@a,\pgfplots@tmpa)
% produces a correct tick line. 
%
% The '@b' variant is only used in case of \pgfplots@ytickposnum = 0
%
% #1 : the current axis (x or y).
% #2 : the axis which is NOT fixed. For x tick lines, this is the y
% axis and for y tick lines, this is the x axis (#1 = x or y)
% #3 : the current tick width
\def\pgfplots@prepare@tick@offsets@for@#1#2#3{%
	\ifcase\csname pgfplots@#1tickposnum\endcsname\relax
		%(\pgfplots@xcoordminTEX-\pgfplots@tick@offset, \pgfplots@tmpa) -- ++( #3, 0pt)
		\edef\pgfplots@tick@beg@a{\pgf@sys@tonumber{\csname pgfplots@#2coordminTEX\endcsname}}%
		\pgfmathsubtract@{\pgfplots@tick@beg@a}{\pgfplots@tick@offset}%
		\let\pgfplots@tick@beg@a=\pgfmathresult
		\pgfmathadd@{\pgfplots@tick@beg@a}{#3}%
		\edef\pgfplots@tick@beg@a{\pgfplots@tick@beg@a pt}%
		\edef\pgfplots@tick@end@a{\pgfmathresult pt}%
		%
		%(\pgfplots@xcoordmaxTEX+\pgfplots@tick@offset, \pgfplots@tmpa)	-- ++(-#3, 0pt)
		\edef\pgfplots@tick@beg@b{\pgf@sys@tonumber{\csname pgfplots@#2coordmaxTEX\endcsname}}%
		\pgfmathadd@{\pgfplots@tick@beg@b}{\pgfplots@tick@offset}%
		\let\pgfplots@tick@beg@b=\pgfmathresult
		\pgfmathsubtract@{\pgfplots@tick@beg@b}{#3}%
		\edef\pgfplots@tick@beg@b{\pgfplots@tick@beg@b pt}%
		\edef\pgfplots@tick@end@b{\pgfmathresult pt}%
	\or
		% (\pgfplots@xcoordminTEX-\pgfplots@tick@offset, \pgfplots@tmpa) -- ++( #3, 0pt);
		\edef\pgfplots@tick@beg@a{\pgf@sys@tonumber{\csname pgfplots@#2coordminTEX\endcsname}}%
		\pgfmathsubtract@{\pgfplots@tick@beg@a}{\pgfplots@tick@offset}%
		\let\pgfplots@tick@beg@a=\pgfmathresult
		\pgfmathadd@{\pgfplots@tick@beg@a}{#3}%
		\edef\pgfplots@tick@beg@a{\pgfplots@tick@beg@a pt}%
		\edef\pgfplots@tick@end@a{\pgfmathresult pt}%
	\or
		% (\pgfplots@ZERO@x      -\pgfplots@tick@offset, \pgfplots@tmpa) -- ++( #3, 0pt);
		\pgf@xa=\csname pgfplots@ZERO@#2\endcsname
		\edef\pgfplots@loc@TMPa{\pgf@sys@tonumber{\pgf@xa}}%
		\pgfmathsubtract@{\pgfplots@loc@TMPa}{\pgfplots@tick@offset}%
		\let\pgfplots@tick@beg@a=\pgfmathresult
		\pgfmathadd@{\pgfplots@tick@beg@a}{#3}%
		\edef\pgfplots@tick@beg@a{\pgfplots@tick@beg@a pt}%
		\edef\pgfplots@tick@end@a{\pgfmathresult pt}%
	\or
		% (\pgfplots@xcoordmaxTEX+\pgfplots@tick@offset, \pgfplots@tmpa)	-- ++(-#3, 0pt);
		\edef\pgfplots@tick@beg@a{\pgf@sys@tonumber{\csname pgfplots@#2coordmaxTEX\endcsname}}%
		\pgfmathadd@{\pgfplots@tick@beg@a}{\pgfplots@tick@offset}%
		\let\pgfplots@tick@beg@a=\pgfmathresult
		\pgfmathsubtract@{\pgfplots@tick@beg@a}{#3}%
		\edef\pgfplots@tick@beg@a{\pgfplots@tick@beg@a pt}%
		\edef\pgfplots@tick@end@a{\pgfmathresult pt}%
	\fi
}%

\def\pgfplots@drawyaxis@placecomputedtick{%
	\pgfpathmoveto{\pgfqpoint{\pgfplots@tick@beg@a}{\pgfplots@tmpa}}%
	\pgfpathlineto{\pgfqpoint{\pgfplots@tick@end@a}{\pgfplots@tmpa}}%
	\ifnum\pgfplots@ytickposnum=0\relax
		\pgfpathmoveto{\pgfqpoint{\pgfplots@tick@beg@b}{\pgfplots@tmpa}}%
		\pgfpathlineto{\pgfqpoint{\pgfplots@tick@end@b}{\pgfplots@tmpa}}%
	\fi
}%
\def\pgfplots@drawyaxis@placecomputedgridline{%
	\pgfpathmoveto{\pgfqpoint{\pgfplots@xcoordminTEX}{\pgfplots@tmpa}}%
	\pgfpathlineto{\pgfqpoint{\pgfplots@xcoordmaxTEX}{\pgfplots@tmpa}}%
}%

\newif\ifpgfplots@needsminorloop

\def\pgfplots@draw@tick@scale@label@for#1{%
	\csname ifpgfplots@#1islinear\endcsname
		\pgfplots@if{pgfplots@scaled@ticks@#1}{%
			\begingroup
				\xdef\pgfplots@glob@TMPa{\csname pgfplots@tick@scale@#1\endcsname}%
				\expandafter\c@pgf@counta\pgfplots@glob@TMPa\relax
				\multiply\c@pgf@counta by-1
				\ifnum\c@pgf@counta=0\relax
					\global\let\pgfplots@glob@TMPa=\pgfutil@empty
				\else
					\xdef\pgfplots@glob@TMPa{\the\c@pgf@counta}%
				\fi
			\endgroup
			\ifx\pgfplots@glob@TMPa\pgfutil@empty
			\else
				\edef\pgfplots@tick@scale@labels{\noexpand\pgfplots@invoke@pgfkeyscode{/pgfplots/tick scale label code/.@cmd}{\pgfplots@glob@TMPa}}%
				\node 
					[%
					xshift=\pgfplots@xcoordminTEX,%
					yshift=\pgfplots@ycoordminTEX,%
					x=\pgfplots@xcoordmaxTEX-\pgfplots@xcoordminTEX,%
					y=\pgfplots@ycoordmaxTEX-\pgfplots@ycoordminTEX,%
					/pgfplots/every tick label,%
					/pgfplots/every #1 tick label,%
					/pgfplots/every #1 tick scale label]
				{\pgfplots@tick@scale@labels};
			\fi
		}{\relax}%
	\fi
}

% Simply invokes the code of PGF key #1 with value #2, that means
% #1#2\pgfeov
\def\pgfplots@invoke@pgfkeyscode#1#2{%
	\pgfkeysgetvalue{#1}\pgfplots@invoke@pgfkeyscode@CODE
	\pgfplots@invoke@pgfkeyscode@CODE#2\pgfeov
}

% Check if the current tick position, stored in \pgfplots@tmpa, 
% does not cross the y-axis.
%
% This is just a special case for centered axis lines.
\def\pgfplots@xtick@check@tickshow{%
	\pgfplots@tickshowtrue
	\ifnum\pgfplots@xaxislinesnum=2\relax
		\ifcase\pgfplots@yaxislinesnum\relax
			\ifdim\pgfplots@tmpa=\pgfplots@xcoordminTEX\relax
				\pgfplots@tickshowfalse
			\fi
			\ifdim\pgfplots@tmpa=\pgfplots@xcoordmaxTEX\relax
				\pgfplots@tickshowfalse
			\fi
		\or
			\ifdim\pgfplots@tmpa=\pgfplots@xcoordminTEX\relax
				\pgfplots@tickshowfalse
			\fi
		\or
			\ifdim\pgfplots@tmpa=\pgfplots@ZERO@x\relax
				\pgfplots@tickshowfalse
			\fi
		\or
			\ifdim\pgfplots@tmpa=\pgfplots@xcoordmaxTEX\relax
				\pgfplots@tickshowfalse
			\fi
		\fi
	\fi
}

\def\pgfplots@drawxaxis@placecomputedtick{%
	\pgfpathmoveto{\pgfqpoint{\pgfplots@tmpa}{\pgfplots@tick@beg@a}}%
	\pgfpathlineto{\pgfqpoint{\pgfplots@tmpa}{\pgfplots@tick@end@a}}%
	\ifnum\pgfplots@xtickposnum=0\relax
		\pgfpathmoveto{\pgfqpoint{\pgfplots@tmpa}{\pgfplots@tick@beg@b}}%
		\pgfpathlineto{\pgfqpoint{\pgfplots@tmpa}{\pgfplots@tick@end@b}}%
	\fi
}%
\def\pgfplots@drawxaxis@placecomputedgridline{%
	\pgfpathmoveto{\pgfqpoint{\pgfplots@tmpa}{\pgfplots@ycoordminTEX}}%
	\pgfpathlineto{\pgfqpoint{\pgfplots@tmpa}{\pgfplots@ycoordmaxTEX}}%
}%

% #1: axis (x or y)
% #2: axis index (0 or 1)
% #3: tick position list
\def\pgfplots@draw@extra@ticks@for#1#2#3{%
	\begingroup
	\pgfplots@scaled@ticks@xfalse
	\pgfplots@scaled@ticks@yfalse
	\csname pgfplots@#1minorticksfalse\endcsname
	\csname pgfplots@#1minorgridsfalse\endcsname
	\expandafter\let\expandafter\axis@TMP\csname pgfplots@extra@#1ticklabel\endcsname
	\expandafter\let\csname pgfplots@#1ticklabel\endcsname=\axis@TMP
	\pgfplotsset{/pgfplots/every extra #1 tick}% FIXME : used 'search path for tikz' before...
	\pgfplots@prepare@ticks@for{#3}{#1}{#2}%
	\pgfplots@drawgridlines@for{#1}{#2}%
	\pgfplots@drawticklines@for{#1}{#2}%
	\pgfplots@drawticklabels@for{#1}{#2}%
	\endgroup
}

\def\pgfplots@drawaxis@innerlines{%
	\ifpgfplots@hide@y\else
		\ifnum\pgfplots@yaxislinesnum=2
			\draw[/pgfplots/every inner y axis line,%
				decorate,%
				ydiscont,%
				decoration={pre length=\ydisstart, post length=\ydisend}]
				(\pgfplots@ZERO@x,	\pgfplots@ycoordminTEX) -- (\pgfplots@ZERO@x,	\pgfplots@ycoordmaxTEX);
		\fi
	\fi
	\ifpgfplots@hide@x\else
		\ifnum\pgfplots@xaxislinesnum=2
			\draw[/pgfplots/every inner x axis line,%
				decorate,%
				xdiscont,%
				decoration={pre length=\xdisstart, post length=\xdisend}]
				(\pgfplots@xcoordminTEX, \pgfplots@ZERO@y) -- (\pgfplots@xcoordmaxTEX, \pgfplots@ZERO@y);
		\fi
	\fi
}%

% Ok, we don't mind whether edges with thick lines look ugly. We just
% draw separate lines. This here is necessary if we want arrow heads.
\def\pgfplots@drawaxis@outerlines@separate{%
	\ifpgfplots@hide@x
	\else
		\scope[/pgfplots/every outer x axis line,
			xdiscont,decoration={pre length=\xdisstart, post length=\xdisend}]
		\ifcase\pgfplots@xaxislinesnum
			\draw decorate { 
					(\pgfplots@xcoordminTEX,\pgfplots@ycoordminTEX) 
				--	(\pgfplots@xcoordmaxTEX,\pgfplots@ycoordminTEX) };
			\draw decorate {
					(\pgfplots@xcoordminTEX,\pgfplots@ycoordmaxTEX)
				--	(\pgfplots@xcoordmaxTEX,\pgfplots@ycoordmaxTEX) };

		\or
			\draw decorate { 
					(\pgfplots@xcoordminTEX,\pgfplots@ycoordminTEX) 
				--	(\pgfplots@xcoordmaxTEX,\pgfplots@ycoordminTEX) };
		\or 
		\or
			\draw decorate {
					(\pgfplots@xcoordminTEX,\pgfplots@ycoordmaxTEX)
				--	(\pgfplots@xcoordmaxTEX,\pgfplots@ycoordmaxTEX) };

		\fi
		\endscope
	\fi
	\ifpgfplots@hide@y
	\else
		\scope[/pgfplots/every outer y axis line,
			ydiscont,decoration={pre length=\ydisstart, post length=\ydisend}]
		\ifcase\pgfplots@yaxislinesnum
			\draw decorate { 
					(\pgfplots@xcoordminTEX,\pgfplots@ycoordminTEX) 
				--	(\pgfplots@xcoordminTEX,\pgfplots@ycoordmaxTEX) };
			\draw decorate {
					(\pgfplots@xcoordmaxTEX,\pgfplots@ycoordminTEX)
				--	(\pgfplots@xcoordmaxTEX,\pgfplots@ycoordmaxTEX) };

		\or
			\draw decorate { 
					(\pgfplots@xcoordminTEX,\pgfplots@ycoordminTEX) 
				--	(\pgfplots@xcoordminTEX,\pgfplots@ycoordmaxTEX) };
		\or 
		\or
			\draw decorate {
					(\pgfplots@xcoordmaxTEX,\pgfplots@ycoordminTEX)
				--	(\pgfplots@xcoordmaxTEX,\pgfplots@ycoordmaxTEX) };

		\fi
		\endscope
	\fi
}%

% This here is complicated: we try to create good edges and draw a
% SINGLE path for the partial or complete rectangle
%
%  -----
%  |   |
%  |   |
%  -----
\def\pgfplots@drawaxis@outerlines@cycledpath{%
	\draw[
		/pgfplots/every outer x axis line, % FIXME! these outer styles need much more attention :-(
		/pgfplots/every outer y axis line]
	(\pgfplots@xcoordminTEX,	\pgfplots@ycoordminTEX)
\ifpgfplots@hide@y
	{ (\pgfplots@xcoordminTEX,	\pgfplots@ycoordmaxTEX) }
\else
 	\ifcase\pgfplots@yaxislinesnum
	    decorate [ydiscont,decoration={pre length=\ydisstart, post length=\ydisend}] { -- (\pgfplots@xcoordminTEX,	\pgfplots@ycoordmaxTEX) }
	\or decorate [ydiscont,decoration={pre length=\ydisstart, post length=\ydisend}] { -- (\pgfplots@xcoordminTEX,	\pgfplots@ycoordmaxTEX) }
	\or { (\pgfplots@xcoordminTEX,	\pgfplots@ycoordmaxTEX) }
	\or { (\pgfplots@xcoordminTEX,	\pgfplots@ycoordmaxTEX) }
	\fi
\fi
\ifpgfplots@hide@x
	{ (\pgfplots@xcoordmaxTEX,	\pgfplots@ycoordmaxTEX) }
\else
	\ifcase\pgfplots@xaxislinesnum
	    decorate [xdiscont,decoration={pre length=\xdisstart, post length=\xdisend}] { -- (\pgfplots@xcoordmaxTEX,	\pgfplots@ycoordmaxTEX) }
	\or { (\pgfplots@xcoordmaxTEX,	\pgfplots@ycoordmaxTEX) }
	\or { (\pgfplots@xcoordmaxTEX,	\pgfplots@ycoordmaxTEX) }
	\or decorate [xdiscont,decoration={pre length=\xdisstart, post length=\xdisend}] { -- (\pgfplots@xcoordmaxTEX,	\pgfplots@ycoordmaxTEX) }
	\fi
\fi
\ifpgfplots@hide@y
	{ (\pgfplots@xcoordmaxTEX,	\pgfplots@ycoordminTEX) }
\else
	\ifcase\pgfplots@yaxislinesnum
	    decorate [ydiscont,decoration={pre length=\ydisend, post length=\ydisstart}] { -- (\pgfplots@xcoordmaxTEX,	\pgfplots@ycoordminTEX) }
	\or { (\pgfplots@xcoordmaxTEX,	\pgfplots@ycoordminTEX) }
	\or { (\pgfplots@xcoordmaxTEX,	\pgfplots@ycoordminTEX) }
	\or decorate [ydiscont,decoration={pre length=\ydisend, post length=\ydisstart}] { -- (\pgfplots@xcoordmaxTEX,	\pgfplots@ycoordminTEX) }
	\fi
\fi
\ifpgfplots@hide@x
	{ (\pgfplots@xcoordminTEX,	\pgfplots@ycoordminTEX) }
\else
	\ifcase\pgfplots@xaxislinesnum
	    decorate [xdiscont,decoration={pre length=\xdisend, post length=\xdisstart}] { -- (\pgfplots@xcoordminTEX,	\pgfplots@ycoordminTEX) }
	\or decorate [xdiscont,decoration={pre length=\xdisend, post length=\xdisstart}] { -- (\pgfplots@xcoordminTEX,	\pgfplots@ycoordminTEX) }
	\or { (\pgfplots@xcoordminTEX,	\pgfplots@ycoordminTEX) }
	\or { (\pgfplots@xcoordminTEX,	\pgfplots@ycoordminTEX) }
	\fi% can't use cycle here!
\fi
	; %	-- cycle;
}%

\def\pgfplots@drawaxis@outerlines{%
	\ifnum\pgfplots@xaxislinesnum>0
		\pgfplots@separate@axis@linestrue
	\fi
	\ifnum\pgfplots@yaxislinesnum>0
		\pgfplots@separate@axis@linestrue
	\fi
	\ifpgfplots@separate@axis@lines
		\pgfplots@drawaxis@outerlines@separate
	\else
		\pgfplots@drawaxis@outerlines@cycledpath
	\fi
}%

\def\pgfplots@drawaxis@lines{%
	\begingroup
	\begingroup
	% this group employs several temporary dimension registers
	% and is therefor scoped:
	\let\ydisstart=\pgf@xa
	\let\ydisend=\pgf@xb
	\let\xdisstart=\pgf@ya
	\let\xdisend=\pgf@yb
	\ydisend=\pgfplots@ycoordmaxTEX
	\advance \ydisend by -\pgfplots@ycoordminTEX
	\ifcase\pgfplots@yaxisdiscontnum\relax
		\let\ydiscontstyle=\pgfutil@empty
	\or
		\def\ydiscontstyle{decoration={zigzag,segment length=12pt, amplitude=4pt}}%
		\advance \ydisend by -16pt
	\or
		\def\ydiscontstyle{decoration={ticks,segment length=4pt, amplitude=8pt}}%
		\advance \ydisend by -8pt
	\fi
	\ifpgfplots@apply@datatrafo@y
		\advance \pgfplots@ycoordmaxTEX by\pgfplots@data@scale@trafo@SHIFT@y pt
	\fi
	\ifdim\pgfplots@ycoordmaxTEX<0pt
		\ydisstart=\ydisend
		\ydisend=4pt
	\else
		\ydisstart=4pt
	\fi
	\ifpgfplots@apply@datatrafo@y
		\advance \pgfplots@ycoordmaxTEX by-\pgfplots@data@scale@trafo@SHIFT@y pt
	\fi
	\xdisend=\pgfplots@xcoordmaxTEX
	\advance \xdisend by -\pgfplots@xcoordminTEX
	\ifcase\pgfplots@xaxisdiscontnum\relax
		\let\xdiscontstyle=\pgfutil@empty
	\or
		\def\xdiscontstyle{decoration={zigzag,segment length=12pt, amplitude=4pt}}%
		\advance \xdisend by -16pt
	\or
		\def\xdiscontstyle{decoration={ticks,segment length=4pt, amplitude=8pt}}%
		\advance \xdisend by -8pt
	\fi
	\ifpgfplots@apply@datatrafo@x
		\advance \pgfplots@xcoordmaxTEX by\pgfplots@data@scale@trafo@SHIFT@x pt
	\fi
	\ifdim\pgfplots@xcoordmaxTEX<0pt
		\xdisstart=\xdisend
		\xdisend=4pt
	\else
		\xdisstart=4pt
	\fi
	\ifpgfplots@apply@datatrafo@x
		\advance \pgfplots@xcoordmaxTEX by-\pgfplots@data@scale@trafo@SHIFT@x pt
	\fi
	% carry local computations outside of group:
	\xdef\pgfplots@glob@TMPa{%
		\noexpand\def\noexpand\xdisstart{\the\xdisstart}%
		\noexpand\def\noexpand\xdisend{\the\xdisend}%
		\noexpand\def\noexpand\ydisstart{\the\ydisstart}%
		\noexpand\def\noexpand\ydisend{\the\ydisend}%
		\noexpand\pgfkeys{%
			/tikz/xdiscont/.style={\xdiscontstyle},%
			/tikz/ydiscont/.style={\ydiscontstyle}}%
	}%
	\endgroup
	\pgfplots@glob@TMPa
	\pgfplots@drawaxis@outerlines%
	\pgfplots@drawaxis@innerlines%
	\endgroup
}%

% Computes final major and minor tick positions into global lists
% \pgfplots@prepared@tick@positions@major@x
% and
% \pgfplots@prepared@tick@positions@minor@x.
%
% The major tick list contains tuples (canvas position,logical position)
% while the minor tick list contains just the canvas position.
%
% #1: the tick list.
% #2: the axis name as character, i.e. 'x' or 'y'
% #3: the axis name as integer, i.e. 0 or 1
\def\pgfplots@prepare@ticks@for#1#2#3{%
	\begingroup
	\expandafter\let\expandafter\ifpgfplots@islinear\csname ifpgfplots@#2islinear\endcsname
	\expandafter\let\expandafter\ifpgfplots@minorticks\csname ifpgfplots@#2minorticks\endcsname
	\expandafter\let\expandafter\ifpgfplots@minorgrids\csname ifpgfplots@#2minorgrids\endcsname
	% these lists need to be global such that I can fill them inside
	% of \foreach statements. And, yes: I have also added a TeX group
	% on my own (but that's not the problem).
	\global\pgfplotslistnewempty\pgfplots@prepared@tick@positions@major
	\global\pgfplotslistnewempty\pgfplots@prepared@tick@positions@minor
	\edef\pgfplots@loc@TMPa{#1}%
	\ifx\pgfplots@loc@TMPa\pgfutil@empty
	\else
		\ifpgfplots@minorticks
			\pgfplots@needsminorlooptrue
		\else
			\ifpgfplots@minorgrids
				\pgfplots@needsminorlooptrue
			\else
				\pgfplots@needsminorloopfalse
			\fi
		\fi
		\ifpgfplots@needsminorloop
			\ifpgfplots@islinear
				\expandafter\let\expandafter\pgfplots@minor@tick@num\csname pgfplots@minor@#2tick@num\endcsname
				\begingroup
				\c@pgf@counta=\pgfplots@minor@tick@num\relax
				\advance\c@pgf@counta by1\relax
				\pgfplots@tmpa=\csname pgfplots@tick@distance@#2\endcsname pt
				\divide\pgfplots@tmpa by\c@pgf@counta
				\edef\pgfmathresult{\pgf@sys@tonumber{\pgfplots@tmpa}}%
				\pgfmath@smuggleone\pgfmathresult
				\endgroup
				\let\pgfplots@minor@tick@dist=\pgfmathresult
			\else
				\def\pgfplots@minor@tick@num{9}%
			\fi
		\fi
		\foreach \x in {#1} {%
			\ifcase#3\relax
				\pgfextractx{\pgfplots@tmpa}{\pgfpointxy{\x}{0}}%
			\or
				\pgfextracty{\pgfplots@tmpa}{\pgfpointxy{0}{\x}}%
			\fi
			\csname pgfplots@#2tick@check@tickshow\endcsname
			%
			\ifpgfplots@tickshow
				\ifdim\pgfplots@tmpa<\csname pgfplots@#2coordminTEX\endcsname
				\else
					\ifdim\pgfplots@tmpa>\csname pgfplots@#2coordmaxTEX\endcsname
					\else
						\edef\pgfplots@loc@TMPa{{\the\pgfplots@tmpa}{\x}}%
						\expandafter\pgfplotslistpushbackglobal\pgfplots@loc@TMPa\to\pgfplots@prepared@tick@positions@major
					\fi
				\fi
			\fi
			% X-Axis ticks bottom and top
			% in log:
			%  log( i*10^k ) = log\pgfplots@i + k\log10 -> draw ticks for i=1..9
			\ifpgfplots@needsminorloop
				\foreach \pgfplots@i in {1,...,\pgfplots@minor@tick@num} {%
					\begingroup
					\ifcase#3\relax
						\ifpgfplots@islinear
							\pgfextractx{\pgfplots@tmpa}{\pgfpointxy{\pgfplots@i*\pgfplots@minor@tick@dist}{0}}%
						\else
							\pgfextractx{\pgfplots@tmpa}{\pgfpointxy{\logi\pgfplots@i}{0}}%
						\fi
					\or
						\ifpgfplots@islinear
							\pgfextracty{\pgfplots@tmpa}{\pgfpointxy{0}{\pgfplots@i*\pgfplots@minor@tick@dist}}%
						\else
							\pgfextracty{\pgfplots@tmpa}{\pgfpointxy{0}{\logi\pgfplots@i}}%
						\fi
					\fi
					\edef\pgfmathresult{\the\pgfplots@tmpa}%
					\pgfmath@smuggleone\pgfmathresult
					\endgroup
					\advance\pgfplots@tmpa by\pgfmathresult\relax
					\ifdim\pgfplots@tmpa<\csname pgfplots@#2coordminTEX\endcsname
					\else
						\ifdim\pgfplots@tmpa>\csname pgfplots@#2coordmaxTEX\endcsname
						\else
							\expandafter\pgfplotslistpushbackglobal\the\pgfplots@tmpa\to\pgfplots@prepared@tick@positions@minor
						\fi
					\fi
				}%
			\fi
		}%
	\fi
	\endgroup
	\expandafter\let\csname pgfplots@prepared@tick@positions@minor@#2\endcsname=\pgfplots@prepared@tick@positions@minor
	\expandafter\let\csname pgfplots@prepared@tick@positions@major@#2\endcsname=\pgfplots@prepared@tick@positions@major
	\global\let\pgfplots@prepared@tick@positions@major=\relax
	\global\let\pgfplots@prepared@tick@positions@minor=\relax
}%

% Converts the tuples in major tick lists into two separate variables.
%
% Usage: 
% \pgfplotslistforeach\pgfplots@prepared@tick@positions@major@x\as\curelement{%
%	 \expandafter\pgfplots@parse@prepared@major@tickpos\curelement\canvas\logical
% }
%
% #1#2 : the tuples as they are found in the prepared major tick list,
% #3   : a dimen register which will be filled with #1
% #4   : a macro which will be assigned with #2
\def\pgfplots@parse@prepared@major@tickpos#1#2#3#4{%
	#3=#1\relax%
	\def#4{#2}%
}%
	

% #1 : the verbatim axis name (either 'x' or 'y')
% #2 : the index of the axis  (either 0 or 1)
\def\pgfplots@drawgridlines@for#1#2{%
	\begingroup
	\expandafter\let\expandafter\ifpgfplots@major\csname ifpgfplots@#1majorgrids\endcsname
	\expandafter\let\expandafter\ifpgfplots@minor\csname ifpgfplots@#1minorgrids\endcsname
	\expandafter\let\expandafter\pgfplots@prepared@tick@positions@major@\csname pgfplots@prepared@tick@positions@major@#1\endcsname
	\expandafter\let\expandafter\pgfplots@prepared@tick@positions@minor@\csname pgfplots@prepared@tick@positions@minor@#1\endcsname
	\pgfplots@loop@CONTINUEfalse
	\ifpgfplots@major
		\pgfplots@loop@CONTINUEtrue
	\fi
	\ifpgfplots@minor
		\pgfplots@loop@CONTINUEtrue
	\fi
	\ifpgfplots@loop@CONTINUE
		\scope
		%\clip 			(\pgfplots@xcoordminTEX\pgfplots@leftover,	\pgfplots@ycoordminTEX\pgfplots@leftover) 
		%	rectangle	(\pgfplots@xcoordmaxTEX\pgfplots@rightover,	\pgfplots@ycoordmaxTEX\pgfplots@rightover);
		\pgfinterruptboundingbox%
		\ifcase#2\relax
			\clip 			(\pgfplots@xcoordminTEX,	\pgfplots@ycoordminTEX-5cm) 
				rectangle	(\pgfplots@xcoordmaxTEX,	\pgfplots@ycoordmaxTEX+5cm);
		\or
			\clip 			(\pgfplots@xcoordminTEX-5cm,	\pgfplots@ycoordminTEX) 
				rectangle	(\pgfplots@xcoordmaxTEX+5cm,	\pgfplots@ycoordmaxTEX);
		\fi
		\endpgfinterruptboundingbox%
		\ifpgfplots@major
			\draw[%
				/pgfplots/every axis grid,
				/pgfplots/every major grid,
				/pgfplots/every axis #1 grid,
				/pgfplots/every major #1 grid]%
			\pgfextra
			\pgfplotslistforeach\pgfplots@prepared@tick@positions@major@\as\pgfplots@curgridpos{%
				\expandafter\pgfplots@parse@prepared@major@tickpos\pgfplots@curgridpos\pgfplots@tmpa\pgfplots@curgridpos
				\csname pgfplots@draw#1axis@placecomputedgridline\endcsname
			}%
			\endpgfextra;
		\fi
		%
		\ifpgfplots@minor
			\draw[%
				/pgfplots/every axis grid,
				/pgfplots/every minor grid,
				/pgfplots/every axis #1 grid,
				/pgfplots/every minor #1 grid]%
			\pgfextra
			\pgfplotslistforeach\pgfplots@prepared@tick@positions@minor@\as\pgfplots@curgridpos{%
				\pgfplots@tmpa=\pgfplots@curgridpos
				\csname pgfplots@draw#1axis@placecomputedgridline\endcsname
			}%
			\endpgfextra;
		\fi
		\endscope
	\fi
	\endgroup
}

% #1 : the verbatim axis name (either 'x' or 'y')
% #2 : the index of the axis  (either 0 or 1)
\def\pgfplots@drawticklines@for#1#2{%
	\scope
	\expandafter\let\expandafter\ifpgfplots@major\csname ifpgfplots@#1majorticks\endcsname
	\expandafter\let\expandafter\ifpgfplots@minor\csname ifpgfplots@#1minorticks\endcsname
	\expandafter\let\expandafter\pgfplots@prepared@tick@positions@major@\csname pgfplots@prepared@tick@positions@major@#1\endcsname
	\expandafter\let\expandafter\pgfplots@prepared@tick@positions@minor@\csname pgfplots@prepared@tick@positions@minor@#1\endcsname
	%\clip 			(\pgfplots@xcoordminTEX\pgfplots@leftover,	\pgfplots@ycoordminTEX\pgfplots@leftover) 
	%	rectangle	(\pgfplots@xcoordmaxTEX\pgfplots@rightover,	\pgfplots@ycoordmaxTEX\pgfplots@rightover);
	\pgfinterruptboundingbox%
	\ifcase#2\relax
		\clip 			(\pgfplots@xcoordminTEX,	\pgfplots@ycoordminTEX-5cm) 
			rectangle	(\pgfplots@xcoordmaxTEX,	\pgfplots@ycoordmaxTEX+5cm);
	\or
		\clip 			(\pgfplots@xcoordminTEX-5cm,	\pgfplots@ycoordminTEX) 
			rectangle	(\pgfplots@xcoordmaxTEX+5cm,	\pgfplots@ycoordmaxTEX);
	\fi
	\endpgfinterruptboundingbox%
	\ifpgfplots@major
		\draw[%
			/pgfplots/every tick,
			/pgfplots/every major tick,
			/pgfplots/every #1 tick,
			/pgfplots/every major #1 tick]%
		\pgfextra
		\pgfmathparse{\pgfplots@tickwidth}%
		\let\pgfplots@tickwidth@=\pgfmathresult
		\edef\pgfplots@tickwidth{\pgfplots@tickwidth@ pt}%
		\ifcase\csname pgfplots@#1tickalignnum\endcsname\relax
			\def\pgfplots@tick@offset{0}
		\or
			\let\pgfplots@tick@offset=\pgfplots@tickwidth@%
		\or
			\pgfmathmultiply@{0.5}{\pgfplots@tickwidth@}%
			\let\pgfplots@tick@offset=\pgfmathresult%
		\fi
		\ifcase#2\relax
			\pgfplots@prepare@tick@offsets@for@{#1}{y}{\pgfplots@tickwidth@}%
		\else
			\pgfplots@prepare@tick@offsets@for@{#1}{x}{\pgfplots@tickwidth@}%
		\fi
		\pgfplotslistforeach\pgfplots@prepared@tick@positions@major@\as\pgfplots@curtickpos{%
			\expandafter\pgfplots@parse@prepared@major@tickpos\pgfplots@curtickpos\pgfplots@tmpa\pgfplots@curtickpos
			\csname pgfplots@draw#1axis@placecomputedtick\endcsname
		}%
		\endpgfextra;
	\fi
	%
	\ifpgfplots@minor
		\draw[%
			/pgfplots/every tick,
			/pgfplots/every minor tick,
			/pgfplots/every #1 tick,
			/pgfplots/every minor #1 tick]%
		\pgfextra
		\pgfmathparse{\pgfplots@subtickwidth}%
		\let\pgfplots@subtickwidth@=\pgfmathresult
		\edef\pgfplots@subtickwidth{\pgfplots@subtickwidth@ pt}%
		\ifcase\csname pgfplots@#1tickalignnum\endcsname\relax
			\def\pgfplots@tick@offset{0}%
		\or
			\let\pgfplots@tick@offset=\pgfplots@subtickwidth@%
		\or
			\pgfmathmultiply@{0.5}{\pgfplots@subtickwidth@}%
			\let\pgfplots@tick@offset=\pgfmathresult%
		\fi
		\ifcase#2\relax
			\pgfplots@prepare@tick@offsets@for@{#1}{y}{\pgfplots@subtickwidth@}%
		\else
			\pgfplots@prepare@tick@offsets@for@{#1}{x}{\pgfplots@subtickwidth@}%
		\fi
		\pgfplotslistforeach\pgfplots@prepared@tick@positions@minor@\as\pgfplots@curtickpos{%
			\pgfplots@tmpa=\pgfplots@curtickpos
			\csname pgfplots@draw#1axis@placecomputedtick\endcsname
		}%
		\endpgfextra;
	\fi
	\endscope
}

% #1 : the verbatim axis name (either 'x' or 'y')
% #2 : the index of the axis  (either 0 or 1)
\def\pgfplots@drawticklabels@for#1#2{%
	\begingroup
	\expandafter\let\expandafter\ifpgfplots@major\csname ifpgfplots@#1majorticks\endcsname
	\expandafter\let\expandafter\ifpgfplots@islinear\csname ifpgfplots@#1islinear\endcsname
	\expandafter\let\expandafter\pgfplots@prepared@tick@positions@major@\csname pgfplots@prepared@tick@positions@major@#1\endcsname
	\ifpgfplots@major
		\ifpgfplots@islinear
			\pgfplots@if{pgfplots@scaled@ticks@#1}{%
				\pgfplots@init@scaled@tick@for{#1}%
			}\relax%
		\fi
		\begingroup
		\pgfkeys{/tikz/every node/.append style={/pgfplots/every tick label,/pgfplots/every #1 tick label}}%
		\ifcase\csname pgfplots@#1tickalignnum\endcsname\relax
			\def\pgfmathresult{0}%
		\or
			\pgfmathparse{\pgfplots@tickwidth}%
		\or
			\pgfmathmultiply{0.5}{\pgfplots@tickwidth}%
		\fi
		\let\pgfplots@tick@offset=\pgfmathresult
		\ifnum\csname pgfplots@#1ticklabelposnum\endcsname=0
			% the choice '[xy]ticklabel pos=default':
			\expandafter\let\expandafter\pgfplots@tmpposnum\csname pgfplots@#1tickposnum\endcsname
		\else
			\expandafter\let\expandafter\pgfplots@tmpposnum\csname pgfplots@#1ticklabelposnum\endcsname
		\fi
		\ifcase#2\relax
			\ifcase\pgfplots@tmpposnum\relax
				\edef\pgfplots@tick@origin{\pgf@sys@tonumber{\pgfplots@ycoordminTEX}}%
			\or
				\edef\pgfplots@tick@origin{\pgf@sys@tonumber{\pgfplots@ycoordminTEX}}%
			\or
				\pgf@xa=\pgfplots@ZERO@y
				\edef\pgfplots@tick@origin{\pgf@sys@tonumber{\pgf@xa}}%
			\or
				\edef\pgfplots@tick@origin{\pgf@sys@tonumber{\pgfplots@ycoordmaxTEX}}%
			\fi
			\def\pgfplots@tickposchoicea{\tikzset{above}}%
			\def\pgfplots@tickposchoiceb{\tikzset{below}}%
		\or
			\ifcase\pgfplots@tmpposnum\relax
				\edef\pgfplots@tick@origin{\pgf@sys@tonumber{\pgfplots@xcoordminTEX}}%
			\or
				\edef\pgfplots@tick@origin{\pgf@sys@tonumber{\pgfplots@xcoordminTEX}}%
			\or
				\pgf@xa=\pgfplots@ZERO@x
				\edef\pgfplots@tick@origin{\pgf@sys@tonumber{\pgf@xa}}%
			\or
				\edef\pgfplots@tick@origin{\pgf@sys@tonumber{\pgfplots@xcoordmaxTEX}}%
			\fi
			\def\pgfplots@tickposchoicea{\tikzset{right}}%
			\def\pgfplots@tickposchoiceb{\tikzset{left}}%
		\fi
		\ifnum\pgfplots@tmpposnum=3
			\pgfplots@tickposchoicea
			\pgfmathadd@{\pgfplots@tick@origin}{\pgfplots@tick@offset}%
		\else
			\pgfplots@tickposchoiceb
			\pgfmathsubtract@{\pgfplots@tick@origin}{\pgfplots@tick@offset}%
		\fi
		\edef\pgfplots@tick@origin{\pgfmathresult pt}%
		\def\pgfplots@ticknum{0}%
		\xdef\pgfplots@show@ticklabel@LASTTICK{}%
		\pgfplotslistforeachungrouped\pgfplots@prepared@tick@positions@major@\as\pgfplots@curtickpos{%
			\expandafter\pgfplots@parse@prepared@major@tickpos\pgfplots@curtickpos\pgfplots@tmpa\pgfplots@curtickpos
			\ifcase#2\relax
				\pgfplots@show@ticklabel
					{#1}{\pgfplots@curtickpos}(\pgfplots@tmpa,\pgfplots@tick@origin)%
					{\pgfplots@ticknum}%
			\or
				\pgfplots@show@ticklabel
					{#1}{\pgfplots@curtickpos}(\pgfplots@tick@origin,\pgfplots@tmpa)%
					{\pgfplots@ticknum}%
			\fi
			\begingroup
			\c@pgf@counta=\pgfplots@ticknum\relax
			\advance\c@pgf@counta by1
			\edef\pgfplots@ticknum{\the\c@pgf@counta}%
			\pgfmath@smuggleone\pgfplots@ticknum
			\endgroup
		}%
		\endgroup
		\pgfplots@draw@tick@scale@label@for #1%
	\fi
	\endgroup
}

\def\pgfplots@rememberplotspec#1{%
	\pgfplotslistpushbackglobal{#1}\to\pgfplots@plotspeclist
}

\def\pgfplots@getautoplotspec into#1{%
	\pgfplotslistsize\autoplotspeclist\to\c@pgf@counta
	\ifnum\c@pgf@counta=0
		\let#1=\pgfutil@empty
	\else
		\c@pgf@countb=\pgfplots@numplots
		% offset modulo size:
		\loop
		\ifnum\c@pgf@countb<\c@pgf@counta
			\pgfplots@loop@CONTINUEfalse
		\else
			\pgfplots@loop@CONTINUEtrue
		\fi
		\ifpgfplots@loop@CONTINUE
			\advance\c@pgf@countb by-\c@pgf@counta
		\repeat
		\pgfplotslistselect\c@pgf@countb\of\autoplotspeclist\to#1
%\pgfplots@message{pgfplots.sty: using \string\autoplotspeclist\ specification no\#\the\c@pgf@countb (of \the\c@pgf@counta): #1}%
	\fi
}

% The main interface to draw a plot into an axis.
%
% Usage:
% \addplot 
% 	plot coordinates {
% 		(0,0)
% 		(1,1)
% 	};
% 
% or
%
% \addplot[color=blue,mark=*]
% 	plot coordinates {
% 		(0,0)
% 		(1,1)
% 	};
% 
% The first syntax will use the next plot specification in the list
% \autoplotspeclist
% and the first will use blue color and * markers. 
%
% \addplot[<style options>]  plot[<behavior options>]  <input type and args> <post plot path> ;
% 
%
% The linespec. will be used in the legend.
%
% Low-level implementation:
%
% \pgfplots@addplot 
% \pgfplots@addplotimpl
% \pgfplots@start@plot@with@behavioroptions <--- \begingroup
% ...
% ... remember options GLOBALLY
% ... update limits GLOBALLY
% ... \pgfplots@addplot@enqueue@coords GLOBALLY
% ...
% \pgfplots@end@plot <--- \endgroup
\long\def\pgfplots@addplot{%
	\pgfutil@ifnextchar+{%
		\pgfplots@getautoplotspec into\nextplotspec
		\pgfplots@addplotimplAPPEND
	}{%
		\pgfutil@ifnextchar[{%
			\pgfplots@addplotimpl%
		}{%
			\pgfplots@getautoplotspec into\nextplotspec
			% the space after ']' is required here:
			% FIXME: 
			% - \addplot[]plot coordinates is NOT allowed!?
			\expandafter\pgfplots@addplotimpl\expandafter[\nextplotspec]%
		}%
	}%
}

\long\def\pgfplots@addplotimplAPPEND+[{%
	\expandafter\pgfplots@addplotimpl\expandafter[\nextplotspec,
}

\long\def\pgfplots@addplotimpl[#1]{%
	\pgfutil@ifnextchar p{%
		\pgfplots@addplotimpl@plot{#1}%
	}{%
		\pgfplots@addplotimpl@plot{#1}plot
	}%
}

\def\pgfplots@addplotimpl@plot#1plot{%
	\pgfutil@ifnextchar[{%
		\pgfplots@addplotimpl@plot@withoptions{#1}%
	}{%
		\pgfplots@addplotimpl@plot@withoptions{#1}[]%
	}%
}

\def\pgfplots@addplotimpl@plot@withoptions#1[#2]{
	\pgfplots@start@plot@with@behavioroptions{#2}%
	\pgfutil@ifnextchar c{%
		\pgfplots@addplotimpl@coordinates{#1}plot 
	}{%
		\pgfutil@ifnextchar f{%
			\pgfplots@addplotimpl@f{#1}%
		}{%
			\pgfutil@ifnextchar t{%
				\pgfplots@addplotimpl@table{#1}%
			}{%
				\pgfutil@ifnextchar ({%
					\pgfplots@addplotimpl@expression{#1}%
				}{%
					\pgfplots@error{Sorry, the supplied plot command is unknown or unsupported by pgfplots! Ignoring it.}%
					\pgfplots@gobble@until@semicolon
				}%
			}%
		}%
	}%
}

\def\pgfplots@gobble@until@semicolon#1;{}

% Currently, plot expression is really inefficient:
%
% 1. it invokes the math parser to get all coordinates. Ok, that's
% what one expects.
%
% 2. It collects the result into one large list instead of calling
% pgfplots' stream methods. That's because \foreach encapsulates its
% code in at least one TeX-group.
%
% 3. It processes the collected list; applying any floating point
% parser routines - it does NOT know that any numbers are already in
% TeX-precision!
%
\long\def\pgfplots@addplotimpl@expression#1(#2,#3)#4;{%
	\pgfplots@PREPARE@COORD@STREAM{#1}{#4}%
	%
	\pgfplots@gettikzinternal@keyval{variable}{tikz@plot@var}{\x}%
	\pgfplots@gettikzinternal@keyval{samples at}{tikz@plot@samplesat}{-5,-4.6,...,5}%
	%
	\edef\pgfplots@plot@data{\noexpand\foreach\expandafter\noexpand\tikz@plot@var in {\tikz@plot@samplesat}}%
	\pgfplotsapplistXXglobalnewempty
	\pgfplots@plot@data{%
		\pgfmathparse{#2}%
		\let\pgfplots@current@point@x=\pgfmathresult
		\pgfmathparse{#3}%
		\let\pgfplots@current@point@y=\pgfmathresult
		\edef\pgfplots@loc@TMPa{(\pgfplots@current@point@x,\pgfplots@current@point@y)}%
		\expandafter\pgfplotsapplistXXglobalpushback\expandafter{\pgfplots@loc@TMPa}%
	}%
	\pgfplotsapplistXXgloballet\pgfplots@loc@TMPa
	\pgfplotsapplistXXglobalclear
	\expandafter\pgfplots@coord@stream@foreach\expandafter{\pgfplots@loc@TMPa}%
}%

\def\pgfplots@addplotimpl@f#1f{%
	\pgfutil@ifnextchar i{\pgfplots@addplotimpl@file{#1}}{\pgfplots@addplotimpl@function{#1}}%
}%

\let\pgfplots@backupof@pgfplotxyfile=\pgfplotxyfile

% the following code 
% results finally in
%
% set format "%.7e";; set samples <...>; plot ...
%
% The windows port of gnuplot doesn't run without the second semicolon
% - for whatever reason.
{
  \catcode`\%=12
  \catcode`\"=12
  \xdef\pgfplots@gnuplot@format{set format "%.7e";}
}

% #1: args of \addplot[...]
% #2: file name
% #3: trailing path commands until ';'
\def\pgfplots@addplotimpl@function#1unction#2#3;{%
	\pgfplots@gettikzinternal@keyval{prefix}{tikz@plot@prefix}{\jobname.}%
	\pgfplots@gettikzinternal@keyval{id}{tikz@plot@id}{pgf-plot}%
	\pgfplots@gettikzinternal@keyval{samples}{tikz@plot@samples}{25}%
	\pgfplots@gettikzinternal@keyval{domain}{tikz@plot@domain}{-5:5}%
	\pgfplots@gettikzinternal@keyval{raw gnuplot}{iftikz@plot@raw@gnuplot}{\iffalse}%
	\pgfplots@gettikzinternal@keyval{parametric}{iftikz@plot@parametric}{\iffalse}%
	%
	\def\pgfplots@plot@filename{\tikz@plot@prefix\tikz@plot@id}%  
	\iftikz@plot@raw@gnuplot%
		\def\pgfplots@plot@data{\pgfplotgnuplot[\pgfplots@plot@filename]{#2}}%
	\else%
		\iftikz@plot@parametric%   
			\def\pgfplots@plot@data{\pgfplotgnuplot[\pgfplots@plot@filename]{%
				\pgfplots@gnuplot@format;
				set samples \tikz@plot@samples;
				set parametric;
				plot [t=\tikz@plot@domain] #2}}%
		\else%
			\def\pgfplots@plot@data{\pgfplotgnuplot[\pgfplots@plot@filename]{%
				\pgfplots@gnuplot@format;
				set samples \tikz@plot@samples;
				plot [x=\tikz@plot@domain] #2}}%
		\fi%
	\fi%
	\def\pgfplotxyfile{\pgfplots@addplotimpl@gnuplotresult{#1}{#3}}%
	\pgfplots@plot@data
	\let\pgfplotxyfile=\pgfplots@backupof@pgfplotxyfile
}%

\def\pgfplots@addplotimpl@gnuplotresult#1#2#3{%
	\begingroup
	\openin1=#3
	\ifeof1
		\pgfplots@error{Sorry, the gnuplot-result file '#3' could not be found. Maybe you need to enable the shell-escape feature? For pdflatex, this is '>> pdflatex -shell-escape'. You can also invoke '>> gnuplot #3' manually.}%
		\aftergroup\pgfplots@loop@CONTINUEfalse
	\else
		\aftergroup\pgfplots@loop@CONTINUEtrue
	\fi
	\closein1
	\endgroup
	\ifpgfplots@loop@CONTINUE
		\pgfplots@addplotimpl@file{#1}ile{#3}#2;%
	\fi
}

% #1: arguments to \addplot[...]
% #2: the file name
% #3: any additional path arguments
\def\pgfplots@addplotimpl@file#1ile{%
	\pgfutil@ifnextchar[{%
		\pgfplots@addplotimpl@file@opt{#1}%
	}{%
		\pgfplots@addplotimpl@file@opt{#1}[]%
	}%
}

% \addplot[#1] file[#2] {#3} #4;
\def\pgfplots@addplotimpl@file@opt#1[#2]#3#4;{%
	\begingroup
	\def\pgfplots@loc@TMPa{#2}%
	\ifx\pgfplots@loc@TMPa\pgfutil@empty
	\else
		\pgfqkeys{/pgfplots/plot file}{#2}%
	\fi
	\pgfplots@PREPARE@COORD@STREAM{#1}{#4}%
	\pgfplots@coord@stream@start
	\openin1=#3
	\ifeof1
		\pgfplots@warning{sorry, plot file{#3} could not be opened!?}%
	\else
		\pgfplots@addplotimpl@file@readall
	\fi
	\pgfplots@coord@stream@end
	\endgroup
}%
\def\pgfplots@addplotimpl@file@readall{%
	\read1 to\pgfplots@file@LINE
	\expandafter\pgfplotstableread@checkspecial@line\pgfplots@file@LINE\pgfplotstable@EOI
	\ifpgfplotstableread@skipline
	\else
		\ifpgfplots@plot@file@skipfirst
			% Silently skip first data row, assuming it is a header.
			\pgfplots@plot@file@skipfirstfalse
		\else
			\expandafter\pgfplots@addplotimpl@file@parsesingle\pgfplots@file@LINE\pgfplots@EOI
		\fi
	\fi
	\ifeof1
	\else
		\expandafter
		\pgfplots@addplotimpl@file@readall
	\fi
}%

\def\pgfplots@addplotimpl@file@parsesingle#1 #2 #3\pgfplots@EOI{%
	\pgfplots@coord@stream@coord{#1}{#2}{}{}%
}%

\def\pgfplots@addplotimpl@table#1table{%
	\pgfutil@ifnextchar[{%
		\pgfplots@addplotimpl@table@getopts{#1}%
	}{%
		\pgfplots@addplotimpl@table@getopts{#1}[x index=0,y index=1]%
	}%
}%

\def\pgfplots@addplotimpl@table@getopts#1[#2]{%
	\pgfutil@ifnextchar f{%
		\pgfplots@addplotimpl@table@fromstructure{#1}{#2}%
	}{%
		\pgfplots@addplotimpl@table@fromfile{#1}{#2}%
	}%
}

% #1: arguments to \addplot[...]
% #2: arguments to table[...]
% #3: the argument of plot table{...}
% #4: trailing path arguments after plot table{...}#4;
\long\def\pgfplots@addplotimpl@table@fromstructure#1#2from#3#4;{%
	\begingroup
	% FIXME : this thing here has runtime O(N^2) !
	% I fear it is faster to simply reload the data .... !?
	%
	% well, for a lot of columns which are used in different contexts
	% and few rows, this here IS more efficient.
	\pgfplotstableset{#2}%
	\pgfplotstablecopy#3\to\pgfplots@table
	\ifx\pgfplots@plot@tbl@x\pgfutil@empty
		\pgfplotstablegetcolumnbyindex\pgfplots@plot@tbl@xindex\of\pgfplots@table\to\addplot@tbl@x
	\else
		\pgfplotstablegetcolumnbyname\pgfplots@plot@tbl@x\of\pgfplots@table\to\addplot@tbl@x
	\fi
	\ifx\pgfplots@plot@tbl@y\pgfutil@empty
		\pgfplotstablegetcolumnbyindex\pgfplots@plot@tbl@yindex\of\pgfplots@table\to\addplot@tbl@y
	\else
		\pgfplotstablegetcolumnbyname\pgfplots@plot@tbl@y\of\pgfplots@table\to\addplot@tbl@y
	\fi
	%
	\ifpgfplots@errorbars@enabled
		\let\addplot@tbl@error@x=\pgfutil@empty
		\let\addplot@tbl@error@y=\pgfutil@empty
		\pgfkeysgetvalue{/pgfplots/table/x error index}\pgfplots@plot@tbl@error@xindex
		\pgfkeysgetvalue{/pgfplots/table/x error}\pgfplots@plot@tbl@error@x
		\pgfkeysgetvalue{/pgfplots/table/y error index}\pgfplots@plot@tbl@error@yindex
		\pgfkeysgetvalue{/pgfplots/table/y error}\pgfplots@plot@tbl@error@y
		\ifx\pgfplots@plot@tbl@error@x\pgfutil@empty
			\ifx\pgfplots@plot@tbl@error@xindex\pgfutil@empty
			\else
				\pgfplotstablegetcolumnbyindex\pgfplots@plot@tbl@error@xindex\of\pgfplots@table\to\addplot@tbl@error@x
			\fi
		\else
			\pgfplotstablegetcolumnbyname\pgfplots@plot@tbl@error@x\of\pgfplots@table\to\addplot@tbl@error@x
		\fi
		\ifx\pgfplots@plot@tbl@error@y\pgfutil@empty
			\ifx\pgfplots@plot@tbl@error@yindex\pgfutil@empty
			\else
				\pgfplotstablegetcolumnbyindex\pgfplots@plot@tbl@error@yindex\of\pgfplots@table\to\addplot@tbl@error@y
			\fi
		\else
			\pgfplotstablegetcolumnbyname\pgfplots@plot@tbl@error@y\of\pgfplots@table\to\addplot@tbl@error@y
		\fi
	\fi
	%
	\pgfplots@PREPARE@COORD@STREAM{#1}{#4}%
	\pgfplots@coord@stream@start
	\loop
	\pgfplotslistcheckempty\addplot@tbl@x
	\ifpgfplotslistempty
		\pgfplots@loop@CONTINUEfalse
	\else
		% This here is just for sanity checking: if the 'y' column is 
		% - for whatever reasons - invalid; provide good error
		%   recovery.
		\pgfplotslistcheckempty\addplot@tbl@y
		\ifpgfplotslistempty
			\pgfplots@loop@CONTINUEfalse
		\else
			\pgfplots@loop@CONTINUEtrue
		\fi
	\fi
	\ifpgfplots@loop@CONTINUE
		\pgfplotslistpopfront\addplot@tbl@x\to\addplot@tbl@cur@x
		\pgfplotslistpopfront\addplot@tbl@y\to\addplot@tbl@cur@y
		\ifpgfplots@errorbars@enabled
			\ifx\addplot@tbl@error@x\pgfutil@empty
				\let\addplot@tbl@error@cur@x=\pgfutil@empty
			\else
				\pgfplotslistpopfront\addplot@tbl@error@x\to\addplot@tbl@error@cur@x
			\fi
			\ifx\addplot@tbl@error@y\pgfutil@empty
				\let\addplot@tbl@error@cur@y=\pgfutil@empty
			\else
				\pgfplotslistpopfront\addplot@tbl@error@y\to\addplot@tbl@error@cur@y
			\fi
			\edef\pgfplots@loc@TMPa{{\addplot@tbl@cur@x}{\addplot@tbl@cur@y}{\addplot@tbl@error@cur@x}{\addplot@tbl@error@cur@y}}%
			\expandafter\pgfplots@coord@stream@coord\pgfplots@loc@TMPa
		\else
			\edef\pgfplots@loc@TMPa{{\addplot@tbl@cur@x}{\addplot@tbl@cur@y}{}{}}%
			\expandafter\pgfplots@coord@stream@coord\pgfplots@loc@TMPa
		\fi
	\repeat
	\pgfplots@coord@stream@end
	\endgroup
}


% #1: arguments to \addplot[...]
% #2: arguments to table[...]
% #3: the argument of plot table{...}
% #4: trailing path arguments after plot table{...}#4;
\long\def\pgfplots@addplotimpl@table@fromfile#1#2#3#4;{%
	%--------------------------------------------------
	% \begingroup
	% \pgfplotstableset{#2}%
	% \pgfplotstableread{#3}\pgfplots@table
	% \pgfplots@addplotimpl@table@fromstructure{#1}{}from{\pgfplots@table}{#4};%
	% \endgroup
	%-------------------------------------------------- 
	\pgfplotsapplistXXglobalnewempty
	\begingroup
	\pgfplotstableset{#2}%
	\let\pgfplots@table@PTR@x=\pgfutil@empty
	\let\pgfplots@table@PTR@y=\pgfutil@empty
	\ifpgfplots@errorbars@enabled
		\let\pgfplots@table@ERRPTR@x=\pgfutil@empty
		\let\pgfplots@table@ERRPTR@y=\pgfutil@empty
		\pgfkeysgetvalue{/pgfplots/table/x error index}\pgfplots@plot@tbl@error@xindex
		\pgfkeysgetvalue{/pgfplots/table/x error}\pgfplots@plot@tbl@error@x
		\pgfkeysgetvalue{/pgfplots/table/y error index}\pgfplots@plot@tbl@error@yindex
		\pgfkeysgetvalue{/pgfplots/table/y error}\pgfplots@plot@tbl@error@y
		\pgfplotstableread{#3} to listener\pgfplots@addplotimpl@table@fromfile@listener@witherrors
	\else
		\pgfplotstableread{#3} to listener\pgfplots@addplotimpl@table@fromfile@listener
	\fi
	\endgroup
	%
	\pgfplots@PREPARE@COORD@STREAM{#1}{#4}%
	\pgfplotsapplistXXgloballet\pgfplots@coordlist
	\pgfplotsapplistXXglobalclear
	\expandafter\pgfplots@coord@stream@foreach\expandafter{\pgfplots@coordlist}%%
}
\def\pgfplots@addplotimpl@table@fromfile@listener{%
	\pgfplots@addplotimpl@table@fromfile@listener@
	\edef\pgfplots@current@point{(\pgfplots@current@point@x,\pgfplots@current@point@y)}%
	\expandafter\pgfplotsapplistXXglobalpushback\expandafter{\pgfplots@current@point}%
}
\def\pgfplots@addplotimpl@table@fromfile@listener@{%
	\ifx\pgfplots@table@PTR@x\pgfutil@empty
		% this here is only evaluated ONCE.
		\ifx\pgfplots@plot@tbl@x\pgfutil@empty
			\pgfplotstablereadgetptrtocolindex{\pgfplots@plot@tbl@xindex}{\pgfplots@table@PTR@x}%
		\else
			\pgfplotstablereadgetptrtocolname{\pgfplots@plot@tbl@x}{\pgfplots@table@PTR@x}%
		\fi
		\ifx\pgfplots@plot@tbl@y\pgfutil@empty
			\pgfplotstablereadgetptrtocolindex{\pgfplots@plot@tbl@yindex}{\pgfplots@table@PTR@y}%
		\else
			\pgfplotstablereadgetptrtocolname{\pgfplots@plot@tbl@y}{\pgfplots@table@PTR@y}%
		\fi
	\fi
	\pgfplotstablereadevalptr\pgfplots@table@PTR@x\pgfplots@current@point@x
	\pgfplotstablereadevalptr\pgfplots@table@PTR@y\pgfplots@current@point@y
}%
\def\pgfplots@addplotimpl@table@fromfile@listener@witherrors{%
	\pgfplots@addplotimpl@table@fromfile@listener@
	%
	\ifx\pgfplots@table@ERRPTR@x\pgfutil@empty
		% this here is only evaluated ONCE.
		\ifx\pgfplots@plot@tbl@error@x\pgfutil@empty
			\ifx\pgfplots@plot@tbl@error@xindex\pgfutil@empty
				\let\pgfplots@table@ERRPTR@x=\relax%
			\else
				\pgfplotstablereadgetptrtocolindex{\pgfplots@plot@tbl@error@xindex}{\pgfplots@table@ERRPTR@x}%
			\fi
		\else
			\pgfplotstablereadgetptrtocolname{\pgfplots@plot@tbl@error@x}{\pgfplots@table@ERRPTR@x}%
		\fi
		\ifx\pgfplots@plot@tbl@error@y\pgfutil@empty
			\ifx\pgfplots@plot@tbl@error@yindex\pgfutil@empty
				\let\pgfplots@table@ERRPTR@y=\relax%
			\else
				\pgfplotstablereadgetptrtocolindex{\pgfplots@plot@tbl@error@yindex}{\pgfplots@table@ERRPTR@y}%
			\fi
		\else
			\pgfplotstablereadgetptrtocolname{\pgfplots@plot@tbl@error@y}{\pgfplots@table@ERRPTR@y}%
		\fi
	\fi
	\ifx\relax\pgfplots@table@ERRPTR@x
		\let\addplot@tbl@error@cur@x=\pgfutil@empty
	\else
		\pgfplotstablereadevalptr\pgfplots@table@ERRPTR@x\addplot@tbl@error@cur@x
	\fi
	\ifx\relax\pgfplots@table@ERRPTR@y
		\let\addplot@tbl@error@cur@y=\pgfutil@empty
	\else
		\pgfplotstablereadevalptr\pgfplots@table@ERRPTR@y\addplot@tbl@error@cur@y
	\fi
	\edef\pgfplots@current@point{(\pgfplots@current@point@x,\pgfplots@current@point@y)+-(\addplot@tbl@error@cur@x,\addplot@tbl@error@cur@y)}%
	\expandafter\pgfplotsapplistXXglobalpushback\expandafter{\pgfplots@current@point}%
}%

% #1:  arguments to \addplot plot[#1]
%   -> these are called 'behavior' options in the manual; they are set
%   immediately.
\def\pgfplots@start@plot@with@behavioroptions#1{%
	\begingroup
	\def\pgfplots@current@point@coordindex{0}% can be used inside of coordinate filters.
	\def\coordindex{\pgfplots@current@point@coordindex}% valid inside of \addplot
	\ifx\pgfplots@execute@at@begin@plot\pgfutil@empty
	\else
		\pgfplots@execute@at@begin@plot
	\fi
	\def\pgfplots@addplot@nonlegend@options{#1}%
	\ifx\pgfplots@addplot@nonlegend@options\pgfutil@empty
	\else
		\pgfplotsset{#1}%
	\fi
	% these styles may contain behavior options (error bars,
	% samples,... ) activate them!
	\pgfplotsset{/pgfplots/every axis plot,/pgfplots/every axis plot no \the\pgfplots@numplots/.try}%
}

% Initialises 
% \pgfplots@coord@stream@start
% \pgfplots@coord@stream@coord
% \pgfplots@coord@stream@end
% such that a following coordinate stream is processed properly. The
% following coordinate stream may come from different input methods.
%
% Arguments:
% #1:  all options of \addplot[...] (the plot style)
% #2:  any trailing path commands after the 'plot' command as such,
%      for example \addplot plot coordinates {...} -- (0,0);
%      would yield #2 =' -- (0,0)'
%
\long\def\pgfplots@PREPARE@COORD@STREAM#1#2{%
	\def\pgfplots@coord@stream@start@{%
		\pgfplotsapplistXXnewempty
		\ifpgfplots@errorbars@enabled
			\pgfplots@streamerrorbar@recordto{\pgfplots@recordederrorbar}%
			\pgfplots@streamerrorbarstart
		\else
			\let\pgfplots@recordederrorbar=\pgfutil@empty
		\fi
		\ifpgfplots@stackedmode
			\pgfplots@stacked@beginplot
		\fi
		%
		%\let\pgfplots@coord@stream@recorded=\pgfutil@empty
		%
	}%
	\let\pgfplots@coord@stream@coord@=\pgfplots@process@one@point
	\def\pgfplots@coord@stream@end@{%
		\ifpgfplots@errorbars@enabled
			\pgfplots@streamerrorbarend
		\fi
		\ifpgfplots@coord@stream@isfirst
			\pgfplots@warning{Empty plot silently dropped.}%
		\else
			\ifpgfplots@stackedmode
				\pgfplots@stacked@endplot
			\fi
			% Idea: use
			%   \scope[plot specification]
			%   <any paths for error bars>
			%   \endscope
			%   \draw plot coordinates {...};
			% to share plot specifications between error bars and plot
			% coordinates. Unfortunately, it is NOT sufficient to use
			% \tikzset{#1}
			\edef\pgfplots@addplot@preoptionsTMP{/pgfplots/every axis plot,/pgfplots/every axis plot no \the\pgfplots@numplots/.try}%
			\expandafter\pgfplots@rememberplotspec\expandafter{\pgfplots@addplot@preoptionsTMP,#1,/pgfplots/every axis plot post}%
			% warning: rememberplotspec calls list macros which
			% overwrite \t@pgfplots@toka
			\t@pgfplots@toka=\expandafter{\pgfplots@addplot@preoptionsTMP,#1,/pgfplots/every axis plot post}%
			\xdef\pgfplots@last@plot@style{\the\t@pgfplots@toka}% store it for \label commands.
			% ATTENTION: do NOT call list macros from here on!
			%
			\ifpgfplots@datascaletrafo@initialised
				\pgfplots@addplot@get@named@startendpoints@command\pgfplots@loc@TMPa
				\t@pgfplots@tokc=\expandafter{\pgfplots@loc@TMPa}%
			\else
				\t@pgfplots@tokc={}%
			\fi
			\ifx\pgfplots@recordederrorbar\pgfutil@empty
				\let\pgfplots@loc@TMPb=\pgfutil@empty%
			\else
				\t@pgfplots@tokb=\expandafter{\pgfplots@recordederrorbar}%
				\def\pgfplots@loc@TMPb{%
					\noexpand\pgfplots@errorbars@finishwithstyleoptions[current plot style]{\the\t@pgfplots@tokb}%
				}%
			\fi
			% assembe a \pgfplots@addplot@enqueue@coords command ...
			% BEGIN HERE ...
			% vvvvvvvvvv
			\xdef\pgfplots@glob@TMPa{%
				\noexpand\pgfplots@addplot@enqueue@coords
				{% precommand:
					\noexpand\def\noexpand\plotnum{\the\pgfplots@numplots}%
					\noexpand\pgfplots@initzerolevelhandler
					\the\t@pgfplots@tokc% named start/end points (if already available)
					\noexpand\pgfkeysdef{/tikz/current plot style}{\noexpand\pgfkeysalso{\the\t@pgfplots@toka}}%
					\pgfplots@loc@TMPb% error bar commands
				}%
				{% draw command:
					\noexpand\draw%
				}%
			}%
			\pgfplotsapplistXXlet\pgfplots@coord@stream@recorded
			\pgfplotsapplistXXclear
			\t@pgfplots@tokc=\expandafter{\pgfplots@coord@stream@recorded}%
			\t@pgfplots@tokb={#2;}%
			\t@pgfplots@toka=\expandafter{\pgfplots@glob@TMPa}%
			\xdef\pgfplots@glob@TMPa{%
				\the\t@pgfplots@toka
				{% coordinates which need to be processed in \endaxis:
					plot coordinates {\the\t@pgfplots@tokc}\the\t@pgfplots@tokb
				}%
				{% postcommand
				}%
			}%
			\pgfplots@glob@TMPa
			%^^^^^^^^^^^^ ... END of \pgfplots@addplot@enqueue@coords HERE
			\pgfplots@end@plot
		\fi
	}%
}%

\def\pgfplots@end@plot{%
	\global\advance\pgfplots@numplots by1\relax%
	\ifx\pgfplots@execute@at@end@plot\pgfutil@empty
	\else
		\pgfplots@execute@at@end@plot
	\fi
	\global\let\pgfplots@glob@TMPa=\relax
	\ifpgfplots@collect@firstplot@astick
		\ifnum\pgfplots@numplots=1\relax
			\t@pgfplots@toka=\expandafter{\pgfplots@firstplot@coords@x}%
			\t@pgfplots@tokb=\expandafter{\pgfplots@firstplot@coords@y}%
			\xdef\pgfplots@glob@TMPa{%
				\noexpand\def\noexpand\pgfplots@firstplot@coords@x{\the\t@pgfplots@toka}%
				\noexpand\def\noexpand\pgfplots@firstplot@coords@y{\the\t@pgfplots@tokb}%
			}%
		\fi
	\fi
	\endgroup
	\pgfplots@glob@TMPa% see above
}

% #1: arguments to \addplot[...]
% #2: the plot coordinates
% #3: any trailing path command before the final ';'. It will be used as-is.
\long\def\pgfplots@addplotimpl@coordinates#1plot coordinates#2#3;{%
%\tracingmacros=2\tracingcommands=2
%\pgfplots@message{processing plots coords with trailing path '#3'}%
	\pgfplots@PREPARE@COORD@STREAM{#1}{#3}%
	\pgfplots@coord@stream@foreach{#2}%
}%

\newif\ifpgfplots@update@limits@for@one@point@ISCLIPPED
\def\pgfplots@math@ONE{1.0}%

\def\pgfplots@streamerrorbarstart{%
}%
\def\pgfplots@streamerrorbarend{%
}%
\def\pgfplots@streamerrorbarcoords#1#2{%
}%

\def\pgfplots@streamerrorbar@recordto#1{%
	\def\pgfplots@streamerrorbarstart{%
		\pgfplotsapplistXnewempty\pgfplots@streamerrorbar@recordto@@
	}%
	\def\pgfplots@streamerrorbarend{%
		\pgfplotsapplistXlet#1=\pgfplots@streamerrorbar@recordto@@
		\pgfplotsapplistXnewempty\pgfplots@streamerrorbar@recordto@@% clear
	}%
	\def\pgfplots@streamerrorbarcoords##1##2{%
		\pgfplotsapplistXpushback{\pgfplots@errorbar@draw{##1}{##2}}\to\pgfplots@streamerrorbar@recordto@@
	}%
}
\def\pgfplots@streamerrorbar@directdraw{%
	\def\pgfplots@streamerrorbarstart{}%
	\def\pgfplots@streamerrorbarend{}%
	\def\pgfplots@streamerrorbarcoords##1##2{%
		\pgfplots@errorbar@draw{##1}{##2}%
	}%
}
	


% Updates the current x and y limits for point (#1,#2).
%
% The point coordinates may be given in floating point format, see
% below.
%
% Please note that if user specified limits are given, automatic
% limits are only applied to points which fall into the user specified
% clipping region.
%
% PRECONDITIONS:
% - the input coordinates have been parsed correctly (floating point
%   format for linear axis, log applied for logarithmic ones)
%
% #3= error for x coord (or empty)
% #4= error for y coord (or empty)
\long\def\pgfplots@update@limits@for@one@point#1#2#3#4{%
%\tracingmacros=2\tracingcommands=2
%\pgfplots@message{Updating limits for (#1,#2) ...}%
	\ifpgfplots@autocomputeanylimits
		\pgfplots@update@limits@for@one@point@ISCLIPPEDfalse
		\ifpgfplots@autocompute@all@limits
		\else
			% check whether we need to clip limits:
			\ifpgfplots@clip@limits
				\ifpgfplots@autocompute@xmin
				\else
					\ifpgfplots@xislinear
						\pgfmathfloatlessthan@{#1}{\pgfplots@xmin}%
						\ifpgfmathfloatcomparison
							\pgfplots@update@limits@for@one@point@ISCLIPPEDtrue
						\fi
					\else
						\pgfmathlessthan@{#1}{\pgfplots@xmin}%
						\ifx\pgfmathresult\pgfplots@math@ONE
							\pgfplots@update@limits@for@one@point@ISCLIPPEDtrue
						\fi
					\fi
				\fi
				\ifpgfplots@autocompute@xmax
				\else
					\ifpgfplots@xislinear
						\pgfmathfloatlessthan@{\pgfplots@xmax}{#1}%
						\ifpgfmathfloatcomparison
							\pgfplots@update@limits@for@one@point@ISCLIPPEDtrue
						\fi
					\else
						\pgfmathlessthan@{\pgfplots@xmax}{#1}%
						\ifx\pgfmathresult\pgfplots@math@ONE
							\pgfplots@update@limits@for@one@point@ISCLIPPEDtrue
						\fi
					\fi
				\fi
				\ifpgfplots@autocompute@ymin
				\else
					\ifpgfplots@yislinear
						\pgfmathfloatlessthan@{#2}{\pgfplots@ymin}%
						\ifpgfmathfloatcomparison
							\pgfplots@update@limits@for@one@point@ISCLIPPEDtrue
						\fi
					\else
						\pgfmathlessthan@{#2}{\pgfplots@ymin}%
						\ifx\pgfmathresult\pgfplots@math@ONE
							\pgfplots@update@limits@for@one@point@ISCLIPPEDtrue
						\fi
					\fi
				\fi
				\ifpgfplots@autocompute@ymax
				\else
					\ifpgfplots@yislinear
						\pgfmathfloatlessthan@{\pgfplots@ymax}{#2}%
						\ifpgfmathfloatcomparison
							\pgfplots@update@limits@for@one@point@ISCLIPPEDtrue
						\fi
					\else
						\pgfmathlessthan@{\pgfplots@ymax}{#2}%
						\ifx\pgfmathresult\pgfplots@math@ONE
							\pgfplots@update@limits@for@one@point@ISCLIPPEDtrue
						\fi
					\fi
				\fi
			\fi
		\fi
		%
		%
		%
		% Update limits:
		\ifpgfplots@update@limits@for@one@point@ISCLIPPED
		\else
			\ifpgfplots@autocompute@xmin
				\ifpgfplots@xislinear
					\pgfmathfloatmin@{\pgfplots@xmin}{#1}%
					\global\let\pgfplots@xmin=\pgfmathresult
				\else
					\pgfmathmin@{\pgfplots@xmin}{#1}%
					\global\let\pgfplots@xmin=\pgfmathresult
				\fi
			\fi
			\ifpgfplots@autocompute@xmax
				\ifpgfplots@xislinear
					\pgfmathfloatmax@{\pgfplots@xmax}{#1}%
					\global\let\pgfplots@xmax=\pgfmathresult
				\else
					\pgfmathmax@{\pgfplots@xmax}{#1}%
					\global\let\pgfplots@xmax=\pgfmathresult
				\fi
			\fi
			\ifpgfplots@autocompute@ymin
				\ifpgfplots@yislinear
					\pgfmathfloatmin@{\pgfplots@ymin}{#2}%
					\global\let\pgfplots@ymin=\pgfmathresult
				\else
					\pgfmathmin@{\pgfplots@ymin}{#2}%
					\global\let\pgfplots@ymin=\pgfmathresult
				\fi
			\fi
			\ifpgfplots@autocompute@ymax
				\ifpgfplots@yislinear
					\pgfmathfloatmax@{\pgfplots@ymax}{#2}%
					\global\let\pgfplots@ymax=\pgfmathresult
				\else
					\pgfmathmax@{\pgfplots@ymax}{#2}%
					\global\let\pgfplots@ymax=\pgfmathresult
				\fi
			\fi
		\fi
	\fi
	%
	% Compute data range:
	\ifpgfplots@autocompute@all@limits
		\global\let\pgfplots@data@xmin=\pgfplots@xmin
		\global\let\pgfplots@data@xmax=\pgfplots@xmax
		\global\let\pgfplots@data@ymin=\pgfplots@ymin
		\global\let\pgfplots@data@ymax=\pgfplots@ymax
	\else
		% Attention: it is only done for linear axis!
		\ifpgfplots@xislinear
			\pgfmathfloatmin@{\pgfplots@data@xmin}{#1}%
			\global\let\pgfplots@data@xmin=\pgfmathresult
			\pgfmathfloatmax@{\pgfplots@data@xmax}{#1}%
			\global\let\pgfplots@data@xmax=\pgfmathresult
		\fi
		\ifpgfplots@yislinear
			\pgfmathfloatmin@{\pgfplots@data@ymin}{#2}%
			\global\let\pgfplots@data@ymin=\pgfmathresult
			\pgfmathfloatmax@{\pgfplots@data@ymax}{#2}%
			\global\let\pgfplots@data@ymax=\pgfmathresult
		\fi
	\fi
%\pgfplots@message{Updated limits: (\pgfplots@xmin,\pgfplots@ymin) rectangle  (\pgfplots@xmax,\pgfplots@ymax).}%
%\tracingmacros=0\tracingcommands=0
}
\let\pgfplots@update@limits@for@one@point@orig=\pgfplots@update@limits@for@one@point

\def\pgfplots@invoke@filter#1#2{%
	\pgfkeysvalueof{/pgfplots/#2 filter/.@cmd}#1\pgfeov%
}%

% #3= error for x coord (or empty)
% #4= error for y coord (or empty)
\def\pgfplots@process@one@point#1#2#3#4{%
	\pgfplots@prepare@xcoord{#1}%
	\expandafter\pgfplots@invoke@filter\expandafter{\pgfmathresult}{x}%
	\let\pgfplots@current@point@x=\pgfmathresult
	%
	\pgfplots@prepare@ycoord{#2}%
	\expandafter\pgfplots@invoke@filter\expandafter{\pgfmathresult}{y}%
	\let\pgfplots@current@point@y=\pgfmathresult
	%
	\ifpgfplots@xislinear
		\ifx\pgfplots@current@point@x\pgfutil@empty
		\else
			\pgfmathfloatparsenumber{\pgfplots@current@point@x}%
			\expandafter\pgfmathfloat@decompose@F\pgfmathresult\relax\c@pgf@counta
			\ifnum\c@pgf@counta>2
				\let\pgfplots@current@point@x=\pgfutil@empty
			\else
				\let\pgfplots@current@point@x=\pgfmathresult
			\fi
		\fi
	\fi
	%
	\ifpgfplots@yislinear
		\ifx\pgfplots@current@point@y\pgfutil@empty
		\else
			\pgfmathfloatparsenumber{\pgfplots@current@point@y}%
			\expandafter\pgfmathfloat@decompose@F\pgfmathresult\relax\c@pgf@counta
			\ifnum\c@pgf@counta>2
				\let\pgfplots@current@point@y=\pgfutil@empty
			\else
				\let\pgfplots@current@point@y=\pgfmathresult
			\fi
		\fi
	\fi
	%
	\ifx\pgfplots@current@point@x\pgfutil@empty
		\ifpgfplots@warn@for@filter@discards
			\pgfplots@message{NOTE: coordinate (#1,#2) has been dropped because of the x-coordinate filter.}%
		\fi
	\else
		\ifx\pgfplots@current@point@y\pgfutil@empty
			\ifpgfplots@warn@for@filter@discards
				\pgfplots@message{NOTE: coordinate (#1,#2) has been dropped because of the y-coordinate filter.}%
			\fi
		\else
			%
			\ifpgfplots@apply@datatrafo
				\ifpgfplots@datascaletrafo@initialised
					% apply data transformation directly.
					\ifpgfplots@apply@datatrafo@x
						\pgfplots@datascaletrafo@x\pgfplots@current@point@x
						\let\pgfplots@current@point@x=\pgfmathresult
					\fi
					\ifpgfplots@apply@datatrafo@y
						\pgfplots@datascaletrafo@y\pgfplots@current@point@y
						\let\pgfplots@current@point@y=\pgfmathresult
					\fi
				\fi
			\fi
			% All following routines (limit updating/stacking/error
			% bars) will use float numerics if necessary (controlled
			% by ifs).
			\ifpgfplots@stackedmode
				\pgfplots@stacked@preparepoint@inmacro{\pgfplots@current@point@x}{\pgfplots@current@point@y}%
				\ifpgfplots@datascaletrafo@initialised% is also true if there is no scale trafo.
					\pgfplots@stacked@finishpoint{\pgfplots@current@point@x}{\pgfplots@current@point@y}%
				\else
					% the finishpoint routine will be invoked at
					% \endaxis.
				\fi
			\fi
			% update also axis / data limits:
			\pgfplots@update@limits@for@one@point{\pgfplots@current@point@x}{\pgfplots@current@point@y}{}{}%
			\ifpgfplots@errorbars@enabled
				\pgfplots@process@errorbar@for{\pgfplots@current@point@x}{\pgfplots@current@point@y}{#3}{#4}{#1}{#2}%
			\fi
			%
			\edef\pgfplots@loc@TMPa{(\pgfplots@current@point@x,\pgfplots@current@point@y)}%
			\expandafter\pgfplotsapplistXXpushback\expandafter{\pgfplots@loc@TMPa}%
			%\t@pgfplots@tokc=\expandafter{\pgfplots@coord@stream@recorded}%
			%\edef\pgfplots@coord@stream@recorded{\the\t@pgfplots@tokc (\pgfplots@current@point@x,\pgfplots@current@point@y)}%
			%
			\ifpgfplots@collect@firstplot@astick
				\ifnum\pgfplots@numplots=0
					\ifx\pgfplots@firstplot@coords@x\pgfutil@empty
						\t@pgfplots@tokc=\expandafter{}%
					\else
						\t@pgfplots@tokc=\expandafter{\pgfplots@firstplot@coords@x,}%
					\fi
					\edef\pgfplots@firstplot@coords@x{\the\t@pgfplots@tokc\pgfplots@current@point@x}%
					\ifx\pgfplots@firstplot@coords@y\pgfutil@empty
						\t@pgfplots@tokc=\expandafter{}%
					\else
						\t@pgfplots@tokc=\expandafter{\pgfplots@firstplot@coords@y,}%
					\fi
					\edef\pgfplots@firstplot@coords@y{\the\t@pgfplots@tokc\pgfplots@current@point@y}%
				\fi
			\fi
		\fi
	\fi
	%
	% increase \pgfplots@current@point@coordindex:
	\begingroup
	\c@pgf@counta=\pgfplots@current@point@coordindex
	\advance\c@pgf@counta by1\relax
	\edef\pgfmathresult{\the\c@pgf@counta}%
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
	\let\pgfplots@current@point@coordindex=\pgfmathresult
}

% Internal stream methods.
%
% Please overwrite \pgfplots@coord@stream@start@,
% \pgfplots@coord@stream@end@ and \pgfplots@coord@stream@coord@
% if you implement streams.
%
% FIXME: REPLACE THIS HERE WITH METHODS OF THE VISUALIZATION FRAMEWORK
\newif\ifpgfplots@coord@stream@isfirst
\def\pgfplots@coord@stream@start{%
	\pgfplots@coord@stream@isfirsttrue
	\pgfplots@coord@stream@start@}%
\def\pgfplots@coord@stream@end{\pgfplots@coord@stream@end@}

% Will be invoked for every point coordinate.
%
% It invokes \pgfplots@coord@stream@coord@.
% It is expected to assign \pgfplots@current@point@x and
% \pgfplots@current@point@y
%
% It is expected to
% (#1,#2) : x, y coordinates
% (#3,#4) : any x, y errors (or empty)
\def\pgfplots@coord@stream@coord#1#2#3#4{%
	\pgfplots@coord@stream@coord@{#1}{#2}{#3}{#4}%
	\ifpgfplots@coord@stream@isfirst
		\ifx\pgfplots@currentplot@firstcoord@x\pgfutil@empty
		\else
			\ifx\pgfplots@currentplot@firstcoord@y\pgfutil@empty
			\else
				\let\pgfplots@currentplot@firstcoord@x=\pgfplots@current@point@x
				\let\pgfplots@currentplot@firstcoord@y=\pgfplots@current@point@y
				\pgfplots@coord@stream@isfirstfalse
			\fi
		\fi
	\fi
	\ifx\pgfplots@current@point@x\pgfutil@empty
	\else
		\ifx\pgfplots@current@point@y\pgfutil@empty
		\else
			\let\pgfplots@currentplot@lastcoord@x=\pgfplots@current@point@x
			\let\pgfplots@currentplot@lastcoord@y=\pgfplots@current@point@y
		\fi
	\fi
}%

% A looping method which applies
% \pgfplots@coord@stream@start
% for each coordinate '(x,y)'  or '(x,y) +- (ex,ey)', call
%   \pgfplots@coord@stream@coord{x}{y}{ex}{ey}
% \pgfplots@coord@stream@end
%
% #1 a sequence of coordinates of the form 
%   '(x,y)'
%   or
%   '(x,y) +- (ex,ey)'
%   separated by white-space.
\long\def\pgfplots@coord@stream@foreach#1{%
	\pgfplots@coord@stream@start
	\pgfplots@foreach@plot@coord@do%
		\pgfplots@coord@stream@coord
	\for
	plot coordinates {#1};%
	\pgfplots@EOI
	\pgfplots@coord@stream@end
}%

% this is a convenience macro to save storage in the long coordinate
% lists.
\def\pgfplots@stream#1#2{\pgfplotstreampoint{\pgfqpoint{#1}{#2}}}

\newif\ifpgfplots@record@marker@stream
% Takes a sequence of PREPARED coordinates which are given in floating
% point representation and applies the data scaling trafo (if
% necessary).
%
% Any coordinate will be plotted with the selected PGF plot handler.
%
% This stream is designed to be done at the end of an axis.
% See \pgfplots@coord@stream@finalize@storedcoords@START
%
% #1 : a macro which will be filled with a pgf plot stream for the
% marker points.
\def\pgfplots@coord@stream@INIT@finalize@storedcoords#1{%
	%
	% Init the plot handlers:
	\pgfplots@getcurrent@plothandler\pgfplots@basiclevel@plothandler
	\pgfplots@gettikzinternal@keyval{mark}{tikz@plot@mark}{}%
	%
	\ifx\tikz@plot@mark\pgfutil@empty
		% mark=none : no need to waste time collecting marker
		% positions.
		\pgfplots@record@marker@streamfalse
	\else
		\ifx\pgfplots@basiclevel@plothandler\pgfplothandlerdiscard
			\ifpgfplots@clip@marker@paths
				% only marks: draw markers directly; no need for the
				% two-pass-approach.
				\let\pgfplots@basiclevel@plothandler=\relax
				\pgfplots@install@plotmark@handler
				\pgfplots@record@marker@streamfalse
			\else
				% collect mark positions... they will be drawn after
				% the clipped axis range. Clipping will only be
				% applied to their *positions*, not their paths.
				\pgfplots@record@marker@streamtrue
			\fi
		\else
			% ok, mark!=none and we also have a plot handler.
			% So, collect mark positions!
			\pgfplots@record@marker@streamtrue
		\fi
	\fi
	\gdef#1{}%
	%
	% Now, set up coordinate streams.
	\def\pgfplots@coord@stream@start@{%
		\ifpgfplots@apply@datatrafo
			\ifpgfplots@stackedmode
				\pgfplots@stacked@beginplot
			\fi
		\fi
		\pgfplots@basiclevel@plothandler
		\pgfplotstreamstart
		\let\pgfplots@data@scaletrafo@result=\pgfutil@empty
		\ifpgfplots@record@marker@stream
			\pgfplotsapplistXXnewempty
			\pgfplotsapplistXXpushback{\pgfplotstreamstart}%
			%\gdef#1{\pgfplotstreamstart}%
		\fi
	}%
	\def\pgfplots@coord@stream@end@{%
		\ifpgfplots@apply@datatrafo
			\ifpgfplots@stackedmode
				\pgfplots@stacked@endplot
			\fi
			\pgfplots@addplot@get@named@startendpoints@command\pgfplots@loc@TMPa
			\pgfplots@loc@TMPa
		\fi
		\pgfplotstreamend
		\ifpgfplots@record@marker@stream
			\pgfplotsapplistXXpushback{\pgfplotstreamend}%
			\pgfplotsapplistXXflushbuffers%
			\global\let#1=\pgfplotsapplistXX
			\pgfplotsapplistXXclear
			%\expandafter\gdef\expandafter#1\expandafter{#1\pgfplotstreamend}%
		\fi
	}%
	\ifpgfplots@apply@datatrafo
		\def\pgfplots@coord@stream@coord@##1##2##3##4{%
			\pgfplots@apply@data@scaletrafo@to@one@point{##1}{##2}{##3}{##4}%
			\pgfplots@coord@stream@finalize@currentpt
		}%
	\else
		\def\pgfplots@coord@stream@coord@##1##2##3##4{%
			\def\pgfplots@current@point@x{##1}%
			\def\pgfplots@current@point@y{##2}%
			\pgfplots@coord@stream@finalize@currentpt
		}%
	\fi
	%
	\def\pgfplots@coord@stream@finalize@currentpt{%
		\pgfqpointxy{\pgfplots@current@point@x}{\pgfplots@current@point@y}%
		\ifpgfplots@record@marker@stream
			\ifdim\pgf@x<\pgfplots@xcoordminTEX
			\else
				\ifdim\pgf@x>\pgfplots@xcoordmaxTEX
				\else
					\ifdim\pgf@y<\pgfplots@ycoordminTEX
					\else
						\ifdim\pgf@y>\pgfplots@ycoordmaxTEX
						\else
							\edef\pgfmathresult{\noexpand\pgfplots@stream{\the\pgf@x}{\the\pgf@y}}%
							\expandafter\pgfplotsapplistXXpushback\expandafter{\pgfmathresult}%
						\fi
					\fi
				\fi
			\fi
		\fi
		\pgfplotstreampoint{}% it will simply take \pgf@x and \pgf@y!
	}%
}
\def\pgfplots@addplot@get@named@startendpoints@command#1{%
	\edef#1{%
		\noexpand\pgfcoordinate{current plot begin}{\noexpand\pgfqpointxy{\pgfplots@currentplot@firstcoord@x}{\pgfplots@currentplot@firstcoord@y}}%
		\noexpand\pgfcoordinate{current plot end}{\noexpand\pgfqpointxy{\pgfplots@currentplot@lastcoord@x}{\pgfplots@currentplot@lastcoord@y}}%
	}%
}%

% INPUT: 
% 	either floating point or fixed point coordinates (depending on the
% 	state of the \ifpgfplots@apply@datatrafo boolean)
%
\long\def\pgfplots@coord@stream@finalize@storedcoords@START plot coordinates #1#2;\pgfplots@EOI{%
	\pgfplots@assert@tikzinternal@exists{tikz@make@last@position}%
	\pgfplots@stored@current@cmd[current plot style]
	\pgfextra
	\tikzset{every plot/.try}%
	\pgfplots@coord@stream@INIT@finalize@storedcoords\pgfplots@recorded@marker@stream%
	\pgfplots@coord@stream@foreach{#1}%
	\tikz@make@last@position{\pgfplotlastpoint}%  
	\endpgfextra
	#2;
	\ifx\pgfplots@recorded@marker@stream\pgfutil@empty
	\else
		\ifpgfplots@clip@marker@paths
			% Draw markers on top of the plot lines:
			%
			% FIXME: inefficient! Use \scope to set variables of 'current plot style' !?
			\pgfplots@stored@current@cmd[current plot style]
			\pgfextra 
				\pgfplots@install@plotmark@handler
				\pgfplots@recorded@marker@stream 
			\endpgfextra
			;
		\else
			% sigh... ok, store the marker list (once more again).
			% They need to be drawn after the clipped area.
			\pgfplots@stored@REMEMBER@MARK@COMMAND
		\fi
	\fi
	\gdef\pgfplots@recorded@marker@stream{}% clear
}%

% This method MUST be called while \pgfplots@stored@plotlist is
% evaluated, that means
% - \pgfplots@stored@* commands need to be valid,
% - the precommand has already been invoked.
% - pgfplots@recorded@marker@stream exists
% - current plot style is valid
\def\pgfplots@stored@REMEMBER@MARK@COMMAND{%
	\pgfkeysgetvalue{/tikz/current plot style/.@cmd}{\pgfplots@loc@TMPa}%
	\t@pgfplots@toka=\expandafter{\pgfplots@loc@TMPa\pgfeov}%
	\t@pgfplots@tokb=\expandafter{\pgfplots@stored@current@cmd[current plot style]}%
	\t@pgfplots@tokc=\expandafter{\pgfplots@recorded@marker@stream}%
	\edef\pgfplots@loc@TMPa{%
		\noexpand\pgfkeysdef{/tikz/current plot style}{\the\t@pgfplots@toka}%
		\the\t@pgfplots@tokb
		\noexpand\pgfextra
		\noexpand\pgfplots@install@plotmark@handler
		\the\t@pgfplots@tokc
		\noexpand\endpgfextra
		;}%
	\expandafter\pgfplotslistpushbackglobal\expandafter{\pgfplots@loc@TMPa}\to\pgfplots@stored@markerlist
}%

\def\pgfplots@install@plotmark@handler{%
	\pgfplots@assert@tikzinternal@exists{tikz@options}%
	% note: I can't check on tikz@transform because it can be
	% '\relax'.
	\pgfplots@gettikzinternal@keyval{mark indices}{tikz@mark@list}{}%
	\pgfplots@gettikzinternal@keyval{mark}{tikz@plot@mark}{}%
	%
	% do not reset \tikz@options: draw color may be acquired
	% from 'current plot style'
	%\let\tikz@options=\pgfutil@empty%
	\let\tikz@transform=\pgfutil@empty%
	\tikzset{every plot/.try,every mark}%
	\tikz@options
	\ifx\tikz@mark@list\pgfutil@empty%
		\pgfplothandlermark{\tikz@transform\pgfuseplotmark{\tikz@plot@mark}}%
	\else
		\pgfplothandlermarklisted{\tikz@transform\pgfuseplotmark{\tikz@plot@mark}}{\tikz@mark@list}%
	\fi
}%

% A looping command to loop through plot coordinates.
% For every point, #1{X}{Y} will be invoked.
%
% No scoping is used during this operation, so you can access outer
% variables.
\long\def\pgfplots@foreach@plot@coord@do#1\for plot coordinates #2;\pgfplots@EOI{%
	\def\pgfplots@foreach@plot@coord@do@CMD{#1}%
	\pgfplots@foreach@plot@coord@ITERATE#2\pgfplots@EOI%
}

\def\pgfplots@foreach@plot@coord@ITERATE{%
	\pgfutil@ifnextchar\pgfplots@EOI{%
		\pgfplots@foreach@plot@coord@FINISH%
	}{%
		\pgfplots@foreach@plot@coord@NEXT%
	}%
}

\def\pgfplots@foreach@plot@coord@NEXT(#1,#2){%
	\pgfutil@ifnextchar+{%
		\pgfplots@foreach@plot@coord@NEXT@WITH@ERRORRANGE{#1}{#2}%
	}{%
		\pgfplots@foreach@plot@coord@do@CMD{#1}{#2}{}{}%
		\pgfplots@foreach@plot@coord@ITERATE
	}%
}

% processing something like '(x,y) +- (error_x,error_y)'
\def\pgfplots@foreach@plot@coord@NEXT@WITH@ERRORRANGE#1#2+-#3({%
	\pgfplots@foreach@plot@coord@NEXT@WITH@ERRORRANGE@{#1}{#2}%
}
\def\pgfplots@foreach@plot@coord@NEXT@WITH@ERRORRANGE@#1#2#3,#4){%
	\pgfplots@foreach@plot@coord@do@CMD{#1}{#2}{#3}{#4}%
	\pgfplots@foreach@plot@coord@ITERATE
}

\def\pgfplots@foreach@plot@coord@FINISH\pgfplots@EOI{}

	
% #1= x coord
% #2= y coord
% #3= error for x coord (or empty)
% #4= error for y coord (or empty)
\def\pgfplots@apply@data@scaletrafo@to@one@point#1#2#3#4{%
	\ifpgfplots@apply@datatrafo@x
		\pgfplots@datascaletrafo@x{#1}%
		\let\pgfplots@current@point@x=\pgfmathresult
	\else
		\def\pgfplots@current@point@x{#1}%
	\fi
	\ifpgfplots@apply@datatrafo@y
		\pgfplots@datascaletrafo@y{#2}%
		\let\pgfplots@current@point@y=\pgfmathresult
	\else
		\def\pgfplots@current@point@y{#2}%
	\fi
	\ifpgfplots@stackedmode
		% all these calls work with pgfmath; no more floating point
		% arithmetics are applied.
		\pgfplots@stacked@getnextzerolevelpoint
		\pgfplots@stacked@finishpoint{\pgfplots@current@point@x}{\pgfplots@current@point@y}%
		\pgfplots@stacked@rememberzerolevelpoint@for@next@plot{(\pgfplots@current@point@x,\pgfplots@current@point@y)}%
	\fi
%	\t@pgfplots@tokc=\expandafter{\pgfplots@data@scaletrafo@result}%
%	\edef\pgfplots@data@scaletrafo@result{\the\t@pgfplots@tokc(\pgfplots@current@point@x,\pgfplots@current@point@y)}%
}

% This thing here shall draw all error bar commands listed in '#2'.
%
% It will be invoked when any plotting commands take effect (that
% means all limits are computed; the axis has been drawn,
% transformations are set up...)
\def\pgfplots@errorbars@finishwithstyleoptions[#1]#2{%
	\scope[/pgfplots/.cd,#1,/pgfplots/every error bar]% it used the /pgfplots/.unknown
	#2%
	\endscope
}

\def\pgfplots@errorbar@draw@float(#1,#2)(#3,#4){%
	\ifpgfplots@apply@datatrafo@x
		\pgfplots@datascaletrafo@x{#1}%
		\let\pgfplots@xarg=\pgfmathresult%
		\pgfplots@datascaletrafo@x{#3}%
		\let\pgfplots@error@xarg=\pgfmathresult%
	\else
		\def\pgfplots@xarg{#1}%
		\def\pgfplots@error@xarg{#3}%
	\fi
	\ifpgfplots@apply@datatrafo@y
		\pgfplots@datascaletrafo@y{#2}%
		\let\pgfplots@yarg=\pgfmathresult%
		\pgfplots@datascaletrafo@y{#4}%
		\let\pgfplots@error@yarg=\pgfmathresult%
	\else
		\def\pgfplots@yarg{#2}%
		\def\pgfplots@error@yarg{#4}%
	\fi
	\edef\pgfplots@loc@TMPa{{(\pgfplots@xarg,\pgfplots@yarg)}{(\pgfplots@error@xarg,\pgfplots@error@yarg)}}%
	\def\pgfplots@loc@TMPb{\pgfkeysvalueof{/pgfplots/error bars/draw error bar/.@cmd}}%
	\expandafter\pgfplots@loc@TMPb\pgfplots@loc@TMPa\pgfeov
}

\def\pgfplots@errorbar@draw#1#2{%
	\begingroup
	\ifpgfplots@apply@datatrafo
		\pgfplots@errorbar@draw@float#1#2
	\else
		\pgfkeysvalueof{/pgfplots/error bars/draw error bar/.@cmd}{#1}{#2}\pgfeov%
	\fi
	\endgroup
}%

% Also provides UNFILTERED arguments x (#5) and y (#6). These are use
% in case of logplots, because we may need to compute log( x + e_x )
% or log( y + e_y ).
\def\pgfplots@process@errorbar@for#1#2#3#4#5#6{%
%	\begingroup
	\edef\pgfplots@xarg{#1}%
	\edef\pgfplots@yarg{#2}%
	\def\pgfplots@xarg@unfiltered{#5}%
	\def\pgfplots@yarg@unfiltered{#6}%
	\edef\pgfplots@error@xarg{#3}%
	\edef\pgfplots@error@yarg{#4}%
	\def\pgfplots@loc@TMPa{0}%
	\ifx\pgfplots@loc@TMPa\pgfplots@error@xarg
		\let\pgfplots@error@xarg=\pgfutil@empty
	\fi
	\ifx\pgfplots@loc@TMPa\pgfplots@error@yarg
		\let\pgfplots@error@yarg=\pgfutil@empty
	\fi
	%  FIXME : INEFFICIENT! This code here does every computation 
	%  multiple times!
	\ifcase\pgfplots@errorbars@xdirection
	\or
		\pgfplots@process@errorbar@@for{x}{+}1%
	\or
		\pgfplots@process@errorbar@@for{x}{-}2%
	\or
		\pgfplots@process@errorbar@@for{x}{+}1%
		\pgfplots@process@errorbar@@for{x}{-}2%
	\fi
	\ifcase\pgfplots@errorbars@ydirection
	\or
		\pgfplots@process@errorbar@@for{y}{+}1%
	\or
		\pgfplots@process@errorbar@@for{y}{-}2%
	\or
		\pgfplots@process@errorbar@@for{y}{+}1%
		\pgfplots@process@errorbar@@for{y}{-}2%
	\fi
%	\endgroup
}

% #1: either 'x' or 'y'
% #2: either '+' or '-'
% #3: an integer representing the argument #2. It is '1' if #2='+'
%     and '2' is #2 = '-'.
\def\pgfplots@process@errorbar@@for#1#2#3{%
	\csname ifpgfplots@#1islinear\endcsname
		\edef\pgfplots@error@src{\csname pgfplots@#1arg\endcsname}%
		\ifcase\csname pgfplots@errorbars@#1mode\endcsname
			% fixed absolute error.
			\edef\pgfplots@error@coord{\csname pgfplots@errorbars@#1fixed\endcsname}%
			\pgfmathfloatparsenumber{\pgfplots@error@coord}%
			\let\pgfplots@error@coord=\pgfmathresult
			\ifnum#3=1
				\pgfmathfloatadd@{\pgfplots@error@src}{\pgfplots@error@coord}%
			\else
				\pgfmathfloatsubtract@{\pgfplots@error@src}{\pgfplots@error@coord}%
			\fi
			\let\pgfplots@error@coord=\pgfmathresult
		\or% fixed relative error:
			\pgfmathparse{(1#2\csname pgfplots@errorbars@#1rel\endcsname)}%
			\let\pgfplots@error@coord=\pgfmathresult
			\pgfmathfloatmultiplyfixed@{\pgfplots@error@src}{\pgfplots@error@coord}%
			\let\pgfplots@error@coord=\pgfmathresult
		\or% explicit absolute:
			\edef\pgfplots@error@coord{\csname pgfplots@error@#1arg\endcsname}%
			\ifx\pgfplots@error@coord\pgfutil@empty
			\else
				\pgfmathfloatparsenumber{\pgfplots@error@coord}%
				\let\pgfplots@error@coord=\pgfmathresult
				\ifnum#3=1
					\pgfmathfloatadd@{\pgfplots@error@src}{\pgfplots@error@coord}%
				\else
					\pgfmathfloatsubtract@{\pgfplots@error@src}{\pgfplots@error@coord}%
				\fi
				\let\pgfplots@error@coord=\pgfmathresult
			\fi
		\or% explicit relative:
			\edef\pgfplots@error@coord{\csname pgfplots@error@#1arg\endcsname}%
			\ifx\pgfplots@error@coord\pgfutil@empty
			\else
				\pgfmathparse{(1#2\pgfplots@error@coord)}%
				\let\pgfplots@error@coord=\pgfmathresult
				\pgfmathfloatmultiplyfixed@{\pgfplots@error@src}{\pgfplots@error@coord}%
				\let\pgfplots@error@coord=\pgfmathresult
			\fi
		\fi
	\else
		% LOGARITHMIC scaling. All errors are interpreted as 
		%   log(x +- e_x)
		% or
		%   log( x*(1+-e_x) )
		\ifcase\csname pgfplots@errorbars@#1mode\endcsname
			% fixed absolute, log( x +- e_x )
			\edef\pgfplots@error@src{\csname pgfplots@#1arg@unfiltered\endcsname}%
			\edef\pgfplots@error@coord{\csname pgfplots@errorbars@#1fixed\endcsname}%
			\pgfmathfloatparsenumber{\pgfplots@error@coord}%
			\let\pgfplots@error@coord=\pgfmathresult
			\pgfmathfloatparsenumber{\pgfplots@error@src}%
			\let\pgfplots@error@src=\pgfmathresult
			\ifnum#3=1
				\pgfmathfloatadd@{\pgfplots@error@src}{\pgfplots@error@coord}%
			\else
				\pgfmathfloatsubtract@{\pgfplots@error@src}{\pgfplots@error@coord}%
			\fi
			\pgfmathlog@float{\pgfmathresult}%
			\let\pgfplots@error@coord=\pgfmathresult
		\or% fixed relative, log( x ( 1+-e_x ) ) = log(x) + log(1+-e_x)
			\edef\pgfplots@error@src{\csname pgfplots@#1arg\endcsname}%
			\pgfmathparse{\pgfplots@error@src + ln(1#2\csname pgfplots@errorbars@#1rel\endcsname)}%
			\let\pgfplots@error@coord=\pgfmathresult%
		\or% explicit absolute
			\edef\pgfplots@error@src{\csname pgfplots@#1arg@unfiltered\endcsname}%
			\edef\pgfplots@error@coord{\csname pgfplots@error@#1arg\endcsname}%
			\ifx\pgfplots@error@coord\pgfutil@empty
			\else
				\pgfmathfloatparsenumber{\pgfplots@error@coord}%
				\let\pgfplots@error@coord=\pgfmathresult
				\pgfmathfloatparsenumber{\pgfplots@error@src}%
				\let\pgfplots@error@src=\pgfmathresult
				\ifnum#3=1
					\pgfmathfloatadd@{\pgfplots@error@src}{\pgfplots@error@coord}%
				\else
					\pgfmathfloatsubtract@{\pgfplots@error@src}{\pgfplots@error@coord}%
				\fi
				\pgfmathlog@float{\pgfmathresult}%
				\let\pgfplots@error@coord=\pgfmathresult
			\fi
		\or% explicit relative:
			\edef\pgfplots@error@src{\csname pgfplots@#1arg\endcsname}%
			\edef\pgfplots@error@coord{\csname pgfplots@error@#1arg\endcsname}%
			\ifx\pgfplots@error@coord\pgfutil@empty
			\else
				\pgfmathparse{\pgfplots@error@src + ln(1#2 \pgfplots@error@coord)}%
				\let\pgfplots@error@coord=\pgfmathresult%
			\fi
		\fi
	\fi
	\ifx\pgfplots@error@coord\pgfutil@empty
	\else
		\def\pgfplots@loc@TMPa{#1}%
		\def\pgfplots@loc@TMPb{x}%
		\ifx\pgfplots@loc@TMPa\pgfplots@loc@TMPb
			\pgfplots@update@limits@for@one@point{\pgfplots@error@coord}{\pgfplots@yarg}{}{}%
			\edef\pgfplots@loc@TMPa{%
				{(\pgfplots@xarg,\pgfplots@yarg)}%
				{(\pgfplots@error@coord,\pgfplots@yarg)}%
			}%
		\else
			\pgfplots@update@limits@for@one@point{\pgfplots@xarg}{\pgfplots@error@coord}{}{}%
			\edef\pgfplots@loc@TMPa{%
				{(\pgfplots@xarg,\pgfplots@yarg)}%
				{(\pgfplots@xarg,\pgfplots@error@coord)}%
			}%
		\fi
		\expandafter\pgfplots@streamerrorbarcoords\pgfplots@loc@TMPa
	\fi
}

\long\def\pgfplots@path#1;{%
	\pgfplots@path@enqueue{#1;}%
}

% This thing here shall be used to replace any '\path' where \axispath
% shall be used.
\long\def\pgfplots@replacement@for@tikz@path#1;{%
	\axispath\path#1;%
}


% Will be available as \closedcycle command inside of an axis.
%
% It closes the current plot by drawing lines to the last "zero
% level".
%
% That means the current plot is connected orthogonally with the
% x-axis, allowing fill commands.
%
% For stacked plots, \closedcycle is special (it connects with the
% previous \addplot command).
%
% Example:
% \addplot coordinates {(3,0.5) (4,2) (5,1)} \closedcycle;
\def\pgfplots@path@closed@cycle{%
	\ifpgfplots@stackedmode
		\pgfplots@stacked@path@closed@cycle
	\else
		\pgfplots@path@closed@cycle@std
	\fi
}
\def\pgfplots@path@closed@cycle@std{%
	|- (perpendicular cs: 
		vertical line through={(current plot begin)}, 
		horizontal line through={(\pgfplots@ZERO@x,\pgfplots@ZERO@y)})
	-- cycle
}%

% Remembers the plotting command #2 and '#3=plot coordinates {...} ...';
% for later postprocessing of the coordinates.
%
% #1: commands which should be executed before issueing the plotting
%        command #2 #3.
% #2:
%    the command which is responsable for drawing.
%    - If #2 is NOT '\pgfutil@empty', we expect #3 to contain only
%      EXPANDABLE DATA.
%      That's important for postponed floating point arithmetics in #3.
%    - If #2='\pgfutil@empty', we don't make any assumption about #3
%      and process it as-is.
%
% #3: see above.
%
% #4: commands which should be executed after '#2 #3'.
%
\long\def\pgfplots@path@enqueue@coords#1#2#3#4{%
	\ifpgfplots@draw@at@end
		\pgfplotslistpushbackglobal{#1}{#2}{#3}{#4}\to\pgfplots@stored@plotlist
	\else
		\begingroup
		#1#2#3#4%
		\endgroup
	\fi
}

% The same as \pgfplots@path@enqueue@coords, but this here also stores
% \pgfplots@addplot@nonlegend@options
\long\def\pgfplots@addplot@enqueue@coords#1#2#3#4{%
	\ifpgfplots@draw@at@end
		\ifx\pgfplots@addplot@nonlegend@options\pgfutil@empty
			\pgfplots@path@enqueue@coords{#1}{#2}{#3}{#4}%
		\else
			\expandafter
			\pgfplots@path@enqueue@coords
				\expandafter{%
				\expandafter\pgfplotsset\expandafter{\pgfplots@addplot@nonlegend@options}%
				#1}{#2}{#3}{#4}%
		\fi
	\else
		\pgfplots@path@enqueue@coords{#1}{#2}{#3}{#4}%
	\fi
}


% Remembers the plotting command #1.
\long\def\pgfplots@path@enqueue#1{%
	\pgfplots@path@enqueue@coords{}{}{#1}{}%
}


% Assigns a legend.
% Syntax:
% \legend{entry 1\\entry2\\entry3}
\def\pgfplots@command@legend{
	\pgfutil@ifnextchar[{%
		\pgfplots@error{Sorry, legend options are now deprecated. Legends are now TikZ-matrizes which provide better alignment and can be placed horizontally. See the manual for details.}%
		\pgfplots@command@legend@impl
	}{%
		\pgfplots@command@legend@impl
	}%
}

\def\pgfplots@command@legend@impl#1{%
	\pgfplots@assign@list\pgfplots@loc@TMPc{#1}%
	\global\let\pgfplots@legend=\pgfplots@loc@TMPc
}


\def\pgfplots@addlegendentry{%
	\pgfutil@ifnextchar[{%
		\pgfplots@addlegendentry@opts
	}{%
		\pgfplots@addlegendentry@opts[]%
	}%
}
\def\pgfplots@addlegendentry@opts[#1]#2{%
	\pgfplotslistpushbackglobal[#1]#2\to\pgfplots@legend
}

\def\pgfplots@pop@next@legend{{%
	\globaldefs=1
	\pgfplotslistcheckempty\pgfplots@plotspeclist
	\ifpgfplotslistempty
		\let\pgfplots@curplotlist=\pgfutil@empty
	\else
		\pgfplotslistpopfront\pgfplots@plotspeclist\to\pgfplots@curplotlist
	\fi
	%
	\pgfplotslistcheckempty\pgfplots@legend
	\ifpgfplotslistempty
		\let\pgfplots@curlegend=\pgfutil@empty
	\else
		\pgfplotslistpopfront\pgfplots@legend\to\pgfplots@curlegend
	\fi
	\advance\pgfplots@numplots by-1
}}

% This routine is called at the begin of every plot.
% It initialised a zero level stream.
%
% The default is to use '0' as zero level streams.
%
% This method is called as "precommand"; before any Tikz drawing
% commands have been started.
\def\pgfplots@initzerolevelhandler{%
	\ifpgfplots@stackedmode
		% ATTENTION: this thing here says:
		%    "draw zero level coordinates from list XYZ."
		% But at the time of this initialisation, the list will be EMPTY!
		%
		% It will be filled later. That's ok, because 
		% \pgfplots@initzerolevelhandler will be
		% used as 'precommand', that means before Tikz sees any
		% coordinates.
		\pgfplots@stacked@initzerolevelhandler
	\else
		\pgfplotxzerolevelstreamconstant{\pgfplots@ZERO@x}%
		\pgfplotyzerolevelstreamconstant{\pgfplots@ZERO@y}%
	\fi
}

\def\pgfplots@try@mirror@plot@handler{%
	\pgfplots@getcurrent@plothandler\pgfplots@basiclevel@plothandler
	% this method assigns '\tikz@plot@handler'.
	% That's ok and does not introduce incompatibilities.
	\ifx\pgfplots@basiclevel@plothandler\pgfplothandlerconstantlineto
		\let\tikz@plot@handler=\pgfplothandlerconstantlinetomarkright
	\else
		\ifx\pgfplots@basiclevel@plothandler\pgfplothandlerconstantlinetomarkright
			\let\tikz@plot@handler=\pgfplothandlerconstantlineto
		\fi
	\fi
}

\long\def\pgfplots@show@small@legendplots#1#2{
	\begingroup
	\def\pgfplots@loc@TMPb{#1}%
	\ifx\pgfplots@loc@TMPb\pgfutil@empty
	\else
		\pgfqkeys{/pgfplots/search path for tikz}{#1}%
	\fi
	\pgfkeysvalueof{/pgfplots/legend image code/.@cmd}#2\pgfeov
	\endgroup
}

\def\pgfplots@split@opts{%
	\pgfutil@ifnextchar[{%
		\pgfplots@split@opts@opts
	}{%
		\pgfplots@split@opts@opts[]%
	}%
}
\def\pgfplots@split@opts@opts[#1]#2\pgfplots@result@to#3#4{%
	\def#3{#2}%
	\def#4{#1}%
}

% Typesets a legend node.
%
% It will either typeset a previously computed legend (which needs to be
% stored in the macro \pgfplots@already@computed@legend@node)
%
% or it creates a legend, stores the commands into the macro named
% above and typesets it.
\def\pgfplots@createlegend{%
	\ifx\pgfplots@already@computed@legend@node\pgfutil@empty
		\pgfplotslistcheckempty\pgfplots@legend
		\ifpgfplotslistempty
			% No legend commands appeared in the document. So,
			% consider the key:
			\pgfkeysgetvalue{/pgfplots/legend entries}\pgfplots@legend
			\expandafter\pgfplots@assign@list\expandafter\pgfplots@legend\expandafter{\pgfplots@legend}%
			\pgfplotslistcheckempty\pgfplots@legend
		\fi
		\ifpgfplotslistempty
		\else
		%
		% 
		\begingroup
			% assemble a 
			% \matrix {
			% 	small plot  & legend1\\
			% 	small plot  & legend2\\
			% 	...
			% };
			% command [and using the 'legend columns' option]
			%
			% \t@pgfplots@toka={
			% 	small plot  & legend1\\
			% 	small plot  & legend2\\
			% 	...
			% }
			% ( I have allocated the token registers in my
			% liststructure.sty)
			% 
			% \global\def\pgfplots@glob@TMPa{
			% 	\matrix {
			% 		\TOKL@TA
			% 	};
			% }
			% -> finally, \pgfplots@glob@TMPa will contain the complete command.
			\t@pgfplots@toka={}%
			\let\curcolumnNum=\c@pgf@counta
			\let\maxcolumnCount=\c@pgf@countb
			\let\legendplotpos=\c@pgf@countc
			\legendplotpos\expandafter=\pgfplots@legend@plot@pos
			\curcolumnNum=0
			\maxcolumnCount=\pgfplots@legend@columns\relax
			%
			\loop
			\ifnum0<\pgfplots@numplots\relax
				\pgfplots@pop@next@legend
				\ifx\pgfplots@curlegend\pgfutil@empty
				\else
					\advance\curcolumnNum by1
					\begingroup
					\expandafter\pgfplots@split@opts\pgfplots@curlegend\pgfplots@result@to{\pgfplots@curlegend}{\pgfplots@curlegend@opts}%
					\ifcase\legendplotpos
						% legend plot pos=left 
						\t@pgfplots@tokb=\expandafter{%
								\expandafter\pgfplots@show@small@legendplots
								\expandafter{\pgfplots@curlegend@opts}}%
						\t@pgfplots@tokb=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\t@pgfplots@tokb\expandafter{\pgfplots@curplotlist}%
								\pgfmatrixnextcell\node}%
						\t@pgfplots@tokb=\expandafter\expandafter\expandafter{%
							\expandafter\the\expandafter\t@pgfplots@tokb
							\expandafter{\pgfplots@curlegend};}%
					\or
						% legend plot pos=right
						\t@pgfplots@tokb=\expandafter{%
							\expandafter\node
							\expandafter{\pgfplots@curlegend};%
							\pgfmatrixnextcell
							\pgfplots@show@small@legendplots}%
						\t@pgfplots@tokb=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\t@pgfplots@tokb\expandafter{\pgfplots@curlegend@opts}}%
						\t@pgfplots@tokb=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\t@pgfplots@tokb\expandafter{\pgfplots@curplotlist}}%
					\or
						% legend plot pos=none
						\t@pgfplots@tokb=\expandafter{\expandafter\node\expandafter{\pgfplots@curlegend};}%
					\fi
					\ifnum\curcolumnNum=\maxcolumnCount
						\t@pgfplots@tokb=\expandafter{\the\t@pgfplots@tokb\\}%
					\else
						\ifnum\pgfplots@numplots=0
							\t@pgfplots@tokb=\expandafter{\the\t@pgfplots@tokb\\}%
						\else
							\t@pgfplots@tokb=\expandafter{\the\t@pgfplots@tokb\pgfmatrixnextcell}%
						\fi
					\fi
					\xdef\pgfplots@glob@TMPa{%
						\the\t@pgfplots@toka
						\the\t@pgfplots@tokb
					}%
					\endgroup
					\ifnum\curcolumnNum=\maxcolumnCount
						\curcolumnNum=0
					\fi
					\expandafter\t@pgfplots@toka\expandafter{\pgfplots@glob@TMPa}%
				\fi
			\repeat
			\t@pgfplots@tokb={\matrix[/pgfplots/every axis legend]}%
			\xdef\pgfplots@glob@TMPa{%
				\noexpand\def\noexpand\plotnum{0}%
				\the\t@pgfplots@tokb {%
					\the\t@pgfplots@toka
				};%
			}%
		\endgroup
		\let\pgfplots@already@computed@legend@node=\pgfplots@glob@TMPa
		\fi
	\fi
%\pgfplots@message{Vor legende: \meaning\pgfplots@already@computed@legend@node}%
	\pgfplots@already@computed@legend@node
}

\newif\ifpgfplots@checkuniform@isfirst
% Checks whether the argument to xtick or ytick is a UNIFORM tick
% sequence.
%
% A uniform tick sequence is 0,...,10 and 3,4,5 and -5,-4,-2 but 
% NOT 0,2,4 or 4,10.
%
% Furthermore, any NON-integer tick arguments are also assumed to be
% NOT uniform.
%
% INPUT:
% #1: a tick argument (i.e. something which can be put to 
%     \foreach \x in {#1})
%
% OUTPUT:
%    \pgfplots@isuniformticktrue
%    or
%    \pgfplots@isuniformtickfalse
% depending on the check.
% This variable will be set globally.
\def\pgfplots@checkisuniformLOGtick#1{%
	\begingroup
	\global\pgfplots@isuniformticktrue
	\pgfplots@checkuniform@isfirsttrue
	\foreach \x in {#1}{%
		\pgfmathmultiply@\x\reciproclogten
		\let\cur=\pgfmathresult
		% check whether
		%  \cur - last == 1 (last = \pgfplots@glob@TMPb)
		\ifpgfplots@checkuniform@isfirst
			\global\pgfplots@checkuniform@isfirstfalse
		\else
			\pgfmathsubtract@\cur\pgfplots@glob@TMPb%
			\pgfmathapproxequalto@\pgfmathresult{1.0}%
			\ifpgfmathcomparison
			\else
				\global\pgfplots@isuniformtickfalse
				\breakforeach
			\fi
		\fi
		\global\let\pgfplots@glob@TMPb=\cur
	}%
	\endgroup
}

% Checks whether the linear tick sequence #1 is a uniform tick.
%
% It also assigns pgfplots@tick@distance@#1  as the distance.
%
% see \pgfplots@checkisuniformLOGtick for details.
%
% #1: a tick sequence (expanded)
% #2: a macro which will be filled with the tick distance. This is
% only valid if \pgfplots@isuniformticktrue.
\def\pgfplots@checkisuniformLINEARtick#1#2{%
	\begingroup
	\global\pgfplots@isuniformticktrue
	\pgfplots@checkuniform@isfirsttrue
	\global\let\pgfplots@glob@TMPb=\pgfutil@empty
	\global\def\pgfplots@glob@TMPa{1}%
	\foreach \x in {#1}{%
		\ifx\pgfplots@glob@TMPb\pgfutil@empty
		\else
			\pgfmathsubtract@\x\pgfplots@glob@TMPb
			\ifpgfplots@checkuniform@isfirst
				% remember first distance h = x_1 - x_0
				\global\let\pgfplots@glob@TMPa=\pgfmathresult
				\global\pgfplots@checkuniform@isfirstfalse
			\else
				% check whether x_i - x_{i-1} = h
				\pgfmathapproxequalto@\pgfmathresult\pgfplots@glob@TMPa%
				\ifpgfmathcomparison
				\else
					\global\pgfplots@isuniformtickfalse
					\breakforeach
				\fi
			\fi
		\fi
		\global\let\pgfplots@glob@TMPb=\x%
	}%
	\endgroup
	\let#2=\pgfplots@glob@TMPa
}

\def\skipsuffixzero#1.#2|{
	{%
	\def\pgfplots@loc@TMPa{#2}%
	\def\pgfplots@loc@TMPb{0}%
	\ifx\pgfplots@loc@TMPa\pgfplots@loc@TMPb
		\global\def\pgfmathresult{#1}%
	\else
		\global\def\pgfmathresult{#1.#2}%
	\fi
	}%
}

\def\pgfmathlogtologten#1{%
	\pgfmathparse{#1}%
	\expandafter\pgfmathlogtologten@\expandafter{\pgfmathresult}%
}

% Simply divides #1 by log(10).
\def\pgfmathlogtologten@#1{%
	\pgfmathmultiply@{#1}\reciproclogten%
}%

% DEPRECATED.
\def\logtologtentomacro#1#2{%
	\pgfmathmultiply@{#1}\reciproclogten%
	\expandafter\skipsuffixzero\pgfmathresult|%
	\let#2=\pgfmathresult
}

% DEPRECATED.
\def\logtologten#1{%
	\pgfmathmultiply@{#1}\reciproclogten%
	\expandafter\skipsuffixzero\pgfmathresult|%
	\pgfmathresult
}

% helper method which computes log10*\x foreach \x in {#1}.
% The result will be \xdef'ed into #2.
\def\pgfplots@compute@tick@times@logten#1\to#2{%
	\global\let#2=\pgfutil@empty
	\foreach \pgfplots@loc@TMPb in {#1} {%
		\pgfmathmultiply@\pgfplots@loc@TMPb\logten%
		\ifx#2\pgfutil@empty
			\xdef#2{\pgfmathresult}%
		\else
			\xdef#2{#2,\pgfmathresult}%
		\fi
	}%
}

\def\pgfplots@enlarge@limit@ifconfigured#1{%
	\pgfplots@enlargelimits@autofalse
	\pgfplots@enlargelimitsfalse
	\pgfplots@enlargelimits@rel@threshfalse
	\pgfkeysgetvalue{/pgfplots/enlarge #1 limits}{\pgfplots@loc@TMPa}%
	%
	\def\pgfplots@loc@TMPb{true}%
	\ifx\pgfplots@loc@TMPa\pgfplots@loc@TMPb
		\pgfplots@enlargelimitstrue
	\else
		\def\pgfplots@loc@TMPb{false}%
		\ifx\pgfplots@loc@TMPa\pgfplots@loc@TMPb
		\else
			\def\pgfplots@loc@TMPb{auto}%
			\ifx\pgfplots@loc@TMPa\pgfplots@loc@TMPb
				\pgfplots@enlargelimits@autotrue
			\else
				\begingroup
				% try to read it as number:
				\pgf@xa\pgfplots@loc@TMPa pt\relax
				\endgroup
				\pgfplots@enlargelimitstrue
				\pgfplots@enlargelimits@rel@threshtrue
			\fi
		\fi
	\fi
	\expandafter\let\expandafter\ifpgfplots@autocompute@@@min\csname ifpgfplots@autocompute@#1min\endcsname
	\expandafter\let\expandafter\ifpgfplots@autocompute@@@max\csname ifpgfplots@autocompute@#1max\endcsname
	\ifpgfplots@enlargelimits
		% relax the sizes.
		%
		% Idea: if the user chose his xmin,xmax tight to his data,
		% this here will look better.
		\pgfplots@enlarge@limit@for{#1}%
	\else
		\ifpgfplots@enlargelimits@auto
			%\ifpgfplots@hide@x
				% there is no axis, so skip this enlargement (unless
				% the user explizitly requests it)
				% WHY!?
			%\else
				% FIXME : this here should be user-configurable!
				\ifpgfplots@autocompute@@@min
					\pgfplots@enlarge@limit@for{#1}%
				\else
					\ifpgfplots@autocompute@@@max
						\pgfplots@enlarge@limit@for{#1}%
					\fi
				\fi
			%\fi
		\fi
	\fi
}

\def\pgfplots@enlarge@limit@for#1{%
	\begingroup
	\expandafter\let\expandafter\pgfplots@@min\expandafter=\csname pgfplots@#1min\endcsname
	\expandafter\let\expandafter\pgfplots@@max\expandafter=\csname pgfplots@#1max\endcsname
	\expandafter\let\expandafter\ifpgfplots@autocompute@@@min\csname ifpgfplots@autocompute@#1min\endcsname
	\expandafter\let\expandafter\ifpgfplots@autocompute@@@max\csname ifpgfplots@autocompute@#1max\endcsname
	\ifpgfplots@enlargelimits@rel@thresh
		\pgfkeysgetvalue{/pgfplots/enlarge #1 limits}{\enlargepercent}%
	\else
		\def\enlargepercent{0.1}% FIXME : pack 10% as default into option 'enlargelimits' or so
	\fi
	\pgfmathsubtract@\pgfplots@@max\pgfplots@@min%
	\pgf@xa\pgfmathresult pt
	\pgf@xb\enlargepercent\pgf@xa
	\ifdim\pgf@xb>0.001pt
		% the case with 
		%   enlargeabsolute ~= 0
		% means that \pgfplots@@min ~= \pgfplots@@max.
		% It is handled in another method.
		\edef\enlargeabsolute{\pgf@sys@tonumber{\pgf@xb}}%
		%
		\ifpgfplots@enlargelimits@auto
			\ifpgfplots@autocompute@@@min
				\pgfmathsubtract@\pgfplots@@min\enlargeabsolute%
				\let\pgfplots@@min=\pgfmathresult
			\fi
			\ifpgfplots@autocompute@@@max
				\pgfmathadd@\pgfplots@@max\enlargeabsolute%
				\let\pgfplots@@max=\pgfmathresult
			\fi
		\else
			% compute xmin := xmin - enlargeabsolute
			\pgfmathsubtract@\pgfplots@@min\enlargeabsolute%
			\let\pgfplots@@min=\pgfmathresult
			\pgfmathadd@\pgfplots@@max\enlargeabsolute%
			\let\pgfplots@@max=\pgfmathresult
		\fi
	\fi
	\xdef\pgfplots@glob@TMPa{\pgfplots@@min}%
	\xdef\pgfplots@glob@TMPb{\pgfplots@@max}%
	\endgroup
	\expandafter\global\expandafter\let\csname pgfplots@#1min\endcsname=\pgfplots@glob@TMPa
	\expandafter\global\expandafter\let\csname pgfplots@#1max\endcsname=\pgfplots@glob@TMPb
}

% Computes tick positions using the current axis limits.
%
% Parameters:
% /pgfplots/max space between ticks
%    Determines the maximum space which is not filled by at least one
%    tick label (approximate, there is some rounding internally)
% /pgfplots/try min ticks
%    see manual
%
% Idea:
% We want ticks at each 
%    { i*H, i in \Z }.
% Of course, there shouldn't be TOO MUCH ticks. 
%
% Our heuristics is to set
%    desirednumticks = round(ACTUAL WIDTH / (max space between ticks) )
% and generate H = (axis range) / (desirednumticks).
%
% Since not all step sizes H look well, restrict H to a set of allowed 
% step sizes such as 
%   { 1, 1/2, 1/5, 1/10 },
% or, to be more precise:
%   { 1*10^e, 2*10^e, 5*10^e }
% -> round to the nearest matching number!
%
% For log-plots, 
% 	H in { j*log(10), j=1,2,3,... }
% where the usual case should be j = 1.
%
% Then, the resulting tick is
% TICK={MIN,MIN+H,...,MAX}
% where
%    MIN = I*H
% is chosen such that 
%    axis minimum limit = I*H + rest; |rest| < H.
%
% Again, log plots follow a slightly different approach: here,
%   MIN = I * log(10)
% is chosen such that
%    axis minimum limit = I*log(10) + rest; |rest| < log(10)
% while H = j*log(10), j>=1.
%
%
% PRECONDITION:
% - limits are correct
% - axis width/height is set correctly
%
% POSTCONDITION:
% - Tick for axis #1 is assigned
% - \ifpgfplots@determinedefaultvalues@needs@check@uniformtick is set
%
% REMARKS:
% - this algorithms works also if the data range has been transformed
%   with a LINEAR transformation.
%   ATTENTION: as of 2008-05-15, the scaling trafo is AFFINE LINEAR.
%   That means we have to eliminate the 'affine' shifting before the
%   algorithms works correctly.
\def\pgfplots@assign@default@tick@foraxis#1{%
	\begingroup
	% Shortcut-names:
	\expandafter\let\expandafter\ifpgfplots@is@datascaled\csname ifpgfplots@apply@datatrafo@#1\endcsname
	% Attention here: use UNSHIFTET scalings, see remark above
	\expandafter\let\expandafter\pgfplots@data@scale@trafo\csname pgfplots@datascaletrafo@#1@noshift\endcsname
	\expandafter\let\expandafter\pgfplots@data@scale@inverse@trafo\csname pgfplots@inverse@datascaletrafo@#1@noshift\endcsname
	\expandafter\let\expandafter\ifpgfplots@cur@is@linear\csname ifpgfplots@#1islinear\endcsname
	%
	\let\desirednumticks=\c@pgf@countd
	\let\Wr=\pgf@xc
	\Wr=\csname pgfplots@#1coordmaxTEX\endcsname
	\advance\Wr by-\csname pgfplots@#1coordminTEX\endcsname
	% r = max place without ticks in pt -> choose desirednumticks >= W/r
	\expandafter\expandafter\divide\Wr\axisdefaulttickwidth
	\pgfmathsetcount{\desirednumticks}{\Wr}%
	\advance\desirednumticks by1
	\csname ifpgfplots@#1islinear\endcsname
		\expandafter\ifnum\axisdefaulttryminticks>\desirednumticks
			\desirednumticks=\axisdefaulttryminticks
		\fi
	\else
		\expandafter\ifnum\pgfplots@default@try@minticks@log>\desirednumticks
			\desirednumticks=\pgfplots@default@try@minticks@log\relax
		\fi
		\expandafter\ifx\csname pgfplots@#1tickten\endcsname\pgfutil@empty
		\else
			% log plot and tickten-option: provide special processing.
			\edef\pgfplots@loc@TMPa{\csname pgfplots@#1tickten\endcsname}%
			\expandafter\pgfplots@compute@tick@times@logten\pgfplots@loc@TMPa\to\pgfplots@glob@TMPa
			\expandafter\let\csname pgfplots@#1tick\endcsname=\pgfplots@glob@TMPa
		\fi
	\fi
	%
	\expandafter\ifx\csname pgfplots@#1tick\endcsname\pgfutil@empty
		% Ok, we have either log or linear axis and need default
		% ticks MIN,MIN+H,...,MAX.
		\let\MINH=\pgf@xa
		\let\H=\pgf@xb
		\let\MAX=\pgf@ya
		\let\MIN=\pgf@yb
		% compute step size 'H':
		\expandafter\MAX\csname pgfplots@#1max\endcsname pt
		\advance\MAX by0.001pt% avoid round errors
		%\expandafter\MIN\the\c@pgf@counta pt
		\expandafter\MIN\csname pgfplots@#1min\endcsname pt
		\H=\MAX
		\advance\H by-\MIN
%\message{Axis limit #1: [\the\MIN:\the\MAX], diff = \the\H.}%
		\c@pgf@counta=\desirednumticks
		\advance\c@pgf@counta by-1
		\divide\H by\c@pgf@counta
%\message{determining ticks for #1-axis: Wr := (width/max space between ticks) = \the\Wr, desirednumticks=max(\axisdefaulttryminticks, trunc(Wr)) = \the\desirednumticks, H#1=(axis range/(desirednumticks-1)) = \the\H}%
		%
		% SEARCH for the NEXT FEASABLE H.
		\edef\Hmacro{\pgf@sys@tonumber\H}%
		\ifpgfplots@cur@is@linear
			% CASE LINEAR AXIS
			\ifpgfplots@is@datascaled
				% This here works if the scaling trafo is linear.
				\expandafter\pgfplots@data@scale@inverse@trafo\expandafter{\Hmacro}%
				\let\Hmacro=\pgfmathresult
			\else
				\pgfmathfloatparsenumber{\Hmacro}%
				\let\Hmacro=\pgfmathresult
			\fi
			\expandafter\pgfmathfloat@decompose\pgfmathresult\relax\pgfmathfloat@a@S\H\pgfmathfloat@a@E
%\message{Got T^{-1}(H#1) = \Hmacro}%
			% modify the mantisse:
			\ifdim\H<2pt
				\ifdim\H<1.5pt
					\H=1.0pt
				\else
					\H=2.0pt
				\fi
			\else
				\ifdim\H<4.9999pt
					\ifdim\H<3.5pt
						\H=2.0pt\relax
					\else
						\H=5.0pt\relax
					\fi
				\else
					\ifdim\H<7.5pt
						\H=5.0pt\relax
					\else
						\H=1.0pt\relax
						\advance\pgfmathfloat@a@E by1
					\fi
				\fi
			\fi
%\message{Computed H#1=\the\H [unscaled]; transforming ... }%
			\pgfmathfloatcreate{\the\pgfmathfloat@a@S}{\pgf@sys@tonumber{\H}}{\the\pgfmathfloat@a@E}%
			\let\Hmacro=\pgfmathresult
			\ifpgfplots@is@datascaled
				\pgfplots@data@scale@trafo\Hmacro
			\else
				\pgfmathfloattofixed\Hmacro
			\fi
			\let\Hmacro=\pgfmathresult
%\message{got H#1=\Hmacro\ [transformed]}%
			\expandafter\H\Hmacro pt
			\expandafter\aftergroup\csname pgfplots@determinedefaultvalues@#1isuniformtrue\endcsname
			%
			% Now, we want to activate the Tick set {i*H, i in \Z}
			% compute I such that
			%   xmin = I * H + rest;  |rest| < H
			% -> I = round(xmin/H)
			% -> MIN = I * H
			%
			% but first: eliminate any 'affine' data scaling!
			\ifpgfplots@is@datascaled
				\advance\MIN by\csname pgfplots@data@scale@trafo@SHIFT@#1\endcsname pt
			\fi
			\pgfmathlog@invoke@expanded\pgfmathdivide@{%
				{\pgf@sys@tonumber\MIN}%
				{\pgf@sys@tonumber\H}%
			}%
			\pgfmathsetcount{\c@pgf@counta}{\pgfmathresult}%
			\ifdim\MIN<0pt
				% the truncation rounds TOWARDS 0 which is not what I want.
				\advance\c@pgf@counta by-1
			\fi
			\MIN=\H
			\multiply\MIN by\c@pgf@counta
			\ifpgfplots@is@datascaled
				\advance\MIN by-\csname pgfplots@data@scale@trafo@SHIFT@#1\endcsname pt
			\fi
		\else
			% CASE LOG AXIS
			%
			% search for the "best" H= j* log(10),  j an integer.
			%
			% And prefer j=1 if that is possible (otherwise minor
			% ticks are not useful).
			\pgfmathmultiply@{\Hmacro}{\reciproclogten}%
			\let\Hmacrobaseten=\pgfmathresult
			\expandafter\H\pgfmathresult pt
%\message{ [ H / log(10) = \pgfmathresult ]}%
			\ifdim\H<2pt
				\H=1pt
			\else
				\ifnum\H<1pt
					\H=1pt
				\else
					\expandafter\pgfmathfloor\expandafter{\pgfmathresult}%
					\expandafter\H\pgfmathresult pt
				\fi
			\fi
			\ifdim\H=1pt
				\expandafter\aftergroup\csname pgfplots@determinedefaultvalues@#1isuniformtrue\endcsname
				\pgfplots@isuniformticktrue
			\else
				\expandafter\aftergroup\csname pgfplots@determinedefaultvalues@#1isuniformfalse\endcsname
				\pgfplots@isuniformtickfalse
			\fi
%\message{final H=\pgf@sys@tonumber{\H} * log(10)}%
			\H=\logten\H\relax
			% Now, we want to activate the Tick set 
			%   {lowest, lowest+H, ..., highest}
			%
			% Where 
			% 	lowest =  I * log(10) + rest, |rest| < log(10).
			% this is conceptionally different from the approach for
			% linear axes, because H = j*log(10).
			%
			% remember the original xmin in MINH:
			\MINH=\MIN
			%
			% and compute I and I*log(10) here:
			\expandafter\MIN\reciproclogten\MIN\relax
			\edef\pgfmathresult{\pgf@sys@tonumber{\MIN}}%
			\pgfmathsetcount{\c@pgf@counta}{\pgfmathresult}%
			\ifdim\MIN<0pt
				% the truncation rounds TOWARDS 0 which is not what I want.
				\advance\c@pgf@counta by-1
			\fi
			\expandafter\MIN\logten pt
			\multiply\MIN by\c@pgf@counta
			\ifpgfplots@isuniformtick
			\else
				% This here is a special case to move the first tick
				% near the lower axis limit.
				%
				% "Near" means either directly above or directly below ymin.
				% 
				% My application example is as follows:
				% Let H = 2*log(10).
				% Furthermore, ymin = 3e-6, ymax= 8e-2. That means we can choose either
				%    10^{-5}, 10^{-3}, 10^{-1}
				% or
				%    10^{-4}, 10^{-2}
				% as ticks. Well, I prefer the first one.
				%
				% HEURISTICS: start as near to ymin as possible!
				%
				% We check here if we can come nearer to ymin if we
				% shift the current tick by log(10):
				%  if( ymin - I * log(10) < 0.5*H ->  use I+1, that means add log(10).
				%
				% that's equivalent to 
				%  2*(ymin - I * log(10)) - H < 0.
				\advance\MINH by-\MIN
				\multiply\MINH by2
				\advance\MINH by-\H
				% 
				\ifdim\MINH<0pt
					\expandafter\advance\expandafter\MIN\logten pt
				\fi
			\fi
		\fi
		\MINH=\MIN
		\advance\MINH by\H
		% Ok, now it can happen that only ONE tick label is placed in
		% this range.
		% That's useless, so check for it.
		%
		% That's the case if
		%    MIN < ORIGMIN && MAX < MIN+2 H 
		% MIN < ORIGMIN by construction (ok, MIN <= ORIGMIN by
		% construction, but I don't care about this case). 
		% So: check only the second condition.
		\pgfplots@tmpa=\MINH
		\advance\pgfplots@tmpa by\H
		\ifdim\MAX<\pgfplots@tmpa
			\expandafter\aftergroup\csname pgfplots@determinedefaultvalues@#1isuniformfalse\endcsname
			% ok, do something special.
			%
			% The idea is now to place ticks at
			% 10^{i*h} with properly choosen 'h'.
			%
			% So: apply basically the SAME code as above for linear
			% axis, just everything log 10!  And keep in mind that all
			% coordinates are actually given as natural logarithms.
			\expandafter\MIN\csname pgfplots@#1min\endcsname pt
			\H=\MAX
			\advance\H by-\MIN
			\H=\reciproclogten\H
%\message{Axis limit #1: [\the\MIN:\the\MAX], diff/log(10) = \the\H.}%
			\c@pgf@counta=\desirednumticks\relax
			\advance\c@pgf@counta by-1
			\ifnum\c@pgf@counta>2
				% subtract one more. This algorithm here produces more
				% ticks than the normal one which is designed for 10^i
				\advance\c@pgf@counta by-1
			\fi
			\divide\H by\c@pgf@counta\relax
%\message{determining ticks for #1-axis: Wr := (width/max space between ticks) = \the\Wr, desirednumticks=max(\axisdefaulttryminticks, trunc(Wr)) = \the\desirednumticks, H#1=(axis range/(desirednumticks-1)) = \the\H}%
			%
			% SEARCH for the NEXT FEASABLE H.
			\edef\Hmacro{\pgf@sys@tonumber\H}%
			\pgfmathfloatparsenumber{\Hmacro}%
			\expandafter\pgfmathfloat@decompose\pgfmathresult\relax\pgfmathfloat@a@S\H\pgfmathfloat@a@E
			% Determine properly snapped mantisse...
			\ifdim\H<2pt
				\ifdim\H<1.5pt
					\H=1.0pt
				\else
					\H=2.0pt
				\fi
			\else
				\ifdim\H<4.9999pt
					\ifdim\H<3.5pt
						\H=2.0pt\relax
					\else
						\H=5.0pt\relax
					\fi
				\else
					\ifdim\H<7.5pt
						\H=5.0pt\relax
					\else
						\H=1.0pt\relax
						\advance\pgfmathfloat@a@E by1
					\fi
				\fi
			\fi
			\pgfmathfloatcreate{\the\pgfmathfloat@a@S}{\pgf@sys@tonumber{\H}}{\the\pgfmathfloat@a@E}%
			\expandafter\pgfmathfloattofixed\expandafter{\pgfmathresult}%
			\let\Hmacro=\pgfmathresult
			\H=\Hmacro pt%
			% Ok, our step size h for 10^{i*h} is ready!
%\message{determined step size 10^{\Hmacro}}%
			% Now, we want to activate the Tick set {10^{i*H}, i in \Z}
			% compute I such that
			%   10^{min} = 10^{I * H + rest};  |rest| < H
			% -> I = round(xmin/H)
			% -> MIN = I * H
			% BUT EVERYTHING to log(10) basis!
			\MIN=\reciproclogten\MIN\relax
			\pgfmathlog@invoke@expanded\pgfmathdivide@{%
				{\pgf@sys@tonumber\MIN}%
				{\Hmacro}%
			}%
			\pgfmathsetcount{\c@pgf@counta}{\pgfmathresult}%
			\ifdim\MIN<0pt
				% the truncation rounds TOWARDS 0 which is not what I want.
				\advance\c@pgf@counta by-1
			\fi
			\MIN=\H\relax
			\multiply\MIN by\c@pgf@counta\relax
			%
			% convert back to basis 'e':
			\MIN=\logten\MIN\relax
			\H=\logten\H\relax
			\MINH=\MIN\relax
			\advance\MINH by\H\relax
		\fi
%\pgfplots@message{final H=\the\H.}%
		\xdef\pgfplots@glob@TMPa{\pgf@sys@tonumber{\MIN},\pgf@sys@tonumber{\MINH},...,\pgf@sys@tonumber{\MAX}}%
		\xdef\pgfplots@glob@TMPb{\pgf@sys@tonumber{\H}}%
		\aftergroup\pgfplots@determinedefaultvalues@needs@check@uniformtickfalse
	\else
		\expandafter\global\expandafter\let\expandafter\pgfplots@glob@TMPa\csname pgfplots@#1tick\endcsname
		\gdef\pgfplots@glob@TMPb{}% will be computed later, in 'check uniform tick'
		\aftergroup\pgfplots@determinedefaultvalues@needs@check@uniformticktrue
	\fi
	\endgroup
	\expandafter\let\csname pgfplots@#1tick\endcsname=\pgfplots@glob@TMPa
	\expandafter\let\csname pgfplots@tick@distance@#1\endcsname=\pgfplots@glob@TMPb
%\pgfplots@message{pgfplots.sty: #1tick set to \csname pgfplots@#1tick\endcsname [#1min=\csname pgfplots@#1min\endcsname, #1max=\csname pgfplots@#1max\endcsname].}%
}

% Helper method for 
%  \pgfplots@apply@data@scale@trafo@to@options@for
% #1: the ticks
% #2: the trafo macro name 
% #3: the output macro name
\long\def\pgfplots@apply@data@scale@trafo@to@user@ticks#1#2\to#3{%
	\let#3=\pgfutil@empty
	\foreach \pgfplots@loc@TMPb in {#1} {%
		\pgfmathfloatparsenumber{\pgfplots@loc@TMPb}%
		\expandafter#2\expandafter{\pgfmathresult}%
		\ifx#3\pgfutil@empty
			\xdef#3{\pgfmathresult}%
		\else
			\xdef#3{#3,\pgfmathresult}%
		\fi
	}%
	%
}%

% Helper method for 
%  \pgfplots@apply@data@scale@trafo@to@options@for
% #1: the ticks ALREADY IN FLOAT FORMAT
% #2: the trafo macro name 
% #3: the output macro name
\long\def\pgfplots@apply@data@scale@trafo@to@user@ticks@isfloat#1#2\to#3{%
	\let#3=\pgfutil@empty
	\foreach \pgfplots@loc@TMPb in {#1} {%
		#2{\pgfplots@loc@TMPb}%
		\ifx#3\pgfutil@empty
			\xdef#3{\pgfmathresult}%
		\else
			\xdef#3{#3,\pgfmathresult}%
		\fi
	}%
	%
}%

% helper for \pgfplots@apply@data@scale@trafo@to@options@for.
\def\pgfplots@compute@number@order@for@trafo@isdimen#1\tocount#2{%
	\edef\pgfplots@loc@TMPa{\pgf@sys@tonumber{#1}}%
	\pgfmathfloatparsenumber{\pgfplots@loc@TMPa}%
	\expandafter\pgfmathfloat@decompose@E\pgfmathresult\relax#2
	\advance#2 by1\relax
}

% helper for \pgfplots@apply@data@scale@trafo@to@options@for.
% 
\def\pgfplots@compute@number@order@for@trafo@isfloat#1\tocount#2{%
	\expandafter\pgfmathfloat@decompose@E#1\relax#2\relax
	\advance#2 by1\relax
}

% Initialises the data scale transformation and applies it to any
% user specified options.
%
% PRECONDITION:
%   - all axis limits are available in float representation
%   - \pgfplots@set@default@size@options has been called before
% POSTCONDITION:
%   - the scaling transformation is set up,
%   - all axis limits are transformed,
%   - any user input (like ticks and tick labels)
%     will reflect the changes.
\def\pgfplots@apply@data@scale@trafo@to@options@for#1{%
	% initialise data scale transformation 
	%   T(x) = 10^{q-m} * x
	%
	\begingroup
	\let\data@max@order=\c@pgf@counta
	\let\data@cur@order=\c@pgf@countb
	\let\data@dimen=\pgf@xa
	\let\data@tmp=\pgf@xb
	\let\data@dimen@order=\c@pgf@countc
	\let\data@EXPONENT=\c@pgf@countd
	\expandafter\let\expandafter\pgfplots@display@min@float\csname pgfplots@#1min\endcsname
	\expandafter\let\expandafter\pgfplots@display@max@float\csname pgfplots@#1max\endcsname
	\expandafter\let\expandafter\pgfplots@data@min@float\csname pgfplots@data@#1min\endcsname
	\expandafter\let\expandafter\pgfplots@data@max@float\csname pgfplots@data@#1max\endcsname
	\expandafter\let\expandafter\pgfplots@actual@trafo\csname pgfplots@datascaletrafo@#1\endcsname
	\ifpgfplots@autocompute@all@limits
	\else
		\pgfmathfloatmax@{\pgfplots@display@max@float}{\pgfplots@data@max@float}%
		\let\pgfplots@data@max@float=\pgfmathresult
		\pgfmathfloatmin@{\pgfplots@display@min@float}{\pgfplots@data@min@float}%
		\let\pgfplots@data@min@float=\pgfmathresult
	\fi
	%
	% Step 1: compute 'm', the data order
	\pgfplots@compute@number@order@for@trafo@isfloat
		\pgfplots@data@min@float
		\tocount\data@cur@order
	%
	\data@max@order=\data@cur@order
	%
	\pgfplots@compute@number@order@for@trafo@isfloat
		\pgfplots@data@max@float
		\tocount\data@cur@order
	%
	\ifnum\data@cur@order>\data@max@order
		\data@max@order=\data@cur@order
	\fi
	%
	% Step 2: compute 'q', the #1-size of the axis.
	\expandafter\ifx\csname pgfplots@#1\endcsname\pgfutil@empty
		% We have 'width' or 'height'.
		%
		% Use the order of these parameters.
		\def\pgfplots@loc@TMPa{#1}%
		\def\pgfplots@loc@TMPb{x}%
		\ifx\pgfplots@loc@TMPa\pgfplots@loc@TMPb
			\data@dimen=\pgfplots@width\relax
		\else
			\def\pgfplots@loc@TMPb{y}%
			\ifx\pgfplots@loc@TMPa\pgfplots@loc@TMPb
				\data@dimen=\pgfplots@height\relax
			\fi
		\fi
		\pgfplots@compute@number@order@for@trafo@isdimen
			\data@dimen
			\tocount\data@dimen@order
		% This here is to avoid inaccuracies in the final
		% axis rectangle size, see \pgfplots@initsizes:
		%\advance\data@dimen@order by-1
	\else
		% FIXME:
		% we have either the 'x=1cm' or 'y=1cm' option!
		% How should I initialise the trafo!?
		\data@dimen@order=3
	\fi
	%
%\message{Direction #1: data max order=\the\data@max@order;  data dimen order=\the\data@dimen@order. }%
	\data@EXPONENT=\data@dimen@order
	\advance\data@EXPONENT by-\data@max@order
	% Now, I introduce a loop which shall avoid cancellation of
	% significant digits.
	%
	% Harmless Example: 
	%  if we have data shift = -3 and 
	%  max = 2e6, min = 1e6, then max-min = 1e6; T(max)-T(min) = 1e3 which is ok.
	%  In this case, the loop won't change anything.
	%
	% Critical Example:
	%  if we have data shift = -3 and
	%  max = 1980, min = 1930 then 
	%    T(max) = 1.98 and T(min) = 1.93
	%  and thus T(max)-T(min) = 0.05 . 
	%  Considering that this is the axis range
	%  in which tick labels and plot points need to be computed, we
	%  only have two or three digits left! That happens because the
	%  prefix '19' is common and is cancelled in the subtraction.
	%  Idea: while T(max)-T(min) < O(10^2) -> increase shift by +1
	%  (and make sure that T(max) < MAX_VALID_TEX_NUMBER).
	%
	\pgfplots@loop@CONTINUEtrue
	\expandafter\edef\csname pgfplots@data@scale@trafo@SHIFT@#1\endcsname{0}%
	\loop
	\expandafter\edef\csname pgfplots@data@scale@trafo@EXPONENT@#1\endcsname{\the\data@EXPONENT}%
	\pgfplots@actual@trafo{\pgfplots@data@min@float}%
	\let\pgfplots@min@fixed=\pgfmathresult
	\ifpgfplots@loop@CONTINUE
		\pgfplots@actual@trafo{\pgfplots@data@max@float}%
		\let\pgfplots@max@fixed=\pgfmathresult
		\expandafter\data@tmp\pgfplots@max@fixed pt
%\message{Current trafo EXPONENT for #1 direction: \the\data@EXPONENT; original #1 data limits: [\pgfplots@data@min@float:\pgfplots@data@max@float]; current transformed #1 limits: [\pgfplots@min@fixed:\pgfplots@max@fixed]; cancellation check max-min running...}%
		\ifdim\data@tmp<0pt
			% I need absolute values here:
			\multiply\data@tmp by-1\relax
		\fi
		\pgfmathsubtract@{\pgfplots@max@fixed}{\pgfplots@min@fixed}%
		\expandafter\data@dimen\pgfmathresult pt
		\pgfplots@loop@CONTINUEfalse
		\ifdim\data@tmp<1500pt% a multiplication with '10' results in max = 15000 which is the upper limit.
			\ifdim\data@dimen<100pt% I guess if max-min = O(100), we have quite good accuracy
				\ifdim\data@dimen<0.0001pt
				\else
					\advance\data@EXPONENT by1
					\pgfplots@loop@CONTINUEtrue
				\fi
			\fi
		\fi
		%--------------------------------------------------
		% \ifdim\data@dimen>1200pt% FIXME : is this here ok!? CHECK IT!
		% 	\ifdim\data@dimen>7999pt
		% 		\advance\data@EXPONENT by-2
		% 	\else
		% 		\advance\data@EXPONENT by-1
		% 	\fi
		% 	\pgfplots@loop@CONTINUEfalse
		% \fi
		%-------------------------------------------------- 
	\repeat
	\xdef\pgfplots@glob@TMPa{\csname pgfplots@data@scale@trafo@EXPONENT@#1\endcsname}%
	\xdef\pgfplots@glob@TMPb{\pgfplots@min@fixed}%
	\endgroup
%\message{Initialising the data scale transformation in direction #1 to 10^\pgfplots@glob@TMPa*#1 - \pgfplots@glob@TMPb...}%
	% COMPLETE INITIALISATION:
	\ifpgfplots@disabledatascaling
		% this here is a waste of time, I know it. One could really
		% safe a lot of CPU time when disabledatascaling is enabled...
		% but it requires so much extra cases; I really don't want
		% that!
		\gdef\pgfplots@glob@TMPa{0}%
		\gdef\pgfplots@glob@TMPb{0}%
	\fi
	\expandafter\let\csname pgfplots@data@scale@trafo@EXPONENT@#1\endcsname\pgfplots@glob@TMPa
	\expandafter\let\csname pgfplots@data@scale@trafo@SHIFT@#1\endcsname\pgfplots@glob@TMPb%
	%
	% ... and apply transformation to any user input
	%
	% Transform axis limits:
%\message{#1- display limits BEFORE data transformation: [\csname pgfplots@#1min\endcsname:\csname pgfplots@#1max\endcsname]}%
	\expandafter\expandafter\csname pgfplots@datascaletrafo@#1\endcsname\expandafter{\csname pgfplots@#1min\endcsname}%
	\expandafter\global\expandafter\let\csname pgfplots@#1min\endcsname=\pgfmathresult
	%
	\expandafter\expandafter\csname pgfplots@datascaletrafo@#1\endcsname\expandafter{\csname pgfplots@#1max\endcsname}%
	\expandafter\global\expandafter\let\csname pgfplots@#1max\endcsname=\pgfmathresult
%\message{#1- display limits after data transformation: [\csname pgfplots@#1min\endcsname:\csname pgfplots@#1max\endcsname]}%
	%
	% Convert any user-specified ticks:
	\edef\pgfplots@loc@TMPa{\csname pgfplots@#1tick\endcsname}%
	% this here should also work with 'xtick=\pgfutil@empty', the "No tick" command.
	\ifx\pgfplots@loc@TMPa\pgfutil@empty
	\else
		\t@pgfplots@tokc=\expandafter{\csname pgfplots@datascaletrafo@#1\endcsname}%
		\def\pgfplots@loc@TMPb{data}%
		\ifx\pgfplots@loc@TMPa\pgfplots@loc@TMPb
			% we have #1tick = data
			%
			% Since we have entered this method, we know that these
			% coordinate ARE ALREADY in floating point representation.
			\expandafter\let\expandafter\pgfplots@loc@TMPa\csname pgfplots@firstplot@coords@#1\endcsname
			\t@pgfplots@toka=\expandafter{\pgfplots@loc@TMPa}%
			\edef\pgfplots@loc@TMPa{{\the\t@pgfplots@toka}\the\t@pgfplots@tokc}%
			\expandafter\pgfplots@apply@data@scale@trafo@to@user@ticks@isfloat\pgfplots@loc@TMPa\to\pgfplots@loc@TMPc
		\else
			\t@pgfplots@toka=\expandafter{\pgfplots@loc@TMPa}%
%\message{Converting #1tick='\csname pgfplots@#1tick\endcsname'}%
			\edef\pgfplots@loc@TMPa{{\the\t@pgfplots@toka}\the\t@pgfplots@tokc}%
			\expandafter\pgfplots@apply@data@scale@trafo@to@user@ticks\pgfplots@loc@TMPa\to\pgfplots@loc@TMPc
		\fi
		\expandafter\let\csname pgfplots@#1tick\endcsname=\pgfplots@loc@TMPc
	\fi
	%
	% Convert any extra-ticks, see above.
	\edef\pgfplots@loc@TMPa{\csname pgfplots@extra@#1tick\endcsname}%
	\ifx\pgfplots@loc@TMPa\pgfutil@empty
	\else
		\t@pgfplots@tokc=\expandafter{\csname pgfplots@datascaletrafo@#1\endcsname}%
		\edef\pgfplots@loc@TMPa{{\csname pgfplots@extra@#1tick\endcsname}\the\t@pgfplots@tokc}%
		\expandafter\pgfplots@apply@data@scale@trafo@to@user@ticks\pgfplots@loc@TMPa\to\pgfplots@loc@TMPc
		\expandafter\let\csname pgfplots@extra@#1tick\endcsname=\pgfplots@loc@TMPc
	\fi
	%
	% Transform any explicit axis unit scalings:
	\expandafter\ifx\csname pgfplots@#1\endcsname\pgfutil@empty
	\else
%\message{Converting #1 unit scale='\csname pgfplots@#1\endcsname' ... }%
		\expandafter\pgfmathparse\expandafter{\csname pgfplots@#1\endcsname}%
		\expandafter\expandafter\csname pgfplots@inverse@datascaletrafo@tofixed@#1@noshift\endcsname\expandafter{\pgfmathresult}%
		\expandafter\edef\csname pgfplots@#1\endcsname{\pgfmathresult pt}%
%\message{to #1='\csname pgfplots@#1\endcsname'.}%
	\fi
}

\newif\ifpgfplots@determinedefaultvalues@xisuniform
\newif\ifpgfplots@determinedefaultvalues@yisuniform
\newif\ifpgfplots@determinedefaultvalues@needs@check@uniformtick
\newif\ifpgfplots@limits@are@computed

\def\pgfplots@handle@invalid@range{%
	% COMPLETELY EMPTY AXIS:
	\pgfplots@warning{You have a plot with empty range. Replacing it with default and clearing plots.}%
	\ifpgfplots@xislinear
		\pgfmathfloatcreate{0}{0.0}{0}%
		\global\let\pgfplots@xmin=\pgfmathresult
		\pgfmathfloatcreate{1}{1.0}{0}%
		\global\let\pgfplots@xmax=\pgfmathresult
		\global\let\pgfplots@data@xmin=\pgfplots@xmin
		\global\let\pgfplots@data@xmax=\pgfplots@xmax
	\else
		\gdef\pgfplots@xmin{0}%
		\gdef\pgfplots@xmax{1}%
	\fi
	\ifpgfplots@yislinear
		\pgfmathfloatcreate{0}{0.0}{0}%
		\global\let\pgfplots@ymin=\pgfmathresult
		\pgfmathfloatcreate{1}{1.0}{0}%
		\global\let\pgfplots@ymax=\pgfmathresult
		\global\let\pgfplots@data@ymin=\pgfplots@ymin
		\global\let\pgfplots@data@ymax=\pgfplots@ymax
	\else
		\gdef\pgfplots@ymin{0}%
		\gdef\pgfplots@ymax{1}%
	\fi
	\def\pgfplots@xtick{}%
	\def\pgfplots@ytick{}%
	\def\pgfplots@extra@xtick{}%
	\def\pgfplots@extra@ytick{}%
	\def\pgfplots@xtickten{}%
	\def\pgfplots@ytickten{}%
	% clear all plots!
	\pgfplots@init@cleared@structures
}
\def\pgfplots@check@invalid@range{%
	\pgfplots@limits@are@computedtrue
	\ifx\pgfplots@xmin\pgfplots@invalidrange@xmin
		\pgfplots@limits@are@computedfalse
	\fi
	\ifx\pgfplots@xmin\pgfplots@invalidrange@xmax
		\pgfplots@limits@are@computedfalse
	\fi
	\ifx\pgfplots@ymin\pgfplots@invalidrange@ymin
		\pgfplots@limits@are@computedfalse
	\fi
	\ifx\pgfplots@ymin\pgfplots@invalidrange@ymax
		\pgfplots@limits@are@computedfalse
	\fi
	\ifpgfplots@limits@are@computed
		\ifx\pgfplots@data@xmin\pgfplots@invalidrange@xmin
			\global\let\pgfplots@data@xmin=\pgfplots@xmin
		\fi
		\ifx\pgfplots@data@xmin\pgfplots@invalidrange@xmax
			\global\let\pgfplots@data@xmax=\pgfplots@xmax
		\fi
		\ifx\pgfplots@data@ymin\pgfplots@invalidrange@ymin
			\global\let\pgfplots@data@ymin=\pgfplots@ymin
		\fi
		\ifx\pgfplots@data@ymin\pgfplots@invalidrange@ymax
			\global\let\pgfplots@data@ymax=\pgfplots@ymax
		\fi
		\ifpgfplots@clip@limits
		\else
			% there is a rare change that min > max.
			% Handle that ...
			\pgfmathfloatmin@{\pgfplots@xmin}{\pgfplots@xmax}%
			\global\let\pgfplots@xmin=\pgfmathresult
			\pgfmathfloatmax@{\pgfplots@xmin}{\pgfplots@xmax}%
			\global\let\pgfplots@xmax=\pgfmathresult
			%
			\pgfmathfloatmin@{\pgfplots@ymin}{\pgfplots@ymax}%
			\global\let\pgfplots@ymin=\pgfmathresult
			\pgfmathfloatmax@{\pgfplots@ymin}{\pgfplots@ymax}%
			\global\let\pgfplots@ymax=\pgfmathresult
		\fi
	\else
		\pgfplots@handle@invalid@range
	\fi
}%


\def\pgfplots@determinedefaultvalues{%
	\pgfplots@check@invalid@range
	%
	%--------------------------------------------------
	%FIXME
	% \ifpgfplots@float@numerics@mode@x
	% 	\pgfmathfloatmin@{\pgfplots@xmin}{\pgfplots@xmax}%
	% 	\let\pgfplots@xmin=\pgfmathresult
	% 	\pgfmathfloatmax@{\pgfplots@xmin}{\pgfplots@xmax}%
	% 	\let\pgfplots@xmax=\pgfmathresult
	% \else
	% 	\pgfmathmin@{\pgfplots@xmin}{\pgfplots@xmax}%
	% 	\let\pgfplots@xmin=\pgfmathresult
	% 	\pgfmathmax@{\pgfplots@xmin}{\pgfplots@xmax}%
	% 	\let\pgfplots@xmax=\pgfmathresult
	% \fi
	% \ifpgfplots@float@numerics@mode@y
	% 	\pgfmathfloatmin@{\pgfplots@ymin}{\pgfplots@ymax}%
	% 	\let\pgfplots@ymin=\pgfmathresult
	% 	\pgfmathfloatmax@{\pgfplots@ymin}{\pgfplots@ymax}%
	% 	\let\pgfplots@ymax=\pgfmathresult
	% \else
	% 	\pgfmathmin@{\pgfplots@ymin}{\pgfplots@ymax}%
	% 	\let\pgfplots@ymin=\pgfmathresult
	% 	\pgfmathmax@{\pgfplots@ymin}{\pgfplots@ymax}%
	% 	\let\pgfplots@ymax=\pgfmathresult
	% \fi
	%-------------------------------------------------- 
%\message{x = [\pgfplots@xmin:\pgfplots@xmax]  y = [\pgfplots@ymin:\pgfplots@ymax]}%
	%
	%
	\pgfplots@set@default@size@options
	%
	%
	\ifpgfplots@apply@datatrafo@x
		\let\pgfplots@xmin@unscaled@as@float=\pgfplots@xmin
		\let\pgfplots@xmax@unscaled@as@float=\pgfplots@xmax
		\pgfplots@apply@data@scale@trafo@to@options@for x%
	\else
		\def\pgfplots@loc@TMPb{data}%
		\ifx\pgfplots@xtick\pgfplots@loc@TMPb
			\let\pgfplots@xtick=\pgfplots@firstplot@coords@x
		\fi
		\let\pgfplots@xmin@unscaled@as@float=\pgfutil@empty
		\let\pgfplots@xmax@unscaled@as@float=\pgfutil@empty
	\fi
	\ifpgfplots@apply@datatrafo@y
		\let\pgfplots@ymin@unscaled@as@float=\pgfplots@ymin
		\let\pgfplots@ymax@unscaled@as@float=\pgfplots@ymax
		\pgfplots@apply@data@scale@trafo@to@options@for y%
	\else
		\def\pgfplots@loc@TMPb{data}%
		\ifx\pgfplots@ytick\pgfplots@loc@TMPb
			\let\pgfplots@ytick=\pgfplots@firstplot@coords@y
		\fi
		\let\pgfplots@ymin@unscaled@as@float=\pgfutil@empty
		\let\pgfplots@ymax@unscaled@as@float=\pgfutil@empty
	\fi
	\pgfplots@datascaletrafo@initialisedtrue
	%
	% From now on, we can always work with pgfmath.
	% We simply need to apply the data scaling trafo before doing so.
	\pgfkeysgetvalue{/pgfplots/minor x tick num}\pgfplots@minor@xtick@num
	\pgfkeysgetvalue{/pgfplots/minor y tick num}\pgfplots@minor@ytick@num
	\ifpgfplots@xislinear
		\ifnum\pgfplots@minor@xtick@num=0\relax
			\pgfplots@xminorticksfalse
			\pgfplots@xminorgridsfalse
		\else
			\pgfplots@xminortickstrue
		\fi
	\fi
	\ifpgfplots@yislinear
		\ifnum\pgfplots@minor@ytick@num=0\relax
			\pgfplots@yminorticksfalse
			\pgfplots@yminorgridsfalse
		\else
			\pgfplots@yminortickstrue
		\fi
	\fi
	%
	\pgfplots@enlarge@limit@ifconfigured x
	\pgfplots@enlarge@limit@ifconfigured y
	%
	\pgfplots@avoid@empty@axis@range@for x%
	\pgfplots@avoid@empty@axis@range@for y%
	%
	\pgfplots@initsizes
	%
	\pgfplots@determinedefaultvalues@xisuniformtrue
	\pgfplots@determinedefaultvalues@yisuniformtrue
	\pgfplots@determinedefaultvalues@needs@check@uniformticktrue
	\ifx\pgfplots@xtick\pgfutil@empty
		\pgfplots@assign@default@tick@foraxis{x}%
	\fi
	\ifpgfplots@determinedefaultvalues@needs@check@uniformtick
		\ifpgfplots@xislinear
			\expandafter\pgfplots@checkisuniformLINEARtick\expandafter{\pgfplots@xtick}{\pgfplots@tick@distance@x}%
			\ifpgfplots@isuniformtick
				\pgfplots@determinedefaultvalues@xisuniformtrue
			\else
				\pgfplots@determinedefaultvalues@xisuniformfalse
			\fi
		\else
			\expandafter\pgfplots@checkisuniformLOGtick\expandafter{\pgfplots@xtick}%
			\ifpgfplots@isuniformtick
				\pgfplots@determinedefaultvalues@xisuniformtrue
			\else
				\pgfplots@determinedefaultvalues@xisuniformfalse
			\fi
		\fi
	\fi
	\ifpgfplots@determinedefaultvalues@xisuniform
	\else
		\pgfplots@xminorticksfalse
	\fi
	%
	%
	%
	\pgfplots@determinedefaultvalues@needs@check@uniformticktrue
	\ifx\pgfplots@ytick\pgfutil@empty
		\pgfplots@assign@default@tick@foraxis{y}%
	\fi
	\ifpgfplots@determinedefaultvalues@needs@check@uniformtick
		\ifpgfplots@yislinear
			\expandafter\pgfplots@checkisuniformLINEARtick\expandafter{\pgfplots@ytick}{\pgfplots@tick@distance@y}%
			\ifpgfplots@isuniformtick
				\pgfplots@determinedefaultvalues@yisuniformtrue
			\else
				\pgfplots@determinedefaultvalues@yisuniformfalse
			\fi
		\else
			\expandafter\pgfplots@checkisuniformLOGtick\expandafter{\pgfplots@ytick}%
			\ifpgfplots@isuniformtick
				\pgfplots@determinedefaultvalues@yisuniformtrue
			\else
				\pgfplots@determinedefaultvalues@yisuniformfalse
			\fi
		\fi
	\fi
	\ifpgfplots@determinedefaultvalues@yisuniform
	\else
		\pgfplots@yminorticksfalse
	\fi
	%
	\ifx\pgfplots@xticklabel\pgfutil@empty
		\ifpgfplots@xislinear
			\def\pgfplots@xticklabel{\axisdefaultticklabel}%
		\else
			\def\pgfplots@xticklabel{\axisdefaultticklabellog}%
		\fi
	\fi
	\ifx\pgfplots@extra@xticklabel\pgfutil@empty
		\let\pgfplots@extra@xticklabel=\pgfplots@xticklabel
	\fi
	\ifx\pgfplots@yticklabel\pgfutil@empty
		\ifpgfplots@yislinear
			\def\pgfplots@yticklabel{\axisdefaultticklabel}%
		\else
			\def\pgfplots@yticklabel{\axisdefaultticklabellog}%
		\fi
	\fi
	\ifx\pgfplots@extra@yticklabel\pgfutil@empty
		\let\pgfplots@extra@yticklabel=\pgfplots@yticklabel
	\fi
	%
	%
	\pgfplots@prepare@ZERO@coordinates
}

% This code is mainly interesting for bar plots.
%
% It precomputes x = 0 and y = 0 - which is not necessarily
% trivial in case of data scaling. Furthermore, it applies
% coordinate clipping to the resulting values and multiplies them
% with x- and y scale vectors.
\def\pgfplots@prepare@ZERO@coordinates{%
	\ifpgfplots@xislinear
		\ifpgfplots@apply@datatrafo@x
			\pgfplots@datascaletrafo@fromfixed@x{0}%
			\global\let\pgfplots@ZERO@x=\pgfmathresult
		\else
			\gdef\pgfplots@ZERO@x{0}%
		\fi
		\pgfmathmax@{\pgfplots@ZERO@x}{\pgfplots@xmin}%
		\global\let\pgfplots@ZERO@x=\pgfmathresult
	\else
		\global\let\pgfplots@ZERO@x=\pgfplots@xmin%
	\fi
	%
	\ifpgfplots@yislinear
		\ifpgfplots@apply@datatrafo@y
			\pgfplots@datascaletrafo@fromfixed@y{0}%
			\global\let\pgfplots@ZERO@y=\pgfmathresult
		\else
			\gdef\pgfplots@ZERO@y{0}%
		\fi
		\pgfmathmax@{\pgfplots@ZERO@y}{\pgfplots@ymin}%
		\global\let\pgfplots@ZERO@y=\pgfmathresult
	\else
		\global\let\pgfplots@ZERO@y=\pgfplots@ymin%
	\fi
	%
	\pgfinterruptboundingbox%
	\pgfpointxy{\pgfplots@ZERO@x}{\pgfplots@ZERO@y}%
	\xdef\pgfplots@ZERO@x{\the\pgf@x}%
	\xdef\pgfplots@ZERO@y{\the\pgf@y}%
	\endpgfinterruptboundingbox%
}%


% Helper method for initsizes.
%
% It computes a scaling such that \pgfplots@width = SCALE * ACTUAL WIDTH.
% 
% The actual width is 
% 	c + x*(xmax-xmin)
% based on
% - x*xmax = \pgfplots@xcoordmaxTEX
% - x*xmin = \pgfplots@xcoordminTEX
% - c = estimated, a constant for the axis label/tick labels
%
% Arguments: 
% #1: the output argument for the SCALE.
\def\pgfplots@initsizes@getXscale\into#1{%
	\begingroup
	\pgf@xa=\pgfplots@width\relax
	% EXPECTED WIDTH = X = \pgfplots@width
	% ACTUAL WIDTH = c + x * (xmax-xmin)
	% where c is a CONSTANT (for the axis labels/tick labels).
	% -> \pgfplots@tmpXscale = (X - c) / (x *(xmax-xmin))
	%
	% \pgf@xa := X-c:
	\ifpgfplots@scale@only@axis
	\else
		\advance\pgf@xa by-45pt% FIXME determine 'c' correctly!
	\fi
	\ifdim\pgf@xa<0pt
		\pgfplots@error{Error: Plot width `\pgfplots@width' is too small. This can't be realised while maintaining constant width for y-labels. Sorry, label width are only approximate. You will need to adjust your width.}%
		\pgf@xa=0pt
	\fi
	% \pgf@xb := x*(xmax-xmin):
	\pgf@xb=\pgfplots@xcoordmaxTEX
	\advance\pgf@xb by-\pgfplots@xcoordminTEX
	\pgfmathlog@invoke@expanded\pgfmathdivide@{%
		{\pgf@sys@tonumber\pgf@xa}%
		{\pgf@sys@tonumber\pgf@xb}%
	}%
%\pgfplots@message{pgfplots.sty: Computing 'x' such that 'width = c + x*(xmax-xmin)';
%	c=estimated, 
%	width-c =\the\pgf@xa,  
%	x*(xmax[=\the\pgfplots@xcoordmaxTEX] - xmin[=\the\pgfplots@xcoordminTEX)]) = \the\pgf@xb  
%	-> x-scale =#1 }%
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
	\let#1=\pgfmathresult
}

% The same as \pgfplots@initsizes@getXscale, just for the height.
\def\pgfplots@initsizes@getYscale\into#1{%
	\begingroup
	\expandafter\pgf@xa\pgfplots@height\relax
	% EXPECTED WIDTH = X = \pgfplots@width
	% ACTUAL WIDTH = c + x * (xmax-xmin)
	% where c is a CONSTANT (for the axis labels/tick labels).
	% -> \pgfplots@tmpXscale = (X - c) / (x *(xmax-xmin))
	%
	% \pgf@xa := X-c:
	\ifpgfplots@scale@only@axis
	\else
		\advance\pgf@xa by-45pt\relax% FIXME determine 'c' correctly!
	\fi
	\ifdim\pgf@xa<0pt
		\pgfplots@error{Error: Plot height `\pgfplots@height' is too small. This can't be realised while maintaining constant height for x-labels. Sorry, label heights are only approximate. You will need to adjust your height.}%
		\pgf@xa=0pt
	\fi
	% \pgf@xb := x*(xmax-xmin):
	\pgf@xb=\pgfplots@ycoordmaxTEX
	\advance\pgf@xb by-\pgfplots@ycoordminTEX
	\pgfmathlog@invoke@expanded\pgfmathdivide@{%
		{\pgf@sys@tonumber\pgf@xa}%
		{\pgf@sys@tonumber\pgf@xb}%
	}%
%\pgfplots@message{pgfplots.sty: Computing 'y' such that 'height = c + y*(ymax-ymin)';
%	height=\pgfplots@height,
%	c=estimated,
%	height-c =\the\pgf@xa,  
%	y*(ymax[=\the\pgfplots@ycoordmaxTEX] - ymin[=\the\pgfplots@ycoordminTEX)]) = \the\pgf@xb  
%	-> y-scale =#1 }%
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
	\let#1=\pgfmathresult
}


\newif\ifpgfplots@avoid@emptyrange@@range@is@approx@equal
% Checks whether axis limits in coordinate #1 are approximately equal.
%
% If that is the case, force a non-zero width of the range.
%
\def\pgfplots@avoid@empty@axis@range@for#1{%
	% Check if axis limits are empty:
	\begingroup
	\expandafter\let\expandafter\if@cur@is@scaled\csname ifpgfplots@apply@datatrafo@#1\endcsname
	\expandafter\let\expandafter\pgfplots@@min\csname pgfplots@#1min\endcsname
	\expandafter\let\expandafter\pgfplots@@max\csname pgfplots@#1max\endcsname
	\let\min@d=\pgf@xa
	\let\max@d=\pgf@xb
	\let\diff=\pgf@xc
	\expandafter\min@d\pgfplots@@min pt
	\expandafter\max@d\pgfplots@@max pt
	\diff=\max@d
	\advance\diff by-\min@d
	% FIXME : I need a RELATIVE check here!
	% but: real number point division is expensive
	\if@cur@is@scaled
		% this here should be sufficient because the axis
		% has absolute values of order O( 10^3 ) or so.
		\ifdim\diff<0.0001pt
			\pgfplots@avoid@emptyrange@@range@is@approx@equaltrue
		\fi
	\else
		% there is no data scaling, so I should be much more defensive
		% with absolute thresholds...
		\ifdim\diff<0.0001pt
			\pgfplots@avoid@emptyrange@@range@is@approx@equaltrue
		\fi
	\fi
	\ifpgfplots@avoid@emptyrange@@range@is@approx@equal
		\pgfplots@warning{Axis range for axis #1 is approximately equal; enlargeing it.}%
		% the case \pgfplots@@min ~= \pgfplots@@max
		%
		% enlarge \pgfplots@@max and shrink \min:
		\ifdim\max@d<0pt
			\ifdim\max@d<-1pt
				\max@d=0.8\max@d
				\min@d=1.2\min@d
			\else
				\advance\max@d by-1pt
				\advance\min@d by1pt
			\fi
		\else
			\ifdim\max@d>1pt
				\max@d=1.2\max@d
				\min@d=0.8\min@d
			\else
				\ifdim\max@d=0pt
					\if@cur@is@scaled
						\expandafter\let\expandafter\min@unscaled\csname pgfplots@#1min@unscaled@as@float\endcsname
						\expandafter\let\expandafter\max@unscaled\csname pgfplots@#1max@unscaled@as@float\endcsname
						% **sigh**. That's really work.
						%
						% This here happens ALWAYS if min == max for
						% linear axis because the scaling
						% transformation will result in T(min) = T(max) = 0
						%
						% -> we need to enlarge limits in floating
						%  point arithmetics.
						%
						\pgfmathfloatcreate{0}{0.0}{0}%
						\let\pgfplotsmath@zero=\pgfmathresult
						%
						\ifx\max@unscaled\pgfplotsmath@zero
							% max == 0
							\pgfmathfloatcreate{1}{1.0}{0}%
							\let\max@unscaled=\pgfmathresult
							\pgfmathfloatcreate{2}{1.0}{0}%
							\let\min@unscaled=\pgfmathresult
						\else
							%
							\pgfmathfloatcreate{1}{1.2}{0}%
							\let\pgfplotsmath@scalea=\pgfmathresult
							\pgfmathfloatcreate{1}{8.0}{-1}%
							\let\pgfplotsmath@scaleb=\pgfmathresult
							%
							\pgfmathfloatlessthan@{\pgfplotsmath@zero}{\max@unscaled}%
							\ifpgfmathfloatcomparison
								% 0 < max
								\pgfmathfloatmultiply@{\max@unscaled}{\pgfplotsmath@scalea}%
								\let\max@unscaled=\pgfmathresult
								\pgfmathfloatmultiply@{\min@unscaled}{\pgfplotsmath@scaleb}%
								\let\min@unscaled=\pgfmathresult
							\else
								\pgfmathfloatmultiply@{\max@unscaled}{\pgfplotsmath@scaleb}%
								\let\max@unscaled=\pgfmathresult
								\pgfmathfloatmultiply@{\min@unscaled}{\pgfplotsmath@scalea}%
								\let\min@unscaled=\pgfmathresult
							\fi
						\fi
						\csname pgfplots@datascaletrafo@#1\endcsname{\min@unscaled}%
						\let\pgfplots@@min=\pgfmathresult
						\csname pgfplots@datascaletrafo@#1\endcsname{\max@unscaled}%
						\let\pgfplots@@max=\pgfmathresult
						\min@d=\pgfplots@@min pt
						\max@d=\pgfplots@@max pt
					\else
						\advance\max@d by1pt
						\advance\min@d by-1pt
					\fi
				\else
					\advance\max@d by1pt
					\advance\min@d by-1pt
				\fi
			\fi
		\fi
		\xdef\pgfplots@glob@TMPa{\pgf@sys@tonumber{\min@d}}%
		\xdef\pgfplots@glob@TMPb{\pgf@sys@tonumber{\max@d}}%
%\pgfplots@message{ -> #1 = \pgfplots@glob@TMPa : \pgfplots@glob@TMPb;}%
	\else
		\global\let\pgfplots@glob@TMPa=\pgfplots@@min%
		\global\let\pgfplots@glob@TMPb=\pgfplots@@max%
	\fi
	\endgroup
	\expandafter\global\expandafter\let\csname pgfplots@#1min\endcsname=\pgfplots@glob@TMPa
	\expandafter\global\expandafter\let\csname pgfplots@#1max\endcsname=\pgfplots@glob@TMPb
}

% PRECONDITION:
% 	none
% POSTCONDITION:
% 	\pgfplots@default@aspect@ratio is set.
\def\pgfplots@compute@default@aspect@ratio{%
	\expandafter\pgfmath@x\axisdefaultwidth
	\expandafter\pgfmath@y\axisdefaultheight
	\pgfmathlog@invoke@expanded\pgfmathdivide@{%
		{\pgf@sys@tonumber{\pgfmath@x}}%
		{\pgf@sys@tonumber{\pgfmath@y}}%
	}%
	\let\pgfplots@default@aspect@ratio=\pgfmathresult
}

\def\pgfplots@set@default@size@options{%
	% The axes 'x' and 'y' vectors will be scaled such that the total
	% size is (\axisdefaultwidth, \axisdefaultheight).
	%
	% If the user specifies ONE of width OR height, 
	% the plot will be resized; keeping the aspect ratio.
	%
	\let\pgfplots@default@aspect@ratio=\pgfutil@empty
	% CASES:
	% hasx := 'x' option non-empty
	% hasy := 'y' option non-empty
	% W := 'width' option non-empty
	% H := 'height' option non-empty
	%
	% hasx = 1 -> width is not interesting; we use 'x' option.
	% hasx = 0 -> determine final width:
	% 		W H
	% 		0 0 -> \axisdefaultwidth 
	% 		0 1 -> determine width out of H and the default aspect ratio
	% 		1 X -> ok, use the user parameter.
	%
	% hasy = 1 -> height is not interesting, we use 'y' option.
	% hasy = 0 -> determine final height:
	% 		W H
	% 		0 0 -> \axisdefaultheight
	% 		X 1 -> ok, use the user parameter
	% 		1 0 -> determine height out of W and the default aspect ratio
	%
	\ifx\pgfplots@x\pgfutil@empty
		\ifx\pgfplots@y\pgfutil@empty
			% hasx=0, hasy=0 
			%
			% -> KEEP ASPECT RATIO if just one W, or H is given!
			\ifx\pgfplots@width\pgfutil@empty
				\ifx\pgfplots@height\pgfutil@empty
					% The case hasx=0, hasy=0,  W=0 H=0:
					\let\pgfplots@width=\axisdefaultwidth
					\let\pgfplots@height=\axisdefaultheight
				\else
					% The case hasx=0, hasy=0,  W=0 H=1:
					\pgfplots@compute@default@aspect@ratio
					\expandafter\pgfmath@y\pgfplots@height
					\pgfmathlog@invoke@expanded\pgfmathmultiply@{%
						{\pgf@sys@tonumber{\pgfmath@y}}%
						{\pgfplots@default@aspect@ratio}%
					}%
					\edef\pgfplots@width{\pgfmathresult pt}%
				\fi
			\else
				\ifx\pgfplots@height\pgfutil@empty
					% The case hasx=0, hasy=0,  W=1 H=0:
					\pgfplots@compute@default@aspect@ratio
					\expandafter\pgfmath@x\pgfplots@width
					\pgfmathlog@invoke@expanded\pgfmathdivide@{%
						{\pgf@sys@tonumber{\pgfmath@x}}%
						{\pgfplots@default@aspect@ratio}%
					}%
					\edef\pgfplots@height{\pgfmathresult pt}%
				\else
					% The case hasx=0, hasy=0,  W=1 H=1:
				\fi
			\fi
		\else
			% hasx=0, hasy=1, W=0:
			\ifx\pgfplots@width\pgfutil@empty
				\let\pgfplots@width=\axisdefaultwidth
			\fi
		\fi
	\else
		\ifx\pgfplots@y\pgfutil@empty
			% hasx=1, hasy=0, H=0
			\ifx\pgfplots@height\pgfutil@empty
				\let\pgfplots@height=\axisdefaultheight
			\fi
		\fi
	\fi
}

% PRECONDITION: 
% 	- final axis limits are given in transformed range
% 	-  \pgfplots@set@default@size@options has been invoked before
% POSTCONDITION: 
% 	- the current x- and y unit vectors are changed;
% 	- \pgfplots@[xy]coord{min,max}TEX  are set
%
\def\pgfplots@initsizes{%
	% INIT.
	%
	%
	\pgfqpointxy{\pgfplots@xmin}{\pgfplots@ymin}%
	\pgfplots@xcoordminTEX=\pgf@x
	\pgfplots@ycoordminTEX=\pgf@y
	\pgfqpointxy{\pgfplots@xmax}{\pgfplots@ymax}%
	\pgfplots@xcoordmaxTEX=\pgf@x
	\pgfplots@ycoordmaxTEX=\pgf@y
	%
	%
	%-----------------------------------------
	% PROCESS THE 'width' and 'height' options
	%-----------------------------------------
	%
	% FIXME: make these variables LOCAL:
	%
	\let\pgfplots@rectangle@width=\pgfutil@empty
	\let\pgfplots@rectangle@height=\pgfutil@empty
	%
	\ifx\pgfplots@x\pgfutil@empty
		\ifx\pgfplots@width\pgfutil@empty
			\pgfplots@error{INTERNAL LOGIC ERROR! WIDTH NOT SET}%
		\fi
		\pgfplots@initsizes@getXscale\into\pgfplots@tmpXscale
		\ifpgfplots@scale@only@axis
			\let\pgfplots@rectangle@width=\pgfplots@width
		\fi
	\else
		\def\pgfplots@tmpXscale{1}%
	\fi
	%
	\ifx\pgfplots@y\pgfutil@empty
		\ifx\pgfplots@height\pgfutil@empty
			\pgfplots@error{INTERNAL LOGIC ERROR! HEIGHT NOT SET}%
		\fi
		\pgfplots@initsizes@getYscale\into\pgfplots@tmpYscale
		\ifpgfplots@scale@only@axis
			\let\pgfplots@rectangle@height=\pgfplots@height
		\fi
	\else
		\def\pgfplots@tmpYscale{1}%
	\fi
	%
	% 
	% assert( \pgfplots@tmpXscale != \pgfutil@empty && \pgfplots@tmpYscale != \pgfutil@empty )
	%
	% Apply scaling:
	\pgfpointxy{\pgfplots@tmpXscale}{\pgfplots@tmpYscale}%
	\edef\pgfplots@tmpscale@x{\the\pgf@x}%
	\edef\pgfplots@tmpscale@y{\the\pgf@y}%
	\ifx\pgfplots@x\pgfutil@empty
		\pgfsetxvec{\pgfqpoint{\pgfplots@tmpscale@x}{0pt}}%
	\else
		\pgfsetxvec{\pgfpoint{\pgfplots@x}{0pt}}%
	\fi
	\ifx\pgfplots@y\pgfutil@empty
		\pgfsetyvec{\pgfqpoint{0pt}{\pgfplots@tmpscale@y}}%
	\else
		\pgfsetyvec{\pgfpoint{0pt}{\pgfplots@y}}%
	\fi
	%
	% Determine final rectangle dimensions.
	% There are the following cases: 
	% 1. the user really wants a fixed dimension,
	%    i.e. he used 'scale only axis'.
	%    Then, we have to work to get the correct dimension!
	%
	%    Up to now, the scaling mechanism looses to many significant
	%    digits such that the final width/height differs by 1-2 pt.
	%
	%    If I am not mistaken, this does ONLY affect the final size,
	%    not the relative plot precision.
	%    
	%    FIXME : really compute the plot precision!
	% 
	% 2. The use specified width and/or height, but not 'scale only
	%    axis'. Accept inaccurate final widths/heights (see above).
	%
	% 3. The user supplied 'x' and or 'y'. Simply use them, its
	% accurate.
	%
	\pgfqpointxy{\pgfplots@xmin}{\pgfplots@ymin}%
	\pgfplots@xcoordminTEX=\pgf@x
	\pgfplots@ycoordminTEX=\pgf@y
	\pgfqpointxy{\pgfplots@xmax}{\pgfplots@ymax}%
	\ifx\pgfplots@rectangle@width\pgfutil@empty
		\pgfplots@xcoordmaxTEX=\pgf@x
	\else
		% this 'if' here should only make a difference of about
		% 1-2pt, not more.
		%
		% and I am quite sure that this inaccuracy (and this
		% work-around) only affects the
		% final size, not the relative plot accuracy.
		\pgfplots@xcoordmaxTEX=\pgfplots@xcoordminTEX
		\expandafter\advance\expandafter\pgfplots@xcoordmaxTEX\pgfplots@width
	\fi
	\ifx\pgfplots@rectangle@height\pgfutil@empty
		\pgfplots@ycoordmaxTEX=\pgf@y
	\else
		\pgfplots@ycoordmaxTEX=\pgfplots@ycoordminTEX
		\expandafter\advance\expandafter\pgfplots@ycoordmaxTEX\pgfplots@height
	\fi
%--------------------------------------------------
% \begingroup
% \pgf@x=\pgfplots@xcoordmaxTEX\advance\pgf@x by-\pgfplots@xcoordminTEX
% \pgf@y=\pgfplots@ycoordmaxTEX\advance\pgf@y by-\pgfplots@ycoordminTEX
% \message{Axis scaling x=\pgfplots@tmpXscale, y=\pgfplots@tmpYscale\ yields lower-left-corner (\pgfplots@xmin,\pgfplots@ymin) = (\the\pgfplots@xcoordminTEX,\the\pgfplots@ycoordminTEX) and upper right (\pgfplots@xmax,\pgfplots@ymax) = (\the\pgfplots@xcoordmaxTEX,\the\pgfplots@ycoordmaxTEX).   Axis dimensions are width=\the\pgf@x, height=\the\pgf@y.}%
% \endgroup
%-------------------------------------------------- 
}

% This here is a low-weight node. It can ONLY be used during axis
% descriptions and is completely useless otherwise.
%
% See pgfplots@low@level@shape below.
\pgfdeclareshape{pgfplots@low@level@shape@INNER}{%
	\nodeparts{image}%
	\anchor{image}{%
		\pgf@x=0pt
		\pgf@y=0pt
	}%
	%
	%
	\anchor{center}{\pgfqpointxy{0.5}{0.5}}%
	\anchor{north}{\pgfqpointxy{0.5}{1}}%
	\anchor{north east}{\pgfqpointxy{1}{1}}%
	\anchor{east}{\pgfqpointxy{1}{0.5}}
	\anchor{south east}{\pgfqpointxy{1}{0}}%
	\anchor{south}{\pgfqpointxy{0.5}{0}}%
	\anchor{south west}{\pgfqpointxy{0}{0}}%
	\anchor{west}{\pgfqpointxy{0}{0.5}}%
	\anchor{north west}{\pgfqpointxy{0}{1}}%
	%%
	\anchor{origin}{\pgfqpoint{\pgfplots@ZERO@x\relax}{\pgfplots@ZERO@y\relax}}%
	\anchor{above origin}{\pgfqpoint{\pgfplots@ZERO@x\relax}{\pgfplots@ycoordmaxTEX}}%
	\anchor{left of origin}{\pgfqpoint{\pgfplots@xcoordminTEX}{\pgfplots@ZERO@y\relax}}%
	\anchor{right of origin}{\pgfqpoint{\pgfplots@xcoordmaxTEX}{\pgfplots@ZERO@y\relax}}%
	\anchor{below origin}{\pgfqpoint{\pgfplots@ZERO@x\relax}{\pgfplots@ycoordminTEX}}%
	%%
	%%
	%%
	%%
	\anchorborder{}%
	\backgroundpath{}%\pgfpathrectangle{\pgfpointorigin}{\upperrightinnercorner}}%
	\foregroundpath{}%
	\behindbackgroundpath{}%
	\beforebackgroundpath{}%
	\behindforegroundpath{}%
	\beforeforegroundpath{}%
}

% This is the main axis shape.
%
% It has one node part, which is the complete image. It provides a lot
% of anchors.
\pgfdeclareshape{pgfplots@low@level@shape}{%
	\savedanchor\upperrightcorner{
		\pgf@x=\wd\pgfnodepartimagebox
		\pgf@y=\ht\pgfnodepartimagebox
	}%
	\savedanchor\lowerleftinnercorner{%
		\pgfqpoint{\pgfplots@savedanchor@inner@lowerleft@x\relax}{\pgfplots@savedanchor@inner@lowerleft@y\relax}%
	}%
	\savedanchor\upperrightinnercorner{%
		\pgfqpoint{\pgfplots@savedanchor@inner@upperright@x\relax}{\pgfplots@savedanchor@inner@upperright@y\relax}%
	}%
	\savedanchor\origin{%
		\pgfqpoint{\pgfplots@ZERO@x\relax}{\pgfplots@ZERO@y\relax}%
	}%
	%
	\nodeparts{image}%
	\anchor{image}{%
		\pgf@x=0pt
		\pgf@y=0pt
	}%
	%
	%
	\anchor{center}{%
		\lowerleftinnercorner
		\pgf@xa=\pgf@x
		\pgf@xb=\pgf@y
		\upperrightinnercorner
		\advance\pgf@xa by\pgf@x
		\pgf@x=.5\pgf@xa
		\advance\pgf@xb by\pgf@y
		\pgf@y=.5\pgf@xb
	}%
	\anchor{north}{%
		\lowerleftinnercorner
		\pgf@xa=\pgf@x
		\pgf@xb=\pgf@y
		\upperrightinnercorner
		\advance\pgf@xa by\pgf@x
		\pgf@x=.5\pgf@xa
	}%
	\anchor{north east}{\upperrightinnercorner}%
	\anchor{east}{%
		\lowerleftinnercorner
		\pgf@xa=\pgf@x
		\pgf@xb=\pgf@y
		\upperrightinnercorner
		\advance\pgf@xb by\pgf@y
		\pgf@y=.5\pgf@xb
	}%
	\anchor{south east}{%
		\lowerleftinnercorner
		\pgf@xa=\pgf@x
		\pgf@xb=\pgf@y
		\upperrightinnercorner
		\pgf@y=\pgf@xb
	}%
	\anchor{south}{%
		\lowerleftinnercorner
		\pgf@xa=\pgf@x
		\pgf@xb=\pgf@y
		\upperrightinnercorner
		\advance\pgf@xa by\pgf@x
		\pgf@x=.5\pgf@xa
		\pgf@y=\pgf@xb
	}%
	\anchor{south west}{\lowerleftinnercorner}%
	\anchor{west}{%
		\lowerleftinnercorner
		\pgf@xa=\pgf@x
		\pgf@xb=\pgf@y
		\upperrightinnercorner
		\pgf@x=\pgf@xa
		\advance\pgf@xb by\pgf@y
		\pgf@y=.5\pgf@xb
	}%
	\anchor{north west}{%
		\lowerleftinnercorner
		\pgf@xa=\pgf@x
		\pgf@xb=\pgf@y
		\upperrightinnercorner
		\pgf@x=\pgf@xa
	}%
	%%
	\anchor{origin}{%
		\origin
	}%
	\anchor{above origin}{%
		\origin
		\pgf@xa=\pgf@x
		\upperrightinnercorner
		\pgf@x=\pgf@xa
	}%
	\anchor{left of origin}{%
		\origin
		\pgf@xa=\pgf@y
		\lowerleftinnercorner
		\pgf@y=\pgf@xa
	}%
	\anchor{right of origin}{%
		\origin
		\pgf@xa=\pgf@y
		\upperrightinnercorner
		\pgf@y=\pgf@xa
	}%
	\anchor{below origin}{%
		\origin
		\pgf@xa=\pgf@x
		\lowerleftinnercorner
		\pgf@x=\pgf@xa
	}%
	%
	%%
	%
	\anchor{outer north}{%
		\upperrightcorner
		\pgf@x=.5\pgf@x
	}%
	\anchor{outer north east}{\upperrightcorner}%
	\anchor{outer east}{%
		\upperrightcorner
		\pgf@y=.5\pgf@y
	}%
	\anchor{outer south east}{%
		\upperrightcorner
		\pgf@y=0pt
	}%
	\anchor{outer south}{%
		\upperrightcorner
		\pgf@x=.5\pgf@x
		\pgf@y=0pt
	}%
	\anchor{outer south west}{%
		\pgf@x=0pt
		\pgf@y=0pt
	}%
	\anchor{outer west}{%
		\upperrightcorner
		\pgf@x=0pt
		\pgf@y=.5\pgf@y
	}%
	\anchor{outer north west}{%
		\upperrightcorner
		\pgf@x=0pt
	}%
	\anchor{outer center}{%
		\upperrightcorner
		\pgf@x=.5\pgf@x
		\pgf@y=.5\pgf@y
	}%
	%
	%
	%%
	%%
	\anchor{above north}{%
		\upperrightcorner
		\pgf@xa=\pgf@y
		\lowerleftinnercorner
		\pgf@xb=\pgf@x
		\upperrightinnercorner
		\advance\pgf@xb by\pgf@x
		\pgf@x=.5\pgf@xb
		\pgf@y=\pgf@xa
	}%
	\anchor{above north east}{%
		\upperrightcorner
		\pgf@xa=\pgf@y
		\upperrightinnercorner
		\pgf@y=\pgf@xa
	}%
	\anchor{right of north east}{%
		\upperrightcorner
		\pgf@xa=\pgf@x
		\upperrightinnercorner
		\pgf@x=\pgf@xa
	}%
	\anchor{right of east}{%
		\upperrightcorner
		\pgf@xa=\pgf@x
		\upperrightinnercorner
		\pgf@xb=\pgf@y
		\lowerleftinnercorner
		\advance\pgf@xb by\pgf@y
		\pgf@x=\pgf@xa
		\pgf@y=.5\pgf@xb
	}%
	\anchor{right of south east}{%
		\upperrightcorner
		\pgf@xa=\pgf@x
		\lowerleftinnercorner
		\pgf@x=\pgf@xa
	}%
	\anchor{below south east}{%
		\upperrightinnercorner
		\pgf@y=0pt
	}%
	\anchor{below south}{%
		\lowerleftinnercorner
		\pgf@xa=\pgf@x
		\upperrightinnercorner
		\pgf@y=0pt
		\advance\pgf@xa by\pgf@x
		\pgf@x=.5\pgf@xa
	}%
	\anchor{below south west}{%
		\lowerleftinnercorner
		\pgf@y=0pt
	}%
	\anchor{left of south west}{%
		\lowerleftinnercorner
		\pgf@x=0pt
	}%
	\anchor{left of west}{%
		\lowerleftinnercorner
		\pgf@xa=\pgf@y
		\upperrightinnercorner
		\advance\pgf@xa by\pgf@y
		\pgf@y=.5\pgf@xa
		\pgf@x=0pt
	}%
	\anchor{left of north west}{%
		\upperrightinnercorner
		\pgf@x=0pt
	}%
	\anchor{above north west}{%
		\upperrightcorner
		\pgf@xa=\pgf@y
		\lowerleftinnercorner
		\pgf@y=\pgf@xa
	}%
	%%
	%%
	\anchorborder{%
		% Call a function that computes a border point. Since this
		% function will modify dimensions like \pgf@x, we must move them to
		% other dimensions.
		\@tempdima=\pgf@x
		\@tempdimb=\pgf@y
		\pgfpointborderrectangle%
			{\pgfpoint{\@tempdima}{\@tempdimb}}%
			{\pgfpointadd{\upperrightcorner}{\pgfpoint{\width}{\height}}}
	}%
	\backgroundpath{\pgfpathrectangle{\pgfpointorigin}{\upperrightcorner}}%
	\foregroundpath{}%
	\behindbackgroundpath{}%
	\beforebackgroundpath{}%
	\behindforegroundpath{}%
	\beforeforegroundpath{}%
}

\def\pgfplots@draw@axis{%
	\ifpgfplots@hide@x\else
		% compute tick position lists
		% 	\pgfplots@prepared@tick@positions@minor@x
		% and
		% 	\pgfplots@prepared@tick@positions@major@x
		\expandafter\pgfplots@prepare@ticks@for\expandafter{\pgfplots@xtick}{x}{0}%
		\pgfplots@drawgridlines@for{x}{0}%
	\fi
	\ifpgfplots@hide@y\else
		\expandafter\pgfplots@prepare@ticks@for\expandafter{\pgfplots@ytick}{y}{1}%
		\pgfplots@drawgridlines@for{y}{1}%
	\fi
	%
	\ifpgfplots@hide@x\else
		\pgfplots@drawticklines@for{x}{0}%
	\fi
	\ifpgfplots@hide@y\else
		\pgfplots@drawticklines@for{y}{1}%
	\fi
	%
	\pgfplots@drawaxis@lines
	%
	\ifpgfplots@hide@x\else
		\pgfplots@drawticklabels@for{x}{0}%
	\fi
	\ifpgfplots@hide@y\else
		\pgfplots@drawticklabels@for{y}{1}%
	\fi
		%
	\ifpgfplots@hide@x\else
		\ifx\pgfplots@extra@xtick\pgfutil@empty
		\else
			\expandafter\pgfplots@draw@extra@ticks@for\expandafter x\expandafter0\expandafter{\pgfplots@extra@xtick}%
		\fi
	\fi
	\ifpgfplots@hide@y\else
		\ifx\pgfplots@extra@ytick\pgfutil@empty
		\else
			\expandafter\pgfplots@draw@extra@ticks@for\expandafter y\expandafter1\expandafter{\pgfplots@extra@ytick}%
		\fi
	\fi
}%

\def\pgfplots@BEGIN@init@and@draw@axis{%
	\pgfplots@determinedefaultvalues
	\setbox\pgfnodepartimagebox=\hbox\bgroup\bgroup
		\pgfinterruptpicture
		\tikzpicture[/pgfplots/every axis]%
		%\pgfqkeys{/tikz}{every axis}%
		% set baseline for sub-picture to default value.
		% the baseline option will be applied to the OUTER picture.
		\pgfsetbaseline{\pgf@picminy}%
		%
		\scope
		\ifpgfplots@axis@on@top
		\else
			\pgfplots@draw@axis
		\fi
		\clip
						(\pgfplots@xcoordminTEX,	\pgfplots@ycoordminTEX) 
			rectangle	(\pgfplots@xcoordmaxTEX,	\pgfplots@ycoordmaxTEX);
}


\def\pgfplots@END@init@and@draw@axis{%
	\endscope%
	%
	\ifpgfplots@axis@on@top
		\pgfplots@draw@axis
	\else
	\fi
	%
	% whats the better sequence for \ifpgfplots@axis@on@top and \ifpgfplots@clip@marker@paths !? 
	% This here looks better, I think... markers should not be obscured by descriptions.
	\ifpgfplots@clip@marker@paths
	\else
		\pgfplotslistforeach\pgfplots@stored@markerlist\as\pgfplots@loc@TMPa{%
			\pgfplots@loc@TMPa
		}%
		\global\pgfplotslistnewempty\pgfplots@stored@markerlist% clear.
	\fi
	%
	\begingroup
	\pgfkeysvalueof{/pgfplots/after end axis/.@cmd}\pgfeov%
	\endgroup
	%
}

% Writes output to \pgfmathresult
\def\pgfplots@filter@input@ticks@with@log#1{%
	\let\pgfplots@glob@TMPa=\pgfutil@empty
	\foreach \pgfplots@loc@TMPb in {#1} {%
		\expandafter\pgfmathlog@\expandafter{\pgfplots@loc@TMPb}%
		\ifx\pgfplots@glob@TMPa\pgfutil@empty
			\xdef\pgfplots@glob@TMPa{\pgfmathresult}%
		\else
			\xdef\pgfplots@glob@TMPa{\pgfplots@glob@TMPa,\pgfmathresult}%
		\fi
	}%
	\let\pgfmathresult=\pgfplots@glob@TMPa
}

% Writes output to \pgfmathresult
% #1: the input ticks
% #2: the transformation command key as macro
\def\pgfplots@filter@input@ticks@with@highleveltrafo#1#2{%
	\let\pgfplots@glob@TMPa=\pgfutil@empty
	\foreach \pgfplots@loc@TMPb in {#1} {%
		\expandafter#2\expandafter{\pgfplots@loc@TMPb}\pgfeov%
		\ifx\pgfplots@glob@TMPa\pgfutil@empty
			\xdef\pgfplots@glob@TMPa{\pgfmathresult}%
		\else
			\xdef\pgfplots@glob@TMPa{\pgfplots@glob@TMPa,\pgfmathresult}%
		\fi
	}%
	\let\pgfmathresult=\pgfplots@glob@TMPa
}

\tikzdeclarecoordinatesystem{axis}{\pgfplots@evalute@tikz@coord@system@interface#1\pgfplots@coord@end}


% Assigns \pgfmathresult := canvas coordinate (#2) for axis #1.
\long\def\pgfplots@evalute@tikz@coord@system@interface@for#1#2{%
	\pgfkeysgetvalue{/pgfplots/#1 coord trafo/.@cmd}\pgfplots@loc@TMPc
	\def\pgfmathresult{#2}%
	\ifx\pgfplots@loc@TMPc\pgfplots@empty@command@key
	\else
		\expandafter\pgfplots@loc@TMPc\expandafter{\pgfmathresult}\pgfeov
	\fi
	\let\pgfplots@loc@TMPc=\pgfmathresult% FIXME: is that necessary? I doubt it... but just to make sure...
	\expandafter\let\expandafter\if@datascaled@cur\csname ifpgfplots@apply@datatrafo@#1\endcsname
	\csname ifpgfplots@#1islinear\endcsname
		\if@datascaled@cur
			\csname pgfplots@datascaletrafo@fromfixed@#1\endcsname{\pgfplots@loc@TMPc}%
		\fi
	\else
		\pgfmathlog@{\pgfplots@loc@TMPc}%
	\fi
}

\long\def\pgfplots@evalute@tikz@coord@system@interface#1,#2\pgfplots@coord@end{%
	\begingroup
	\pgfplots@evalute@tikz@coord@system@interface@for{x}{#1}%
	\let\pgfplots@evaluate@tikz@coord@x=\pgfmathresult
	\pgfplots@evalute@tikz@coord@system@interface@for{y}{#2}%
	\xdef\pgfplots@glob@TMPa{\pgfplots@evaluate@tikz@coord@x}%
	\xdef\pgfplots@glob@TMPb{\pgfmathresult}%
	\endgroup
	\pgfqpointxy{\pgfplots@glob@TMPa}{\pgfplots@glob@TMPb}%
}

% In case of (semi-) logplots, this command will 
% - assign a filter which invokes \pgfmathlog@{} for each coordinate
% - replace any user-specified coordinate by its log.
%
% All subsequent commands will then work with logarithmic coordinates.
%
% PRECONDITION: 
% - The user input options have been set correctly, 
% - the options have been set, but are not applied
%
% POSTCONDITION: 
% - any user input for log-axis has been replaced by its log
% - coordinate filters to compute logs are installed
%
% See also:
%     \pgfplots@apply@data@scale@trafo@to@options@for
\def\pgfplots@prepare@coord@filtering@for#1{%
	\pgfkeysgetvalue{/pgfplots/#1 coord trafo/.@cmd}\pgfplots@loc@TMPc
	\expandafter\let\csname pgfplots@highlevel@trafo@#1\endcsname=\pgfplots@loc@TMPc
	\ifx\pgfplots@loc@TMPc\pgfplots@empty@command@key
		% no high-level external coord trafos.
		% Simply use identity:
		\expandafter\def\csname pgfplots@prepare@#1coord\endcsname##1{%
			\def\pgfmathresult{##1}%
		}%
	\else
		% Apply external coordinate trafo to all input values:
		\expandafter\edef\csname pgfplots@prepare@#1coord\endcsname##1{%
			\noexpand\def\noexpand\pgfmathresult{##1}%
			\expandafter\noexpand\csname pgfplots@highlevel@trafo@#1\endcsname{##1}\noexpand\pgfeov
		}%
		%
		% The transformation is now \pgfplots@loc@TMPc
		%
		% any user-specified axis limits:
		\expandafter\let\expandafter\pgfplots@loc@TMPa\csname pgfplots@#1min\endcsname
		\ifx\pgfplots@loc@TMPa\pgfutil@empty
		\else
			\expandafter\pgfplots@loc@TMPc\expandafter{\pgfplots@loc@TMPa}\pgfeov%
			\expandafter\global\expandafter\let\csname pgfplots@#1min\endcsname=\pgfmathresult
		\fi
		\expandafter\let\expandafter\pgfplots@loc@TMPa\csname pgfplots@#1max\endcsname
		\ifx\pgfplots@loc@TMPa\pgfutil@empty
		\else
			\expandafter\pgfplots@loc@TMPc\expandafter{\pgfplots@loc@TMPa}\pgfeov%
			\expandafter\global\expandafter\let\csname pgfplots@#1max\endcsname=\pgfmathresult
		\fi
		%
		% any user specified axis ticks:
		\expandafter\let\expandafter\pgfplots@loc@TMPa\csname pgfplots@#1tick\endcsname
		\ifx\pgfplots@loc@TMPa\pgfutil@empty
		\else
			\def\pgfplots@loc@TMPb{data}%
			\ifx\pgfplots@loc@TMPa\pgfplots@loc@TMPb
			\else
				\expandafter\pgfplots@filter@input@ticks@with@highleveltrafo\expandafter{\pgfplots@loc@TMPa}{\pgfplots@loc@TMPc}%
				\expandafter\edef\csname pgfplots@#1tick\endcsname{\pgfmathresult}%
			\fi
		\fi
		\expandafter\let\expandafter\pgfplots@loc@TMPa\csname pgfplots@extra@#1tick\endcsname
		\ifx\pgfplots@loc@TMPa\pgfutil@empty
		\else
			\expandafter\pgfplots@filter@input@ticks@with@highleveltrafo\expandafter{\pgfplots@loc@TMPa}{\pgfplots@loc@TMPc}%
			\expandafter\edef\csname pgfplots@extra@#1tick\endcsname{\pgfmathresult}%
		\fi
		%
	\fi
	%
	\pgfkeysgetvalue{/pgfplots/#1filter}\pgfplots@loc@TMPa
	\ifx\pgfplots@loc@TMPa\pgfutil@empty
	\else
		\expandafter\let\csname pgfplots@#1filter@backwcompat\endcsname=\pgfplots@loc@TMPa
		\t@pgfplots@tokc={/pgfplots/#1filter is deprecated. Please use /pgfplots/#1 filter/.code={\def\pgfmathresult{\#1}}}%
		\pgfplots@warning{\the\t@pgfplots@tokc}%
		\pgfkeys{/pgfplots/#1 filter/.code={\csname pgfplots@#1filter@backwcompat\endcsname{##1}\to\pgfmathresult}}%
	\fi
	\csname ifpgfplots@#1islinear\endcsname
		\csname pgfplots@apply@datatrafo@#1true\endcsname
		\pgfplots@apply@datatrafotrue
		\ifpgfplots@apply@datatrafo
			% Check for any existing axis limits:
			\expandafter\let\expandafter\pgfplots@loc@TMPa\csname pgfplots@#1min\endcsname
			\ifx\pgfplots@loc@TMPa\pgfutil@empty
			\else
				\expandafter\pgfmathfloatparsenumber\expandafter{\pgfplots@loc@TMPa}%
				\expandafter\global\expandafter\let\csname pgfplots@#1min\endcsname=\pgfmathresult
			\fi
			\expandafter\let\expandafter\pgfplots@loc@TMPa\csname pgfplots@#1max\endcsname
			\ifx\pgfplots@loc@TMPa\pgfutil@empty
			\else
				\expandafter\pgfmathfloatparsenumber\expandafter{\pgfplots@loc@TMPa}%
				\expandafter\global\expandafter\let\csname pgfplots@#1max\endcsname=\pgfmathresult
			\fi
		\fi
	\else
		% This here could be done using a high level coord trafo as
		% well! However, I don't want to risk accidentally overwritten
		% keys, so I replicate it here.
		\ifpgfplots@disablelogfilter
		\else
			% any user-specified axis limits:
			\expandafter\let\expandafter\pgfplots@loc@TMPa\csname pgfplots@#1min\endcsname
			\ifx\pgfplots@loc@TMPa\pgfutil@empty
			\else
				\expandafter\pgfmathlog@\expandafter{\pgfplots@loc@TMPa}%
				\expandafter\global\expandafter\let\csname pgfplots@#1min\endcsname=\pgfmathresult
			\fi
			\expandafter\let\expandafter\pgfplots@loc@TMPa\csname pgfplots@#1max\endcsname
			\ifx\pgfplots@loc@TMPa\pgfutil@empty
			\else
				\expandafter\pgfmathlog@\expandafter{\pgfplots@loc@TMPa}%
				\expandafter\global\expandafter\let\csname pgfplots@#1max\endcsname=\pgfmathresult
			\fi
			%
			% any user specified axis ticks:
			\expandafter\let\expandafter\pgfplots@loc@TMPa\csname pgfplots@#1tick\endcsname
			\ifx\pgfplots@loc@TMPa\pgfutil@empty
			\else
				\def\pgfplots@loc@TMPb{data}%
				\ifx\pgfplots@loc@TMPa\pgfplots@loc@TMPb
				\else
					\expandafter\pgfplots@filter@input@ticks@with@log\expandafter{\pgfplots@loc@TMPa}%
					\expandafter\edef\csname pgfplots@#1tick\endcsname{\pgfmathresult}%
				\fi
			\fi
			\expandafter\let\expandafter\pgfplots@loc@TMPa\csname pgfplots@extra@#1tick\endcsname
			\ifx\pgfplots@loc@TMPa\pgfutil@empty
			\else
				\expandafter\pgfplots@filter@input@ticks@with@log\expandafter{\pgfplots@loc@TMPa}%
				\expandafter\edef\csname pgfplots@extra@#1tick\endcsname{\pgfmathresult}%
			\fi
			%
			% append logarithm to prepare coord.
			%
			\pgfkeysgetvalue{/pgfplots/#1 coord trafo/.@cmd}\pgfplots@loc@TMPc
			\ifx\pgfplots@loc@TMPc\pgfplots@empty@command@key
				\expandafter\def\csname pgfplots@prepare@#1coord\endcsname##1{%
					\pgfmathlog@{##1}%
				}%
			\else
				% This is a bit complicated... but it works.
				\t@pgfplots@toka=\expandafter\expandafter\expandafter{\csname pgfplots@prepare@#1coord\endcsname{##1}\expandafter\pgfmathlog@\expandafter{\pgfmathresult}}%
				\edef\pgfplots@loc@TMPa{\the\t@pgfplots@toka}%
				\expandafter\def\expandafter\pgfplots@loc@TMPa\expandafter##\expandafter1\expandafter{\pgfplots@loc@TMPa}%
				\expandafter\let\csname pgfplots@prepare@#1coord\endcsname=\pgfplots@loc@TMPa
			\fi
		\fi
	\fi
}

\def\pgfplots@create@axis@descriptions{%
	\ifpgfplots@hide@x
	\else
		\pgfkeysgetvalue{/pgfplots/xlabel}{\pgfplots@label@}%
		\ifx\pgfplots@label@\pgfutil@empty
		\else
			\pgfplots@show@label{x}{\pgfplots@label@}%
		\fi
	\fi
	\ifpgfplots@hide@y
	\else
		\pgfkeysgetvalue{/pgfplots/ylabel}{\pgfplots@label@}%
		\ifx\pgfplots@label@\pgfutil@empty
		\else
			\pgfplots@show@label{y}{\pgfplots@label@}%
		\fi
	\fi
	%
	\pgfkeysgetvalue{/pgfplots/title}\pgfplots@loc@TMPa
	\ifx\pgfplots@loc@TMPa\pgfutil@empty
	\else
		\expandafter\pgfplots@show@title\expandafter{\pgfplots@loc@TMPa}%
	\fi
	\pgfplots@createlegend
}

\def\pgfplots@datascaletrafo@undoshift@x#1{%
	\pgfmathsubtract@{#1}{\pgfplots@data@scale@trafo@SHIFT@x}%
}%
\def\pgfplots@datascaletrafo@redoshift@x#1{%
	\pgfmathadd@{#1}{\pgfplots@data@scale@trafo@SHIFT@x}%
}%
\def\pgfplots@datascaletrafo@undoshift@y#1{%
	\pgfmathsubtract@{#1}{\pgfplots@data@scale@trafo@SHIFT@y}%
}%
\def\pgfplots@datascaletrafo@redoshift@y#1{%
	\pgfmathadd@{#1}{\pgfplots@data@scale@trafo@SHIFT@y}%
}%

% DATA TRANSFORMATION T(x) = X - xmin
%
% Input: 
%    a number in the original data range, given in **floating** point representation
% Output: 
%    a fixed point number in transformed range
%    stored in \pgfmathresult
% @see
% \pgfplots@datascaletrafo@fromfixed@x
\def\pgfplots@datascaletrafo@x#1{%
	\pgfmathfloatshift@{#1}{\pgfplots@data@scale@trafo@EXPONENT@x}%
	\expandafter\pgfmathfloattofixed\expandafter{\pgfmathresult}%
	\expandafter\pgfmathsubtract@\expandafter{\pgfmathresult}{\pgfplots@data@scale@trafo@SHIFT@x}%
}
\def\pgfplots@datascaletrafo@x@noshift#1{%
	\pgfmathfloatshift@{#1}{\pgfplots@data@scale@trafo@EXPONENT@x}%
	\expandafter\pgfmathfloattofixed\expandafter{\pgfmathresult}%
}

% Overloaded function.
% Input:
%     a FIXED point number instead of a floating point one.
% @see \pgfplots@datascaletrafo@x
\def\pgfplots@datascaletrafo@fromfixed@x#1{%
	\pgfmathfloatparsenumber{#1}%
	\expandafter\pgfplots@datascaletrafo@x\expandafter{\pgfmathresult}%
}

\def\pgfplots@datascaletrafo@y#1{%
	\pgfmathfloatshift@{#1}{\pgfplots@data@scale@trafo@EXPONENT@y}%
	\expandafter\pgfmathfloattofixed\expandafter{\pgfmathresult}%
	\expandafter\pgfmathsubtract@\expandafter{\pgfmathresult}{\pgfplots@data@scale@trafo@SHIFT@y}%
}
\def\pgfplots@datascaletrafo@fromfixed@y#1{%
	\pgfmathfloatparsenumber{#1}%
	\expandafter\pgfplots@datascaletrafo@y\expandafter{\pgfmathresult}%
}
\def\pgfplots@datascaletrafo@y@noshift#1{%
	\pgfmathfloatshift@{#1}{\pgfplots@data@scale@trafo@EXPONENT@y}%
	\expandafter\pgfmathfloattofixed\expandafter{\pgfmathresult}%
}

% INVERSE transformation x = T^{-1}( X )
% Input: 
%    a fixed point number in transformed domain
% Output:
%    a number in the data domain, given in floating point
%    representation
%
% If the input number is approximately X=0, we will return x=0 as
% well.
%
% This allows to handle rounding inaccuracies and should not pose any
% problems.
\def\pgfplots@inverse@datascaletrafo@x#1{%
	\begingroup
	\pgfmathadd@{#1}{\pgfplots@data@scale@trafo@SHIFT@x}%
	\let\pgfplots@inverse@datascaletrafo@@shifted=\pgfmathresult
	\pgfmathapproxequalto@{\pgfplots@inverse@datascaletrafo@@shifted}{0.0}%
	\ifpgfmathcomparison
		\pgfmathfloatcreate{0}{0.0}{0}%
	\else
		\pgfmathfloatparsenumber{\pgfplots@inverse@datascaletrafo@@shifted}%
		\edef\pgfplots@data@scale@trafo@EXPONENT@x{-\pgfplots@data@scale@trafo@EXPONENT@x}%
		\expandafter\pgfmathfloatshift@\expandafter{\pgfmathresult}{\pgfplots@data@scale@trafo@EXPONENT@x}%
	\fi
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}
\def\pgfplots@inverse@datascaletrafo@x@noshift#1{%
	\begingroup
	\pgfmathapproxequalto@{#1}{0.0}%
	\ifpgfmathcomparison
		\pgfmathfloatcreate{0}{0.0}{0}%
	\else
		\pgfmathfloatparsenumber{#1}%
		\edef\pgfplots@data@scale@trafo@EXPONENT@x{-\pgfplots@data@scale@trafo@EXPONENT@x}%
		\expandafter\pgfmathfloatshift@\expandafter{\pgfmathresult}{\pgfplots@data@scale@trafo@EXPONENT@x}%
	\fi
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}

\def\pgfplots@inverse@datascaletrafo@y#1{%
	\begingroup
	\pgfmathadd@{#1}{\pgfplots@data@scale@trafo@SHIFT@y}%
	\let\pgfplots@inverse@datascaletrafo@@shifted=\pgfmathresult
	\pgfmathapproxequalto@{\pgfplots@inverse@datascaletrafo@@shifted}{0.0}%
	\ifpgfmathcomparison
		\pgfmathfloatcreate{0}{0.0}{0}%
	\else
		\pgfmathfloatparsenumber{\pgfplots@inverse@datascaletrafo@@shifted}%
		\edef\pgfplots@data@scale@trafo@EXPONENT@y{-\pgfplots@data@scale@trafo@EXPONENT@y}%
		\expandafter\pgfmathfloatshift@\expandafter{\pgfmathresult}{\pgfplots@data@scale@trafo@EXPONENT@y}%
	\fi
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}
% Overloaded function. This one does only apply the scaling, no shift.
\def\pgfplots@inverse@datascaletrafo@y@noshift#1{%
	\begingroup
	\pgfmathapproxequalto@{#1}{0.0}%
	\ifpgfmathcomparison
		\pgfmathfloatcreate{0}{0.0}{0}%
	\else
		\pgfmathfloatparsenumber{#1}%
		\edef\pgfplots@data@scale@trafo@EXPONENT@y{-\pgfplots@data@scale@trafo@EXPONENT@y}%
		\expandafter\pgfmathfloatshift@\expandafter{\pgfmathresult}{\pgfplots@data@scale@trafo@EXPONENT@y}%
	\fi
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}

% Overloaded function.
%
% In contrast to \pgfplots@inverse@datascaletrafo@x, this method
% returns a number in FIXED point representation.
% @see \pgfplots@inverse@datascaletrafo@x
\def\pgfplots@inverse@datascaletrafo@tofixed@x#1{%
	\pgfplots@inverse@datascaletrafo@x{#1}%
	\expandafter\pgfmathfloattofixed\expandafter{\pgfmathresult}%
}
\def\pgfplots@inverse@datascaletrafo@tofixed@y#1{%
	\pgfplots@inverse@datascaletrafo@y{#1}%
	\expandafter\pgfmathfloattofixed\expandafter{\pgfmathresult}%
}

% Overloaded function.
%
% This one does only apply the scale, no shift.
\def\pgfplots@inverse@datascaletrafo@tofixed@x@noshift#1{%
	\pgfplots@inverse@datascaletrafo@x@noshift{#1}%
	\expandafter\pgfmathfloattofixed\expandafter{\pgfmathresult}%
}
\def\pgfplots@inverse@datascaletrafo@tofixed@y@noshift#1{%
	\pgfplots@inverse@datascaletrafo@y@noshift{#1}%
	\expandafter\pgfmathfloattofixed\expandafter{\pgfmathresult}%
}

% Parses all options in #1 which are known in the currently active families.
%
% The result will be stored back into the TikZ-style named #1 without 
% further processing.
%
% Example:
% \tikzstyle{every axis}=[xmin=0,xmax=1,line width=1pt
% \pgfplots@set@keys@from@tikz@style\tmpmacro{every axis}{/pgfplots}
% 
% - sets axis options 'xmin' and 'xmax'
% - calls \tikzstyle{every axis}={line width=1pt}
% 
% I assume that this method is called within local TeX groups so
% nothing will be destroyed outside.
%
% #1:  A style name.
\def\pgfplots@set@keys@from@tikz@style#1{%
	\let\pgfplots@rmopts=\pgfutil@empty
	\pgfqkeysfiltered{/pgfplots}{/pgfplots/#1}%
	\pgfplots@set@keymacro@to@style\pgfplots@rmopts{#1}%
}

% The same as \pgfplots@set@keys@from@tikz@style  but this one appends
% unmatched options to style #2.
%
% #1:  A style name.
% #2:  A style name which will be filled with unprocessed options.
\def\pgfplots@set@keys@from@tikz@style@append@to#1#2{%
	\let\pgfplots@rmopts=\pgfutil@empty
	\pgfqkeysfiltered{/pgfplots}{/pgfplots/#1}%
	\pgfplots@append@keymacro@to@style\pgfplots@rmopts{#2}%
}

% #1:  A sequence of options.
% #2:  A style name which will be filled with unprocessed options.
\def\pgfplots@set@keys@and@append@remaining@to@style#1#2{%
	\let\pgfplots@rmopts=\pgfutil@empty
	\pgfqkeysfiltered{/pgfplots}{#1}%
	\pgfplots@append@keymacro@to@style\pgfplots@rmopts{#2}%
}%

% #1: input macro
\def\pgfplots@setkeys@from@macro#1{%
	\let\pgfplots@rmopts=\pgfutil@empty
	\def\pgfplots@loc@TMPa{\pgfqkeysfiltered{/pgfplots}}%
	\expandafter\pgfplots@loc@TMPa\expandafter{#1}%
}

% #1: macro
% #2: style name
\long\def\pgfplots@append@keymacro@to@style#1#2{%
	\t@pgfplots@toka={#2/.append style=}%
	\t@pgfplots@tokb=\expandafter{#1}%
	\edef\pgfplots@setkeys@TMP{\the\t@pgfplots@toka{\the\t@pgfplots@tokb}}%
	\expandafter\pgfplotsset\expandafter{\pgfplots@setkeys@TMP}%
%\pgfplots@message{tikzstyle{#2}+=[#1]}%
}

% #1: macro
% #2: style name
\long\def\pgfplots@set@keymacro@to@style#1#2{%
	\t@pgfplots@toka={#2/.style=}%
	\t@pgfplots@tokb=\expandafter{#1}%
	\edef\pgfplots@setkeys@TMP{\the\t@pgfplots@toka{\the\t@pgfplots@tokb}}%
	\expandafter\pgfplotsset\expandafter{\pgfplots@setkeys@TMP}%
%\pgfplots@message{tikzstyle{#2}=[#1]}%
}

% backwards compatibility:
\let\prettyprintnumber=\pgfmathprintnumber%

\def\pgfplots@set@options#1{%
	\pgfutil@ifundefined{tikz@lastx}{%
		% no warning. Its not that important anyway, I think.
		\def\pgfplots@at{\pgfpointorigin}%
	}{%
		\def\pgfplots@at{\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
	}%
	%
	% Temporarily assign families to 'name' and 'alias' options.
	% This allows to get the names - they should not be appended to
	% 'every axis'!
	\pgfkeys{%
		/tikz/domain/.belongs to family=/pgfplots,
		/pgfplots/domain/.code={\pgfkeysalso{/tikz/domain=##1}},
		/tikz/name/.belongs to family=/pgfplots/naming commands,
		/tikz/alias/.belongs to family=/pgfplots/naming commands,
		% and provide aliases in the '/pgfplots/' tree to avoid 
		% search path problems just for these two options:
		/pgfplots/name/.belongs to family=/pgfplots/naming commands,
		/pgfplots/alias/.belongs to family=/pgfplots/naming commands,
		/pgfplots/name/.code={\pgfkeysalso{/tikz/name=##1}},
		/pgfplots/alias/.code={\pgfkeysalso{/tikz/alias=##1}},
		%
		%
		/pgf/key filter handlers/append filtered to/.install key filter handler=\pgfplots@rmopts,
	}%
	\let\tikz@alias=\pgfutil@empty
	\let\tikz@fig@name=\pgfutil@empty
	%
	% Step 1: acquire ONLY 'xmode' and 'ymode' (necessary to decide
	% which axis style shall be loaded):
		\let\pgfplots@rmopts=\pgfutil@empty
		\pgfkeysinstallkeyfilter
			{/pgf/key filters/active families or no family}
			{{/pgf/key filters/false}{/pgf/key filters/false}}
		%
		\pgfqkeysactivatesinglefamilyandfilteroptions{/pgfplots/scale}%
			{/pgfplots}
			{#1}%
	\let\pgfplots@remaining@input=\pgfplots@rmopts
	%
	% Step 2: parse any pgfplots options out of styles.
	\pgfkeysactivatefamily{/pgfplots/style commands}%
	\pgfkeysinstallkeyfilter
		{/pgf/key filters/active families or no family}% DEBUG}
		{{/pgf/key filters/is descendant of=/pgfplots}% for keys without family
		 {/pgf/key filters/false}% for unknown keys
		}%
	%
	\pgfkeysactivatefamilies
		{/pgfplots,/pgfplots/naming commands,/pgfplots/tick,/pgfplots/legend,/pgfplots/descriptions,/pgfplots/scale}
		{\pgfplots@deactivefamiliescmd}%
		\pgfplots@set@keys@from@tikz@style{every axis}%
		\pgfkeysdeactivatefamily{/pgfplots/scale}%
		%
		\ifpgfplots@xislinear
			\ifpgfplots@yislinear
				\pgfplots@set@keys@from@tikz@style@append@to{every linear axis}{every axis}%
			\else
				\pgfplots@set@keys@from@tikz@style@append@to{every semilogy axis}{every axis}%
			\fi
		\else
			\ifpgfplots@yislinear
				\pgfplots@set@keys@from@tikz@style@append@to{every semilogx axis}{every axis}%
			\else
				\pgfplots@set@keys@from@tikz@style@append@to{every loglog axis}{every axis}%
			\fi
		\fi
	\pgfplots@deactivefamiliescmd
	%
	% Acquire style commands and nameing commands from direct input
	% options '#1' BEFORE the 'every' styles are processed:
	\pgfkeysactivatefamily{/pgfplots/naming commands}%
		\pgfplots@setkeys@from@macro\pgfplots@remaining@input%
		\let\pgfplots@remaining@input=\pgfplots@rmopts
	\pgfkeysdeactivatefamily{/pgfplots/naming commands}%
	%
	% Now, any 'name' and 'alias' options have been processed. 
	%
	% Remember their current meaning and reset the tikz options!
	\let\pgfplots@fig@name=\tikz@fig@name
	\let\pgfplots@fig@alias=\tikz@alias
	\let\tikz@alias=\pgfutil@empty
	\let\tikz@fig@name=\pgfutil@empty
	%
	% And protocol all named sub-nodes! Their positions need to be
	% updated later.
	\let\pgfplots@named@child@node@list=\pgfutil@empty
	\pgfkeysgetvalue{/tikz/name/.@cmd}\pgfplots@old@name@impl
	\pgfkeysgetvalue{/tikz/alias/.@cmd}\pgfplots@old@alias@impl
	\pgfkeysdef{/tikz/name}{%
		\xdef\pgfplots@named@child@node@list{\pgfplots@named@child@node@list,{##1}}%
		\pgfplots@old@name@impl##1\pgfeov
	}%
	\pgfkeysdef{/tikz/alias}{%
		\xdef\pgfplots@named@child@node@list{\pgfplots@named@child@node@list,{##1}}%
		\pgfplots@old@alias@impl##1\pgfeov
	}%
	%
	% Now, continue to process the 'every' styles. Please note that
	% the 'legend style={}' like options have already been processed;
	% their values are already inside of the associated 'every'
	% styles.
	%
	% What I am doing here is: set every pgfplots-option directly, and
	% discard it from the every-style. Any non-pgfplots-option will
	% be set in its context.
	%
	\pgfkeysactivatefamily{/pgfplots/legend}%
		\pgfplots@set@keys@from@tikz@style{every axis legend}%
	\pgfkeysdeactivatefamily{/pgfplots/legend}%
	%
	%
	\pgfkeysactivatefamily{/pgfplots/descriptions}%
		\pgfplots@set@keys@from@tikz@style{every axis label}%
		\pgfplots@set@keys@from@tikz@style{every axis x label}%
		\pgfplots@set@keys@from@tikz@style{every axis y label}%
		\pgfplots@set@keys@from@tikz@style{every axis title}%
	\pgfkeysdeactivatefamily{/pgfplots/descriptions}%
	%
	\pgfkeysactivatefamily{/pgfplots/tick}%
		\pgfplots@set@keys@from@tikz@style{every tick}%
		\pgfplots@set@keys@from@tikz@style{every minor tick}%
		\pgfplots@set@keys@from@tikz@style{every major tick}%
		\pgfplots@set@keys@from@tikz@style{every axis grid}%
		\pgfplots@set@keys@from@tikz@style{every minor grid}%
		\pgfplots@set@keys@from@tikz@style{every major grid}%
	\pgfkeysdeactivatefamily{/pgfplots/tick}%
	%
	%--------------------------------------------------
	% \pgfkeysactivatefamily{/pgfplots}%
	% 	\pgfplots@set@keys@from@tikz@style{every axis plot}%
	% \pgfkeysdeactivatefamily{/pgfplots}%
	%-------------------------------------------------- 
	%
	\pgfkeysactivatefamily{/pgfplots/descriptions}%
	\pgfkeysactivatefamily{/pgfplots/tick}%
		\pgfplots@set@keys@from@tikz@style{every x tick label}%
		\pgfplots@set@keys@from@tikz@style{every y tick label}%
		\pgfplots@set@keys@from@tikz@style{every tick label}%
	\pgfkeysdeactivatefamily{/pgfplots/tick}%
	\pgfkeysdeactivatefamily{/pgfplots/descriptions}%
	%
	% Step 3: Set all remaining options of '#1'. They should have
	% highest precedence.
	\pgfkeysactivatefamilies
		{/pgfplots,/pgfplots/tick,/pgfplots/legend,/pgfplots/descriptions}%
		{\pgfplots@deactivefamiliescmd}%
		\expandafter
			\pgfplots@set@keys@and@append@remaining@to@style
		\expandafter
			{\pgfplots@remaining@input}%
			{every axis}%
	\pgfplots@deactivefamiliescmd
%\pgfkeysgetvalue{/tikz/every axis/.@cmd}\pgfplots@loc@TMPa
%\message{every axis is now '\meaning\pgfplots@loc@TMPa'}%
	%
	\pgfkeysdeactivatefamily{/pgfplots/style commands}%
	\global\pgfkeysgetvalue{/pgfplots/xmin}{\pgfplots@xmin}%
	\global\pgfkeysgetvalue{/pgfplots/xmax}{\pgfplots@xmax}%
	\global\pgfkeysgetvalue{/pgfplots/ymin}{\pgfplots@ymin}%
	\global\pgfkeysgetvalue{/pgfplots/ymax}{\pgfplots@ymax}%
	%
	\def\pgfplots@loc@TMPa{data}%
	\pgfplots@collect@firstplot@astickfalse
	\ifx\pgfplots@xtick\pgfplots@loc@TMPa
		\pgfplots@collect@firstplot@asticktrue
	\fi
	\ifx\pgfplots@ytick\pgfplots@loc@TMPa
		\pgfplots@collect@firstplot@asticktrue
	\fi
	\ifpgfplots@collect@firstplot@astick
		\let\pgfplots@firstplot@coords@x=\pgfutil@empty
		\let\pgfplots@firstplot@coords@y=\pgfutil@empty
	\fi
	\pgfkeysdef{/pgfplots/.unknown}{%
		\let\pgfplots@searchname=\pgfkeyscurrentname
		\pgfkeysalso{/tikz/\pgfplots@searchname=##1}%
	}%
}

\def\pgfplots@install@abbrev@commands{
	\let\pgfplots@orig@path=\path
	\let\pgfplots@orig@plot=\plot
	%
	\let\axispath=\pgfplots@path
	\let\pgfplotsinterruptdatabb=\pgfplots@interruptdatabb
	\let\endpgfplotsinterruptdatabb=\endpgfplots@interruptdatabb
	%
	\let\addplot=\pgfplots@addplot
	\let\plot=\addplot
	%
	\def\logten{2.3025851}%
	\def\reciproclogten{0.434294}%
	%
	\def\logi##1{%
		\ifcase##1
		\or0
		\or0.693147
		\or1.098612
		\or1.386294
		\or1.60943791
		\or1.7917594
		\or1.94591014
		\or2.07944154
		\or2.197224
		\fi
	}%
	\def\axisdefaultticklabel{$\pgfmathprintnumber{\tick}$}%
	\def\axisdefaultticklabellog{%
		\pgfkeysgetvalue{/pgfplots/log number format code/.@cmd}\pgfplots@log@label@style
		\expandafter\pgfplots@log@label@style\tick\pgfeov
	}%
	%
	\let\legend=\pgfplots@command@legend
	\let\addlegendentry=\pgfplots@addlegendentry
}

\def\pgfplots@environment{%
	\pgfutil@ifnextchar[{%
		\pgfplots@environment@opt
	}{%
		\pgfplots@environment@opt[]%
	}%
}%

% temporary (local) variables inside of axis
\newif\ifpgfplots@autocomputeanylimits
\newif\ifpgfplots@autocompute@all@limits
\newif\ifpgfplots@autocompute@xmin
\newif\ifpgfplots@autocompute@xmax
\newif\ifpgfplots@autocompute@ymin
\newif\ifpgfplots@autocompute@ymax
\newif\ifpgfplots@apply@datatrafo@x
\newif\ifpgfplots@apply@datatrafo@y
\newif\ifpgfplots@apply@datatrafo
\newif\ifpgfplots@datascaletrafo@initialised
\newif\ifpgfplots@draw@at@end

% Extracts single components of an entry of
% \pgfplots@stored@plotlist
%
% They are defined as
% \pgfplots@stored@current@precmd
% \pgfplots@stored@current@cmd
% \pgfplots@stored@current@data
% \pgfplots@stored@current@postcmd
\def\pgfplots@stored@plotlist@EXTRACTENTRY#1#2#3#4{%
	\def\pgfplots@stored@current@precmd{#1}%
	\def\pgfplots@stored@current@cmd{#2}%
	\def\pgfplots@stored@current@data{#3}%
	\def\pgfplots@stored@current@postcmd{#4}%
}

\def\pgfplots@init@cleared@structures{%
	\global\pgfplotslistnewempty\pgfplots@plotspeclist
	\global\pgfplotslistnewempty\pgfplots@legend
	\global\pgfplotslistnewempty\pgfplots@stored@plotlist
	\global\pgfplots@numplots=0
	\let\pgfplots@already@computed@legend@node=\pgfutil@empty
}

% The implementation for \label{foo} after \addplot. It allows to
% \ref{foo} (it inserts the 'legend image code').
%
% I only need to overwrite '\label'; the rest is done by LaTeX.
%
% THIS IS INCOMPATIBLE WITH plain TeX and ConTeXt! Don't use it, it
% doesn't hurt.
\def\pgfplots@plot@label#1{%
	\ifx\pgfplots@last@plot@style\pgfutil@empty
		\pgfplots@error{Can't create \string\label{#1}: it needs to be called after \string\addplot.}%
	\else
		\begingroup
		% I'd like to get all options which are INDEPENDENT of
		% pgfplots. Idea: expand all /pgfplots-keys and collect
		% everything which belongs NOT to /pgfplots. This is the
		% completely expanded rest. At least, I hope so and it appears
		% to work.
		\pgfkeysinstallkeyfilter
			{/pgf/key filters/and}
				{{/pgf/key filters/is descendant of=/pgfplots}%
				 {/pgf/key filters/defined}}%
		\def\pgfplots@label@tikzopts{}%
		\pgfkeysinstallkeyfilterhandler{/pgf/key filter handlers/append filtered to}{\pgfplots@label@tikzopts}%
		\def\pgfplots@loc@TMPa{\pgfqkeysfiltered{/tikz}}%
		\expandafter\pgfplots@loc@TMPa\expandafter{\pgfplots@last@plot@style}%
		%
		\pgfkeysgetvalue{/pgfplots/every crossref picture/.@cmd}{\pgfplots@crossref@pic}%
		\pgfkeysgetvalue{/pgfplots/legend image code/.@cmd}{\pgfplots@curlegendcode}%
		\t@pgfplots@toka=\expandafter{\pgfplots@curlegendcode current plot style\pgfeov}%
		\t@pgfplots@tokb=\expandafter{\pgfplots@label@tikzopts}%
		\t@pgfplots@tokc=\expandafter{\pgfplots@crossref@pic\pgfeov}%
		\edef\pgfplots@loc@TMPa{%
			\noexpand\begingroup
			\noexpand\pgfkeysdef{/tikz/current plot style}{\noexpand\pgfkeysalso{\the\t@pgfplots@tokb}}%
			\noexpand\pgfkeysdef{/pgfplots/every crossref picture}{\the\t@pgfplots@tokc}%
			\noexpand\tikz[/pgfplots/every crossref picture]{\the\t@pgfplots@toka}%
			\noexpand\endgroup%
		}%
		\pgfplots@command@to@string{\pgfplots@loc@TMPa}{\pgfplots@loc@TMPa}%
		\global\let\pgfplots@glob@TMPb=\pgfplots@loc@TMPa
		\endgroup
		\let\@currentlabel=\pgfplots@glob@TMPb
		\pgfplots@original@LaTeX@label{#1}%
	\fi
}%

\def\pgfplots@interruptdatabb{%
	\def\pgfplots@update@limits@for@one@point##1##2##3##4{}%
}%
\def\endpgfplots@interruptdatabb{%
	\let\pgfplots@update@limits@for@one@point=\pgfplots@update@limits@for@one@point@orig
}%

\def\pgfplots@environment@opt[#1]{%
	\begingroup
	\pgfplots@install@abbrev@commands
	\pgfplots@stacked@initialise
	%
	%
	% The explicit specification of 'x' and 'y' as 1pt is to avoid
	% numeric overflow/underflow during scale computations:
	%
	% The scaling (i.e. proper values for 'x' and 'y') will be
	% determined later-on, dependend on the axis limits.  Since axis
	% limits are implicitly in units of 1pt, it is reasonable to use
	% '1pt' here as well.
	\pgfsetxvec{\pgfqpoint{1pt}{0pt}}%
	\pgfsetyvec{\pgfqpoint{0pt}{1pt}}%
	%
	\pgfplots@set@options{#1}%
	%
	% --------------------
	% Allocations:
	% --------------------
	\pgfplots@init@cleared@structures
	%
	% --------------------
	% Option preprocessing
	% --------------------
	\pgfplots@prepare@coord@filtering@for x
	\pgfplots@prepare@coord@filtering@for y
	\ifpgfplots@apply@datatrafo
		\pgfplots@datascaletrafo@initialisedfalse
	\else
		\pgfplots@datascaletrafo@initialisedtrue% there is no trafo.
	\fi
	%
	\ifpgfplots@xislinear
		\pgfmathfloatcreate{1}{1.0}{2147483645}%
		\let\pgfplots@invalidrange@xmin=\pgfmathresult
		\pgfmathfloatcreate{2}{1.0}{2147483645}%
		\let\pgfplots@invalidrange@xmax=\pgfmathresult
	\else
		\def\pgfplots@invalidrange@xmin{16300}%
		\def\pgfplots@invalidrange@xmax{-16300}%
	\fi
	\ifpgfplots@yislinear
		\pgfmathfloatcreate{1}{1.0}{2147483645}%
		\let\pgfplots@invalidrange@ymin=\pgfmathresult
		\pgfmathfloatcreate{2}{1.0}{2147483645}%
		\let\pgfplots@invalidrange@ymax=\pgfmathresult
	\else
		\def\pgfplots@invalidrange@ymin{16300}%
		\def\pgfplots@invalidrange@ymax{-16300}%
	\fi
	%
	% These numbers will ONLY be filled for linear axis!
	\global\let\pgfplots@data@xmin=\pgfplots@invalidrange@xmin
	\global\let\pgfplots@data@xmax=\pgfplots@invalidrange@xmax
	\global\let\pgfplots@data@ymin=\pgfplots@invalidrange@ymin
	\global\let\pgfplots@data@ymax=\pgfplots@invalidrange@ymax
	%
	\pgfplots@autocompute@all@limitstrue
	\ifx\pgfplots@xmin\pgfutil@empty
		\pgfplots@autocompute@xmintrue
		\global\let\pgfplots@xmin=\pgfplots@invalidrange@xmin
		\pgfplots@autocomputeanylimitstrue
	\else
		\pgfplots@autocompute@all@limitsfalse
	\fi
	\ifx\pgfplots@xmax\pgfutil@empty
		\pgfplots@autocompute@xmaxtrue
		\global\let\pgfplots@xmax=\pgfplots@invalidrange@xmax
		\pgfplots@autocomputeanylimitstrue
	\else
		\pgfplots@autocompute@all@limitsfalse
	\fi
	\ifx\pgfplots@ymin\pgfutil@empty
		\pgfplots@autocompute@ymintrue
		\global\let\pgfplots@ymin=\pgfplots@invalidrange@ymin
		\pgfplots@autocomputeanylimitstrue
	\else
		\pgfplots@autocompute@all@limitsfalse
	\fi
	\ifx\pgfplots@ymax\pgfutil@empty
		\pgfplots@autocompute@ymaxtrue
		\global\let\pgfplots@ymax=\pgfplots@invalidrange@ymax
		\pgfplots@autocomputeanylimitstrue
	\else
		\pgfplots@autocompute@all@limitsfalse
	\fi
	%
	% autocomputelimits := at least one limit needs to be updated.
	\ifpgfplots@autocomputeanylimits
		\pgfplots@draw@at@endtrue
	\fi
	%
	%
	% --------------------
	% Start axis:
	% either postponed to \end or directly.
	% --------------------
	%
	% Since I've introduced a public \numplots macro, I should 
	% make sure it's filled correctly:
	\pgfplots@draw@at@endtrue
	%
	\ifpgfplots@collect@firstplot@astick
		\pgfplots@draw@at@endtrue
	\fi
	\ifpgfplots@apply@datatrafo
		% ALWAYS TRUE. This allows to use inline plots because the data
		% scale transformation will be applied after I know that it should
		% be disabled.
		\pgfplots@draw@at@endtrue
	\fi
	\ifpgfplots@stackedmode
		% Stacked plots require special attention: they are drawn in
		% REVERSE order.
		\pgfplots@draw@at@endtrue
	\else
		% we have no stacked plots and thus no reversing.
		\pgfplots@stacked@reversefalse
	\fi
	%
	\pgfutil@ifundefined{label}{\relax}{%
		\let\pgfplots@original@LaTeX@label=\label
		\let\label=\pgfplots@plot@label
	}%
	\global\let\pgfplots@last@plot@style=\pgfutil@empty
	%
	% any \path command is invalid inside of an axis.
	% Use \axispath instead:
	\def\numplots{\the\pgfplots@numplots}%
	\let\path=\pgfplots@replacement@for@tikz@path
	\let\closedcycle=\pgfplots@path@closed@cycle
	\ifpgfplots@draw@at@end
		\let\pgfplots@nextcommand=\relax
	\else
		\def\pgfplots@nextcommand{\pgfplots@BEGIN@init@and@draw@axis}%
	\fi
	\pgfplots@nextcommand
}
\def\endpgfplots@environment@opt{%
	\xdef\numplots{\the\pgfplots@numplots}%
	\pgfkeysvalueof{/pgfplots/before end axis/.@cmd}\pgfeov%
	%
	% restore old \path command:
	\let\path=\pgfplots@orig@path
	\let\plot=\pgfplots@orig@plot
	%
	%\end{axis}:
	% --------------------
	%  All plotting commands have been read.
	%  -> apply postponed drawing commands!
	% --------------------
	\ifpgfplots@draw@at@end% ALWAYS TRUE - this is obsolete
		\def\pgfplots@nextcommand{%
			\pgfplots@BEGIN@init@and@draw@axis
			\pgfplots@stacked@initialise
			\global\pgfplotslistnewempty\pgfplots@stored@markerlist
			\ifpgfplots@stacked@reverse
				% This here applies any scaling trafos and assembles a
				% NEW \pgfplots@stored@plotlist!
				\pgfplots@stacked@finalize@stored@plots
			\fi
			\pgfplotslistforeach\pgfplots@stored@plotlist\as\pgfplots@loc@TMPa{%
				\expandafter\pgfplots@stored@plotlist@EXTRACTENTRY\pgfplots@loc@TMPa
%\message{Processing stored plot with precommand '\meaning\pgfplots@stored@current@precmd';  pgfplots@plotcmd '\meaning\pgfplots@stored@current@cmd' postcommand '\meaning\pgfplots@stored@current@postcmd'}%
				% The precmd processed any error bars.
				\pgfplots@stored@current@precmd
				\ifx\pgfplots@stored@current@cmd\pgfutil@empty
					\pgfplots@stored@current@data%
				\else
					% this code here means we REALLY have a plotting
					% command!
					\ifpgfplots@stacked@reverse
						% has already been processed above, in \pgfplots@stacked@finalize@stored@plots.
						\pgfplots@stacked@draw@reversed@plot
					\else
						% modifies \pgfplots@stored@markerlist if necessary.
						\expandafter\pgfplots@coord@stream@finalize@storedcoords@START\pgfplots@stored@current@data\pgfplots@EOI
					\fi
				\fi
				\pgfplots@stored@current@postcmd
			}%
			\global\pgfplotslistnewempty\pgfplots@stored@plotlist% delete contents.
		}%
	\else
		\let\pgfplots@nextcommand=\relax
	\fi
	\pgfplots@nextcommand
	\pgfplots@END@init@and@draw@axis
	%
	%
	\begingroup
		% set coordinate system to (0,0) rectangle (1,1) for descriptions:
		\pgftransformxshift{\pgfplots@xcoordminTEX}%
		\pgftransformyshift{\pgfplots@ycoordminTEX}%
		%
		% create a 'current axis' node for anchor references. 
		\pgfmultipartnode{pgfplots@low@level@shape@INNER}{south west}{current axis}{\pgfusepath{discard}}%
		%
		\pgfplots@tmpa=\pgfplots@xcoordmaxTEX
		\advance\pgfplots@tmpa by-\pgfplots@xcoordminTEX
		\pgfsetxvec{\pgfqpoint{\pgfplots@tmpa}{0cm}}%
		%
		\pgfplots@tmpa=\pgfplots@ycoordmaxTEX
		\advance\pgfplots@tmpa by-\pgfplots@ycoordminTEX
		\pgfsetyvec{\pgfqpoint{0cm}{\pgfplots@tmpa}}%
		%
		\pgfplots@create@axis@descriptions
		\pgfkeysvalueof{/pgfplots/extra description/.@cmd}\pgfeov%
	\endgroup
	\endtikzpicture%
	\begingroup
		% Protocol sizes for the axis-shape.
		% I fear that needs to be done globally, do avoid all those
		% \endgroup's in and after \endpgfinterruptpicture ...
		\ifdim\pgf@picmaxx=-16000pt\relax%
			\pgf@picmaxx=0pt\relax%
			\pgf@picminx=0pt\relax%
			\pgf@picmaxy=0pt\relax%
			\pgf@picminy=0pt\relax%
		\fi%
		%
		\xdef\pgfplots@saveddimen@picminx{\the\pgf@picminx}%
		\xdef\pgfplots@saveddimen@picminy{\the\pgf@picminy}%
		%
		\pgf@xa=\pgfplots@xcoordmaxTEX
		\advance\pgf@xa by-\pgf@picminx
		\xdef\pgfplots@savedanchor@inner@upperright@x{\the\pgf@xa}%
		%
		\pgf@xa=\pgfplots@xcoordminTEX
		\advance\pgf@xa by-\pgf@picminx
		\xdef\pgfplots@savedanchor@inner@lowerleft@x{\the\pgf@xa}%
		%
		\pgf@xa=\pgfplots@ycoordmaxTEX
		\advance\pgf@xa by-\pgf@picminy
		\xdef\pgfplots@savedanchor@inner@upperright@y{\the\pgf@xa}%
		%
		\pgf@xa=\pgfplots@ycoordminTEX
		\advance\pgf@xa by-\pgf@picminy
		\xdef\pgfplots@savedanchor@inner@lowerleft@y{\the\pgf@xa}%
		%
		\pgf@xa=\pgfplots@ZERO@x
		\advance\pgf@xa by-\pgf@picminx
		\xdef\pgfplots@ZERO@x{\the\pgf@xa}%
		%
		\pgf@xa=\pgfplots@ZERO@y
		\advance\pgf@xa by-\pgf@picminy
		\xdef\pgfplots@ZERO@y{\the\pgf@xa}%
	\endgroup
	\endpgfinterruptpicture
	\egroup\egroup% end of pgfnodepartimagebox
	%
	\let\tikz@fig@name=\pgfplots@fig@name
	\tikz@fig@mustbenamed
    \pgftransformshift{\pgfplots@at}%
	\pgfmultipartnode{pgfplots@low@level@shape}{\pgfplots@anchorname}{\tikz@fig@name}{\pgfusepath{discard}}%
	\pgfplots@fig@alias
	\pgfnodealias{current axis}{\tikz@fig@name}%
	%
	\pgfplots@finally@correct@child@node@positions
	\pgfplots@stacked@finalize
	\endgroup
}

% Now, we need to process all named nodes inside of our
% axis-image.
%
% The situation at this point is as follows:
% 1. the complete axis image has been "typeset" into a box. That
% means its coordinate system is LOST up to those variables
% which have been saved explicitly.
%
% 2. the \pgfmultipartnode above knows about all axis anchors and
% saved dimensions.
%
% 3. All sub-nodes don't know about their position any more. Any
% saved anchors are wrong.
%
% The approach:
% 1. we shift each named node's saved anchors such that it's
% coordinate is valid inside of the TeX box.
%
% 2. we also shift each named node's saved anchors to reflect the
% axis' anchor.
%
% Afterwards, everything should be fine.
\def\pgfplots@finally@correct@child@node@positions{%
   \ifx\pgfplots@named@child@node@list\pgfutil@empty%
   \else%
      	\begingroup
		\pgftransformreset% FIXME: what's that for!? Copied from matrix code...
		%
		% Use the 'image' anchor here - the internal anchor
		% transformation matrix already has the shift for
		% \pgfplots@anchorname.
		\pgfpointanchor{\tikz@fig@name}{image}%
		\pgf@xa=\pgf@x
		\pgf@xb=\pgf@y
		\pgf@process{\pgfqpoint{\pgfplots@saveddimen@picminx}{\pgfplots@saveddimen@picminy}}%
		\advance\pgf@xa by-\pgf@x
		\advance\pgf@xb by-\pgf@y
		\pgf@x=\pgf@xa
		\pgf@y=\pgf@xb
		\edef\pgfplots@offset{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
		%
		\pgfutil@for\pgfplots@child@node@name:=\pgfplots@named@child@node@list\do{%
			\ifx\pgfplots@child@node@name\pgfutil@empty
			\else
				\expandafter\ifx\csname pgfplots@child@node@visited@\pgfplots@child@node@name\endcsname\relax%
					\pgfutil@ifundefined{pgf@sh@nt@\pgfplots@child@node@name}{%
						\pgfplots@warning{could not adjust coordinates of named node '\pgfplots@child@node@name' for reasons I do not understand! After finishing the image, it did no longer exist!? Sorry.}%
					}{%
						\pgf@shift@node{\pgfplots@child@node@name}{\pgfplots@offset}%
						\expandafter\let\csname pgfplots@child@node@visited@\pgfplots@child@node@name\endcsname=\pgfutil@empty%
					}%
				\fi
			\fi
		}%
		\endgroup
    \fi%
}%

\def\pgfplots@environment@axis{%
	\pgfutil@ifnextchar[{\pgfplots@@environment@axis}{\pgfplots@@environment@axis[]}%
}
\let\endpgfplots@environment@axis=\endpgfplots@environment@opt
\def\pgfplots@@environment@axis[#1]{%
	\pgfplots@environment@opt[/pgfplots/xmode=linear,/pgfplots/ymode=linear,#1]%
}

\def\pgfplots@environment@semilogxaxis{%
	\pgfutil@ifnextchar[{\pgfplots@@environment@semilogxaxis}{\pgfplots@@environment@semilogxaxis[]}%
}
\let\endpgfplots@environment@semilogxaxis=\endpgfplots@environment@opt
\def\pgfplots@@environment@semilogxaxis[#1]{%
	\pgfplots@environment@opt[/pgfplots/xmode=log,/pgfplots/ymode=linear,#1]%
}

\def\pgfplots@environment@semilogyaxis{%
	\pgfutil@ifnextchar[{\pgfplots@@environment@semilogyaxis}{\pgfplots@@environment@semilogyaxis[]}%
}
\let\endpgfplots@environment@semilogyaxis=\endpgfplots@environment@opt
\def\pgfplots@@environment@semilogyaxis[#1]{%
	\pgfplots@environment@opt[/pgfplots/xmode=linear,/pgfplots/ymode=log,#1]%
}

\def\pgfplots@environment@loglogaxis{%
	\pgfutil@ifnextchar[{\pgfplots@@environment@loglogaxis}{\pgfplots@@environment@loglogaxis[]}%
}
\let\endpgfplots@environment@loglogaxis=\endpgfplots@environment@opt
\def\pgfplots@@environment@loglogaxis[#1]{%
	\pgfplots@environment@opt[/pgfplots/xmode=log,/pgfplots/ymode=log,#1]%
}


\pgfutil@ifundefined{tikzaddtikzonlycommandshortcutlet}{%
	\def\tikzaddtikzonlycommandshortcutlet#1#2{%
		\expandafter\def\expandafter\tikz@installcommands\expandafter{\tikz@installcommands
			\let#1=#2
		}%
	}%
}{}

\tikzaddtikzonlycommandshortcutlet\axis\pgfplots@environment@axis
\tikzaddtikzonlycommandshortcutlet\endaxis\endpgfplots@environment@axis

\tikzaddtikzonlycommandshortcutlet\semilogxaxis\pgfplots@environment@semilogxaxis
\tikzaddtikzonlycommandshortcutlet\endsemilogxaxis\endpgfplots@environment@semilogxaxis

\tikzaddtikzonlycommandshortcutlet\semilogyaxis\pgfplots@environment@semilogyaxis
\tikzaddtikzonlycommandshortcutlet\endsemilogyaxis\endpgfplots@environment@semilogyaxis

\tikzaddtikzonlycommandshortcutlet\loglogaxis\pgfplots@environment@loglogaxis
\tikzaddtikzonlycommandshortcutlet\endloglogaxis\endpgfplots@environment@loglogaxis


==> pgfplots.stackedplots.code.tex <==
%--------------------------------------------
%
% Package pgfplots
%
% Provides a user-friendly interface to create function plots (normal
% plots, semi-logplots and double-logplots).
% 
% It is based on Till Tantau's PGF package.
%
% Copyright 2007/2008 by Christian Feuersänger.
%
% This program is free software: you can redistribute it and/or modify
% it under the terms of the GNU General Public License as published by
% the Free Software Foundation, either version 3 of the License, or
% (at your option) any later version.
% 
% This program is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
% GNU General Public License for more details.
% 
% You should have received a copy of the GNU General Public License
% along with this program.  If not, see <http://www.gnu.org/licenses/>.
%
%--------------------------------------------

%
% This file contains the implementation for stacked plots.
%
% Stacked plots always keep record of the last plotted coordinates.
% Any new plot will be ADDED on top of the last plotted coordinates.
% 
% Terminology: "last plotted coordinates" are called "zero levels"
% because they actually work like shifts.
%
% Programming Structure:
%
% 1. We keep TWO lists of coordinates: a list of CURRENT zero level
% coordinates and a list of NEXT zero level coordinates.
%
% The first one will be queried whenever a zero level coordinate is
% requested.
%
% The second one will be used to form zero levels for the next plot.
%
% 2. At the beginning and end of each plot, the lists in 1.) are
% initialised properly.
%
% 3. While plot coordinates are processed, the following methods
% interact with the stacked API:
% \pgfplots@stacked@preparepoint@inmacro
% 	-> compute the 'stacked' sum.
% 	This may need to be done with floating point arithmetics because
% 	the data scaling trafo is not yet initialised
%
% \pgfplots@stacked@finishpoint
% 	-> takes coordinates as they will be given to Tikz. This method is
% 	used to 
% 		- communicate zero level coordinates to Tikz
% 		- implement the 'closed paths' option (allows filled stacked plots).
%
% \pgfplots@stacked@rememberzerolevelpoint@for@next@plot
% \pgfplots@stacked@getnextzerolevelpoint
%
% 4. Zero levels are communicated to Tikz by
% \pgfplots@stacked@initzerolevelhandler. This routine initialises an
% input stream for Tikz plot handlers which produces a sequence of
% zero levels. It is used by [xy]comb and [xy]bar.
%
%
% REMARK:
% the state of the boolean \ifpgfplots@datascaletrafo@initialised
% determines whether these routines expect and return floating point
% numbers or fixed point numbers.

\let\pgfplots@stacked@zerolevelpoint@x=\pgfutil@empty
\let\pgfplots@stacked@zerolevelpoint@y=\pgfutil@empty
\newif\ifpgfplots@stacked@isfirstplot
\newif\ifpgfplots@stacked@isinitialised

% Pre-initialisation.
% Needs to be called before the first call to
% \pgfplots@stacked@beginplot.
\def\pgfplots@stacked@initialise{%
	\pgfplots@stacked@isfirstplottrue
	\pgfplots@stacked@isinitialisedtrue
}%

% Cleanup method. Truncates any global variables to reduce string
% space.
\def\pgfplots@stacked@finalize{%
	\global\pgfplotslistnewempty\pgfplots@stacked@zerolevellist
	\global\pgfplotslistnewempty\pgfplots@stacked@nextzerolevellist
	\pgfplots@stacked@isinitialisedfalse
}%

% (Re)defines the macro \pgfplots@stacked@getnextzerolevelpoint
% at the beginning of each plot.
%
% The macro \pgfplots@stacked@getnextzerolevelpoint fills
% \pgfplots@stacked@zerolevelpoint@[xy].
%
% ATTENTION: call \pgfplots@stacked@initialise before the first call
% to beginplot!
\def\pgfplots@stacked@beginplot{%
%\message{pgfplots@stacked@beginplot: PLOT STARTED.}%
	\ifpgfplots@stacked@isinitialised
	\else
		\pgfplots@error{LOGIC ERROR: please call \string\pgfplots@stacked@initialise.}%
	\fi
	\global\pgfplotslistnewempty\pgfplots@stacked@PGFzerolevels
	% accumulate this command here for \closedcycle:
	\let\pgfplots@stacked@closedcycle@impl=\pgfutil@empty
	\ifpgfplots@stacked@isfirstplot
		\global\pgfplotslistnewempty\pgfplots@stacked@zerolevellist
		\def\pgfplots@stacked@zerolevelpoint@x{0}%
		\def\pgfplots@stacked@zerolevelpoint@y{0}%
		% only work with float if its really necessary - for
		% example if the scaling trafo which maps to pgfmath is
		% not yet initialised.
		\ifpgfplots@datascaletrafo@initialised
		\else
			\ifpgfplots@xislinear
				\pgfmathfloatcreate{0}{0.0}{0}%
				\let\pgfplots@stacked@zerolevelpoint@x=\pgfmathresult
			\fi
			\ifpgfplots@yislinear
				\pgfmathfloatcreate{0}{0.0}{0}%
				\let\pgfplots@stacked@zerolevelpoint@y=\pgfmathresult
			\fi
		\fi
		\def\pgfplots@stacked@getnextzerolevelpoint{}% will remain constant anyway.
	\else
		{\globaldefs=1
		\pgfplotslistcopy\pgfplots@stacked@nextzerolevellist\to\pgfplots@stacked@zerolevellist
		}%
		\def\pgfplots@stacked@getnextzerolevelpoint{%
			{\globaldefs=1
			\pgfplotslistpopfront\pgfplots@stacked@zerolevellist\to\pgfmathresult
			}%
			\expandafter\pgfplots@stacked@parsezerolevelpoint\pgfmathresult
		}%
	\fi
	\global\pgfplotslistnewempty\pgfplots@stacked@nextzerolevellist
}%

\def\pgfplots@stacked@parsezerolevelpoint(#1,#2){%
	\def\pgfplots@stacked@zerolevelpoint@x{#1}%
	\def\pgfplots@stacked@zerolevelpoint@y{#2}%
}

\def\pgfplots@stacked@endplot{%
	\ifpgfplots@stacked@isfirstplot
		\let\pgfplots@stacked@closedcycle@impl=\pgfplots@path@closed@cycle@std
	\else
		\t@pgfplots@tokc=\expandafter{\pgfplots@stacked@closedcycle@impl}%
		\edef\pgfplots@stacked@closedcycle@impl{%
			[mark=none,/utils/exec=\noexpand\pgfplots@try@mirror@plot@handler]
			--plot coordinates{\the\t@pgfplots@tokc}
			--cycle
		}%
	\fi
	\global\pgfplots@stacked@isfirstplotfalse
%\message{pgfplots@stacked@endplot: PLOT ENDED}%
}%

% WARNING: when this method is called, NEITHER
% \ifpgfplots@stacked@isfirstplot NOR the zero level lists are
% initialised!
\def\pgfplots@stacked@initzerolevelhandler{%
	\ifpgfplots@stacked@x
		\pgfplotxzerolevelstream@@list
		\pgfplotyzerolevelstreamconstant{\pgfplots@ZERO@y}%
	\else
		\pgfplotxzerolevelstreamconstant{\pgfplots@ZERO@x}%
		\pgfplotyzerolevelstream@@list
	\fi
}%

\def\pgfplots@stacked@rememberzerolevelpoint@for@next@plot#1{%
	\edef\pgfplots@loc@TMPa{#1}%
	\expandafter\pgfplotslistpushbackglobal\pgfplots@loc@TMPa\to\pgfplots@stacked@nextzerolevellist
}

\def\pgfplots@stacked@finishpoint#1#2{%
	\ifpgfplots@stacked@isfirstplot
	\else
		\pgfpointxy{\pgfplots@stacked@zerolevelpoint@x}{\pgfplots@stacked@zerolevelpoint@y}%
		\ifpgfplots@stacked@x
			\edef\pgfplots@loc@TMPa{\the\pgf@x}%
		\else
			\edef\pgfplots@loc@TMPa{\the\pgf@y}%
		\fi
		\expandafter\pgfplotslistpushbackglobal\pgfplots@loc@TMPa\to\pgfplots@stacked@PGFzerolevels
		\t@pgfplots@toka=\expandafter{\pgfplots@stacked@closedcycle@impl}%
		\edef\pgfplots@stacked@closedcycle@impl{%
			(\pgfplots@stacked@zerolevelpoint@x,\pgfplots@stacked@zerolevelpoint@y)%
			\the\t@pgfplots@toka}%
	\fi
}%

\def\pgfplots@stacked@preparepoint@inmacro#1#2{%
	\pgfplots@stacked@getnextzerolevelpoint
	\ifpgfplots@stacked@x
		\ifpgfplots@stacked@plus
			\let\pgfplots@stacked@op=\pgfmathadd@
		\else
			\let\pgfplots@stacked@op=\pgfmathsubtract@
		\fi
		\ifpgfplots@xislinear
			\ifpgfplots@datascaletrafo@initialised
			\else
				\ifpgfplots@stacked@plus
					\let\pgfplots@stacked@op=\pgfmathfloatadd@
				\else
					\let\pgfplots@stacked@op=\pgfmathfloatsubtract@
				\fi
			\fi
		\fi
		\pgfplots@stacked@op{\pgfplots@stacked@zerolevelpoint@x}{#1}%
		\let#1=\pgfmathresult
	\else
		\ifpgfplots@stacked@plus
			\let\pgfplots@stacked@op=\pgfmathadd@
		\else
			\let\pgfplots@stacked@op=\pgfmathsubtract@
		\fi
		\ifpgfplots@yislinear
			\ifpgfplots@datascaletrafo@initialised
			\else
				\ifpgfplots@stacked@plus
					\let\pgfplots@stacked@op=\pgfmathfloatadd@
				\else
					\let\pgfplots@stacked@op=\pgfmathfloatsubtract@
				\fi
			\fi
		\fi
		\pgfplots@stacked@op{\pgfplots@stacked@zerolevelpoint@y}{#2}%
		\let#2=\pgfmathresult
	\fi
	\pgfplots@stacked@rememberzerolevelpoint@for@next@plot{(#1,#2)}%
}

% This here is a re-implementation of the stored plot processing.
%
% The idea is simple, although it requires quite some work:
%
% If we stack plots on top of each other, early drawing commands
% (early plots) will be OVERDRAWN by later drawing commands (later
% plots). This is especially unfortunate if we use filled bar plots
% or comb plots.
%
% IDEA: draw plots in REVERSE order. The positioning, styles and
% whatever must not be affected, only the sequence of drawing commands
% shall change.
%
% So, this command here does all numerics which is to be done and
% assembles a NEW, REVERSED STORED PLOT LIST.
\def\pgfplots@stacked@finalize@stored@plots{%
	\pgfplotslistnewempty\pgfplots@stored@plotlist@reversed
	\begingroup
	\pgfplotslistforeachungrouped\pgfplots@stored@plotlist\as\pgfplots@loc@TMPa{%
		\expandafter\pgfplots@stored@plotlist@EXTRACTENTRY\pgfplots@loc@TMPa
		\ifx\pgfplots@stored@current@cmd\pgfutil@empty
		\else
			% Apply the data scaling transformation and compute
			% stacked coordinates, but do NOT
			% issue any drawing commands:
			\expandafter\pgfplots@stacked@finalize@stored@coords@START\pgfplots@stored@current@data
				\to
				{\pgfplots@stored@current@data}%
				{\pgfplots@stored@current@precmdappend}%
			% store preparation commands into "precmd":
			\t@pgfplots@tokb=\expandafter{\pgfplots@stored@current@precmd}%
			\t@pgfplots@toka=\expandafter{\pgfplots@stored@current@precmdappend}%
			\edef\pgfplots@stored@current@precmd{\the\t@pgfplots@tokb\the\t@pgfplots@toka}%
		\fi
		% Now, we need to insert all stored entities into the new,
		% reversed list. We only expand them ONCE.
		\t@pgfplots@toka=\expandafter{\pgfplots@stored@current@precmd}%
		\t@pgfplots@tokb=\expandafter{\pgfplots@stored@current@cmd}%
		\edef\pgfplots@loc@TMPa{%
			{\the\t@pgfplots@toka}{\the\t@pgfplots@tokb}}%
		\t@pgfplots@tokc=\expandafter{\pgfplots@loc@TMPa}%
		\t@pgfplots@toka=\expandafter{\pgfplots@stored@current@data}%
		\t@pgfplots@tokb=\expandafter{\pgfplots@stored@current@postcmd}%
		\edef\pgfplots@loc@TMPa{%
			\the\t@pgfplots@tokc
			{\the\t@pgfplots@toka}{\the\t@pgfplots@tokb}}%
		% Reverse sequence:
		\expandafter\pgfplotslistpushfront\pgfplots@loc@TMPa\to\pgfplots@stored@plotlist@reversed
	}%
	% Now, overwrite the original list:
	\global\let\pgfplots@stored@plotlist=\pgfplots@stored@plotlist@reversed
	\global\let\pgfplots@stored@plotlist@reversed=\relax
	\endgroup
}%

% This command finalizes the stored plot data. It records a coordinate
% stream into '#3' and assembles a macro '#4' which contains all
% preparation commands to ensure the functionality of
% \pgfplots@stacked@finalize@stored@plots
%
% Instead, it generates a macro #4 which - if used as "precommand"
% befor a draw operation - restores all required options and performs
% pre-drawing.
\long\def\pgfplots@stacked@finalize@stored@coords@START plot coordinates #1#2;\to#3#4{%
	\pgfplots@stacked@beginplot
	\pgfplots@coord@stream@INIT@finalize@stackedcoords@recordto{#3}{\pgfplots@recorded@marker@stream}%
	\pgfplots@coord@stream@foreach{#1}%
	\pgfplots@stacked@endplot
	\pgfplots@stacked@savestateto\pgfplots@loc@TMPa
	\t@pgfplots@toka=\expandafter{\pgfplots@loc@TMPa\def\pgfplots@stacked@stored@postpath{#2}}%
	\pgfplots@addplot@get@named@startendpoints@command\pgfplots@loc@TMPa
	\t@pgfplots@tokc=\expandafter{\pgfplots@loc@TMPa}%
	\ifpgfplots@record@marker@stream
		\t@pgfplots@tokb=\expandafter{\pgfplots@recorded@marker@stream}%
	\else
		\t@pgfplots@tokb={}%
	\fi
	\edef#4{%
		\the\t@pgfplots@tokc
		\noexpand\gdef\noexpand\pgfplots@recorded@marker@stream{\the\t@pgfplots@tokb}%
		\the\t@pgfplots@toka
	}%
}%

% #1: for coordinates
% #2: for markers
\def\pgfplots@coord@stream@INIT@finalize@stackedcoords@recordto#1#2{%
	\pgfplots@record@marker@streamtrue
	%
	\def\pgfplots@coord@stream@start@{%
		\gdef#1{\pgfplotstreamstart}%
		\ifpgfplots@record@marker@stream
			\pgfplotsapplistXnewempty\pgfplots@stacked@record@mark@cmds
			\pgfplotsapplistXpushback\pgfplotstreamstart\to\pgfplots@stacked@record@mark@cmds
		\fi
	}%
	\def\pgfplots@coord@stream@end@{%
		\expandafter\gdef\expandafter#1\expandafter{#1\pgfplotstreamend}%
		\ifpgfplots@record@marker@stream
			\pgfplotsapplistXpushback\pgfplotstreamend\to\pgfplots@stacked@record@mark@cmds
			\pgfplotsapplistXlet\pgfplots@loc@TMPa=\pgfplots@stacked@record@mark@cmds
			\global\let#2=\pgfplots@loc@TMPa
		\fi
	}%
	\ifpgfplots@apply@datatrafo
		\def\pgfplots@coord@stream@coord@##1##2##3##4{%
			\pgfplots@apply@data@scaletrafo@to@one@point{##1}{##2}{##3}{##4}%
			\pgfplots@coord@stream@finalize@currentpt
		}%
	\else
		\def\pgfplots@coord@stream@coord@##1##2##3##4{%
			\def\pgfplots@current@point@x{##1}%
			\def\pgfplots@current@point@y{##2}%
			\pgfplots@coord@stream@finalize@currentpt
		}%
	\fi
	\def\pgfplots@coord@stream@finalize@currentpt{%
		\pgfqpointxy{\pgfplots@current@point@x}{\pgfplots@current@point@y}%
		\edef\pgfmathresult{{\the\pgf@x}{\the\pgf@y}}%
		\t@pgfplots@toka=\expandafter{#1}%
		\t@pgfplots@tokb=\expandafter{\pgfmathresult}%
		\xdef#1{\the\t@pgfplots@toka
			\noexpand\pgfplots@stream\the\t@pgfplots@tokb}%
		%
		\ifpgfplots@record@marker@stream
			\ifdim\pgf@x<\pgfplots@xcoordminTEX
			\else
				\ifdim\pgf@x>\pgfplots@xcoordmaxTEX
				\else
					\ifdim\pgf@y<\pgfplots@ycoordminTEX
					\else
						\ifdim\pgf@y>\pgfplots@ycoordmaxTEX
						\else
							\edef\pgfmathresult{\noexpand\pgfplots@stream{\the\pgf@x}{\the\pgf@y}}%
							\expandafter\pgfplotsapplistXpushback\expandafter{\pgfmathresult}\to\pgfplots@stacked@record@mark@cmds%
						\fi
					\fi
				\fi
			\fi
		\fi
	}%
}

% This command gets called after the sequence reversal has been done.
% It unpacks everything prepared by 
% \pgfplots@stacked@finalize@stored@coords@START
% and draws the plot (and markers).
\def\pgfplots@stacked@draw@reversed@plot{%
	\pgfplots@stored@current@cmd[current plot style]
	\pgfextra
		\tikzset{every plot/.try}%
		\pgfplots@getcurrent@plothandler\pgfplots@basiclevel@plothandler
		\pgfplots@basiclevel@plothandler
		% this here contains a recorded plot stream, see above. 
		\pgfplots@stored@current@data
		%
		\pgfplots@assert@tikzinternal@exists{tikz@make@last@position}%
		\tikz@make@last@position{\pgfplotlastpoint}%  
	\expandafter
	\endpgfextra
	\pgfplots@stacked@stored@postpath
	;
	% this here has been assigned by the precommand as well.
	\ifx\pgfplots@recorded@marker@stream\pgfutil@empty
	\else
		\ifpgfplots@clip@marker@paths
			\pgfplots@stored@current@cmd[current plot style]
			\pgfextra 
				\pgfplots@install@plotmark@handler
				\pgfplots@recorded@marker@stream 
			\endpgfextra
			;
		\else
			\pgfplots@stored@REMEMBER@MARK@COMMAND
		\fi
	\fi
	\gdef\pgfplots@recorded@marker@stream{}% clear
}%


\def\pgfplots@stacked@path@closed@cycle{%
	\pgfplots@stacked@closedcycle@impl
}

% Saves the finalized variables into macro #1 such that a call to #1
% restores them.
%
% This affects pgf zero level handlers and whether this here is the
% first plot or not..
\def\pgfplots@stacked@savestateto#1{%
	\t@pgfplots@toka=\expandafter{\pgfplots@stacked@PGFzerolevels}%
	\ifpgfplots@stacked@isfirstplot
		\t@pgfplots@tokb={\pgfplots@stacked@isfirstplottrue}%
	\else
		\t@pgfplots@tokb={\pgfplots@stacked@isfirstplotfalse}%
	\fi
	\t@pgfplots@tokc=\expandafter{\pgfplots@stacked@closedcycle@impl}%
	\edef#1{%
		\noexpand\gdef\noexpand\pgfplots@stacked@PGFzerolevels{\the\t@pgfplots@toka}%
		\the\t@pgfplots@tokb
		\noexpand\def\noexpand\pgfplots@stacked@closedcycle@impl{\the\t@pgfplots@tokc}%
	}%
}

% PGF interfaces:
\def\pgfplotxzerolevelstream@@list{%
	\def\pgf@plotxzerolevelstreamstart{%
		\global\let\pgfplotxzerolevelstream@@list@@backup=\pgfplots@stacked@PGFzerolevels
		\gdef\pgf@plotxzerolevelstreamnext{%
			\pgfplotslistcheckempty\pgfplots@stacked@PGFzerolevels
			\ifpgfplotslistempty
				\global\pgf@x=\pgfplots@ZERO@x\relax
			\else
				{\globaldefs=1\relax
				\pgfplotslistpopfront\pgfplots@stacked@PGFzerolevels\to\pgfmathresult
				}%
				\global\pgf@x=\pgfmathresult\relax
			\fi
		}%
	}%
	\def\pgf@plotxzerolevelstreamend{%
		\global\let\pgfplots@stacked@PGFzerolevels=\pgfplotxzerolevelstream@@list@@backup
	}%
}%

\def\pgfplotyzerolevelstream@@list{%
	\def\pgf@plotyzerolevelstreamstart{%
		\global\let\pgfplotyzerolevelstream@@list@@backup=\pgfplots@stacked@PGFzerolevels
		\gdef\pgf@plotyzerolevelstreamnext{%
			\pgfplotslistcheckempty\pgfplots@stacked@PGFzerolevels
			\ifpgfplotslistempty
				\global\pgf@x=\pgfplots@ZERO@y\relax
			\else
				{\globaldefs=1\relax
				\pgfplotslistpopfront\pgfplots@stacked@PGFzerolevels\to\pgfmathresult
				}%
				\global\pgf@x=\pgfmathresult\relax
			\fi
		}%
	}%
	\def\pgf@plotyzerolevelstreamend{%
		\global\let\pgfplots@stacked@PGFzerolevels=\pgfplotyzerolevelstream@@list@@backup
	}%
}%


==> pgfplotsarray.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% This is a helper package with an elementary array datastructure,
% featuring O(1) index access and O(N) creation, deletion, copy.
%
% The following macros are supplied:
%
% \pgfplotsarraynewempty
% \pgfplotsarraynew
% \pgfplotsarraycopy
% \pgfplotsarraypushback
% \pgfplotsarraysize
% \pgfplotsarrayselect
% \pgfplotsarrayletentry
% \pgfplotsarraycheckempty
% \pgfplotsarrayforeach
%
% Copyright 2007/2008 by Christian Feuersänger.
%
% This program is free software: you can redistribute it and/or modify
% it under the terms of the GNU General Public License as published by
% the Free Software Foundation, either version 3 of the License, or
% (at your option) any later version.
% 
% This program is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
% GNU General Public License for more details.
% 
% You should have received a copy of the GNU General Public License
% along with this program.  If not, see <http://www.gnu.org/licenses/>.
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcount\c@pgfplotsarray@tmp
\newif\ifpgfplotsarrayempty

% Creates a new, empty array.
\long\def\pgfplotsarraynewempty#1{%
	\pgfplotsarray@@def{#1@size}{0}%
}

% Creates a new array with an abirtrary number of elements.
% Arguments:
% #1: the array's name (a macro name)
% #2: the elements in the form 
%     first\\second\\third\\ ...\\
%     like in tabular with one column.
%
% Example:
% \pgfplotsarraynew\fooarray{First Element\\Second Element\\Third Element\\}
%
% WARNING: do NOT forget the final '\\'!
\long\def\pgfplotsarraynew#1#2{%
	\pgfplotsarraynewempty{#1}%
	\long\def\pgfplotsarraynew@impl@rest{#2}%
	\pgfutil@loop
	\ifx\pgfplotsarraynew@impl@rest\pgfutil@empty
		\pgfplots@loop@CONTINUEfalse
	\else
		\pgfplots@loop@CONTINUEtrue
	\fi
	\ifpgfplots@loop@CONTINUE
		\expandafter\pgfplotsarraynew@impl\pgfplotsarraynew@impl@rest\toarray#1\relax
	\pgfutil@repeat
}

% helper macro for \pgfplotsarraynew
\long\def\pgfplotsarraynew@impl#1\\#2\toarray#3{%
	\pgfplotsarraypushback#1\to#3\relax%
	\def\pgfplotsarraynew@impl@rest{#2}%
}


\def\pgfplotsarray@@let#1=#2{%
	\def\pgfplotsarray@TMP@@{\expandafter\let\csname\string#1\endcsname}%
	\expandafter\pgfplotsarray@TMP@@\expandafter=\csname\string#2\endcsname
}%

\def\pgfplotsarray@@def#1{%
	\expandafter\def\csname\string#1\endcsname
}%
\def\pgfplotsarray@@edef#1{%
	\expandafter\edef\csname\string#1\endcsname
}%

\def\pgfplotsarray@@getsizeto#1#2{%
	\pgfplotsarraysize{#1}\to\c@pgfplotsarray@tmp
	\edef#2{\the\c@pgfplotsarray@tmp}%
}%

% Copies array #1 to array #2.
\def\pgfplotsarraycopy#1\to#2{%
	\pgfplotsarray@@let{#2@size}={#1@size}%
	\pgfplotsarray@@getsizeto{#1}{\pgfplotsarray@TMP}%
	\c@pgfplotsarray@tmp=0
	\pgfutil@loop
	\ifnum\c@pgfplotsarray@tmp<\pgfplotsarray@TMP
	\pgfplotsarray@@let{#2@\the\c@pgfplotsarray@tmp}={#1@\the\c@pgfplotsarray@tmp}%
	\advance\c@pgfplotsarray@tmp by1
	\pgfutil@repeat
}



% #1: the item to append
% #2: the array as macro name
% Example:
% \pgfplotsarraypushback Next last element\to\fooarray
\long\def\pgfplotsarraypushback#1\to#2{%
	\pgfplotsarraysize{#2}\to\c@pgfplotsarray@tmp
	\pgfplotsarray@@def{#2@\the\c@pgfplotsarray@tmp}{#1}%
	\advance\c@pgfplotsarray@tmp by1
	\pgfplotsarray@@edef{#2@size}{\the\c@pgfplotsarray@tmp}%
}


% Counts the number of elements in array #1, storing it into the count
% register #2.
% Example:
% \pgfplotsarraysize\foo\to{\count0}%
% \the\count0
\long\def\pgfplotsarraysize#1\to#2{%
	#2=\csname\string#1@size\endcsname\relax
}

% Returns the #1th element of array #2 into macro #3
% Arguments:
% #1: a count 0,...,N-1 where N is the array size.
%     You may specify a number of a count.
% #2: a array
% #3: a macro name
% Example:
%   Element 0:
%   \pgfplotsarrayselect0\of\foo\to\elem
%   \elem
%   Element \count1:
%   \pgfplotsarrayselect\count1\of\foo\to\elem
\long\def\pgfplotsarrayselect#1\of#2\to#3{%
	\c@pgfplotsarray@tmp=#1\relax
	\expandafter\let\expandafter#3\expandafter=\csname\string#2@\the\c@pgfplotsarray@tmp\endcsname%
}
\long\def\pgfplotsarrayletentry#1\of#2=#3{%
	\c@pgfplotsarray@tmp=#1\relax
	\expandafter\let\csname\string#2@\the\c@pgfplotsarray@tmp\endcsname=#3\relax
}

% Sets the boolean \ifpgfplotsarrayempty depending on whether array #1 is empty
% or not.
% Example:
%
% \pgfplotsarraycheckempty\fooarray
% \ifpgfplotsarrayempty
%    List fooarray is empty!
% \else
%    List is not empty.
% \fi
\def\pgfplotsarraycheckempty#1{%
	\pgfplotsarraysize{#1}\to\c@pgfplotsarray@tmp
	\ifnum\c@pgfplotsarray@tmp=0\relax
		\pgfplotsarrayemptytrue
	\else
		\pgfplotsarrayemptyfalse
	\fi
}


% Iterates through each array element, names it #2 and calls code #3.
% Example:
% \pgfplotsarraynew\fooarray{Eins\\Zwei\\Drei\\}%
% \pgfplotsarrayforeach\fooarray\as\foo{Element \foo\par}%
% results in
%  Element Eins
%  Element Zwei
%  Element Drei
% Each single element will be grouped with TeX groups.
\long\def\pgfplotsarrayforeach#1\as#2#3{%
	\pgfplotsarray@@getsizeto{#1}{\pgfplotsarray@TMP}%
	\c@pgfplotsarray@tmp=0\relax
	\pgfutil@loop
	\ifnum\c@pgfplotsarray@tmp<\pgfplotsarray@TMP\relax
	\begingroup
	\expandafter\let\expandafter#2\expandafter=\csname\string#1@\the\c@pgfplotsarray@tmp\endcsname%
	#3%
	\endgroup
	\advance\c@pgfplotsarray@tmp by1
	\pgfutil@repeat
}

% The same but without groups around #3.
\long\def\pgfplotsarrayforeachungrouped#1\as#2#3{%
	\pgfplotsarray@@getsizeto{#1}{\pgfplotsarray@TMP}%
	\c@pgfplotsarray@tmp=0\relax
	\pgfutil@loop
	\ifnum\c@pgfplotsarray@tmp<\pgfplotsarray@TMP\relax
	\expandafter\let\expandafter#2\expandafter=\csname\string#1@\the\c@pgfplotsarray@tmp\endcsname%
	#3%
	\advance\c@pgfplotsarray@tmp by1
	\pgfutil@repeat
}


==> pgfplotsliststructure.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% This is a helper package with an elementary list datastructure.
%
% Its implementation is based on Knuth's list macros in "The TeXbook".
%
% It features a convenient set of list macros, but it is not fast.
% In fact, every elementary operation requires time O(N), so working 
% with this list easily leads to O(N^2) runtime.
%
% The following macros are supplied:
%
% \pgfplotslistnewempty
% \pgfplotslistnew
% \pgfplotslistcopy
% \pgfplotslistpopfront
% \pgfplotslistfront
% \pgfplotslistpushback
% \pgfplotslistpushfront
% \pgfplotslistsize
% \pgfplotslistselect
% \pgfplotslistcheckempty
% \pgfplotslistforeach
%
% @see \pgfplotsapplist a "real" list with O(1) pushback, but limited application.
% @see \pgfplotsapplistX a preasymptotical fast list to accumulate elements.
% @see \pgfplotsapplistXX an optimized version of \pgfplotsapplistX.
%
% Copyright 2007/2008 by Christian Feuersänger.
%
% This program is free software: you can redistribute it and/or modify
% it under the terms of the GNU General Public License as published by
% the Free Software Foundation, either version 3 of the License, or
% (at your option) any later version.
% 
% This program is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
% GNU General Public License for more details.
% 
% You should have received a copy of the GNU General Public License
% along with this program.  If not, see <http://www.gnu.org/licenses/>.
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newif\ifpgfplotslistempty


\newif\ifpgfplots@loop@CONTINUE
\newif\ifpgfplotslist@is@backslash@terminated

% Creates a new, empty list.
\long\def\pgfplotslistnewempty#1{\let#1=\pgfutil@empty}

% Creates a new list with an abirtrary number of elements.
% Arguments:
% #1: the list's name (a macro name)
% #2: the elements in the form 
%     first\\second\\third\\ ...\\
%     like in tabular with one column.
%     You can also use comma-separated lists
%     first,second,third
%
% Example:
% 1.
%  \pgfplotslistnew\foolist{First Element\\Second Element\\Third Element\\}
%   WARNING: do NOT forget the final '\\'!
%
% 2.
% \pgfplotslistnew\foolist{First Element,Second Element,Third Element}
%
% Use braces '{}' to use '\\' or ',' as arguments.
%
\long\def\pgfplotslistnew#1#2{%
	\pgfplotslistnewempty{#1}%
	\long\def\pgfplotslistnew@impl@rest{#2}%
	\pgfplotslist@check@backslash@list #2\\\pgfplotslist@EOI
	\ifpgfplotslist@is@backslash@terminated
	\else
		\expandafter\def\expandafter\pgfplotslistnew@impl@rest\expandafter{\pgfplotslistnew@impl@rest,}%
	\fi
	\pgfutil@loop
	\ifx\pgfplotslistnew@impl@rest\pgfutil@empty
		\pgfplots@loop@CONTINUEfalse
	\else
		\pgfplots@loop@CONTINUEtrue
	\fi
	\ifpgfplots@loop@CONTINUE
		\ifpgfplotslist@is@backslash@terminated
			\expandafter\pgfplotslistnew@impl\pgfplotslistnew@impl@rest\tolist#1\relax
		\else
			\expandafter\pgfplotslistnew@impl@comma\pgfplotslistnew@impl@rest\tolist#1\relax
		\fi
	\pgfutil@repeat
}
\def\pgfplotslist@EOI{\pgfplotslist@EOI}

\def\pgfplotslist@check@backslash@list#1\\#2\pgfplotslist@EOI{%
	\def\pgfplotslist@loc@TMPa{#2}%
	\ifx\pgfplotslist@loc@TMPa\pgfutil@empty
		\pgfplotslist@is@backslash@terminatedfalse
	\else
		\pgfplotslist@is@backslash@terminatedtrue
	\fi
}%

% Copies list #1 to list #2.
\def\pgfplotslistcopy#1\to#2{\let#2=#1}


% helper macro for \pgfplotslistnew
\long\def\pgfplotslistnew@impl#1\\#2\tolist#3{%
	\pgfplotslistpushback#1\to#3\relax%
	\def\pgfplotslistnew@impl@rest{#2}%
}
\long\def\pgfplotslistnew@impl@comma#1,#2\tolist#3{%
	\pgfplotslistpushback#1\to#3\relax%
	\def\pgfplotslistnew@impl@rest{#2}%
}


% #1: the item to prepend
% #2: the list as macro name
% Example:
% \pgfplotslistpushfront Next first Element\to\foolist
\long\def\pgfplotslistpushfront#1\to#2{%
	\t@pgfplots@toka={\pgfpl@@{#1}}%
	\t@pgfplots@tokb=\expandafter{#2}%
  	\edef#2{\the\t@pgfplots@toka\the\t@pgfplots@tokb}%
}

% Assembles a low-level list item representation into the token
% register #2.
\def\pgfplotslist@assembleentry#1\into#2{%
	#2={\pgfpl@@{#1}}%
}

% #1: the item to append
% #2: the list as macro name
% Example:
% \pgfplotslistpushback Next last element\to\foolist
\long\def\pgfplotslistpushback#1\to#2{%
	\t@pgfplots@toka={\pgfpl@@{#1}}%
	\ifx#2\pgfutil@empty
		\t@pgfplots@tokb={}%
	\else
		\t@pgfplots@tokb=\expandafter{#2}%
	\fi
 	\edef#2{\the\t@pgfplots@tokb\the\t@pgfplots@toka}%
}
% Adds '#1' to the GLOBAL list '#2'.
\long\def\pgfplotslistpushbackglobal#1\to#2{%
	\t@pgfplots@toka={\pgfpl@@{#1}}%
	\ifx#2\pgfutil@empty
		\t@pgfplots@tokb={}%
	\else
		\t@pgfplots@tokb=\expandafter{#2}%
	\fi
 	\xdef#2{\the\t@pgfplots@tokb\the\t@pgfplots@toka}%
}

% Concatenates two lists #2 and #3 into #1
% Example:
% \pgfplotslistconcat\result=\foolist&\bar
\long\def\pgfplotslistconcat#1=#2&#3{%
	\t@pgfplots@toka=\expandafter{#2}%
	\t@pgfplots@tokb=\expandafter{#3}%
	\edef#1{\the\t@pgfplots@toka\the\t@pgfplots@tokb}%
}

% implements #2 := pop_front(#1)
% Example:
% \pgfplotslistpopfront\foolist\to\poppedfirstelem
\long\def\pgfplotslistpopfront#1\to#2{%
	\pgfplotslistcheckempty#1\relax
	\ifpgfplotslistempty
		\pgfplots@error{ERROR: \string\pgfplotslistpopfront\ from \string#1\ although list is EMPTY}%
		\let#2=\pgfutil@empty
	\else
		\expandafter\pgfplotslistpopfront@impl#1\pgfplotslistpopfront@macronames#1#2%
	\fi
}
\long\def\pgfplotslistfront#1\to#2{%
	\pgfplotslistcheckempty#1\relax
	\ifpgfplotslistempty
		\pgfplots@error{ERROR: \string\pgfplotslistfront\ from \string#1\ although list is EMPTY}%
		\let#2=\pgfutil@empty
	\else
		\expandafter\pgfplotslistfront@impl#1\pgfplotslistpopfront@macronames#2%
	\fi
}

% implementation helper for listpopfront
\long\def\pgfplotslistpopfront@impl\pgfpl@@#1#2\pgfplotslistpopfront@macronames#3#4{%
	\def#4{#1}%
	\def#3{#2}%
}
\long\def\pgfplotslistfront@impl\pgfpl@@#1#2\pgfplotslistpopfront@macronames#3{%
	\def#3{#1}%
}

% Counts the number of elements in list #1, storing it into the count
% register #2.
% Example:
% \pgfplotslistsize\foo\to{\count0}%
% \the\count0
\long\def\pgfplotslistsize#1\to#2{%
	#2=0%
	\long\def\pgfpl@@##1{\advance#2 by 1 }%
	#1%
}

% Returns the #1th element of list #2 into macro #3
% Arguments:
% #1: a count 0,...,N-1 where N is the list size.
%     You may specify a number of a count.
% #2: a list
% #3: a macro name
% Example:
%   Element 0:
%   \pgfplotslistselect0\of\foo\to\elem
%   \elem
%   Element \count1:
%   \pgfplotslistselect\count1\of\foo\to\elem
\def\pgfplotslistselect#1\of#2\to#3{%
	\global\def\pgfplotslistselect@tmp{\def#3{}\pgfplots@error{The requested list entry with index #1 of \string#2 is too large; this list has not enough elements.}}%
	\pgfplotslistselect@{#1}\of{#2}\to{#3}%
}
\def\pgfplotslistselect@#1\of#2\to#3{%
	\begingroup
	\count0=#1\relax
 	\long\def\pgfpl@@##1{%
		\advance\count0 by-1\relax
		\ifnum\count0=-1\relax
			\global\def\pgfplotslistselect@tmp{\def#3{##1}}%
		\fi%
	}%
	#2%
	\endgroup
	\pgfplotslistselect@tmp
}
\def\pgfplotslistselectorempty#1\of#2\to#3{%
	\global\def\pgfplotslistselect@tmp{\def#3{}}%
	\pgfplotslistselect@{#1}\of{#2}\to{#3}%
}

% Sets the boolean \ifpgfplotslistempty depending on whether list #1 is empty
% or not.
% Example:
%
% \pgfplotslistcheckempty\foolist
% \ifpgfplotslistempty
%    List foolist is empty!
% \else
%    List is not empty.
% \fi
\def\pgfplotslistcheckempty#1{%
	\ifx#1\pgfutil@empty
		\pgfplotslistemptytrue
	\else
		\ifx#1\relax
			\pgfplots@warning{WARNING: possible logic error in script code: the command \string\pgfplotslistcheckempty{\string#1} encountered an undefined argument.}%
			\pgfplotslistemptytrue
		\else
			\pgfplotslistemptyfalse
		\fi
	\fi
}


% Iterates through each list element, names it #2 and calls code #3.
% Example:
% \pgfplotslistnew\foolist{Eins\\Zwei\\Drei\\}%
% \pgfplotslistforeach\foolist\as\foo{Element \foo\par}%
% results in
%  Element Eins
%  Element Zwei
%  Element Drei
% Each single element will be grouped with TeX groups.
\long\def\pgfplotslistforeach#1\as#2#3{%
	\begingroup
	\long\def\pgfpl@@##1{\def#2{##1}%
		\begingroup
		#3
		\endgroup}%
	#1\relax
	\endgroup
}

\newif\ifpgfplotslistforeachungroupedrunning

% The same but without groups around #3.
\long\def\pgfplotslistforeachungrouped#1\as#2#3{%
	\ifpgfplotslistforeachungroupedrunning
		\pgfplots@error{Sorry, you can't nest pgfplotslistforeachungrouped.}%
	\else
		\pgfplotslistforeachungroupedrunningtrue
		\long\def\pgfpl@@##1{\def#2{##1}#3}%
		#1\relax
		\pgfplotslistforeachungroupedrunningfalse
	\fi
}


==> pgfplotsliststructureext.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% This is a helper package with an elementary list datastructure.
% In contrast to \pgfplotslist, this one features fast append and fast
% copy-to-macro.
%
% The 'pgfplotsapplist' is a list which has ONLY the features
%
%  \pgfplotsapplistnewempty 
%  \pgfplotsapplistpushback O(1)
%  \pgfplotsapplistedefcontenttomacro (N)
%  \pgfplotsapplistxdefcontenttomacro (N)
%
% It has been designed to accumulate macro content in O(N) (in
% contrast to TeX's macro append routines which lead to O(N^2)
% runtime).
%
% Furthermore, there is the 
%
%  \pgfplotsapplistXnewempty 
%  \pgfplotsapplistXpushback
%  \pgfplotsapplistXedefcontenttomacro (N)
%  \pgfplotsapplistXxdefcontenttomacro (N)
%  \pgfplotsapplistXlet (N)
%
% structure which features **preasymptotical** constant runtime for
% pushback. That means, as long as N < 80000, the runtime is linear.
% It is only slightly slower than \pgfplotsapplist, and that only due
% to its generality. It could easily be adopted to be FASTER than
% \pgfplotsapplist.
%
% Credits for \pgfplotsapplist go to Till Tantau: he developped it for
% the PGF kernel.
%
%
% Copyright 2007/2008 by Christian Feuersänger.
%
% This program is free software: you can redistribute it and/or modify
% it under the terms of the GNU General Public License as published by
% the Free Software Foundation, either version 3 of the License, or
% (at your option) any later version.
% 
% This program is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
% GNU General Public License for more details.
% 
% You should have received a copy of the GNU General Public License
% along with this program.  If not, see <http://www.gnu.org/licenses/>.
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% the applist defines one macro for each element, like
% 
% \def\element<i>{<content>\element<i+1>}
% \def\element<i+1>{<content>\element<i+2>}
% \def\element<i+2>{}
%
% The '<i>' value belongs to the private interface and is part of the
% macro name.
%
% It features:
% - real O(1) pushback
% - O(N) edef to macro
% - O(N) execute
% - it requires O(N) different macros.
% - it ***can't*** be copied outside of the current TeX group!
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Time: O(1), number of macros: 3
\def\pgfplotsapplistnewempty#1{%
	\expandafter\def\csname\string#1@endno\endcsname{0}%
	\edef#1{\expandafter\noexpand\csname\string#1@0\endcsname}%
	\expandafter\def\csname\string#1@0\endcsname{}%
}%

% Time: O(1), number of macros per list: about N
% #1: the item to append
% #2: the list as macro name
\def\pgfplotsapplistpushback#1\to#2{%
	\expandafter\let\expandafter\pgfplots@loc@TMPa\csname\string#2@endno\endcsname
	\begingroup
	\c@pgf@counta=\pgfplots@loc@TMPa\relax
	\advance\c@pgf@counta by1
	\xdef\pgfplots@glob@TMPa{\the\c@pgf@counta}%
	\endgroup
	\expandafter\let\csname\string#2@endno\endcsname=\pgfplots@glob@TMPa%
	\t@pgfplots@toka={#1}%
	\t@pgfplots@tokb=\expandafter{\csname\string#2@\pgfplots@glob@TMPa\endcsname}%
	\expandafter\edef\csname\string#2@\pgfplots@loc@TMPa\endcsname{\the\t@pgfplots@toka\the\t@pgfplots@tokb}%
	\expandafter\let\the\t@pgfplots@tokb=\pgfutil@empty
}%
	
% time O(N)
% Expands the complete content of list #1 as-is into the macro #2.
\def\pgfplotsapplistedefcontenttomacro#1\to#2{\edef#2{#1}}
\def\pgfplotsapplistxdefcontenttomacro#1\to#2{\xdef#2{#1}}

% Foreach list element, the stored value will simply be processed by
% TeX. Characters will be printed and commands will be executed.
% time O(N)
\def\pgfplotsapplistexecute#1{#1}%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
% This list here is a general re-implementation of the list used in
% the PGF system layer.
% It employs two collect-buffers to reduce the runtime.
%
% - It has preasymptotical runtime O(N), but is O(N^2) asymptotically.
% - It requires only 5 macros per list.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Usage: 
% \pgfplotsapplistXnewempty\macro
% \pgfplotsapplistXnewempty[to global]\macro
%
% The 'to global' flag will configure the list such that all
% assignments to \macro are global. The list accumulation is
% LOCAL, however: 'to global' is to be used inside of a local
% group such that the final result, when all buffers are flushed,
% is assigned globally.
\def\pgfplotsapplistXnewempty{%
	\pgfutil@ifnextchar[{%
		\pgfplotsapplistXnewempty@opt
	}{%
		\pgfplotsapplistXnewempty@opt[]%
	}%
}

\def\pgfplotsapplistXnewempty@opt@TOGLOBAL{to global}

\def\pgfplotsapplistXnewempty@opt[#1]#2{%
	\def\pgfplots@loc@TMPa{#1}%
	\ifx\pgfplots@loc@TMPa\pgfutil@empty
		\expandafter\let\csname\string#2@let\endcsname=\let%
		\expandafter\let\csname\string#2@edef\endcsname=\edef
	\else
		\ifx\pgfplots@loc@TMPa\pgfplotsapplistXnewempty@opt@TOGLOBAL
			\expandafter\def\csname\string#2@let\endcsname{\global\let}%
			\expandafter\let\csname\string#2@edef\endcsname=\xdef
		\else
			\pgfplots@error{Sorry, the argument '#1' to \string\pgfplotsapplistXnewempty\ is unknown. Accepted is 'to global' or empty.}%
		\fi
	\fi
	\pgfplotsapplistXnewempty@{#2}%
}%

\def\pgfplotsapplistXnewempty@#1{%
	\csname\string#1@let\endcsname#1=\pgfutil@empty
	\expandafter\let\csname\string#1@smallbuf\endcsname=\pgfutil@empty
	\expandafter\let\csname\string#1@bigbuf\endcsname=\pgfutil@empty
	\expandafter\def\csname\string#1@smallbuf@c\endcsname{0}%
	\expandafter\def\csname\string#1@bigbuf@c\endcsname{0}%
}%

% #1: the item to append
% #2: the list as macro name
\def\pgfplotsapplistXpushback#1\to#2{%
	\begingroup
		\c@pgf@counta=\csname\string#2@smallbuf@c\endcsname\relax
		\advance\c@pgf@counta by1
		\xdef\pgfplots@glob@TMPa{\the\c@pgf@counta}%
	\endgroup
	\expandafter\let\csname\string#2@smallbuf@c\endcsname=\pgfplots@glob@TMPa
	\ifnum\csname\string#2@smallbuf@c\endcsname<40
		\t@pgfplots@toka=\expandafter\expandafter\expandafter{\csname\string#2@smallbuf\endcsname#1}%
		\expandafter\edef\csname\string#2@smallbuf\endcsname{\the\t@pgfplots@toka}%
	\else
		\pgfplotsapplistXpushback@smallbufoverfl{#1}{#2}%
	\fi
}%
\def\pgfplotsapplistXpushback@smallbufoverfl#1#2{%
	\begingroup
		\c@pgf@counta=\csname\string#2@bigbuf@c\endcsname\relax
		\advance\c@pgf@counta by1
		\xdef\pgfplots@glob@TMPa{\the\c@pgf@counta}%
	\endgroup
	\expandafter\let\csname\string#2@bigbuf@c\endcsname=\pgfplots@glob@TMPa
	%
	\ifnum\csname\string#2@bigbuf@c\endcsname<30
		\t@pgfplots@toka=\expandafter\expandafter\expandafter{\csname\string#2@bigbuf\endcsname}%
		\t@pgfplots@tokb=\expandafter\expandafter\expandafter{\csname\string#2@smallbuf\endcsname#1}%
		\expandafter\edef\csname\string#2@bigbuf\endcsname{\the\t@pgfplots@toka\the\t@pgfplots@tokb}%
		\expandafter\let\csname\string#2@smallbuf\endcsname=\pgfutil@empty
		\expandafter\def\csname\string#2@smallbuf@c\endcsname{0}%
	\else%
		\t@pgfplots@toka=\expandafter{#2}%
		\t@pgfplots@tokb=\expandafter\expandafter\expandafter{\csname\string#2@bigbuf\endcsname}%
		\t@pgfplots@tokc=\expandafter\expandafter\expandafter{\csname\string#2@smallbuf\endcsname#1}%
		\csname\string#2@edef\endcsname#2{\the\t@pgfplots@toka\the\t@pgfplots@tokb\the\t@pgfplots@tokc}%
		\expandafter\let\csname\string#2@smallbuf\endcsname=\pgfutil@empty
		\expandafter\def\csname\string#2@smallbuf@c\endcsname{0}%
		\expandafter\let\csname\string#2@bigbuf\endcsname=\pgfutil@empty
		\expandafter\def\csname\string#2@bigbuf@c\endcsname{0}%
	\fi%
}%
\def\pgfplotsapplistXflushbuffers#1{%
	\t@pgfplots@toka=\expandafter{#1}%
	\t@pgfplots@tokb=\expandafter\expandafter\expandafter{\csname\string#1@bigbuf\endcsname}%
	\t@pgfplots@tokc=\expandafter\expandafter\expandafter{\csname\string#1@smallbuf\endcsname}%
	\csname\string#1@edef\endcsname#1{\the\t@pgfplots@toka\the\t@pgfplots@tokb\the\t@pgfplots@tokc}%
	\expandafter\let\csname\string#1@smallbuf\endcsname=\pgfutil@empty
	\expandafter\def\csname\string#1@smallbuf@c\endcsname{0}%
	\expandafter\let\csname\string#1@bigbuf\endcsname=\pgfutil@empty
	\expandafter\def\csname\string#1@bigbuf@c\endcsname{0}%
}%

	
% Expands the complete content of list #1 as-is into the macro #2.
\def\pgfplotsapplistXedefcontenttomacro#1\to#2{%
	\pgfplotsapplistXflushbuffers#1%
	\edef#2{#1}}
\def\pgfplotsapplistXxdefcontenttomacro#1\to#2{%
	\pgfplotsapplistXflushbuffers#1%
	\xdef#2{#1}}
\def\pgfplotsapplistXlet#1=#2{%
	\pgfplotsapplistXflushbuffers#2%
	\let#1=#2}

% Foreach list element, the stored value will simply be processed by
% TeX. Characters will be printed and commands will be executed.
\def\pgfplotsapplistXexecute#1{%
	\pgfplotsapplistXflushbuffers#1%
	#1}%






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
% 
% This list \pgfplotsapplistXX here is essentially the SAME as \pgfplotslistX.
%
% But there can only be one such list at a time, so it is faster than
% \pgfplotslistX.
%
% This here is probably the fastest list.
%
% It is nothing else but a copy of Till Tantau's pgf kernel list.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5



% WARNING: call \pgfplotsapplistclear if there is another list active.
\def\pgfplotsapplistXXnewempty{%
	\pgfutil@ifundefined{pgfplotsapplistXX}{}{%
		\ifx\pgfplotsapplistXX\pgfutil@empty
		\else
			\pgfplots@error{\string\pgfplotsapplistXXnewempty: there is already another list which is *not* empty. It currently contains '\meaning\pgfplotsapplistXX'. Please call '\string\pgfplotsapplistXXclear' before using a new list to ensure clean separations.}%
		\fi
	}%
	\let\pgfplotsapplistXX=\pgfutil@empty
	\let\pgfplotsapplistXX@smallbuf=\pgfutil@empty
	\let\pgfplotsapplistXX@bigbuf=\pgfutil@empty
	\def\pgfplotsapplistXX@smallbuf@c{0}%
	\def\pgfplotsapplistXX@bigbuf@c{0}%
}%


\def\pgfplotsapplistXXclear{%
	\pgfutil@ifundefined{pgfplotsapplistXX}{}{%
		\let\pgfplotsapplistXX=\pgfutil@empty
		\let\pgfplotsapplistXX@smallbuf=\pgfutil@empty
		\let\pgfplotsapplistXX@bigbuf=\pgfutil@empty
		\def\pgfplotsapplistXX@smallbuf@c{0}%
		\def\pgfplotsapplistXX@bigbuf@c{0}%
	}%
}%

% #1: the item to append
% #2: the list as macro name
\def\pgfplotsapplistXXpushback#1{%
	\begingroup
		\c@pgf@counta=\pgfplotsapplistXX@smallbuf@c\relax
		\advance\c@pgf@counta by1
		\xdef\pgfplots@glob@TMPa{\the\c@pgf@counta}%
	\endgroup
	\let\pgfplotsapplistXX@smallbuf@c=\pgfplots@glob@TMPa
	\ifnum\pgfplotsapplistXX@smallbuf@c<40
		\t@pgfplots@toka=\expandafter{\pgfplotsapplistXX@smallbuf#1}%
		\edef\pgfplotsapplistXX@smallbuf{\the\t@pgfplots@toka}%
	\else
		\pgfplotsapplistXXpushback@smallbufoverfl{#1}%
	\fi
}%
\def\pgfplotsapplistXXpushback@smallbufoverfl#1{%
	\begingroup
		\c@pgf@counta=\pgfplotsapplistXX@bigbuf@c\relax
		\advance\c@pgf@counta by1
		\xdef\pgfplots@glob@TMPa{\the\c@pgf@counta}%
	\endgroup
	\let\pgfplotsapplistXX@bigbuf@c=\pgfplots@glob@TMPa
	%
	\ifnum\pgfplotsapplistXX@bigbuf@c<30
		\t@pgfplots@toka=\expandafter{\pgfplotsapplistXX@bigbuf}%
		\t@pgfplots@tokb=\expandafter{\pgfplotsapplistXX@smallbuf#1}%
		\edef\pgfplotsapplistXX@bigbuf{\the\t@pgfplots@toka\the\t@pgfplots@tokb}%
		\let\pgfplotsapplistXX@smallbuf=\pgfutil@empty
		\def\pgfplotsapplistXX@smallbuf@c{0}%
	\else%
		\t@pgfplots@toka=\expandafter{\pgfplotsapplistXX}%
		\t@pgfplots@tokb=\expandafter{\pgfplotsapplistXX@bigbuf}%
		\t@pgfplots@tokc=\expandafter{\pgfplotsapplistXX@smallbuf#1}%
		\edef\pgfplotsapplistXX{\the\t@pgfplots@toka\the\t@pgfplots@tokb\the\t@pgfplots@tokc}%
		\let\pgfplotsapplistXX@smallbuf=\pgfutil@empty
		\def\pgfplotsapplistXX@smallbuf@c{0}%
		\let\pgfplotsapplistXX@bigbuf=\pgfutil@empty
		\def\pgfplotsapplistXX@bigbuf@c{0}%
	\fi%
}%
\def\pgfplotsapplistXXflushbuffers{%
	\t@pgfplots@toka=\expandafter{\pgfplotsapplistXX}%
	\t@pgfplots@tokb=\expandafter{\pgfplotsapplistXX@bigbuf}%
	\t@pgfplots@tokc=\expandafter{\pgfplotsapplistXX@smallbuf}%
	\edef\pgfplotsapplistXX{\the\t@pgfplots@toka\the\t@pgfplots@tokb\the\t@pgfplots@tokc}%
	\let\pgfplotsapplistXX@smallbuf=\pgfutil@empty
	\def\pgfplotsapplistXX@smallbuf@c{0}%
	\let\pgfplotsapplistXX@bigbuf=\pgfutil@empty
	\def\pgfplotsapplistXX@bigbuf@c{0}%
}%

	
% Expands the complete content of list #1 as-is into the macro #2.
\def\pgfplotsapplistXXedefcontenttomacro#1{%
	\pgfplotsapplistXXflushbuffers
	\edef#1{\pgfplotsapplistXX}}
\def\pgfplotsapplistXXxdefcontenttomacro#1{%
	\pgfplotsapplistXXflushbuffers%
	\xdef#1{\pgfplotsapplistXX}}
\def\pgfplotsapplistXXlet#1{%
	\pgfplotsapplistXXflushbuffers%
	\let#1=\pgfplotsapplistXX}

% Foreach list element, the stored value will simply be processed by
% TeX. Characters will be printed and commands will be executed.
\def\pgfplotsapplistXXexecute#1{%
	\pgfplotsapplistXXflushbuffers
	#1}%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
% 
% \pgfplotslistXXglobal  assigns to a global list.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\def\pgfplotsapplistXXglobalnewempty{%
	\pgfutil@ifundefined{pgfplotsapplistXXglobal}{}{%
		\ifx\pgfplotsapplistXXglobal\pgfutil@empty
		\else
			\pgfplots@error{\string\pgfplotsapplistXXglobalnewempty: there is already another list which is *not* empty. It currently contains '\meaning\pgfplotsapplistXXglobal'. Please call '\string\pgfplotsapplistXXglobalclear' before using a new list to ensure clean separations.}%
		\fi
	}%
	\global\let\pgfplotsapplistXXglobal=\pgfutil@empty
	\global\let\pgfplotsapplistXXglobal@smallbuf=\pgfutil@empty
	\global\let\pgfplotsapplistXXglobal@bigbuf=\pgfutil@empty
	\gdef\pgfplotsapplistXXglobal@smallbuf@c{0}%
	\gdef\pgfplotsapplistXXglobal@bigbuf@c{0}%
}%


\def\pgfplotsapplistXXglobalclear{%
	\pgfutil@ifundefined{pgfplotsapplistXXglobal}{}{%
		\global\let\pgfplotsapplistXXglobal=\pgfutil@empty
		\global\let\pgfplotsapplistXXglobal@smallbuf=\pgfutil@empty
		\global\let\pgfplotsapplistXXglobal@bigbuf=\pgfutil@empty
		\gdef\pgfplotsapplistXXglobal@smallbuf@c{0}%
		\gdef\pgfplotsapplistXXglobal@bigbuf@c{0}%
	}%
}%

% #1: the item to append
% #2: the list as macro name
\def\pgfplotsapplistXXglobalpushback#1{%
	\begingroup
		\c@pgf@counta=\pgfplotsapplistXXglobal@smallbuf@c\relax
		\advance\c@pgf@counta by1
		\xdef\pgfplots@glob@TMPa{\the\c@pgf@counta}%
	\endgroup
	\global\let\pgfplotsapplistXXglobal@smallbuf@c=\pgfplots@glob@TMPa
	\ifnum\pgfplotsapplistXXglobal@smallbuf@c<40
		\t@pgfplots@toka=\expandafter{\pgfplotsapplistXXglobal@smallbuf#1}%
		\xdef\pgfplotsapplistXXglobal@smallbuf{\the\t@pgfplots@toka}%
	\else
		\pgfplotsapplistXXglobalpushback@smallbufoverfl{#1}%
	\fi
}%
\def\pgfplotsapplistXXglobalpushback@smallbufoverfl#1{%
	\begingroup
		\c@pgf@counta=\pgfplotsapplistXXglobal@bigbuf@c\relax
		\advance\c@pgf@counta by1
		\xdef\pgfplots@glob@TMPa{\the\c@pgf@counta}%
	\endgroup
	\global\let\pgfplotsapplistXXglobal@bigbuf@c=\pgfplots@glob@TMPa
	%
	\ifnum\pgfplotsapplistXXglobal@bigbuf@c<30
		\t@pgfplots@toka=\expandafter{\pgfplotsapplistXXglobal@bigbuf}%
		\t@pgfplots@tokb=\expandafter{\pgfplotsapplistXXglobal@smallbuf#1}%
		\xdef\pgfplotsapplistXXglobal@bigbuf{\the\t@pgfplots@toka\the\t@pgfplots@tokb}%
		\global\let\pgfplotsapplistXXglobal@smallbuf=\pgfutil@empty
		\gdef\pgfplotsapplistXXglobal@smallbuf@c{0}%
	\else%
		\t@pgfplots@toka=\expandafter{\pgfplotsapplistXXglobal}%
		\t@pgfplots@tokb=\expandafter{\pgfplotsapplistXXglobal@bigbuf}%
		\t@pgfplots@tokc=\expandafter{\pgfplotsapplistXXglobal@smallbuf#1}%
		\xdef\pgfplotsapplistXXglobal{\the\t@pgfplots@toka\the\t@pgfplots@tokb\the\t@pgfplots@tokc}%
		\global\let\pgfplotsapplistXXglobal@smallbuf=\pgfutil@empty
		\gdef\pgfplotsapplistXXglobal@smallbuf@c{0}%
		\global\let\pgfplotsapplistXXglobal@bigbuf=\pgfutil@empty
		\gdef\pgfplotsapplistXXglobal@bigbuf@c{0}%
	\fi%
}%
\def\pgfplotsapplistXXglobalflushbuffers{%
	\t@pgfplots@toka=\expandafter{\pgfplotsapplistXXglobal}%
	\t@pgfplots@tokb=\expandafter{\pgfplotsapplistXXglobal@bigbuf}%
	\t@pgfplots@tokc=\expandafter{\pgfplotsapplistXXglobal@smallbuf}%
	\xdef\pgfplotsapplistXXglobal{\the\t@pgfplots@toka\the\t@pgfplots@tokb\the\t@pgfplots@tokc}%
	\global\let\pgfplotsapplistXXglobal@smallbuf=\pgfutil@empty
	\gdef\pgfplotsapplistXXglobal@smallbuf@c{0}%
	\global\let\pgfplotsapplistXXglobal@bigbuf=\pgfutil@empty
	\gdef\pgfplotsapplistXXglobal@bigbuf@c{0}%
}%

	
% Expands the complete content of list #1 as-is into the macro #2.
%
% this assigns locally into #1.
\def\pgfplotsapplistXXglobaledefcontenttomacro#1{%
	\pgfplotsapplistXXglobalflushbuffers
	\edef#1{\pgfplotsapplistXXglobal}}
% this assigns locally into #1.
\def\pgfplotsapplistXXglobalxdefcontenttomacro#1{%
	\pgfplotsapplistXXglobalflushbuffers%
	\xdef#1{\pgfplotsapplistXXglobal}}
% this assigns locally into #1.
\def\pgfplotsapplistXXgloballet#1{%
	\pgfplotsapplistXXglobalflushbuffers%
	\let#1=\pgfplotsapplistXXglobal}

% Foreach list element, the stored value will simply be processed by
% TeX. Characters will be printed and commands will be executed.
% this assigns locally into #1.
\def\pgfplotsapplistXXglobalexecute#1{%
	\pgfplotsapplistXXglobalflushbuffers
	#1}%


==> pgfplotsoldpgfsupp_loader.code.tex <==
%--------------------------------------------------
% \pgfutil@ifundefined{pgfmathfloattosci}
% 	{}%
% 	{\endinput}%
%-------------------------------------------------- 
\pgfkeysifdefined{/pgf/number format/@dec sep mark}{\endinput}{}

\immediate\write16{Package pgfplots: loading complementary code for your PGF version...}
\input pgfplotsoldpgfsupp_misc.code.tex
\input pgfplotsoldpgfsupp_pgfkeysfiltered.code.tex
\input pgfplotsoldpgfsupp_pgfmathfloat.code.tex
\input pgfplotsoldpgfsupp_pgflibraryplothandlers.code.tex


==> pgfplotsoldpgfsupp_misc.code.tex <==

% ======================================================
% compatibility with PGF 2.0
\def\pgfkeysaddvalue#1#2#3{%
  {%
    \toks0{#2}%
    \pgfkeysifdefined{#1}
    {\pgfkeys@temptoks\expandafter\expandafter\expandafter{\csname pgfk@#1\endcsname}}%
    {\pgfkeys@temptoks{}}%
    \toks1{#3}%
    \xdef\pgfkeys@global@temp{\the\toks0 \the\pgfkeys@temptoks \the\toks1}% believe or don't: the spaces are important
  }%
  \pgfkeyslet{#1}\pgfkeys@global@temp%
}

\def\pgfkeys@try{%
  \pgfkeysifdefined{\pgfkeyscurrentpath/.@cmd}%
  {%
    \pgfkeysgetvalue{\pgfkeyscurrentpath/.@cmd}{\pgfkeys@code}%
    \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text% Hmm... no value
      \pgfkeysifdefined{\pgfkeyscurrentpath/.@def}%
      {\pgfkeysgetvalue{\pgfkeyscurrentpath/.@def}{\pgfkeyscurrentvalue}}
      {}% no default, so leave it
    \fi%
	\let\pgfkeyscurrentkey=\pgfkeyscurrentpath% make sure that \pgfkeys@code doesn't know about 'try'. Important for .is choice
	% FIXME: maybe there are more things like that - also adjust currentname!?
    \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov%
    \pgfkeyssuccesstrue%
  }%
  {%
    \pgfkeysifdefined{\pgfkeyscurrentpath}%
    {%
      \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text%
        \pgfkeysvalueof{\pgfkeyscurrentpath}%
      \else%
        \pgfkeyslet{\pgfkeyscurrentpath}\pgfkeyscurrentvalue%
      \fi%
      \pgfkeyssuccesstrue%
    }%
    {\pgfkeyssuccessfalse}%
  }%
}
% ======================================================


% pgfutil@loop (from plain.tex)

\def\pgfutil@loop#1\pgfutil@repeat{\def\pgfutil@body{#1}\pgfutil@iterate}
\def\pgfutil@iterate{\pgfutil@body \let\pgfutil@next\pgfutil@iterate \else\let\pgfutil@next\relax\fi \pgfutil@next}
\let\pgfutil@repeat=\fi % this makes \loop...\if...\repeat skippable

\def\pgfqpointxy#1#2{%
  \pgf@x=#1\pgf@xx%
  \advance\pgf@x by #2\pgf@yx%
  \pgf@y=#1\pgf@xy%
  \advance\pgf@y by #2\pgf@yy}
\def\pgfqpointxyz#1#2#3{%
  \pgf@x=#1\pgf@xx%
  \advance\pgf@x by #2\pgf@yx%
  \advance\pgf@x by #3\pgf@zx%
  \pgf@y=#1\pgf@xy%
  \advance\pgf@y by #2\pgf@yy%
  \advance\pgf@y by #3\pgf@zy}
\def\pgfcoordinate#1#2{%
  \edef\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty% do nothing
  \else%
    \pgf@process{\pgfpointtransformed{#2}}%
    \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{coordinate}%
    \expandafter\xdef\csname pgf@sh@np@#1\endcsname{%
      \noexpand\def\noexpand\centerpoint{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    }
    \expandafter\gdef\csname pgf@sh@nt@#1\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
    \expandafter\global\expandafter\let\csname pgf@sh@ma@#1\endcsname\pgfutil@empty%
    \expandafter\gdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}%
  \fi%
}
% ======================================================

\def\pgfutilensuremath#1{%
	\ifmmode#1\else$#1$\fi
}

\tikzoption{ybar}[]{\let\tikz@plot@handler=\pgfplothandlerybar}
\tikzoption{xbar}[]{\let\tikz@plot@handler=\pgfplothandlerxbar}
\tikzoption{ybar interval}[]{\let\tikz@plot@handler=\pgfplothandlerybarinterval}
\tikzoption{xbar interval}[]{\let\tikz@plot@handler=\pgfplothandlerxbarinterval}
\tikzoption{const plot}[]{\let\tikz@plot@handler=\pgfplothandlerconstantlineto}
\tikzoption{const plot mark left}[]{\let\tikz@plot@handler=\pgfplothandlerconstantlineto}
\tikzoption{const plot mark right}[]{\let\tikz@plot@handler=\pgfplothandlerconstantlinetomarkright}
\tikzoption{jump mark right}[]{\let\tikz@plot@handler=\pgfplothandlerjumpmarkright}
\tikzoption{jump mark left}[]{\let\tikz@plot@handler=\pgfplothandlerjumpmarkleft}

% the 'every mark' style is new:
\tikzset{
	every mark/.style={},
	mark options/.style={%
		every mark/.style={#1}%
	}}
\def\tikz@@@plot{%
    \def\pgfplotlastpoint{\pgfpointorigin}%
    \tikz@plot@handler%
    \tikz@plot@data%
    \global\let\tikz@@@temp=\pgfplotlastpoint%
    \ifx\tikz@plot@mark\pgfutil@empty%
    \else%
      % Marks are drawn after the path.
      \setbox\tikz@figbox=\hbox{%
        \unhbox\tikz@figbox%
        \hbox{{%
          \pgfinterruptpath%
            \pgfscope%
              \let\tikz@options=\pgfutil@empty%
              \let\tikz@transform=\pgfutil@empty%
			  \tikzset{every mark}%
              \tikz@options%
              \ifx\tikz@mark@list\pgfutil@empty%
                \pgfplothandlermark{\tikz@transform\pgfuseplotmark{\tikz@plot@mark}}%
              \else
                \pgfplothandlermarklisted{\tikz@transform\pgfuseplotmark{\tikz@plot@mark}}{\tikz@mark@list}%
              \fi
              \tikz@plot@data%
            \endpgfscope
          \endpgfinterruptpath%
        }}%
      }%
    \fi%
    \global\setbox\tikz@tempbox=\copy\tikz@figbox%
    %\global\let\tikz@after@path@smuggle=\tikz@after@path
  \endgroup%
  \setbox\tikz@figbox=\box\tikz@tempbox%  
  \tikz@make@last@position{\tikz@@@temp}%  
  %\expandafter\tikz@scan@next@command\tikz@after@path@smuggle%
  \tikz@scan@next@command%
}




% ======================================================


\newif\ifpgfmathcomparison

% Assigns \pgfmathresult to 1.0 if #1 ~= #1.
%
% It will also set the boolean \ifpgfmathcomparison accordingly
% (globally).
\def\pgfmathapproxequalto#1#2{%
	\edef\pgfmath@marshal{%
		\noexpand\pgfmathparse{#2}
		\noexpand\let\noexpand\pgfmath@arg\noexpand\pgfmathresult%
		\noexpand\pgfmathparse{#1}%
	}%
	\pgfmath@marshal%
	\pgfmathapproxequalto@{\pgfmathresult}{\pgfmath@arg}}
\def\pgfmathapproxequalto@#1#2{%
	\begingroup%
		\pgfmath@x#1pt%
		\pgfmath@y#2pt%
		\advance\pgfmath@x-\pgfmath@y%
		\ifdim\pgfmath@x<0pt
			\multiply\pgfmath@x by-1
		\fi
		\ifdim\pgfmath@x<0.0001pt\relax%
			\def\pgfmathresult{1.0}%
			\global\pgfmathcomparisontrue
		\else%
			\def\pgfmathresult{0.0}%
			\global\pgfmathcomparisonfalse
		\fi%
	\pgfmath@smuggleone\pgfmathresult
	\endgroup%
}


==> pgfplotsoldpgfsupp_pgfkeysfiltered.code.tex <==
% Copyright 2008 by Christian Feuersaenger
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.
% 
% This file contains additions to pgfkeys.code.tex (loaded
% automatically at the end of pgfkeys.code.tex)
%
% Improvements:
%
% - option filtering 
%   you provide
%     - a boolean predicate
%     - a "filter handler" which will be invoked for non-matching options,
%     - a key=value list as usual.
%   The filter sets only matching options and invokes the handler for
%   unmatching ones.
%
% - Fast family support as in xkeyval.
%   - A key like /my tree/my option  can be associated with /my family
%   - You can efficiently set keys which belong to a set of "active"
%     families.
%  Remaining options can be collected into a macro.

% WARNING:
% this file overwrites
% \pgfkeys@addpath
% \pgfkeys@nevermind
%
% all other features are 'additive'


% these implementations will be switched dynamically with their
% filtered versions (in \pgfkeys@install@filter@and@invoke)
\let\pgfkeys@orig@case@one=\pgfkeys@case@one
\let\pgfkeys@orig@@set=\pgfkeys@@set
\let\pgfkeys@orig@@qset=\pgfkeys@@qset
\let\pgfkeys@orig@try=\pgfkeys@try
\let\pgfkeys@orig@unknown=\pgfkeys@unknown

\newif\ifpgfkeysfilteringisactive
\newif\ifpgfkeysfiltercontinue
\let\pgfkeys@key@predicate=\pgfkeys@empty
\let\pgfkeys@filtered@handler=\pgfkeys@empty
\newtoks\pgfkeys@tmptoks

% Performs 'filtered' key settings.
%
% For every option for which the path prefixing has already been done, 
% the current key filter predicate will be invoked. If the predicate
% returns true, pgfkeys will process this key in the normal manner.
% If not, a key filter handler will be invoked.
%
% The *predicate* and *handler* semantics are as follows:
% PRECONDITION:
% 		1. The variables
% 			\pgfkeyscurrentkey (full path including name)
% 			\pgfkeyscurrentkeyRAW (the current key as it has been
% 			                       found in the key=value list
% 			                       without path modification)
% 			\pgfkeyscurrentvalue
% 			are all set. If the current key is a handler variable,
%	 			\pgfkeyscurrentname 
%	 		and
% 				\pgfkeyscurrentpath
% 			are also set.
%		2. The type of option has already been checked, that means
%			case (1) whether '.@cmd' exists
%			case (2) whether the key as such has its value
%			case (3) it is a handler like '.code', '.cd' or whatever.
%			case (0) it is unknown.
%			The actual case number (0-3) will be provided as contents
%			of the macro
%				\pgfkeyscasenumber.
%			Please note that unknown options will be processed with
%			the usual '.unknown' handlers unless the key filter takes
%			control over unknown options as well.
%
% POSTCONDITION:
% 		the predicate sets 
% 			\pgfkeysfiltercontinuetrue 
% 		or
% 			\pgfkeysfiltercontinuefalse
% 		(the boolean \ifpgfkeysfiltercontinue).
% Depending on this 'if', option processing will be continued or
% skipped.
%
% The handler can do anything with the option, for example collect
% unmatched ones.
%
% ATTENTION: \pgfkeysfiltered can't be nested (yet). Use the
% \pgfkeyspredicateAND if you need multiple predicates at once.
% Nesting would produce unexpected results because the current filter
% state can't be stored/restored without TeX-groups, therefor it is
% disabled.
%
% ATTENTION: you can't filter error messages.
%
% REMARK: In case (3), the macros \pgfkeyscurrentpath and
% \pgfkeyscurrentname have already been computed, you do not need to
% invoke \pgfkeyssplitpath. In any other case, neither path nor name
% are required for the options processing - if you need them for
% predicates/handlers, you need to compute them by hand.
% 
%
% Example:
%   \def\unmatched{}
%   \pgfkeys{/pgf/key filters/is descendant of/.install key filter=/my group}
%   \pgfkeys{/pgf/key filter handlers/append filtered to/.install key filter handler=\unmatched}
%   \pgfkeysfiltered%
%   	{/my group/option 1=value 1,/tikz/option 2=value 2}
% ->
%  will set '/my group/option 1' as usual, but '/tikz/option 2' will not
%  be set. Instead, it will be appended to '\unmatched' such that 
%  \unmatched = {/tikz/option 2=value2}
%  after the operation.
%
% Arguments:
% #1:  key-value list.
\def\pgfkeysfiltered{%
	% produce 
	% '{<default path>}'
	% each expanded exactly one time into the register:  
	\expandafter\pgfkeysfiltered@@install\expandafter{\pgfkeysdefaultpath}%
}

% #1: old value of default path.
% #2: key-value-list.
\def\pgfkeysfiltered@@install#1#2{%
	\pgfkeys@install@filter@and@invoke{%
		\let\pgfkeysdefaultpath\pgfkeys@root%
		\pgfkeys@parse#2,\pgfkeys@mainstop%
		\def\pgfkeysdefaultpath{#1}%
	}%
}

% Assuming that macro #1 contains a key=value list, this command
% performs an \pgfkeysalso command for the content of macro #1.
%
% It can be used in conjunction with 
%   - \pgfkeysfiltered and
%   - \pgfkeysappendfilterednamestomacro:
% the first pass fill only process options matching the filter, then,
% a \pgfkeysalsofrom can be used at a later time to set the remaining
% options.
%
% Example:
% \pgfkeys{/my group/.cd,/utils/exec=\pgfkeysalsofrom\filtered}
\def\pgfkeysalsofrom#1{%
	\expandafter\pgfkeysalso\expandafter{#1}%
}

% The same as \pgfkeysalsofrom, but it invokes \pgfkeysalsofiltered.
\def\pgfkeysalsofilteredfrom#1{%
	\expandafter\pgfkeysalsofiltered\expandafter{#1}%
}

% #1 = options
\long\def\pgfkeysalsofiltered#1{%
	\pgfkeys@install@filter@and@invoke{\pgfkeysalso{#1}}%
}%

% The same like \pgfkeysfiltered, but with quick search path setting.
%
% #1: default path
% #2: key-value-pairs
\def\pgfqkeysfiltered#1{%
	\expandafter\pgfqkeysfiltered@@install\expandafter{\pgfkeysdefaultpath}{#1}%
}

% #1: old value of default path.
% #2: default path
% #3: key-value-list.
\def\pgfqkeysfiltered@@install#1#2#3{%
	\pgfkeys@install@filter@and@invoke{%
		\def\pgfkeysdefaultpath{#2/}\pgfkeys@parse#3,\pgfkeys@mainstop\def\pgfkeysdefaultpath{#1}%
	}%
}

% Family management
%
% The family code provides the following features:
% 1. every key can be associated with 0 or 1 'family'.
% 2. Families are a loose association which are independend of the key
% hierarchy.
%   For example, /my tree/key1  can belong to family /tikz.
%
% 3. It is possible to "activate" or "deactivate" single families.
%    Furthermore, it is possible to set only keys which belong to 
%    active families (using \pgfkeysfiltered).
% 4. Runtime complexities:
%    If you have N options and you only want to process K active
%    families, the runtime is O( N + K ):
%      - activate every family O(K)
%      - use \pgfkeyshasactivefamily as filter predicate O(N)
%      - deactivate every family O(K)


% Activates family #1.
%
% #1 maybe a macro.
\def\pgfkeysactivatefamily#1{%
	\pgfkeysiffamilydefined
		{#1}%
		{\csname pgfk@#1/familyactivetrue\endcsname}%
		{\pgfkeysvalueof{/errors/family unknown/.@cmd}{#1}\pgfeov}%
%\message{[ACTIVATING FAMILY #1]}%
}

% Deactivates family #1.
%
% #1 maybe a macro.
\def\pgfkeysdeactivatefamily#1{
	\pgfkeysiffamilydefined
		{#1}%
		{\csname pgfk@#1/familyactivefalse\endcsname}%
		{\pgfkeysvalueof{/errors/family unknown/.@cmd}{#1}\pgfeov}%
%\message{[DEACTIVATING FAMILY #1]}%
}

% Activates all families in the comma separated list #1.
%
% It will also generate code for deactivation of all those families
% into the command #2.
%
% #1: a comma-separated list of fully qualified family names.
% #2: a command which will be filled with a deactivate-all command.
\def\pgfkeysactivatefamilies#1#2{%
	\pgfkeyssavekeyfilterstateto\pgfkeys@cur@state
	\expandafter\pgfkeysactivatefamilies@impl\expandafter{\pgfkeys@cur@state}{#1}{#2}%
}
% #1: commands needed to restore the old filtering state
% #2: family name list
% #3: macro name for de-activate command
\def\pgfkeysactivatefamilies@impl#1#2#3{%
	\pgfkeysinstallkeyfilter{/pgf/key filters/false}{}%
	\let#3=\pgfkeys@empty%
	\def\pgfkeys@filtered@handler{\pgfkeys@family@activate@handler{#3}}%
	\pgfkeysalsofiltered{#2}%
	#1%
}

\def\pgfkeys@family@activate@handler#1{%
	\pgfkeysactivatefamily{\pgfkeyscurrentkey}%
	% produce 
	%   <old list> '\pgfkeysdeactivatefamily{' <current key> '}'
	\pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter#1\expandafter\pgfkeysdeactivatefamily\expandafter{\pgfkeyscurrentkey}}%
	\edef#1{\the\pgfkeys@tmptoks}%
}

% If for testing whether a family exists.
%
% #1 = fully qualified family name
% #2 = if-case
% #3 = else-case
%
% Description:
%
% If the family exists, #2 will be executed. Otherwise, #3 will be
% called.
\long\def\pgfkeysiffamilydefined#1#2#3{\pgfkeys@ifcsname ifpgfk@#1/familyactive\endcsname#2\else#3\fi}

% Sets the TeX boolean 
%   \ifpgfkeysfiltercontinue := ( family #1 is active )
% 
% Argument:
% #1 the family name. Maybe a macro.
\def\pgfkeysisfamilyactive#1{%
	\pgfkeysiffamilydefined{#1}{%
		\expandafter\let\expandafter\ifpgfkeysfiltercontinue\csname ifpgfk@#1/familyactive\endcsname
	}{%
		\pgfkeysvalueof{/errors/family unknown/.@cmd}{#1}\pgfeov%
		\expandafter\expandafter\expandafter\let\csname ifpgfkeysfiltercontinue\endcsname\csname iffalse\endcsname
	}%
}%

% Retrieve the family of full key #1 into macro #2.
%
% Will set the TeX boolean \ifpgfkeyssuccess to whether the full key
% really has a family.
%
% The family for any key is stored in the sub-key #1/family.
%
% Parameters:
% #1:  the full key name for which the family is requested. Maybe a
%      macro.
% #2:  a macro name which will be filled with the result.
\def\pgfkeysgetfamily#1#2{%
	\pgfkeysifdefined{#1/family}{\pgfkeysgetvalue{#1/family}{#2}\pgfkeyssuccesstrue}{\pgfkeyssuccessfalse}%
}
	


% Sets \ifpgfkeysfiltercontinue to true iff the current key belongs to
% the /errors tree.
\long\def\pgfkeys@cur@is@descendant@of@errors{%
	\expandafter\pgfkeys@cur@is@descendant@of@errors@impl\pgfkeyscurrentkey/errors\pgf@@eov
}%
\long\def\pgfkeys@cur@is@descendant@of@errors@impl#1/errors#2\pgf@@eov{%
	\def\pgfkeyspred@TMP{#1}%
	\ifx\pgfkeyspred@TMP\pgfkeys@empty
%\message{[SPECIAL CHECK] '\pgfkeyscurrentkey' is descendant of '/errors': TRUE.}%
		\pgfkeysfiltercontinuetrue
	\else
%\message{[SPECIAL CHECK] '\pgfkeyscurrentkey' is descendant of '/errors': FALSE.}%
		\pgfkeysfiltercontinuefalse
	\fi
}%

% \pgfkeysinterruptkeyfilter
% ...
% \endpgfkeysinterruptkeyfilter
% temporarily interrupts key filtering and enables it in
% \endpgfkeysinterruptkeyfilter.
%
% If key filtering it not active, this has no effect at all.
%
% REMARK:
% \pgfkeysinterruptkeyfilter...\endpgfkeysinterruptkeyfilter does NOT
% introduce a \TeX-group.
\def\pgfkeysinterruptkeyfilter{%
	\ifpgfkeysfilteringisactive
		\let\pgfkeys@case@one=\pgfkeys@orig@case@one
		\let\pgfkeys@try=\pgfkeys@orig@try
		\let\pgfkeys@unknown=\pgfkeys@orig@unknown
	\fi
}

\def\endpgfkeysinterruptkeyfilter{%
	\ifpgfkeysfilteringisactive
		\let\pgfkeys@case@one=\pgfkeys@case@one@filtered
		\let\pgfkeys@try=\pgfkeys@try@filtered
		\let\pgfkeys@unknown=\pgfkeys@unknown@filtered
	\fi
}

% Activates families #1, calls \pgfkeysfiltered and deactivates the
% families afterwards.
%
% REMARK: you need to install a family-based key filter predicate
% manually to benefit from the activated families!
%
% #1: comma separated family list
% #2: key-value pairs
%
% @see \pgfkeysactivatefamiliesandfilteroptions
\def\pgfkeysactivatefamiliesandfilteroptions#1#2{%
	\pgfkeysactivatefamilies{#1}{\pgfkeys@family@deactivation}%
	\pgfkeysfiltered{#2}%
	\pgfkeys@family@deactivation
}

% The "quick" variant of \pgfkeysactivatefamiliesandfilteroptions: it
% also assigns a default path.
%
% #1: comma separated family list
% #2: default path
% #3: key-value pairs
\def\pgfqkeysactivatefamiliesandfilteroptions#1#2#3{%
	\pgfkeysactivatefamilies{#1}{\pgfkeys@family@deactivation}%
	\pgfqkeysfiltered{#2}{#3}%
	\pgfkeys@family@deactivation
}

% Public version of split path:
\def\pgfkeyssplitpath{\pgfkeys@split@path}%


% The same as \pgfkeysactivatefamiliesandfilteroptions but just for
% ONE family.
%
% #1: family (maybe a macro)
% #2: key-value pairs
\def\pgfkeysactivatesinglefamilyandfilteroptions#1#2{%
	\pgfkeysactivatefamily{#1}%
	\pgfkeysfiltered{#2}%
	\pgfkeysdeactivatefamily{#1}%
}

% The "quick" variant of \pgfkeysactivatesinglefamilyandfilteroptions
%
% #1: family (maybe a macro)
% #2: default path
% #3: key-value pairs
\def\pgfqkeysactivatesinglefamilyandfilteroptions#1#2#3{%
	\pgfkeysactivatefamily{#1}%
	\pgfqkeysfiltered{#2}{#3}%
	\pgfkeysdeactivatefamily{#1}%
}

% Installs the key filter '#1' with argument '#2'.
% This is equivalent to
%    \pgfkeys{#1/.install key filter=#2}
%
% The current values of the key filter handler is stored into the public
% macros
% \pgfkeyscurrentkeyfilter
% and
% \pgfkeyscurrentkeyfilterargs
%
% #1: a full key name; may be a macro
% #2: optional arguments for the key. If the key expects more than one
% argument, supply '{{first}{second}}'
\def\pgfkeysinstallkeyfilter#1#2{%
	\pgfkeysifdefined{#1/.@cmd}{%
		\edef\pgfkeyscurrentkeyfilter{#1}%
		\def\pgfkeyscurrentkeyfilterargs{#2}%
		\pgfkeysgetvalue{#1/.@cmd}{\pgfkeys@key@predicate@}%
		\def\pgfkeys@key@predicate{\pgfkeys@key@predicate@#2\pgfeov}%
	}{%
		\pgfkeysvalueof{/errors/no such key filter/.@cmd}{#1}{#2}\pgfeov%
	}%
}

% Installs the key filter handler '#1' with argument '#2'.
% This is equivalent to
%    \pgfkeys{#1/.install key filter handler=#2}
% 
% The current values of the key filter handler is stored into the public
% macros
% \pgfkeyscurrentkeyfilterhandler
% and
% \pgfkeyscurrentkeyfilterhandlerargs
%
% #1: a full key name; may be a macro
% #2: optional arguments for the handler. If the handler expects more than one
% argument, supply '{{first}{second}}'
\def\pgfkeysinstallkeyfilterhandler#1#2{%
	\pgfkeysifdefined{#1/.@cmd}{%
		\edef\pgfkeyscurrentkeyfilterhandler{#1}%
		\def\pgfkeyscurrentkeyfilterhandlerargs{#2}%
		\pgfkeysgetvalue{#1/.@cmd}{\pgfkeys@filtered@handler@}%
		\def\pgfkeys@filtered@handler{\pgfkeys@filtered@handler@#2\pgfeov}%
	}{%
		\pgfkeysvalueof{/errors/no such key filter handler/.@cmd}{#1}{#2}\pgfeov%
	}%
}

% Creates a macro which contains commands to re-activate the current
% key filter and key filter handler. It can be used to temporarily
% switch the key filter.
\def\pgfkeyssavekeyfilterstateto#1{%
	% produce the string
	% \pgfkeysinstallkeyfilter{...}{...}
	% \pgfkeysinstallkeyfilterhandler{...}{...}
	% where each argument is expanded once
	% FIXME: Do the same with less overhead!
	\pgfkeys@tmptoks={\pgfkeysinstallkeyfilter}%
	\pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfkeys@tmptoks\expandafter{\pgfkeyscurrentkeyfilter}}%
	\pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfkeys@tmptoks\expandafter{\pgfkeyscurrentkeyfilterargs}\pgfkeysinstallkeyfilterhandler}%
	\pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfkeys@tmptoks\expandafter{\pgfkeyscurrentkeyfilterhandler}}%
	\pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfkeys@tmptoks\expandafter{\pgfkeyscurrentkeyfilterhandlerargs}}%
	\edef#1{%
		\the\pgfkeys@tmptoks
	}%
}


\pgfkeys{%
	/errors/family unknown/.code=\pgfkeys@error{%
		Sorry, I do not know family '#1' and can't work with any assoicated family handling. Perhaps you misspelled it?},
	/errors/no such key filter/.code 2 args=\pgfkeys@error{Sorry, there is no such key filter '#1'.},
	/errors/no such key filter handler/.code 2 args=\pgfkeys@error{Sorry, there is no such key filter handler '#1'.},
	% HANDLERS:
	%
	% .is family should
	%  1. '.cd' into the families' path,
	%  2. define booleans to activate/deactive the family 
	%     (see \pgfkeysisfamilyactive)
	%  3. make sure that \pgfkeyshasactivefamily returns true for
	%     the family itsself.
	/handlers/.is family/.append code={%
		%\newif is an \outer macro in plain tex, so this here is not portable:
		%\expandafter\newif\csname if\pgfkeyscurrentpath/familyactive\endcsname
		\edef\pgfkeyspred@TMP{pgfk@\pgfkeyscurrentpath/familyactive}%
		\expandafter\pgfkeys@non@outer@newif\expandafter{\pgfkeyspred@TMP}%
		\edef\pgfkeyspred@TMP{\pgfkeyscurrentpath/.belongs to family=\pgfkeyscurrentpath}%
		\expandafter\pgfkeysalso\expandafter{\pgfkeyspred@TMP}%
	},%
	/handlers/.activate family/.code=\pgfkeysactivatefamily{\pgfkeyscurrentpath},
	/handlers/.deactivate family/.code=\pgfkeysdeactivatefamily{\pgfkeyscurrentpath},
	/handlers/.belongs to family/.code={%
			\pgfkeysiffamilydefined{#1}{%
				\pgfkeyssetvalue{\pgfkeyscurrentpath/family}{#1}%
			}{%
				\pgfkeysalso{/errors/family unknown=#1}%
			}%
	},%
	%
	%
	% An addition to the '.try' and '.retry' handlers:
	%
	% It is the same as '.retry', but if the option is still unknown, the
	% usual handlers for unknown keys will be invoked.
	/handlers/.lastretry/.code={%
		\ifpgfkeyssuccess\else
			\pgfkeys@try
			\ifpgfkeyssuccess\else
				% discard the '.lastretry' suffix:
				\edef\pgfkeyscurrentkey{\pgfkeyscurrentpath}%
				\pgfkeys@split@path%
				\pgfkeys@unknown
			\fi
		\fi
	},
	%
	%
	/handlers/.install key filter/.code={%
		\pgfkeysinstallkeyfilter{\pgfkeyscurrentpath}{#1}%
	},%
	/handlers/.install key filter handler/.code={%
		\pgfkeysinstallkeyfilterhandler{\pgfkeyscurrentpath}{#1}%
	},%
	%
	%
	% KEY FILTER HANDLERS:
	%
	/pgf/key filter handlers/append filtered to/.code={%
		% Produce
		%  <orig key> '={' <value> '}'
		% where both, the key and the value are expanded just ONCE:
		\pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter\pgfkeyscurrentkeyRAW\expandafter=\expandafter{\pgfkeyscurrentvalue}}%
		\ifx#1\pgfkeys@empty
		\else
			% Produce <old list> ','  <orig key> '={' <value> '}'
			\pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter#1\expandafter,\the\pgfkeys@tmptoks}%
		\fi
		\edef#1{\the\pgfkeys@tmptoks}%
	},%
	/pgf/key filter handlers/ignore/.code={},
	/pgf/key filter handlers/ignore/.install key filter handler,
	/pgf/key filter handlers/log/.code={%
		\immediate\write16{LOG: the option '\pgfkeyscurrentkey' (was originally '\pgfkeyscurrentkeyRAW') (case \pgfkeyscasenumber) has not been processed due to pgfkeysfiltered.}%
	},
	%
	% 
	% KEY FILTER PREDICATES:
	%
	% Returns true iff the currently processed key belongs to an active family.
	% A family is active if it has been activated before.
	/pgf/key filters/active families/.code={%
		\ifnum\pgfkeyscasenumber=0
			% unknown options shall be processed with the
			% unknown-handlers.
			\pgfkeysfiltercontinuetrue
		\else
			\ifnum\pgfkeyscasenumber=3
				\pgfkeysgetfamily\pgfkeyscurrentpath\pgfkeyspred@TMP
			\else
				\pgfkeysgetfamily\pgfkeyscurrentkey\pgfkeyspred@TMP
			\fi
			\ifpgfkeyssuccess
				\pgfkeysisfamilyactive{\pgfkeyspred@TMP}%
			\else% Ok, it does not belong to any family.
				\pgfkeysfiltercontinuefalse
			\fi
		\fi
	},%
	%
	%
	%
	% This filter works as follows:
	% 1. if the current key belongs to a family:
	% 	return whether its family is active,
	% 2. if the current key does NOT belong to a family:
	%   return the result of criterion '#1',
	% 3. the current key is unknown:
	% 	return the result of criterion '#2'.
	%
	% Arguments:
	% #1: the predicate which will be invoked in case 2.
	%   It will be invoked with the current case number as argument.
	% #2: the predicate which will be invoked in case 3 with 
	%   the current case number as argument.
	/pgf/key filters/active families or no family/.code 2 args={%
		\ifnum\pgfkeyscasenumber=0
			\pgfkeysevalkeyfilterwith{#2}%
		\else
			\ifnum\pgfkeyscasenumber=3
				\pgfkeysgetfamily\pgfkeyscurrentpath\pgfkeyspred@TMP
			\else
				\pgfkeysgetfamily\pgfkeyscurrentkey\pgfkeyspred@TMP
			\fi
			\ifpgfkeyssuccess
				\pgfkeysisfamilyactive{\pgfkeyspred@TMP}%
			\else% Ok, it does not belong to any family.
				\pgfkeysevalkeyfilterwith{#1}%
			\fi
		\fi
	},
	/pgf/key filters/active families or no family DEBUG/.code 2 args={%
		\ifnum\pgfkeyscasenumber=0
			\immediate\write16{[pgfkeyshasactivefamilyornofamily(\pgfkeyscurrentkey, \pgfkeyscasenumber) invoking unknown handler '#2']}%
			\pgfkeysevalkeyfilterwith{#2}%
		\else
			\ifnum\pgfkeyscasenumber=3
				\pgfkeysgetfamily\pgfkeyscurrentpath\pgfkeyspred@TMP
			\else
				\pgfkeysgetfamily\pgfkeyscurrentkey\pgfkeyspred@TMP
			\fi
			\ifpgfkeyssuccess
				\pgfkeysisfamilyactive{\pgfkeyspred@TMP}%
				\ifpgfkeysfiltercontinue
					\immediate\write16{[pgfkeyshasactivefamilyornofamily(\pgfkeyscurrentkey, \pgfkeyscasenumber) family is ACTIVE]}%
				\else
					\immediate\write16{[pgfkeyshasactivefamilyornofamily(\pgfkeyscurrentkey, \pgfkeyscasenumber) family is NOT active.]}%
				\fi
			\else% Ok, it does not belong to any family.
				\immediate\write16{[pgfkeyshasactivefamilyornofamily(\pgfkeyscurrentkey, \pgfkeyscasenumber) invoking has-no-family-handler '#1']}%
				\pgfkeysevalkeyfilterwith{#1}%
			\fi
		\fi
	},
	%
	% Processes only options which are childs of #1.
	% Example:
	%   is descendant of/.install key filter=/foo
	% will be true for
	%  /foo/bar/x=y
	%  /foo/.cd
	%  /foo/bar/.style=...
	% but not for
	%  /bar/foo/...
	/pgf/key filters/is descendant of/.code={%
		\ifnum\pgfkeyscasenumber=0
%\message{'\pgfkeyscurrentkey' (case \pgfkeyscasenumber) is UNKNOWN. Calling unknown handler.}%
			% unknown options shall be processed with the
			% unknown-handlers.
			\pgfkeysfiltercontinuetrue
		\else
			% string prefix comparison:
			\long\def\pgfkeysisdescendantof@impl##1#1##2\pgf@@eov{%
				\def\pgfkeyspred@TMP{##1}%
				\ifx\pgfkeyspred@TMP\pgfkeys@empty
%\message{'\pgfkeyscurrentkey' (case \pgfkeyscasenumber) is descendant of '#1': TRUE.}%
					\pgfkeysfiltercontinuetrue
				\else
%\message{'\pgfkeyscurrentkey' (case \pgfkeyscasenumber) is descendant of '#1': FALSE.}%
					\pgfkeysfiltercontinuefalse
				\fi
			}%
			\expandafter\pgfkeysisdescendantof@impl\pgfkeyscurrentkey#1\pgf@@eov
		\fi
	},%
	%
	%
	% 
	% Returns true if the currently processed full key equals #2.
	/pgf/key filters/equals/.code={%
		\ifnum\pgfkeyscasenumber=0
			% Unknown option:
			\pgfkeysfiltercontinuetrue
		\else
			\def\pgfkeyspred@TMP{#1}%
			\ifx\pgfkeyscurrentkey\pgfkeyspred@TMP
				\pgfkeysfiltercontinuetrue
			\else
				\pgfkeysfiltercontinuefalse
			\fi
		\fi
	},%
	%
	%
	% Argument #1 can be any other (evaluated) filter predicate, its logical return
	% value will be inverted.
	% Example:
	%   not/.install key filter={is descendend of=/tikz}
	% will install a key filter which evaluates 'is descendant of' with argument '/tikz' and returns the logical negation of the result.
	/pgf/key filters/not/.code={%
		\pgfkeysevalkeyfilterwith{#1}%
		\ifpgfkeysfiltercontinue
			\pgfkeysfiltercontinuefalse
		\else
			\pgfkeysfiltercontinuetrue
		\fi
	},%
	/pgf/key filters/and/.code 2 args={%
		\pgfkeysevalkeyfilterwith{#1}%
		\ifpgfkeysfiltercontinue
			\pgfkeysevalkeyfilterwith{#2}%
		\fi
	},%
	/pgf/key filters/or/.code 2 args={%
		\pgfkeysevalkeyfilterwith{#1}%
		\ifpgfkeysfiltercontinue
		\else
			\pgfkeysevalkeyfilterwith{#2}%
		\fi
	},%
	/pgf/key filters/true/.code={\pgfkeysfiltercontinuetrue},%
	/pgf/key filters/true/.install key filter,
	/pgf/key filters/false/.code={\pgfkeysfiltercontinuefalse},%
	%
	% Returns false if the current key is unknown, which avoids calling
	% the unknown handlers.
	/pgf/key filters/defined/.code={%
		\ifnum\pgfkeyscasenumber=0
			\pgfkeysfiltercontinuefalse
		\else
			\pgfkeysfiltercontinuetrue
		\fi
	},
}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Private IMPLEMENTATION
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% This command does THE SAME work as \pgfkeys@case@one,
% but it applies filtering whenever it identified the type of an
% option.
\def\pgfkeys@case@one@filtered{%
	\pgfkeys@cur@is@descendant@of@errors
	\ifpgfkeysfiltercontinue
		\pgfkeys@orig@case@one
	\else
		\pgfkeysfiltercontinuetrue
		\pgfkeysifdefined{\pgfkeyscurrentkey/.@cmd}{%
			% CASE ONE: a command option
			\def\pgfkeyscasenumber{1}%
			\pgfkeys@key@predicate%
			\ifpgfkeysfiltercontinue
%\message{PROCESSING KEY \pgfkeyscurrentkey!}%
				\pgfkeysgetvalue{\pgfkeyscurrentkey/.@cmd}{\pgfkeys@code}%
				\expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov
			\else
%\message{FILTEReD OUT  KEY \pgfkeyscurrentkey!}%
				\pgfkeys@filtered@handler%
			\fi
		}{%
			% CASE TWO: a normal value option
			\pgfkeysifdefined{\pgfkeyscurrentkey}{%
				\def\pgfkeyscasenumber{2}%
				\pgfkeys@key@predicate%
				\ifpgfkeysfiltercontinue
%\message{PROCESSING KEY \pgfkeyscurrentkey!}%
					\pgfkeys@case@two@extern
				\else
%\message{FILTEReD OUT  KEY \pgfkeyscurrentkey!}%
					\pgfkeys@filtered@handler%
				\fi
			}{%
				\pgfkeys@split@path
				% CASE THREE: a handler
				\pgfkeysifdefined{/handlers/\pgfkeyscurrentname/.@cmd}{%
					\def\pgfkeyscasenumber{3}%
					\pgfkeys@key@predicate%
					\ifpgfkeysfiltercontinue
%\message{PROCESSING KEY \pgfkeyscurrentkey!}%
						\pgfkeysgetvalue{/handlers/\pgfkeyscurrentname/.@cmd}{\pgfkeys@code}%
						\expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov
					\else
%\message{FILTERED OUT  KEY \pgfkeyscurrentkey!}%
						\pgfkeys@filtered@handler%
					\fi
				}{%
					\pgfkeys@unknown
				}%
			}%
		}%
	\fi
}%

\def\pgfkeys@unknown@filtered{%
	% CASE ZERO: an unknown option.
	\def\pgfkeyscasenumber{0}%
	\pgfkeys@key@predicate%
	\ifpgfkeysfiltercontinue
%\message{PROCESSING  KEY \pgfkeyscurrentkey!}%
		% start normal 'unknown' handlers:
		\pgfkeys@orig@unknown
	\else
%\message{FILTEReD OUT  KEY \pgfkeyscurrentkey!}%
		\pgfkeys@filtered@handler%
	\fi
}

% Does the same as \pgfkeys@try, but it also invokes the key filters.
\def\pgfkeys@try@filtered{%
	\ifpgfkeysfiltercontinue
		\pgfkeys@orig@try
	\else
		\pgfkeysfiltercontinuetrue
		\pgfkeysifdefined{\pgfkeyscurrentpath/.@cmd}%
		{%
			% CASE ONE: a command option
			\def\pgfkeyscasenumber{1}%
			\pgfkeys@key@predicate%
			\ifpgfkeysfiltercontinue
				\pgfkeysgetvalue{\pgfkeyscurrentkey/.@cmd}{\pgfkeys@code}%
				\ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text% Hmm... no value
					\pgfkeysifdefined{\pgfkeyscurrentpath/.@def}%
					{\pgfkeysgetvalue{\pgfkeyscurrentpath/.@def}{\pgfkeyscurrentvalue}}
					{}% no default, so leave it
				\fi%
				\expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov%
			\else
				\pgfkeys@filtered@handler%
			\fi
			\pgfkeyssuccesstrue%
		}%
		{%
			\pgfkeysifdefined{\pgfkeyscurrentpath}%
			{% CASE TWO: a normal value option
				\def\pgfkeyscasenumber{2}%
				\pgfkeys@key@predicate%
				\ifpgfkeysfiltercontinue
					\ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text%
						\pgfkeysvalueof{\pgfkeyscurrentpath}%
					\else%
						\pgfkeyslet{\pgfkeyscurrentpath}\pgfkeyscurrentvalue%
					\fi%
				\else
					\pgfkeys@filtered@handler%
				\fi
				\pgfkeyssuccesstrue%
			}%
			{\pgfkeyssuccessfalse}%
		}%
	\fi
}


% #1 the code to invoke after init and before cleanup
\def\pgfkeys@install@filter@and@invoke#1{%
	\ifpgfkeysfilteringisactive
		\pgfkeys@error{Sorry, nested calls to key filtering routines are not allowed. (reason: It is not possible to properly restore the previous filtering state after returning from the nested call)}%
	\fi
	\pgfkeysfilteringisactivetrue
	\let\pgfkeys@case@one=\pgfkeys@case@one@filtered
	\let\pgfkeys@try=\pgfkeys@try@filtered
	\let\pgfkeys@unknown=\pgfkeys@unknown@filtered
	#1%
	\let\pgfkeys@case@one=\pgfkeys@orig@case@one
	\let\pgfkeys@try=\pgfkeys@orig@try
	\let\pgfkeys@unknown=\pgfkeys@orig@unknown
	\pgfkeysfilteringisactivefalse
}


%--------------------------------------------------
% \def\pgfkeys@eval@key@filter@subroutine@case@one{%
% 	\pgfkeysifdefined{\pgfkeyscurrentkey/.@cmd}{%
% 		\pgfkeysgetvalue{\pgfkeyscurrentkey/.@cmd}{\pgfkeys@code}%
% 		\let\pgfkeyspred@TMP=\pgfkeyscurrentvalue
% 		\pgfkeys@eval@key@filter@subroutine@restorestate
% 		\expandafter\pgfkeys@code\pgfkeyspred@TMP\pgfeov
% 	}{%
% 		\pgfkeysvalueof{/errors/no such key filter/.@cmd}\pgfkeyscurrentkey\pgfkeyscurrentvalue\pgfeov%
% 	}%
% }
% % THIS VERSION IS TOO SLOW. See below.
% \def\pgfkeysevalkeyfilterwith#1{%
% 	\edef\pgfkeys@eval@key@filter@subroutine@restorestate{%
% 		\noexpand\def\noexpand\pgfkeyscurrentkey{\pgfkeyscurrentkey}%
% 		\noexpand\def\noexpand\pgfkeyscurrentkeyRAW{\pgfkeyscurrentkeyRAW}%
% 		\noexpand\def\noexpand\pgfkeyscurrentname{\pgfkeyscurrentname}%
% 		\noexpand\def\noexpand\pgfkeyscurrentvalue{\pgfkeyscurrentvalue}%
% 		\noexpand\pgfkeys@pathtoks={\pgfkeyscurrentpath}%
% 	}%
% 	\pgfkeysinterruptkeyfilter
% 	\let\pgfkeys@case@one=\pgfkeys@eval@key@filter@subroutine@case@one
% 	\pgfkeysalso{#1}%
% 	\endpgfkeysinterruptkeyfilter% this here also restored \pgfkeys@case@one.
% 	\pgfkeys@eval@key@filter@subroutine@restorestate
% }%
%-------------------------------------------------- 


% Evaluates a key filter '#1'. Example:
% \pgfkeysevalkeyfilterwith{/pgf/key filters/equals=/tikz}
%
% \pgfkeysevalkeyfilterwith works only if key filtering is
% active.
%
% The argument '#1' MUST be a FULL KEY.
%
% The implementation employs a subset of the \pgfkeysalso code.
\def\pgfkeysevalkeyfilterwith#1{%
	\pgfkeys@eval@key@filter@subroutine@unpack#1=\pgfkeysnovalue=\pgfkeys@stop
}%
\def\pgfkeys@eval@key@filter@subroutine@unpack#1=#2=#3\pgfkeys@stop{%
	\pgfkeys@spdef\pgfkeyspred@TMP{#1}%
	\edef\pgfkeyspred@TMP{\pgfkeyspred@TMP}%
	\pgfkeys@spdef\pgfkeyspred@TMPB{#2}% TMPB=value
	\ifx\pgfkeyspred@TMPB\pgfkeysnovalue@text% Hmm... no value
		\pgfkeysifdefined{\pgfkeyspred@TMP/.@def}%
		{\pgfkeysgetvalue{\pgfkeyspred@TMP/.@def}{\pgfkeyspred@TMPB}}
		{}% no default, so leave it
	\fi%
	\ifx\pgfkeyspred@TMPB\pgfkeysvaluerequired%
		\pgfkeysvalueof{/errors/value required/.@cmd}\pgfkeyspred@TMP\pgfkeyspred@TMPB\pgfeov%
	\else%
		\pgfkeysifdefined{\pgfkeyspred@TMP/.@cmd}{%
			\pgfkeysgetvalue{\pgfkeyspred@TMP/.@cmd}{\pgfkeys@code}%
			\expandafter\pgfkeys@code\pgfkeyspred@TMPB\pgfeov
		}{%
			\pgfkeysvalueof{/errors/no such key filter/.@cmd}\pgfkeyspred@TMP\pgfkeyspred@TMPB\pgfeov%
		}%
	\fi%
}


\def\pgfkeys@nevermind#1\relax{\let\pgfkeyscurrentkeyRAW=\pgfkeyscurrentkey}
\def\pgfkeys@addpath#1\relax{\def\pgfkeyscurrentkeyRAW{#1}% old @addpath:	
	\edef\pgfkeyscurrentkey{\pgfkeysdefaultpath#1}%
}

\def\pgfkeys@non@outer@newif@#1#2{%
	\expandafter\edef\csname #2true\endcsname{\noexpand\let\noexpand#1=\noexpand\iftrue}%
	\expandafter\edef\csname #2false\endcsname{\noexpand\let\noexpand#1=\noexpand\iffalse}%
	\csname #2false\endcsname
}%

% For latex and context, this here has the same effect as a \newif
% applied to 'if#1'. For plain tex, it has also the same effect, but
% it is not an \outer macro as the plain-tex \newif.
\def\pgfkeys@non@outer@newif#1{%
	\expandafter\pgfkeys@non@outer@newif@\csname if#1\endcsname{#1}%
}
\endinput


==> pgfplotsoldpgfsupp_pgflibraryplothandlers.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgfplots/pgfplots/generic/pgfplots/oldpgfcompatib/pgfplotsoldpgfsupp_pgflibraryplothandlers.code.tex,v 1.3 2008/06/07 17:08:33 ludewich Exp $

\newif\ifpgf@plot@started


% This handler converts each plot stream command into a curveto
% command, except for the first, which is converted to the previously
% specified action.
%
% Example:
%
% \pgfpathmoveto{\pgfpointorigin}
% \pgfsetlinetofirstplotpoint
% \pgfplothandlercurveto
% \pgfplotxyfile{mytable}

\def\pgfplothandlercurveto{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@curveto@handler@initial%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\pgf@plot@curveto@handler@finish%
    \global\pgf@plot@startedfalse%
  }%
}

\def\pgf@plot@curveto@handler@initial#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@plot@first@action{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \xdef\pgf@plot@curveto@first{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
  \global\let\pgf@plot@curveto@first@support=\pgf@plot@curveto@first%
  \global\let\pgf@plotstreampoint=\pgf@plot@curveto@handler@second%
}

\def\pgf@plot@curveto@handler@second#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@curveto@second{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \global\let\pgf@plotstreampoint=\pgf@plot@curveto@handler@third%
  \global\pgf@plot@startedtrue%
}

\def\pgf@plot@curveto@handler@third#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@curveto@current{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  % compute difference vector:
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{\pgf@plot@curveto@first}
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  % compute support directions:
  \pgf@xa=\pgf@plottension\pgf@xa%
  \pgf@ya=\pgf@plottension\pgf@ya%
  % first marshal:
  \pgf@process{\pgf@plot@curveto@second}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xb by-\pgf@xa%
  \advance\pgf@yb by-\pgf@ya%
  \advance\pgf@xc by\pgf@xa%
  \advance\pgf@yc by\pgf@ya%
  \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgf@plot@curveto@first@support}%
    {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgf@plot@curveto@second}}%
  {\pgf@marshal}%
  % Prepare next:
  \global\let\pgf@plot@curveto@first=\pgf@plot@curveto@second%
  \global\let\pgf@plot@curveto@second=\pgf@plot@curveto@current%
  \xdef\pgf@plot@curveto@first@support{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
}

\def\pgf@plot@curveto@handler@finish{%
  \ifpgf@plot@started%
    \pgfpathcurveto{\pgf@plot@curveto@first@support}{\pgf@plot@curveto@second}{\pgf@plot@curveto@second}%
  \fi%
}


% This commands sets the tension for smoothing of plots.
%
% #1 = tension of curves. A value of 1 will yield a circle when the
%      control points are at quarters of a circle. A smaller value
%      will result in a tighter curve. Default is 0.5. 
%
% Example:
%
% \pgfsetplottension{0.2}

\def\pgfsetplottension#1{%
  \pgf@x=#1pt\relax%
  \pgf@x=0.2775\pgf@x\relax%
  \edef\pgf@plottension{\pgf@sys@tonumber\pgf@x}}
\pgfsetplottension{0.5}


% This handler converts the plot stream command into a curveto
% command that is closed using a closepath.
%
% Example:
%
% \pgfpathmoveto{\pgfpointorigin}
% \pgfplothandlerclosedcurve
% \pgfplotxyfile{mytable}

\def\pgfplothandlerclosedcurve{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@closedcurve@handler@initial%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\pgf@plot@closedcurve@handler@finish%
  }%
}

\def\pgf@plot@closedcurve@handler@initial#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \xdef\pgf@plot@closedcurve@initial{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
  \global\let\pgf@plotstreampoint=\pgf@plot@closedcurve@handler@second%
  \global\pgf@plot@startedfalse%
}

\def\pgf@plot@closedcurve@handler@second#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@closedcurve@after@initial{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  {\pgfpathmoveto{}}%
  \global\let\pgf@plotstreampoint=\pgf@plot@closedcurve@handler@third%
}

\def\pgf@plot@closedcurve@handler@third#1{%
  \global\pgf@plot@startedtrue%
  \pgf@process{#1}%
  \xdef\pgf@plot@closedcurve@current{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  % compute difference vector:
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{\pgf@plot@closedcurve@initial}
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  % compute support directions:
  \pgf@xa=\pgf@plottension\pgf@xa%
  \pgf@ya=\pgf@plottension\pgf@ya%
  % first marshal:
  \pgf@process{\pgf@plot@closedcurve@after@initial}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xb by-\pgf@xa%
  \advance\pgf@yb by-\pgf@ya%
  \advance\pgf@xc by\pgf@xa%
  \advance\pgf@yc by\pgf@ya%
  \global\let\pgf@plot@closedcurve@first=\pgf@plot@closedcurve@after@initial%
  \global\let\pgf@plot@closedcurve@second=\pgf@plot@closedcurve@current%
  \xdef\pgf@plot@closedcurve@after@initial@presupport{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
  \xdef\pgf@plot@closedcurve@first@support{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
  \global\let\pgf@plotstreampoint=\pgf@plot@closedcurve@handler@fourth%
}

\def\pgf@plot@closedcurve@handler@fourth#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@closedcurve@current{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  % compute difference vector:
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{\pgf@plot@closedcurve@first}
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  % compute support directions:
  \pgf@xa=\pgf@plottension\pgf@xa%
  \pgf@ya=\pgf@plottension\pgf@ya%
  % first marshal:
  \pgf@process{\pgf@plot@closedcurve@second}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xb by-\pgf@xa%
  \advance\pgf@yb by-\pgf@ya%
  \advance\pgf@xc by\pgf@xa%
  \advance\pgf@yc by\pgf@ya%
  \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgf@plot@closedcurve@first@support}%
    {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgf@plot@closedcurve@second}}%
  {\pgf@marshal}%
  % Prepare next:
  \global\let\pgf@plot@closedcurve@first=\pgf@plot@closedcurve@second%
  \global\let\pgf@plot@closedcurve@second=\pgf@plot@closedcurve@current%
  \xdef\pgf@plot@closedcurve@first@support{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
}

\def\pgf@plot@closedcurve@handler@finish{%
  \ifpgf@plot@started
    %
    % first, draw line from 2nd last to last:
    %
    \pgf@process{\pgf@plot@closedcurve@initial}%
    % compute difference vector:
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\pgf@plot@closedcurve@first}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    % compute support directions:
    \pgf@xa=\pgf@plottension\pgf@xa%
    \pgf@ya=\pgf@plottension\pgf@ya%
    % first marshal:
    \pgf@process{\pgf@plot@closedcurve@second}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \advance\pgf@xb by-\pgf@xa%
    \advance\pgf@yb by-\pgf@ya%
    \advance\pgf@xc by\pgf@xa%
    \advance\pgf@yc by\pgf@ya%
    \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgf@plot@closedcurve@first@support}%
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgf@plot@closedcurve@second}}%
    {\pgf@marshal}%
    \xdef\pgf@plot@closedcurve@first@support{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    %
    % second, draw line from last point to start:
    %
    \pgf@process{\pgf@plot@closedcurve@after@initial}%
    % compute difference vector:
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\pgf@plot@closedcurve@second}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    % compute support directions:
    \pgf@xa=\pgf@plottension\pgf@xa%
    \pgf@ya=\pgf@plottension\pgf@ya%
    % first marshal:
    \pgf@process{\pgf@plot@closedcurve@initial}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \advance\pgf@xb by-\pgf@xa%
    \advance\pgf@yb by-\pgf@ya%
    \advance\pgf@xc by\pgf@xa%
    \advance\pgf@yc by\pgf@ya%
    \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgf@plot@closedcurve@first@support}%
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgf@plot@closedcurve@initial}}%
    {\pgf@marshal}%
    %
    % third, draw line from first to second point:
    %
    \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      {\noexpand\pgf@plot@closedcurve@after@initial@presupport}{\noexpand\pgf@plot@closedcurve@after@initial}}%
    {\pgf@marshal}%
    \pgfpathclose%
  \fi%
}





% This handler converts each point in a stream into a line from the
% $y$-axis to the given points coordinate, resulting in a
% ``comb.'' 
%
% Example:
%
% \pgfplothandlerxcomb
% \pgfplotxyfile{mytable}

\def\pgfplothandlerxcomb{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@xcomb@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\pgfplotxzerolevelstreamend%
	\pgfplotxzerolevelstreamstart
  }%
}

\def\pgf@plot@xcomb@handler#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \begingroup
  \pgfplotxzerolevelstreamnext
  \endgroup
  \pgf@yb=\pgf@x
  \pgfpathmoveto{\pgfqpoint{\pgf@yb}{\pgf@ya}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
}


% This handler converts each point in a stream into a line from the
% $x$-axis straight up to the given points coordinate, resulting in a
% ``comb.'' 
%
% Example:
%
% \pgfplothandlerycomb
% \pgfplotxyfile{mytable}

\def\pgfplothandlerycomb{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@ycomb@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\pgfplotyzerolevelstreamend%
	\pgfplotyzerolevelstreamstart
  }%
}

\def\pgf@plot@ycomb@handler#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \begingroup
  \pgfplotyzerolevelstreamnext
  \endgroup
  \pgf@yb=\pgf@x
  \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
}

% PGF Bar or comb plots usually draw something from zero to the current plot's coordinate.
% 
% The 'zero' offset can be changed using an input stream.
%
% There are two such streams which can be configured independently.
% The first one returns "zeros" for coordinate x, the second one
% returns "zeros" for coordinate y.
% 
% \pgfplotxzerolevelstreamstart
% \pgfplotxzerolevelstreamnext % assigns \pgf@x globally
% \pgfplotxzerolevelstreamnext
% \pgfplotxzerolevelstreamnext
% \pgfplotxzerolevelstreamend
%
% and 
% \pgfplotyzerolevelstreamstart
% \pgfplotyzerolevelstreamnext % assigns \pgf@x globally
% \pgfplotyzerolevelstreamend
%
\def\pgfplotxzerolevelstreamstart{\pgf@plotxzerolevelstreamstart}%
\def\pgfplotxzerolevelstreamend{\pgf@plotxzerolevelstreamend}%
\def\pgfplotxzerolevelstreamnext{\pgf@plotxzerolevelstreamnext}
\def\pgfplotyzerolevelstreamstart{\pgf@plotyzerolevelstreamstart}%
\def\pgfplotyzerolevelstreamend{\pgf@plotyzerolevelstreamend}%
\def\pgfplotyzerolevelstreamnext{\pgf@plotyzerolevelstreamnext}

% This zero level stream always returns '#1' (a dimension).
\def\pgfplotxzerolevelstreamconstant#1{%
	\edef\pgfplotxzerolevelstreamconstant@val{#1}%
	\def\pgf@plotxzerolevelstreamstart{%
		\global\let\pgf@plotxzerolevelstreamend=\relax
		\gdef\pgf@plotxzerolevelstreamnext{\global\pgf@x=\pgfplotxzerolevelstreamconstant@val\relax}%
	}%
}%
\pgfplotxzerolevelstreamconstant{0pt}%

% This zero level stream always returns '#1'.
\def\pgfplotyzerolevelstreamconstant#1{%
	\edef\pgfplotyzerolevelstreamconstant@val{#1}%
	\def\pgf@plotyzerolevelstreamstart{%
		\global\let\pgf@plotyzerolevelstreamend=\relax
		\gdef\pgf@plotyzerolevelstreamnext{\global\pgf@x=\pgfplotyzerolevelstreamconstant@val\relax}%
	}%
}%
\pgfplotyzerolevelstreamconstant{0pt}%

\def\pgfplotbarwidth{\pgfkeysvalueof{/pgf/bar width}}

\pgfqkeys{/pgf}{%
	bar width/.initial=10pt,
	bar shift/.initial=0pt,
	bar interval width/.initial=1,
	bar interval shift/.initial=0.5,
}

% This handler places a rectangle at each point in the plot stream, a
% rectangle which touches the x-axis at one end and the current point
% at the other end:
%    --(X)--
%    |     |
%    |     |
%    |     |
%    --(0)--
% Example:
%
% \pgfplothandlerybar
% \pgfplotxyfile{mytable}
\def\pgfplothandlerybar{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@ybar@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\pgfplotyzerolevelstreamend%
	\pgfmathparse{\pgfplotbarwidth}%
	\xdef\pgfplotbarwidth@{\pgfmathresult pt}%
	\pgfmathparse{\pgfkeysvalueof{/pgf/bar shift}}%
	\xdef\pgfplotbarshift@{\pgfmathresult pt}%
	\pgfplotyzerolevelstreamstart
  }%
}

\def\pgf@plot@ybar@handler#1{%
  \pgf@process{#1}%
  \pgf@ya=\pgf@y
  \expandafter\pgf@xb\pgfplotbarwidth@\relax
  \pgf@xc=\pgf@x
  \advance\pgf@xc by-.5\pgf@xb
  \advance\pgf@xc by\pgfplotbarshift@\relax
  \begingroup
  \pgfplotyzerolevelstreamnext
  \endgroup
  \pgf@yb=\pgf@x
  \advance\pgf@ya by-\pgf@yb
  \pgfpathrectangle
	{\pgfqpoint{\pgf@xc}{\pgf@yb}}%
	{\pgfqpoint{\pgf@xb}{\pgf@ya}}%
}

% This handler places a rectangle at each point in the plot stream, a
% rectangle which touches the y-axis at one end and the current point
% at the other end:
%    ---------
%    |       |
%   (0)     (X)
%    |       |
%    ---------
% Example:
%
% \pgfplothandlerxbar
% \pgfplotxyfile{mytable}
\def\pgfplothandlerxbar{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@xbar@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\pgfplotxzerolevelstreamend%
	\pgfmathparse{\pgfplotbarwidth}%
	\xdef\pgfplotbarwidth@{\pgfmathresult pt}%
	\pgfmathparse{\pgfkeysvalueof{/pgf/bar shift}}%
	\xdef\pgfplotbarshift@{\pgfmathresult pt}%
	\pgfplotxzerolevelstreamstart
  }%
}

\def\pgf@plot@xbar@handler#1{%
  \pgf@process{#1}%
  \pgf@ya=\pgf@x
  \expandafter\pgf@xb\pgfplotbarwidth@\relax
  \pgf@xc=\pgf@y
  \advance\pgf@xc by-.5\pgf@xb
  \advance\pgf@xc by\pgfplotbarshift@\relax
  \begingroup
  \pgfplotxzerolevelstreamnext
  \endgroup
  \pgf@yb=\pgf@x
  \advance\pgf@ya by-\pgf@yb
  \pgfpathrectangle
	{\pgfqpoint{\pgf@yb}{\pgf@xc}}%
	{\pgfqpoint{\pgf@ya}{\pgf@xb}}%
}

% This handler is a variant of \pgfplothandlerybar which works with
% intervals instead of points.
% 
% Bars are drawn between successive input coordinates and the width is
% determined relatively to the interval length.
%
% It looks like this:
%
%    |---|      |-----| 
%    |   |      |     |    
%    |   |      |     |     
%    |   |      |     |       
% (X)------(X)-----------(X)
%
% where (X) denotes the x-axis offsets of input coordinates.
%
% In more detail, if (x_i,y_i) and (x_{i+1},y_{i+1}) denote successive
% input coordinates, the bar will be placed above the
% interval [x_i,x_{i+1}], centered at
%
%    x_i + \pgfkeysvalueof{/pgf/bar interval shift} * (x_{i+1} - x_i)
%
% with width
%
%    \pgfkeysvalueof{/pgf/bar interval width} * (x_{i+1} - x_i).
%
% If you have N+1 input points, you will get N bars (one for each
% interval). The y_i value of the last bar will be ignored.
%
% Example:
%
% \pgfplothandlerybarinterval
% \pgfplotxyfile{mytable}
\def\pgfplothandlerybarinterval{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@ybarinterval@handler@first%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\pgfplotyzerolevelstreamend%
	\pgfmathparse{\pgfkeysvalueof{/pgf/bar interval width}}%
	\xdef\pgfplotbarintervalwidth@{\pgfmathresult}%
	\pgfmathparse{\pgfkeysvalueof{/pgf/bar interval shift}}%
	\xdef\pgfplotbarintervalshift@{\pgfmathresult}%
	\pgfplotyzerolevelstreamstart
  }%
}

\def\pgf@plot@ybarinterval@handler@first#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@barinterval@intervalstart{\the\pgf@x}%
  \xdef\pgf@plot@barinterval@bar{\the\pgf@y}%
  \global\let\pgf@plotstreampoint=\pgf@plot@ybarinterval@handler%
}
\def\pgf@plot@ybarinterval@handler#1{%
  \pgf@process{#1}%
  \pgf@ya=\pgf@plot@barinterval@bar
  \xdef\pgf@plot@barinterval@bar{\the\pgf@y}%
  \pgf@xc=\pgf@plot@barinterval@intervalstart\relax
  \xdef\pgf@plot@barinterval@intervalstart{\the\pgf@x}%
  \pgf@xb=\pgf@x
  \advance\pgf@xb by-\pgf@xc
  \advance\pgf@xc by\pgfplotbarintervalshift@\pgf@xb
  \pgf@xb=\pgfplotbarintervalwidth@\pgf@xb
  \advance\pgf@xc by-.5\pgf@xb% center
  \begingroup
  \pgfplotyzerolevelstreamnext
  \endgroup
  \pgf@yb=\pgf@x
  \advance\pgf@ya by-\pgf@yb
  \pgfpathrectangle
	{\pgfqpoint{\pgf@xc}{\pgf@yb}}%
	{\pgfqpoint{\pgf@xb}{\pgf@ya}}%
}

% Like \pgfplothandlerybarinterval but for xbar.
\def\pgfplothandlerxbarinterval{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@xbarinterval@handler@first%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\pgfplotxzerolevelstreamend%
	\pgfmathparse{\pgfkeysvalueof{/pgf/bar interval width}}%
	\xdef\pgfplotbarintervalwidth@{\pgfmathresult}%
	\pgfmathparse{\pgfkeysvalueof{/pgf/bar interval shift}}%
	\xdef\pgfplotbarintervalshift@{\pgfmathresult}%
	\pgfplotxzerolevelstreamstart
  }%
}

\def\pgf@plot@xbarinterval@handler@first#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@barinterval@intervalstart{\the\pgf@y}%
  \xdef\pgf@plot@barinterval@bar{\the\pgf@x}%
  \global\let\pgf@plotstreampoint=\pgf@plot@xbarinterval@handler%
}
\def\pgf@plot@xbarinterval@handler#1{%
  \pgf@process{#1}%
  \pgf@ya=\pgf@plot@barinterval@bar
  \xdef\pgf@plot@barinterval@bar{\the\pgf@x}%
  \pgf@xc=\pgf@plot@barinterval@intervalstart\relax
  \xdef\pgf@plot@barinterval@intervalstart{\the\pgf@y}%
  \pgf@xb=\pgf@y
  \advance\pgf@xb by-\pgf@xc
  \advance\pgf@xc by\pgfplotbarintervalshift@\pgf@xb
  \pgf@xb=\pgfplotbarintervalwidth@\pgf@xb
  \advance\pgf@xc by-.5\pgf@xb% center
  \begingroup
  \pgfplotxzerolevelstreamnext
  \endgroup
  \pgf@yb=\pgf@x
  \advance\pgf@ya by-\pgf@yb
  \pgfpathrectangle
	{\pgfqpoint{\pgf@yb}{\pgf@xc}}%
	{\pgfqpoint{\pgf@ya}{\pgf@xb}}%
}


% This handler is very similar to \pgfplothandlerlineto, but it
% produces CONSTANT connected pieces of the form
%
%          x
%          |
%   x---   |
%   |  x----
% x-|
%
% Example:
%
% \pgfplothandlerconstantlineto
% \pgfplotxyfile{mytable}
\def\pgfplothandlerconstantlineto{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@const@line@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\relax%
  }%
}
\def\pgf@plot@const@line@handler#1{%
  \pgf@plot@first@action{#1}%
  \xdef\pgf@plot@const@line@handler@last{\the\pgf@y}%
  \global\let\pgf@plotstreampoint=\pgf@plot@const@line@handler@@%
}
\def\pgf@plot@const@line@handler@@#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x
  \pgf@ya=\pgf@y
  \expandafter\pgf@yb\pgf@plot@const@line@handler@last
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \xdef\pgf@plot@const@line@handler@last{\the\pgf@ya}%
}

% A variant of \pgfplothandlerconstantlineto which places its mark on
% the right line ends.
% 
%       |---x
% ---x  |
%    |--x
% x
%
% Example:
%
% \pgfplothandlerconstantlinetomarkright
% \pgfplotxyfile{mytable}
\def\pgfplothandlerconstantlinetomarkright{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@const@line@mark@right@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\relax%
  }%
}
\def\pgf@plot@const@line@mark@right@handler#1{%
  \pgf@plot@first@action{#1}%
  \xdef\pgf@plot@const@line@handler@last{\the\pgf@x}%
  \global\let\pgf@plotstreampoint=\pgf@plot@const@line@mark@right@handler@@%
}
\def\pgf@plot@const@line@mark@right@handler@@#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x
  \pgf@ya=\pgf@y
  \expandafter\pgf@yb\pgf@plot@const@line@handler@last
  \pgfpathlineto{\pgfqpoint{\pgf@yb}{\pgf@ya}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \xdef\pgf@plot@const@line@handler@last{\the\pgf@xa}%
}

% This handler is in fact a variant of \pgfplothandlerconstantlineto,
% but it does not draw vertical lines. It produces a sequence of
% line-to and move-to operations such that plot marks are placed at
% each right end:
%
%          ---x
%   ---x   
%       ---x
% --x
%
% Example:
%
% \pgfplothandlerjumpmarkright
% \pgfplotxyfile{mytable}
\def\pgfplothandlerjumpmarkright{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@jumpmarkright@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\relax%
  }%
}
\def\pgf@plot@jumpmarkright@handler#1{%
  \pgf@plot@first@action{#1}%
  \xdef\pgf@plot@const@line@handler@last{\the\pgf@x}%
  \global\let\pgf@plotstreampoint=\pgf@plot@jumpmarkright@handler@@%
}
\def\pgf@plot@jumpmarkright@handler@@#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x
  \pgf@ya=\pgf@y
  \expandafter\pgf@yb\pgf@plot@const@line@handler@last
  \pgfpathmoveto{\pgfqpoint{\pgf@yb}{\pgf@ya}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \xdef\pgf@plot@const@line@handler@last{\the\pgf@xa}%
}

% This handler is in fact a variant of \pgfplothandlerconstantlineto,
% but it does not draw vertical lines. It produces a sequence of
% line-to and move-to operations such that plot marks are placed at
% each left end:
%
%          x---
%   x---   
%       x---
% x--
%
% Example:
%
% \pgfplothandlerjumpmarkleft
% \pgfplotxyfile{mytable}
\def\pgfplothandlerjumpmarkleft{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@jumpmarkleft@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\relax%
  }%
}
\def\pgf@plot@jumpmarkleft@handler#1{%
  \pgf@plot@first@action{#1}%
  \xdef\pgf@plot@const@line@handler@last{\the\pgf@y}%
  \global\let\pgf@plotstreampoint=\pgf@plot@jumpmarkleft@handler@@%
}
\def\pgf@plot@jumpmarkleft@handler@@#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x
  \pgf@ya=\pgf@y
  \expandafter\pgf@yb\pgf@plot@const@line@handler@last
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}%
  \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \xdef\pgf@plot@const@line@handler@last{\the\pgf@ya}%
}



% This handler converts each point in a stream into a line from the
% origin to the point's coordinate, resulting in a ``star''.
%
% Example:
%
% \pgfplothandlerpolarcomb
% \pgfplotxyfile{mytable}

\def\pgfplothandlerpolarcomb{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@polarcomb@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\relax%
  }%
}

\def\pgf@plot@polarcomb@handler#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgfpathmoveto{\pgfpointorigin}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
}




% This handler draws a given mark at each point. 
%
% #1 = some code to be executed at each point (with the coordinate
%      system translated to that point).
%      Typically, this code will be \pgfuseplotmark{whatever}.
%
% Example:
%
% \pgfplothandlermark{\pgfuseplotmark{*}}
% \pgfplotxyfile{mytable}

\def\pgfplothandlermark#1{%
  \pgf@plothandlermark{%
    \ifnum\pgf@plot@mark@count<\pgf@plot@mark@repeat\relax%
    \else%
      \global\pgf@plot@mark@count=0\relax%
      #1%
    \fi%
    }%
}

\newcount\pgf@plot@mark@count
\def\pgf@plot@mark@phase{0}

\def\pgf@plothandlermark#1{%
  \def\pgf@plot@mark{#1}%
  \def\pgf@plotstreamstart{%
    \global\pgf@plot@mark@count=\pgf@plot@mark@repeat\relax%
    \global\advance\pgf@plot@mark@count by-\pgf@plot@mark@phase\relax%
    \global\let\pgf@plotstreampoint=\pgf@plot@mark@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\relax%
  }%
}

\def\pgf@plot@mark@handler#1{%
  \global\advance\pgf@plot@mark@count by1\relax%
  {\pgftransformshift{#1}\pgf@plot@mark}%
}


% Set the repeat count for marks. For example, if 3 is given as a
% value, only every third point will get a mark.
%
% #1 = repeat count
%
% Example:
%
% \pgfsetplotmarkrepeat{2}

\def\pgfsetplotmarkrepeat#1{\def\pgf@plot@mark@repeat{#1}}
\pgfsetplotmarkrepeat{1}


% Set the phase for marks. For example, if 3 is the repeat and 3 is 
% the phase, already the first point will be marked. 
%
% #1 = the index of the first point that should be marked.
%
% Example:
%
% \pgfsetplotmarkphase{3}

\def\pgfsetplotmarkphase#1{\def\pgf@plot@mark@phase{#1}}
\pgfsetplotmarkphase{1}



% This handler draws a given mark at those points whose number is
% given in the (pgffor-like) list.
%
% #1 = some code to be executed at each point (with the coordinate
%      system translated to that point).
%      Typically, this code will be \pgfuseplotmark{whatever}.
% #2 = list of positions like "1,2,4,...,9,10"
%
% Example:
%
% \pgfplothandlermarklisted{\pgfuseplotmark{*}}{1,2,4,...,9}
% \pgfplotxyfile{mytable}

\def\pgfplothandlermarklisted#1#2{%
  \let\pgf@plot@mark@list=\pgfutil@empty%
  \edef\pgf@marshal{\noexpand\foreach\noexpand\pgf@temp in{#2}}
  \pgf@marshal{\xdef\pgf@plot@mark@list{\pgf@plot@mark@list(\pgf@temp)}}%
  \pgf@plothandlermark{%
    \edef\pgf@marshal{\noexpand\pgfutil@in@{(\the\pgf@plot@mark@count)}{\pgf@plot@mark@list}}%
    \pgf@marshal%
    \ifpgfutil@in@#1\fi}%
}


% Define a new plot mark for use with \pgfplotmark.
%
% #1 = a plot mark mnemonic
% #2 = code for drawing the mark
%
% Example:
%
% \pgfdeclareplotmark{*}{\pgfpathcircle{\pgfpointorigin}{2pt}\pgfusepathqfill}

\def\pgfdeclareplotmark#1#2{\expandafter\def\csname pgf@plot@mark@#1\endcsname{#2}}


% Set the size of plot marks. For circles, this will be the radius,
% for other shapes it should be about half the width/height.
%
% Example:
%
% \pgfsetplotmarksize{1pt}

\def\pgfsetplotmarksize#1{\pgfmathsetlength\pgfplotmarksize{#1}}

\newdimen\pgfplotmarksize
\pgfplotmarksize=2pt


% Insert a plot mark's code at the origin.
%
% #1 = plot mark mnemonic
%
% Example:
%
% \pgfuseplotmark{*}

\def\pgfuseplotmark#1{\csname pgf@plot@mark@#1\endcsname}


% A stroke-filled circle mark

\pgfdeclareplotmark{*}
{%
  \pgfpathcircle{\pgfpointorigin}{\pgfplotmarksize}
  \pgfusepathqfillstroke
}


% A plus-sign like mark

\pgfdeclareplotmark{+}
{%
  \pgfpathmoveto{\pgfqpoint{-\pgfplotmarksize}{0pt}}
  \pgfpathlineto{\pgfqpoint{\pgfplotmarksize}{0pt}}
  \pgfpathmoveto{\pgfqpoint{0pt}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{0pt}{-\pgfplotmarksize}}
  \pgfusepathqstroke
}


% An x-shaped mark

\pgfdeclareplotmark{x}
{%
  \pgfpathmoveto{\pgfqpoint{-.70710678\pgfplotmarksize}{-.70710678\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{.70710678\pgfplotmarksize}{.70710678\pgfplotmarksize}}
  \pgfpathmoveto{\pgfqpoint{-.70710678\pgfplotmarksize}{.70710678\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{.70710678\pgfplotmarksize}{-.70710678\pgfplotmarksize}}
  \pgfusepathqstroke
}

% See pgflibraryplotmarks for more plot marks






\endinput


==> pgfplotsoldpgfsupp_pgfmathfloat.code.tex <==
% Copyright 2008 by Christian Feuersaenger
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.
%
% This file contains methods for basic floating point arithmetics, rounding
% to arbitrary precision and number pretty printing.
%
% Version 0.9.4 2008/03/18

\global\newif\ifpgfmathfloatcomparison
\newif\ifpgfmathfloatroundhasperiod
\newif\ifpgfmathprintnumberskipzeroperiod


% used internally in grouped macros:
\toksdef\pgfmathfloat@tmptoks=1
\newif\ifpgfmathfloat@fixed@digits@after@period
\newif\ifpgfmathfloatroundmayneedrenormalize
\toksdef\pgfmathfloat@a@Mtok=0

%% WARNING: avoid conflicting register names!
\let\pgfmathfloat@a@S=\c@pgf@counta
\let\pgfmathfloat@a@M=\pgf@xa
\let\pgfmathfloat@a@E=\c@pgf@countb
\let\pgfmathfloat@b@S=\c@pgf@countc
\let\pgfmathfloat@b@M=\pgf@xb
\let\pgfmathfloat@b@E=\c@pgf@countd

% can be changed with options.
\def\pgfmathfloat@round@precision{2}

\gdef\pgfmathfloat@glob@TMP{}


% Computes a normalised floating point representation for #1 of the
% form
%   [FLAGS] MANTISSE EXPONENT
% meaning
%   [+-]X.XXXXXXX*10^C
% where 
%   X.XXXXXX is a mantisse with first number != 0, C is an integer and
% FLAGS contains the sign and some other special cases.
%
% This method does NOT use TeX Registers to represent the numbers! The
% computation is COMPLETELY STRING BASED.
% This allows numbers such at 10000000 or 5.23e-10 to be represented
% properly, although TeX-registers would produce overflow/underflow
% errors in these cases. 
%
% It is to be used to compute logs, because log(X*10^Y) = log(X) + log(10)*Y
%
% Arguments:
% #1:  an arbitrary number which shall be parsed. Maybe a macro.
%     Examples:
%     [+-]XXXXX.XXXXXX
%     [+-]XXXXX.XXXXXXeXXXX
%     [+-]0.0000XXXXXX
%     [+-]0.0000XXXXXXeXXXX
%     [+-]inf
%     nan
%    Maybe a macro containing such a number.
%
% Return value:
% \pgfmathresult will be \def'ed to
%  FLAGS MANTISSE 'e' EXPONENT
% where
% FLAGS is a number in [0-5] where
% 		0 == '0' (the number is +- 0.0),
% 		1 == '+', 
% 		2 == '-',
% 		3 == 'not a number'
% 		4 == '+ infinity'
% 		5 == '- infinity'
%
% MANTISSE is a normalised number 1 <= M < 10. It always contains a
% period and at least one digit after the period.
%
% EXPONENT is an integer value.
%
% Example:
% \pgfmathfloatparsenumber{1}
% -> \pgfmathresult = 11.0e0
% \pgfmathfloatparsenumber{141.212}
% -> \pgfmathresult = 11.41212e2
\def\pgfmathfloatparsenumber#1{%
	\begingroup
	\edef\pgfmathresult{#1}%
	\expandafter\pgfmathfloatparsenumber@impl\pgfmathresult\pgfmathfloat@EOI
	\ifpgfmathfloatparsenumberpendingperiod
		\pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok.0}%
	\fi
	\edef\pgfmathresult{%
		\the\pgfmathfloat@a@S\the\pgfmathfloat@a@Mtok e\the\pgfmathfloat@a@E}%
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}

% The same as \pgfmathfloatparsenumber, but does not perform sanity checking.
\def\pgfmathfloatqparsenumber#1{%
	\begingroup
	\let\pgfmathfloatparsenumber@sanitize@digit=\relax
	\edef\pgfmathresult{#1}%
	\expandafter\pgfmathfloatparsenumber@impl\pgfmathresult\pgfmathfloat@EOI
	\ifpgfmathfloatparsenumberpendingperiod
		\pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok.0}%
	\fi
	\edef\pgfmathresult{%
		\the\pgfmathfloat@a@S\the\pgfmathfloat@a@Mtok e\the\pgfmathfloat@a@E}%
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}


% decomposes a lowlevel floating point representation into flags,
% mantisse and exponent.
%
% #4: integer register for the flags.
% #5: dimen registers for the mantisse.
% #6: integer register for the exponent.
\def\pgfmathfloat@decompose#1#2e#3\relax#4#5#6{%
   #4=#1\relax
   #5=#2pt%
   #6=#3\relax%
}
% overloaded, #5 needs to be a token register for the mantisse.
\def\pgfmathfloat@decompose@tok#1#2e#3\relax#4#5#6{%
   #4=#1\relax
   #5={#2}%
   #6=#3\relax%
}
% overloaded, returns only ONE of the three components into #4:
\def\pgfmathfloat@decompose@F#1#2e#3\relax#4{#4=#1\relax}%
\def\pgfmathfloat@decompose@M#1#2e#3\relax#4{#4=#2pt}%
\def\pgfmathfloat@decompose@Mtok#1#2e#3\relax#4{#4={#2}}%
\def\pgfmathfloat@decompose@E#1#2e#3\relax#4{#4=#3\relax}%

% Takes a floating point number #1 as input and writes flags to macro
% #2, mantisse to macro #3 and exponent to macro #4.
\def\pgfmathfloattomacro#1#2#3#4{%
	\begingroup
	\expandafter\pgfmathfloat@decompose@tok#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
	\xdef\pgfmathfloat@glob@TMP{%
		\noexpand\def\noexpand#2{\the\pgfmathfloat@a@S}%
		\noexpand\def\noexpand#3{\the\pgfmathfloat@a@Mtok}%
		\noexpand\def\noexpand#4{\the\pgfmathfloat@a@E}%
	}%
	\endgroup
	\pgfmathfloat@glob@TMP
}

% Takes a floating point number #1 as input and writes flags to count
% register #2, mantisse to dimen register #3 and exponent to count
% register #4.
\def\pgfmathfloattoregisters#1#2#3#4{%
	\expandafter\pgfmathfloat@decompose#1\relax{#2}{#3}{#4}%
}

% the same, but writes the mantisse into a token register.
\def\pgfmathfloattoregisterstok#1#2#3#4{%
	\expandafter\pgfmathfloat@decompose@tok#1\relax{#2}{#3}{#4}%
}

% Extracts the flags of #1 into the count register #2.
\def\pgfmathfloatgetflags#1#2{%
	\expandafter\pgfmathfloat@decompose@F#1\relax{#2}%
}
% Extracts the mantisse of #1 into the dimen register #2.
\def\pgfmathfloatgetmantisse#1#2{%
	\expandafter\pgfmathfloat@decompose@M#1\relax{#2}%
}
% Extracts the mantisse of #1 into the token register #2.
\def\pgfmathfloatgetmantissetok#1#2{%
	\expandafter\pgfmathfloat@decompose@Mtok#1\relax{#2}%
}
% Extracts the exponent of #1 into the count register #2.
\def\pgfmathfloatgetexponent#1#2{%
	\expandafter\pgfmathfloat@decompose@E#1\relax{#2}%
}

% Defines \pgfmathresult as the floating point number encoded by
% the flags #1, mantisse #2 and exponent #3.
%
% All arguments are characters and will be expanded using '\edef'.
\def\pgfmathfloatcreate#1#2#3{%
	\edef\pgfmathresult{#1#2e#3}%
}%


% Compares #1 with #2 and sets \pgfmathresult either to 1.0 or 0.0.
% 
% It also sets the boolean \ifpgfmathfloatcomparison (globally.
\def\pgfmathfloatlessthan@#1#2{%
%\def\pgfmathfloatlessthan#1#2#3\and#4#5#6{%
	\global\pgfmathfloatcomparisonfalse
	\begingroup
	\expandafter\pgfmathfloat@decompose#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@M\pgfmathfloat@a@E
	\expandafter\pgfmathfloat@decompose#2\relax\pgfmathfloat@b@S\pgfmathfloat@b@M\pgfmathfloat@b@E
	\ifcase\pgfmathfloat@a@S
		% x = 0 -> (x<y <=> y >0)
		\ifnum1=\pgfmathfloat@b@S
			\global\pgfmathfloatcomparisontrue
		\fi
	\or
		% x > 0 -> (x<y <=> ( y > 0 && |x| < |y|) )
		\ifnum1=\pgfmathfloat@b@S
			% y>0:
			\pgfmathfloatlessthan@positive
		\fi
	\or
		% x < 0 -> (x<y <=> (y >= 0 ||   |x| > |y|) )
		\ifnum2=\pgfmathfloat@b@S
			% 'y<0':
			\pgfmathfloatgreaterthan@positive
		\else
			\global\pgfmathfloatcomparisontrue
		\fi
	\else
		\pgfmath@error{Sorry, 'pgfmathfloatlessthan@{#1}{#2}' not yet supported.}%
	\fi
	\endgroup
	\ifpgfmathfloatcomparison
		\def\pgfmathresult{1.0}%
	\else
		\def\pgfmathresult{0.0}%
	\fi
}
\let\pgfmathfloatlessthan=\pgfmathfloatlessthan@

% compares \pgfmathfloat@a@[SME] < \pgfmathfloat@b@[SME]
\def\pgfmathfloatlessthan@positive{%
	\ifnum\pgfmathfloat@a@E<\pgfmathfloat@b@E
		\global\pgfmathfloatcomparisontrue
	\else
		\ifnum\pgfmathfloat@a@E=\pgfmathfloat@b@E
			\ifdim\pgfmathfloat@a@M<\pgfmathfloat@b@M
				\global\pgfmathfloatcomparisontrue
			\fi
		\fi
	\fi
}

% compares \pgfmathfloat@a@[SME] > \pgfmathfloat@b@[SME]
\def\pgfmathfloatgreaterthan@positive{%
	\ifnum\pgfmathfloat@a@E>\pgfmathfloat@b@E
		\global\pgfmathfloatcomparisontrue
	\else
		\ifnum\pgfmathfloat@a@E=\pgfmathfloat@b@E
			\ifdim\pgfmathfloat@a@M>\pgfmathfloat@b@M
				\global\pgfmathfloatcomparisontrue
			\fi
		\fi
	\fi
}


\def\pgfmathfloatmax@#1#2{%
	\pgfmathfloatlessthan{#1}{#2}%
	\ifpgfmathfloatcomparison
		\edef\pgfmathresult{#2}%
	\else
		\edef\pgfmathresult{#1}%
	\fi
}
\let\pgfmathfloatmax=\pgfmathfloatmax@

\def\pgfmathfloatmin@#1#2{%
	\pgfmathfloatlessthan{#1}{#2}%
	\ifpgfmathfloatcomparison
		\edef\pgfmathresult{#1}%
	\else
		\edef\pgfmathresult{#2}%
	\fi
}
\let\pgfmathfloatmin=\pgfmathfloatmin@

% Renormalizes #1 to extended precision mantisse, meaning
% 100 <= m < 1000
% instead of 1 <= m < 10.
% 
% The 'extended precision' means we have higher accuracy when we apply pgfmath operations to mantisses.
%
% The input argument is expected to be a normalized floating point number; the output argument is a non-normalized floating point number (well, normalized to extended precision).
%
% The operation is supposed to be very fast.
\def\pgfmathfloattoextentedprecision#1{%
	\begingroup
	\pgfmathfloattoextentedprecision@a{#1}%
	\pgfmathfloatcreate{\pgfmathfloat@a@S}{\pgfmathresult}{\pgfmathfloat@a@E}%
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}%

\def\pgfmathfloattoextentedprecision@@zero#1\pgfmathfloat@EOI{%
	\edef\pgfmathresult{#1}%
}%
\def\pgfmathfloattoextentedprecision@@one#1.#2#3\pgfmathfloat@EOI{%
	\edef\pgfmathresult{#1#2.#3}%
}%
\def\pgfmathfloattoextentedprecision@@two#1.#2#3#4\pgfmathfloat@EOI{%
	\edef\pgfmathresult{#1#2#3.#4}%
}%

% Sets extended precision to 10^#1.
%
% The default is 10^2, which means mantissas in extended precision are
% normalised to  100 <= m < 1000.
%
% The case 10^1 means they are normalised to 10 <= m < 100 and 10^0
% deactivates extended precision.
%
% #1 is the exponent, #1 = 0,1 or 2.
%
% This setting applies to \pgfmathfloattoextentedprecision.
\def\pgfmathfloatsetextprecision#1{%
	\ifcase#1\relax
		\let\pgfmathfloattoextentedprecision@@=\pgfmathfloattoextentedprecision@@zero
		\def\pgfmathfloatextprec@shift{0}%
	\or
		\let\pgfmathfloattoextentedprecision@@=\pgfmathfloattoextentedprecision@@one
		\def\pgfmathfloatextprec@shift{1}%
	\else
		\let\pgfmathfloattoextentedprecision@@=\pgfmathfloattoextentedprecision@@two
		\def\pgfmathfloatextprec@shift{2}%
	\fi
}%
\pgfmathfloatsetextprecision{2}%

% Does the same work as \pgfmathfloattoextentedprecision, but this one here fills the 
% registers \pgfmathfloat@a@S and \pgfmathfloat@a@E with the flags and (renormalized) exponent.
% It destroys the content of \pgfmathfloat@a@Mtok.
\def\pgfmathfloattoextentedprecision@a#1{%
	\expandafter\pgfmathfloat@decompose@tok#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
	\ifnum\pgfmathfloat@a@S<3
		\advance\pgfmathfloat@a@E by-\pgfmathfloatextprec@shift\relax% compensate for shift
		\expandafter\pgfmathfloattoextentedprecision@@\the\pgfmathfloat@a@Mtok 00\pgfmathfloat@EOI
	\else
		\edef\pgfmathresult{#1}%
	\fi
}%


% Similar to \pgfmathfloattoextentedprecision@a, this one here fills the '@b' registers.
\def\pgfmathfloattoextentedprecision@b#1{%
	\expandafter\pgfmathfloat@decompose@tok#1\relax\pgfmathfloat@b@S\pgfmathfloat@a@Mtok\pgfmathfloat@b@E
	\ifnum\pgfmathfloat@b@S<3
		\advance\pgfmathfloat@b@E by-\pgfmathfloatextprec@shift\relax
		\expandafter\pgfmathfloattoextentedprecision@@\the\pgfmathfloat@a@Mtok 00\pgfmathfloat@EOI
	\else
		\edef\pgfmathresult{#1}%
	\fi
}%

% Addition of two floating point numbers using 8 significant digits.
\def\pgfmathfloatadd@#1#2{%
	\begingroup
	%
	% renormalize argument to 100 <= m < 1000 for extended accuracy:
	\pgfmathfloattoextentedprecision@a{#1}%
	\let\pgfmathfloat@arga=\pgfmathresult
	%
	\pgfmathfloattoextentedprecision@b{#2}%
	\let\pgfmathfloat@argb=\pgfmathresult
	%
	\pgfmathfloatcomparisontrue% re-use this boolean here to handle special cases.
	\ifcase\pgfmathfloat@a@S
		\edef\pgfmathresult{#2}%
		\pgfmathfloatcomparisonfalse
	\or
	\or
		\edef\pgfmathfloat@arga{-\pgfmathfloat@arga}%
	\else
		\pgfmathfloatcomparisonfalse
		\pgfmathfloatcreate{\the\pgfmathfloat@a@S}{0.0}{0}%
	\fi
	\ifcase\pgfmathfloat@b@S
		\edef\pgfmathresult{#1}%
		\pgfmathfloatcomparisonfalse
	\or
	\or
		\edef\pgfmathfloat@argb{-\pgfmathfloat@argb}%
	\else
		\pgfmathfloatcomparisonfalse
		\pgfmathfloatcreate{\the\pgfmathfloat@b@S}{0.0}{0}%
	\fi
	\ifpgfmathfloatcomparison
		% Shift lesser mantisse to fit the larger one:
		\ifnum\pgfmathfloat@a@E<\pgfmathfloat@b@E
			\pgfmathfloatadd@shift{\pgfmathfloat@arga}{\pgfmathfloat@a@E}{\pgfmathfloat@b@E}%
		\else
			\pgfmathfloatadd@shift{\pgfmathfloat@argb}{\pgfmathfloat@b@E}{\pgfmathfloat@a@E}%
		\fi
		% add them!
		\pgfmathadd@{\pgfmathfloat@arga}{\pgfmathfloat@argb}%
		% renormalize sum. This is the only part were an expensive routine comes into play:
		\edef\pgfmathresult{\pgfmathresult e\the\pgfmathfloat@a@E}%
		\expandafter\pgfmathfloatqparsenumber\expandafter{\pgfmathresult}%
	\fi
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}%


% #1=mantisse which needs to be shifted (with smaller exponent)
% #2=smaller exponent
% #3=larger exponent
% 
% ATTENTION: this helper method DESTROYS contents of \pgfmathfloat@a@S.
\def\pgfmathfloatadd@shift#1#2#3{%
	\pgf@xa=#1 pt%
	\pgfmathfloat@a@S=#3\relax
	\advance\pgfmathfloat@a@S by-#2\relax
	\ifcase\pgfmathfloat@a@S
	\or
		\divide\pgf@xa by10\relax
	\or
		\divide\pgf@xa by100\relax
	\or
		\divide\pgf@xa by1000\relax
	\or
		\divide\pgf@xa by10000\relax
	\or
		\divide\pgf@xa by10000\relax
		\divide\pgf@xa by10\relax
	\or
		\divide\pgf@xa by10000\relax
		\divide\pgf@xa by100\relax
	\or
		\divide\pgf@xa by10000\relax
		\divide\pgf@xa by1000\relax
	\or
		\divide\pgf@xa by10000\relax
		\divide\pgf@xa by10000\relax
	\else
		\pgf@xa=0pt%
	\fi
	#2=#3\relax
	\edef#1{\pgf@sys@tonumber\pgf@xa}%
}

\let\pgfmathfloatadd=\pgfmathfloatadd@


% Subtracts two floating point numbers.
\def\pgfmathfloatsubtract@#1#2{%
	\begingroup
	\expandafter\pgfmathfloat@decompose@tok#2\relax\pgfmathfloat@b@S\pgfmathfloat@a@Mtok\pgfmathfloat@b@E
	\ifcase\pgfmathfloat@b@S
		\edef\pgfmathresult{#1}%
	\or
		\pgfmathfloatcreate{2}{\the\pgfmathfloat@a@Mtok}{\the\pgfmathfloat@b@E}%
		\let\pgfmathfloatsub@arg=\pgfmathresult
		\pgfmathfloatadd@{#1}{\pgfmathfloatsub@arg}%
	\or
		\pgfmathfloatcreate{1}{\the\pgfmathfloat@a@Mtok}{\the\pgfmathfloat@b@E}%
		\let\pgfmathfloatsub@arg=\pgfmathresult
		\pgfmathfloatadd@{#1}{\pgfmathfloatsub@arg}%
	\else
		\pgfmathfloatcreate{\the\pgfmathfloat@b@S}{0.0}{0}%
	\fi
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}%

\let\pgfmathfloatsubtract=\pgfmathfloatsubtract@

% Scales a floating point number #1 with a fixed point number #2 using pgfmathmultiply.
% 
% Use this method if #2 is small number.
\def\pgfmathfloatmultiplyfixed@#1#2{%
	\begingroup
	%
	% renormalize argument to 100 <= m < 1000 for extended accuracy:
	\pgfmathfloattoextentedprecision@a{#1}%
	\let\pgfmathfloat@arga=\pgfmathresult
	%
	\pgfmathfloatcomparisontrue% re-use this boolean here to handle special cases.
	\ifcase\pgfmathfloat@a@S
		\edef\pgfmathresult{#1}%
		\pgfmathfloatcomparisonfalse
	\or
	\or
		\edef\pgfmathfloat@arga{-\pgfmathfloat@arga}%
	\else
		\pgfmathfloatcomparisonfalse
		\pgfmathfloatcreate{\the\pgfmathfloat@a@S}{0.0}{0}%
	\fi
	\ifpgfmathfloatcomparison
		\pgfmathmultiply@{\pgfmathfloat@arga}{#2}%
		% renormalize product. This is the only part were an expensive routine comes into play:
		\edef\pgfmathresult{\pgfmathresult e\the\pgfmathfloat@a@E}%
		\expandafter\pgfmathfloatqparsenumber\expandafter{\pgfmathresult}%
	\fi
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}%

\let\pgfmathfloatmultiplyfixed=\pgfmathfloatmultiplyfixed@


\def\pgfmathfloatmultiply@#1#2{%
	\begingroup
	\pgfmathfloatsetextprecision{1}%
	\pgfmathfloattoextentedprecision@a{#1}%
	\let\pgfmathfloat@arga=\pgfmathresult
	%
	\pgfmathfloattoextentedprecision@b{#2}%
	\let\pgfmathfloat@argb=\pgfmathresult
	%
	\pgfmathfloatcomparisontrue% re-use this boolean here to handle special cases.
	\ifcase\pgfmathfloat@a@S
	% 0
		\pgfmathfloatcreate{0}{0.0}{0}%
		\pgfmathfloatcomparisonfalse
	\or% +
		\ifcase\pgfmathfloat@b@S
			\pgfmathfloatcreate{0}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\def\pgfmathresult@S{1}%
		\or
			\def\pgfmathresult@S{2}%
		\else
			\expandafter\pgfmathfloatcreate\the\pgfmathfloat@b@S{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\fi
	\or% -
		\ifcase\pgfmathfloat@b@S
			\pgfmathfloatcreate{0}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\def\pgfmathresult@S{2}%
		\or
			\def\pgfmathresult@S{1}%
		\or
			\pgfmathfloatcreate{3}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{5}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{4}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\fi
	\or% nan
		\pgfmathfloatcreate{3}{0.0}{0}%
		\pgfmathfloatcomparisonfalse
	\or% +infty
		\ifcase\pgfmathfloat@b@S
			\pgfmathfloatcreate{0}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{4}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{5}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{3}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{4}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{5}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\fi
	\or% -infty
		\ifcase\pgfmathfloat@b@S
			\pgfmathfloatcreate{0}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{5}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{4}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{3}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{5}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{4}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\fi
	\fi
	\ifpgfmathfloatcomparison
		\pgfmathmultiply@{\pgfmathfloat@arga}{\pgfmathfloat@argb}%
		\advance\pgfmathfloat@a@E by\pgfmathfloat@b@E
		% renormalize sum. This is the only part were an expensive routine comes into play:
		\edef\pgfmathresult{\pgfmathresult e\the\pgfmathfloat@a@E}%
		\expandafter\pgfmathfloatqparsenumber\expandafter{\pgfmathresult}%
		\expandafter\pgfmathfloat@decompose@tok\pgfmathresult\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
		\pgfmathfloatcreate{\pgfmathresult@S}{\the\pgfmathfloat@a@Mtok}{\the\pgfmathfloat@a@E}%
	\fi
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}%
\let\pgfmathfloatmultiply=\pgfmathfloatmultiply@

\def\pgfmathfloatdivide@#1#2{%
	\begingroup
	\pgfmathfloatsetextprecision{1}%
	\pgfmathfloattoextentedprecision@a{#1}%
	\let\pgfmathfloat@arga=\pgfmathresult
	%
	\pgfmathfloattoextentedprecision@b{#2}%
	\let\pgfmathfloat@argb=\pgfmathresult
	%
	\pgfmathfloatcomparisontrue% re-use this boolean here to handle special cases.
	\ifcase\pgfmathfloat@a@S
	% 0
		\pgfmathfloatcreate{0}{0.0}{0}%
		\pgfmathfloatcomparisonfalse
	\or% +
		\ifcase\pgfmathfloat@b@S
			\pgfmathfloatcreate{4}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\def\pgfmathresult@S{1}%
		\or
			\def\pgfmathresult@S{2}%
		\or
			\pgfmathfloatcreate{3}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\else
			\pgfmathfloatcreate{0}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\fi
	\or% -
		\ifcase\pgfmathfloat@b@S
			\pgfmathfloatcreate{5}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\def\pgfmathresult@S{2}%
		\or
			\def\pgfmathresult@S{1}%
		\or
			\pgfmathfloatcreate{3}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\else
			\pgfmathfloatcreate{0}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\fi
	\or% nan
		\pgfmathfloatcreate{3}{0.0}{0}%
		\pgfmathfloatcomparisonfalse
	\or% +infty
		\ifcase\pgfmathfloat@b@S
			\pgfmathfloatcreate{4}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{4}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{5}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{3}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{4}{0.0}{0}% what is inf/inf ?
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{5}{0.0}{0}% or inf/-inf ?
			\pgfmathfloatcomparisonfalse
		\fi
	\or% -infty
		\ifcase\pgfmathfloat@b@S
			\pgfmathfloatcreate{5}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{5}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{4}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{3}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{5}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\or
			\pgfmathfloatcreate{4}{0.0}{0}%
			\pgfmathfloatcomparisonfalse
		\fi
	\fi
	\ifpgfmathfloatcomparison
		\pgfmathdivide@{\pgfmathfloat@arga}{\pgfmathfloat@argb}%
		\advance\pgfmathfloat@a@E by-\pgfmathfloat@b@E
		% renormalize sum. This is the only part were an expensive routine comes into play:
		\edef\pgfmathresult{\pgfmathresult e\the\pgfmathfloat@a@E}%
		\expandafter\pgfmathfloatqparsenumber\expandafter{\pgfmathresult}%
		\expandafter\pgfmathfloat@decompose@tok\pgfmathresult\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
		\pgfmathfloatcreate{\pgfmathresult@S}{\the\pgfmathfloat@a@Mtok}{\the\pgfmathfloat@a@E}%
	\fi
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}%
\let\pgfmathfloatdivide=\pgfmathfloatdivide@

% Converts a composed floating point representation to fixed point.
%
% Example:
% \pgfmathfloattofixed{142e1}
% -> \pgfmathresult = 42.0
\def\pgfmathfloattofixed@#1{%
	\begingroup
	\expandafter\pgfmathfloat@decompose@tok#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
	\ifcase\pgfmathfloat@a@S
		\def\pgfmathresult{0.0}%
	\or
		\expandafter\pgfmathfloattofixed@impl\the\pgfmathfloat@a@Mtok\relax
	\or
		\expandafter\pgfmathfloattofixed@impl\the\pgfmathfloat@a@Mtok\relax
		\edef\pgfmathresult{-\pgfmathresult}%
	\or\def\pgfmathresult{nan}%
	\or\def\pgfmathresult{inf}%
	\or\def\pgfmathresult{-inf}%
	\fi
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}
\let\pgfmathfloattofixed=\pgfmathfloattofixed@

% Converts a floating point number to scientific format 1.234e5.
%
% This operation is very fast.
\def\pgfmathfloattosci@#1{%
	\begingroup
	\expandafter\pgfmathfloat@decompose@tok#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
	\ifcase\pgfmathfloat@a@S
		\def\pgfmathresult{0.0e0}%
	\or
		\edef\pgfmathresult{\the\pgfmathfloat@a@Mtok e\the\pgfmathfloat@a@E}%
	\or
		\edef\pgfmathresult{-\the\pgfmathfloat@a@Mtok e\the\pgfmathfloat@a@E}%
	\or\def\pgfmathresult{nan}%
	\or\def\pgfmathresult{inf}%
	\or\def\pgfmathresult{-inf}%
	\fi
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}%
\let\pgfmathfloattosci=\pgfmathfloattosci@

% Divides or multiplies the input number by 10^#4 using an arithmetic
% left/right shift.
%
% Input:
% #1 a normalised floating point number.
% #2 a positive or negative integer number denoting the shift.
%
% Example:
% \pgfmathfloatshift{11e3}{4}%
% -> pgfmathresult = 11e7
\def\pgfmathfloatshift@#1#2{%
	\begingroup
	\expandafter\pgfmathfloat@decompose@tok#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
	\expandafter\advance\expandafter\pgfmathfloat@a@E#2\relax
	\edef\pgfmathresult{\the\pgfmathfloat@a@S\the\pgfmathfloat@a@Mtok e\the\pgfmathfloat@a@E}%
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}
\let\pgfmathfloatshift=\pgfmathfloatshift@

% Computes a good guess for log(X.XXXX) where the input number should
% be between 0 < x < 10.
%
% If it is not in this range, the returned value will be bad.
%
% For use in the newton implementation of log(x). Please note that we
% first compute a normalized floating point representation of x, and
% the mantisse is always between 0 and 10.
\def\pgfmathlog@smaller@ten@newton@startval#1.#2\to#3{%
	\ifcase#1
	\pgfmath@error{pgfmathlog@newton: INTERNAL ERROR: should not happen! 
		[\#1=0 should have been caught before!]}%
	\or#3=0.530628pt
	\or#3=0.993pt
	\or#3=1.308pt
	\or#3=1.5pt
	\or#3=1.71pt
	\or#3=1.872pt
	\or#3=2.01pt
	\or#3=2.145pt
	\or#3=2.24pt
	\fi
}

% FIXME : eliminate \pgfmathlog@invoke@expanded ?

% Expands #2 using \edef and invokes #1 with the resulting string.
%
% Example:
%   \pgfmath@y=7.9pt
%   \pgfmathlog@invoke@expanded\pgfmathexp@{{\pgf@sys@tonumber{\pgfmath@y}}}%
% will invoke
%   \pgfmathexp@{7.9}
\def\pgfmathlog@invoke@expanded#1#2{%
	\edef\pgfmath@resulttemp{#2}%
	\expandafter#1\pgfmath@resulttemp
}

% This implementation of log(X) is done with a newton method applied to x-exp(y) = 0.
% The implementation \pgfmathexp is used for exp(y).
%
% see \pgfmathlog@
\def\pgfmathlog@newton#1{%
	\pgfmathfloatparsenumber{#1}%
	\pgfmathlog@newton@float{\pgfmathresult}%
}

% the same as \pgfmathlog@newton, but this one takes a floating point number as input.
\def\pgfmathlog@newton@float#1{%
	\begingroup%
		% compute #1 = M*10^E with normalised mantisse M = [+-]*[1-9].XXXXX
		\expandafter\pgfmathfloat@decompose#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@M\pgfmathfloat@a@E
		\let\pgfmathlog@loopcount=\pgfmathfloat@b@S% this counter is not used here... use it as loop counter.
		%
		\ifnum\pgfmathfloat@a@S=1
		% Now, compute log(#1) = log(M) + E*log(10)
			\expandafter\pgfmathlog@smaller@ten@newton@startval\the\pgfmathfloat@a@M.\to\pgfmathfloat@b@M
			\pgfmathlog@loopcount=0
			\pgfutil@loop
			\ifnum\pgfmathlog@loopcount<3
				\pgfmathlog@invoke@expanded\pgfmathexp@{{\pgf@sys@tonumber{\pgfmathfloat@b@M}}}%
				\let\pgfmathlog@tmp=\pgfmathresult
				\pgfmathlog@invoke@expanded\pgfmathdivide@{{\pgf@sys@tonumber{\pgfmathfloat@a@M}}{\pgfmathlog@tmp}}%
				\expandafter\pgfmath@ya\pgfmathresult pt
				\advance\pgfmathfloat@b@M by\pgfmath@ya
				\advance\pgfmathfloat@b@M by-1pt
				\advance\pgfmathlog@loopcount by1
			\pgfutil@repeat
			\pgfmathfloat@a@M=2.302585pt% = log(10)
			\multiply\expandafter\pgfmathfloat@a@M\pgfmathfloat@a@E
			\advance\pgfmathfloat@b@M by\pgfmathfloat@a@M
			\edef\pgfmathresult{\pgf@sys@tonumber{\pgfmathfloat@b@M}}%
		\else
			\let\pgfmathresult=\pgfutil@empty%
		\fi
	\pgfmath@smuggleone\pgfmathresult
	\endgroup%
}

% Computes log(x) into \pgfmathresult.
%
% REMARK
% This method does NOT use TeX Registers to represent the numbers! The
% computation is COMPLETELY STRING BASED.
% This allows numbers such at 10000000 or 5.23e-10 to be represented
% properly, although TeX-registers would produce overflow/underflow
% errors in these cases. 
%
% The natural logarithm is computed using log(X*10^Y) = log(X) + log(10)*Y
\let\pgfmathlog@=\pgfmathlog@newton

\let\pgfmathlog@float=\pgfmathlog@newton@float

% Public interface method. This is expected to use \pgfmathparse but
% it DOESN'T do that. \pgfmathparse naturally can't handle numbers
% which exceed TeX's numerical capabilities. However, exponentials are
% typically either too large or too small for TeX.
%
% @see \pgfmathnormalisedfloatingpoint for how we parse arguments.
% @see \pgfmathlog@
\let\pgfmathlog=\pgfmathlog@newton

% Rounds a fixed point number #1 to \pgfmathfloat@round@precision digits precision and returns
% the result into \pgfmathresult.
%
% Any trailing zeros after the period are discarded.
% See \pgfmathroundtozerofill if you want trailing zeros and fixed
% width.
%
% This method is PURELY text based and can work with arbirtrary
% precision (well, limited to TeX's stack size and integer size).
%
% Examples:
% \pgfmathroundto{1}
% -> \pgfmathresult = '1'
%
% \pgfmathroundto{19999.9996}
% -> \pgfmathresult = '20000'
%
% Arguments:
% #1 may be either a number or a macro expanding to a number.
%
% SIDE EFFECT: the global variable \ifpgfmathfloatroundhasperiod will be set.
\def\pgfmathroundto#1{%
	\pgfmathfloatroundhasperiodtrue
	\begingroup
	\pgfmathfloat@fixed@digits@after@periodfalse
	\pgfmathroundto@impl{#1}%
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}


% Overloaded method. 
%
% This variant always uses a FIXED number behind the period and fills
% in zeros if necessary.
% Examples:
% \pgfmathroundtozerofill{1}
% -> \pgfmathresult = '1.00'
%
% \pgfmathroundtozerofill{19999.9996}
% -> \pgfmathresult = '20000.00'
%
% SIDE EFFECT: the global variable \ifpgfmathfloatroundhasperiod will be set.
\def\pgfmathroundtozerofill#1{%
	\pgfmathfloatroundhasperiodtrue
	\begingroup
	\pgfmathfloat@fixed@digits@after@periodtrue
	\pgfmathroundto@impl{#1}%
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}

% see \pgfmathprintnumber@fixed@style for docs
\def\pgfmathprintnumber@fixed@styleDEFAULT#1#2#3e#4\relax{%
	\begingroup
	\pgfkeysgetvalue{/pgf/number format/set decimal separator}\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP
	\pgfkeysgetvalue{/pgf/number format/@dec sep mark}\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP@MARK
	\pgfkeysgetvalue{/pgf/number format/set thousands separator}\pgfmathprintnumber@fixed@styleDEFAULT@THOUSAND@SEP
	\c@pgf@counta=#4\relax
	\def\pgfmathresult{}%
	\ifpgfmathfloatroundhasperiod
		\expandafter\pgfmathprintnumber@fixed@styleDEFAULT@impl@period#1\pgfmathfloat@EOI
	\else
		\expandafter\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod#1\pgfmathfloat@EOI\pgfmathfloat@EOI\pgfmathfloat@EOI%
		\begingroup
		\toks0=\expandafter{\pgfmathresult}%
		\toks1=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP@MARK}%
		\xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 }%
		\endgroup
		\let\pgfmathresult=\pgfmathfloat@glob@TMP
	\fi
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@period#1.#2\pgfmathfloat@EOI{%
	\ifpgfmathprintnumberskipzeroperiod
		\def\pgfmathfloat@loc@TMPb{#1}%
		\ifx\pgfmathfloatparsenumber@tok@ZERO\pgfmathfloat@loc@TMPb
		\else
			\def\pgfmathfloat@loc@TMPc{-0}%
			\ifx\pgfmathfloat@loc@TMPc\pgfmathfloat@loc@TMPb
				\def\pgfmathresult{-}%
			\else
				\def\pgfmathfloat@loc@TMPc{+0}%
				\ifx\pgfmathfloat@loc@TMPc\pgfmathfloat@loc@TMPb
					\def\pgfmathresult{+}%
				\else
					\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod#1\pgfmathfloat@EOI\pgfmathfloat@EOI\pgfmathfloat@EOI
				\fi
			\fi
		\fi
	\else
		\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod#1\pgfmathfloat@EOI\pgfmathfloat@EOI\pgfmathfloat@EOI
	\fi
	\begingroup
	\toks0=\expandafter{\pgfmathresult}%
	\toks1=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP@MARK}%
	\toks2=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP #2}%
	\xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 \the\toks2 }%
	\endgroup
	\let\pgfmathresult=\pgfmathfloat@glob@TMP
}%
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod{%
	\ifx\pgfmathprintnumber@fixed@styleDEFAULT@THOUSAND@SEP\pgfutil@empty
		\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
			\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printall}%
	\else
		\ifnum\c@pgf@counta<0\relax
			\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
				\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printall}%
		\else
			\advance\c@pgf@counta by1% counta:= total number of digits, N.
			\c@pgf@countb=\c@pgf@counta
			\divide\c@pgf@countb by3%  countb := N DIV 3
			\c@pgf@countc=\c@pgf@countb
			\multiply\c@pgf@countc by3
			\advance\c@pgf@counta by-\c@pgf@countc% now counta := N MOD 3
			\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
				\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printsign
			}%
		\fi
	\fi
	\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT
}
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printsign#1{%
	\def\pgfmathfloat@loc@TMPb{#1}%
	\ifx\pgfmathfloat@loc@TMPb\pgfmathfloatparsenumber@tok@MINUS
		\expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult #1}%
		\let\pgfmathfloat@loc@TMPb=\pgfutil@empty
	\else
		\ifx\pgfmathfloat@loc@TMPb\pgfmathfloatparsenumber@tok@PLUS
			\expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult #1}%
			\let\pgfmathfloat@loc@TMPb=\pgfutil@empty
		\else
			\ifpgfmathprintnumber@showpositive
				\expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult +}%
			\fi
		\fi
	\fi
	\ifnum\c@pgf@counta>0
		\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
			\expandafter\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printtrailingdigits\pgfmathfloat@loc@TMPb
		}%
	\else
		\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
			\expandafter\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@counteverythird\pgfmathfloat@loc@TMPb
		}%
	\fi
	\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT
}
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printtrailingdigits#1#2{%
	\ifcase\c@pgf@counta
	\or
		\expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult #1}%
		\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
			\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@counteverythird#2%
		}%
	\or
		\expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult #1#2}%
		\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
			\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@counteverythird%
		}%
	\fi
	\ifnum\c@pgf@countb>0\relax
		\begingroup
		\toks0=\expandafter{\pgfmathresult}%
		\toks1=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@THOUSAND@SEP}%
		\xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 }%
		\endgroup
		\let\pgfmathresult=\pgfmathfloat@glob@TMP
	\fi
	\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT
}
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@counteverythird#1#2#3{%
	\ifnum\c@pgf@countb>0\relax
		\expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult #1#2#3}%
		\advance\c@pgf@countb by-1
		\ifnum\c@pgf@countb>0\relax
			\begingroup
			\toks0=\expandafter{\pgfmathresult}%
			\toks1=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@THOUSAND@SEP}%
			\xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 }%
			\endgroup
			\let\pgfmathresult=\pgfmathfloat@glob@TMP
		\fi
		\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
			\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@counteverythird%
		}%
	\else
		% in thise case, #1#2#3 are expected to be
		% \pgfmathfloat@EOI\pgfmathfloat@EOI\pgfmathfloat@EOI
		%--------------------------------------------------
		% \def\pgfmathfloat@loc@TMPb{\pgfmathfloat@EOI\pgfmathfloat@EOI\pgfmathfloat@EOI}%
		% \def\pgfmathfloat@loc@TMPc{#1#2#3}%
		% \ifx\pgfmathfloat@loc@TMPc\pgfmathfloat@loc@TMPb
		% \else
		% 	\pgfmath@error{INTERNAL ERROR in fixed style - The input sequence did not terminate as expected; which indicates a wrong exponent argument provided to \string\pgfmathprintnumber@fixed@style}%
		% \fi
		%-------------------------------------------------- 
		\let\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT=\relax
	\fi
	\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT
}
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printall#1{%
	\def\pgfmathfloat@loc@TMPb{#1}%
	\let\pgfmathfloat@loc@TMPc=\pgfutil@empty
	\ifx\pgfmathfloat@loc@TMPb\pgfmathfloatparsenumber@tok@MINUS
	\else
		\ifx\pgfmathfloat@loc@TMPb\pgfmathfloatparsenumber@tok@PLUS
		\else
			\ifpgfmathprintnumber@showpositive
				\def\pgfmathfloat@loc@TMPc{+}%
			\fi
		\fi
	\fi
	\expandafter\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printall@\pgfmathfloat@loc@TMPc#1%
}
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printall@#1\pgfmathfloat@EOI\pgfmathfloat@EOI\pgfmathfloat@EOI{%
	\expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult #1}%
}%

% #1 maybe a macro
\def\pgfmathprintnumber@fixed@stylePERIOD#1#2#3e#4\relax{%
	\def\pgfmathresult{#1}%
}

% #1 maybe a macro
\def\pgfmathprintnumber@fixed@styleCOMMA#1#2#3e#4\relax{%
	\ifpgfmathfloatroundhasperiod
		\expandafter\pgfmathprintnumber@fixed@styleCOMMA@impl#1\pgfmathfloat@EOI
	\else
		\def\pgfmathresult{#1}%
	\fi
}
\def\pgfmathprintnumber@fixed@styleCOMMA@impl#1.#2\pgfmathfloat@EOI{\def\pgfmathresult{#1{,}#2}}

% The default style to display fixed point numbers.
%
% It does not apply numerics, but it is responsable to typeset the
% rounded number.
% It can access the \ifpgfmathfloatroundhasperiod boolean.
%
% Arguments:
% #1#2#3e#4\relax

% Input: 
% #1  the fixed point number to be displayed (maybe a macro).
% #2#3e#4:  the (possibly unformatted) floating point representation which belongs to #1.
%     It is used to determine sign and exponent.
\let\pgfmathprintnumber@fixed@style=\pgfmathprintnumber@fixed@styleDEFAULT


% Rounds a normalized floating point number to \pgfmathfloat@round@precision 
% digits precision and writes the result to \pgfmathresult.
%
% This method uses \pgfmathroundto for the mantisse.
%
% @see pgfmathfloatroundzerofill
%
% SIDE EFFECT: the global variable \ifpgfmathfloatroundhasperiod will be set to
% whether the final mantisse #5 has a period or not.
\def\pgfmathfloatround#1{%
	\pgfmathfloatroundhasperiodtrue
	\begingroup
	\pgfmathfloat@fixed@digits@after@periodfalse
	\expandafter\pgfmathfloat@decompose@tok#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
	\pgfmathfloatround@impl
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}

% Overload.
%
% This method uses a fixed width for the mantisse and fills in zeros
% if necessary.
%
% This method uses \pgfmathroundtozerofill for the mantisse.
%
% SIDE EFFECT: the global variable \ifpgfmathfloatroundhasperiod will be set to
% whether the final mantisse #5 has a period or not.
\def\pgfmathfloatroundzerofill#1{%
	\pgfmathfloatroundhasperiodtrue
	\begingroup
	\pgfmathfloat@fixed@digits@after@periodtrue
	\expandafter\pgfmathfloat@decompose@tok#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
	\pgfmathfloatround@impl
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}

\newif\ifpgfmathfloatround@allow@empty@mantisse
\def\pgfmathfloatround@mantisse@ONE{1.0}%

% #1: sign
% #2: mantisse
% #3: exponent
% #4: CODE to display if the mantisse is drawn.
% #5: CODE to display if the mantisse is NOT draw. (unused)
% #6: CODE to display the exponent.
\def\pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\relax#4#5#6{%
	\pgfkeysgetvalue{/pgf/number format/@sci exponent mark}\pgfmathfloatrounddisplaystyle@e@mark
	\ifcase#1\relax
		\pgfmathprintnumber@fixed@style{#2}#1#2e0\relax%
		\expandafter\pgfmathfloatrounddisplaystyle@shared@impl@\expandafter{\pgfmathresult}{#4#6}%
	\or\pgfmathprintnumber@fixed@style{#2}#1#2e0\relax%
		\expandafter\pgfmathfloatrounddisplaystyle@shared@impl@\expandafter{\pgfmathresult}{#4#6}%
	\or\pgfmathprintnumber@fixed@style{-#2}#1#2e0\relax%
		\expandafter\pgfmathfloatrounddisplaystyle@shared@impl@\expandafter{\pgfmathresult}{#4#6}%
	\or
		\pgfmathfloatrounddisplaystyle@shared@impl@{NaN}{}%
	\or
		\ifpgfmathprintnumber@showpositive
			\pgfmathfloatrounddisplaystyle@shared@impl@{+\infty}{}%
		\else
			\pgfmathfloatrounddisplaystyle@shared@impl@{\infty}{}%
		\fi
	\or
		\pgfmathfloatrounddisplaystyle@shared@impl@{-\infty}{}%
	\fi
}

% #1: the part before the exponent code
% #2: the part for the exponent code.
\def\pgfmathfloatrounddisplaystyle@shared@impl@#1#2{%
	{\toks0={#1}%
	\toks1=\expandafter{\pgfmathfloatrounddisplaystyle@e@mark #2}%
	\xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 }%
	}%
	\let\pgfmathresult=\pgfmathfloat@glob@TMP
}%

\def\pgfmathfloatrounddisplaystyle@std#1#2e#3\relax{%
	\pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\relax{\cdot}{}{10^{#3}}%
}
\def\pgfmathfloatrounddisplaystyle@subscript#1#2e#3\relax{%
	\pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\relax{}{1}{_{#3}}%
}
\def\pgfmathfloatrounddisplaystyle@e#1#2e#3\relax{%
	\ifnum#3<0\relax
		{\count0=#3\relax
		\multiply\count0 by-1
		\xdef\pgfmathfloat@glob@TMP{e{-}\the\count0}%
		}%
		\let\pgfmathresult=\pgfmathfloat@glob@TMP
	\else
		\def\pgfmathresult{e{+}#3}%
	\fi
	\def\pgfmathfloat@loc@TMPb{\pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\relax{}{1}}%
	\expandafter\pgfmathfloat@loc@TMPb\expandafter{\pgfmathresult}%
}
\def\pgfmathfloatrounddisplaystyle@E#1#2e#3\relax{%
	\ifnum#3<0\relax
		{\count0=#3\relax
		\multiply\count0 by-1
		\xdef\pgfmathfloat@glob@TMP{E{-}\the\count0}%
		}%
		\let\pgfmathresult=\pgfmathfloat@glob@TMP
	\else
		\def\pgfmathresult{E{+}#3}%
	\fi
	\def\pgfmathfloat@loc@TMPb{\pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\relax{}{1}}%
	\expandafter\pgfmathfloat@loc@TMPb\expandafter{\pgfmathresult}%
}

% A macro which takes three arguments, sign, mantisse and exponent and
% expands to the final TeX-representation for that floating point
% number.
%
% PRECONDITION:
%   the floating point number has already been rounded properly and
%   the mantisse has been rounded correcty.
%
% #1: SIGN
% #2: MANTISSE
% #3: EXPONENT
\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@std
\newif\ifpgfmathfloat@usezerofill@sci
\newif\ifpgfmathfloat@usezerofill@fixed
\newif\ifpgfmathprintnumber@assumemathmode
\newif\ifpgfmathprintnumber@showpositive

\pgfkeys{%
	/pgf/number format/.is family,
	/pgf/number format,
	fixed/.code=			\pgfmath@set@number@printer{pgfmathprintnumber@FIXED},
	sci/.code=				\pgfmath@set@number@printer{pgfmathprintnumber@SCI},
	std/.code=				\pgfmath@set@number@printer{pgfmathprintnumber@STD},
	int detect/.code=		\pgfmath@set@number@printer{pgfmathprintnumber@INT@DETECT},
	int trunc/.code=		\pgfmath@set@number@printer{pgfmathprintnumber@INT@TRUNC},
	assume math mode/.is if=pgfmathprintnumber@assumemathmode,
	assume math mode/.default=true,
	fixed zerofill/.is if=	pgfmathfloat@usezerofill@fixed,
	fixed zerofill/.default=true,
	sci zerofill/.is if=	pgfmathfloat@usezerofill@sci,
	sci zerofill/.default=true,
	zerofill/.style=		{/pgf/number format/fixed zerofill=#1,/pgf/number format/sci zerofill=#1},
	zerofill/.default=		true,
	precision/.store in=	\pgfmathfloat@round@precision,
	fixed default/.code=		{\let\pgfmathprintnumber@fixed@style=\pgfmathprintnumber@fixed@styleDEFAULT},
	set decimal separator/.initial=,
	dec sep/.style={/pgf/number format/set decimal separator=#1},
	@dec sep mark/.initial=,
	@sci exponent mark/.initial=,
	set thousands separator/.initial=,
	1000 sep/.style={/pgf/number format/set thousands separator=#1},
	use period/.style=		{/pgf/number format/set decimal separator={.},/pgf/number format/set thousands separator={{{,}}}},
	use comma/.style=		{/pgf/number format/set decimal separator={{{,}}},/pgf/number format/set thousands separator={.}},
	showpos/.is if=pgfmathprintnumber@showpositive,
	showpos/.default=true,
	print sign/.is if=pgfmathprintnumber@showpositive,
	print sign/.default=true,
	skip 0./.is if=pgfmathprintnumberskipzeroperiod,
	skip 0./.default=true,
	skip 0.= false,
	use period,
	sci 10^e/.code=			{\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@std},
	sci 10e/.code=			{\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@std},
	sci e/.code=			{\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@e},
	sci E/.code=			{\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@E},
	sci subscript/.code=	{\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@subscript},
%	sci may skip mantisse/.is if=pgfmathfloatround@allow@empty@mantisse,
%	sci may skip mantisse/.default=true,
}



\def\pgfmathprintnumber@STD#1{%
	% parse the input:
	\pgfmathfloatparsenumber{#1}%
	\expandafter\pgfmathprintnumber@STD@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@STD@issci#1#2e#3\relax{%
	\expandafter\ifnum#1<3
		\expandafter\ifnum#3>4
			\pgfmathprintnumber@SCI@issci#1#2e#3\relax%
		\else
			\begingroup
			\c@pgf@counta=\pgfmathfloat@round@precision\relax
			\divide\c@pgf@counta by-2\relax
			\ifnum#3<\c@pgf@counta
				\pgfmathprintnumber@SCI@issci#1#2e#3\relax%
			\else
				\pgfmathprintnumber@FIXED@issci#1#2e#3\relax%
			\fi
			\pgfmath@smuggleone\pgfmathresult
			\endgroup
		\fi
	\else% nan or inf:
		\pgfmathfloatrounddisplaystyle#1#2e#3\relax%
	\fi
}


\def\pgfmathprintnumber@INT@TRUNC#1{%
	\pgfmathfloatparsenumber{#1}%
	\expandafter\pgfmathprintnumber@INT@TRUNC@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@INT@TRUNC@impl#1.#2\relax#3#4e#5\relax{%
	\pgfmathfloatroundhasperiodfalse
	\pgfmathprintnumber@fixed@style{#1}#3#4e#5\relax%
}
\def\pgfmathprintnumber@INT@TRUNC@issci#1#2e#3\relax{%
	\ifnum#1<3\relax
		\pgfmathfloattofixed{#1#2e#3}%
		\expandafter\pgfmathprintnumber@INT@TRUNC@impl\pgfmathresult\relax#1#2e#3\relax
	\else
		\pgfmathfloatrounddisplaystyle#1#2e#3\relax%
	\fi
}


\def\pgfmathprintnumber@INT@DETECT#1{%
	\pgfmathfloatparsenumber{#1}%
	\expandafter\pgfmathprintnumber@INT@DETECT@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@INT@DETECT@issci#1#2e#3\relax{%
	\begingroup
	\ifnum#1<3\relax
		\pgfmathfloattofixed{#1#2e#3}%
		\def\pgfmathfloat@round@precision{6}%
		\expandafter\pgfmathroundto\expandafter{\pgfmathresult}%
		\ifpgfmathfloatroundhasperiod
			\pgfmathprintnumber@SCI@issci#1#2e#3\relax
		\else
			\expandafter\pgfmathprintnumber@fixed@style\expandafter{\pgfmathresult}#1#2e#3\relax
		\fi
	\else
		\pgfmathfloatrounddisplaystyle#1#2e#3\relax%
	\fi
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}

\def\pgfmathprintnumber@FIXED#1{%
	\pgfmathfloatparsenumber{#1}%
	\expandafter\pgfmathprintnumber@FIXED@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@FIXED@issci#1#2e#3\relax{%
	\begingroup
	\ifnum#1<3
		\pgfmathfloattofixed{#1#2e#3}%
		\ifpgfmathfloat@usezerofill@fixed
			\expandafter\pgfmathroundtozerofill\expandafter{\pgfmathresult}%
		\else
			\expandafter\pgfmathroundto\expandafter{\pgfmathresult}%
		\fi
		\ifpgfmathfloatroundmayneedrenormalize
			\pgfmathfloat@a@E=#3\relax
			\advance\pgfmathfloat@a@E by1
			\edef\pgfmathfloat@loc@TMPb{\noexpand\pgfmathprintnumber@fixed@style{\pgfmathresult}#1#2e\the\pgfmathfloat@a@E}%
			\pgfmathfloat@loc@TMPb\relax%
		\else
			\expandafter\pgfmathprintnumber@fixed@style\expandafter{\pgfmathresult}#1#2e#3\relax%
		\fi
	\else% nan or inf:
		\pgfmathfloatrounddisplaystyle#1#2e#3\relax%
	\fi
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
}


\def\pgfmathprintnumber@SCI#1{%
	\pgfmathfloatparsenumber{#1}%
	\expandafter\pgfmathprintnumber@SCI@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@SCI@issci#1#2e#3\relax{%
	\ifpgfmathfloat@usezerofill@sci
		\pgfmathfloatroundzerofill{#1#2e#3}%
	\else
		\pgfmathfloatround{#1#2e#3}%
	\fi
	\expandafter\pgfmathfloatrounddisplaystyle\pgfmathresult\relax
}

% Prints argument #1 using the current pretty printer environment (all
% variables in /pgf/number format).
%
% You may specify optional arguments with \pgfmathprintnumber[...].
\def\pgfmathprintnumber{%
	\pgfutil@ifnextchar[%
		{\pgfmathprintnumber@OPT}%
		{\pgfmathprintnumber@noopt}%
}

\def\pgfmathprintnumber@noopt#1{%
	\pgfmathprintnumber@{#1}%
	\ifpgfmathprintnumber@assumemathmode
	\else
		\pgfutilensuremath{\pgfmathresult}%
	\fi
}%
\def\pgfmathprintnumber@OPT[#1]#2{%
	\begingroup
	\pgfqkeys{/pgf/number format}{#1}%
	\pgfmathprintnumber@{#2}%
	\ifpgfmathprintnumber@assumemathmode
	\else
		\pgfutilensuremath{\pgfmathresult}%
	\fi
	\endgroup
}%

% As \pgfmathprintnumber, but it produces its output into the second
% argument.
\def\pgfmathprintnumberto{%
	\pgfutil@ifnextchar[%
		{\pgfmathprintnumberto@OPT}%
		{\pgfmathprintnumberto@noopt}%
}

\def\pgfmathprintnumberto@noopt#1#2{%
	\begingroup
	\pgfmathprintnumber@{#1}%
	\ifpgfmathprintnumber@assumemathmode
		\global\let\pgfmathfloat@glob@TMP=\pgfmathresult
	\else
		\toks0=\expandafter{\pgfmathresult}%
		\xdef\pgfmathfloat@glob@TMP{\noexpand\pgfutilensuremath{\the\toks0 }}%
	\fi
	\endgroup
	\let#2=\pgfmathfloat@glob@TMP
}%
\def\pgfmathprintnumberto@OPT[#1]#2#3{%
	\begingroup
	\pgfqkeys{/pgf/number format}{#1}%
	\pgfmathprintnumber@{#2}%
	\ifpgfmathprintnumber@assumemathmode
		\global\let\pgfmathfloat@glob@TMP=\pgfmathresult
	\else
		\toks0=\expandafter{\pgfmathresult}%
		\xdef\pgfmathfloat@glob@TMP{\noexpand\pgfutilensuremath{\the\toks0 }}%
	\fi
	\endgroup
	\let#3=\pgfmathfloat@glob@TMP
}%
	

% Changes the current number pretty printer to #1.
%
% #1 is the macro base name for the pretty print routine, without the
% leading '\'.
\def\pgfmath@set@number@printer#1{%
	\expandafter\let\expandafter\pgfmathprintnumber@\csname #1\endcsname
	\expandafter\let\expandafter\pgfmathprintnumber@issci\csname #1@issci\endcsname
}

\pgfmath@set@number@printer{pgfmathprintnumber@STD}
%\pgfmath@set@number@printer{pgfmathprintnumber@FIXED}
%\pgfmath@set@number@printer{pgfmathprintnumber@FIXED@ZEROFILL}
%\pgfmath@set@number@printer{pgfmathprintnumber@SCI@ZEROFILL}
%\pgfmath@set@number@printer{pgfmathprintnumber@SCI}

%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% IMPL
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

% equals only itsself when compared with \ifx:
\def\pgfmathfloat@EOI{\pgfmathfloat@EOI}%

% Re-use counters internally.
%
% They are always grouped and only used inside of the rounding
% routines.
\let\c@pgfmathroundto@prec=\pgfmathfloat@b@S% ATTENTION: DOUBLE-USED REGISTERS!
\let\c@pgfmathroundto@offsetbehindperiod=\pgfmathfloat@b@E
\newcount\c@pgfmathroundto@lastzeros

\newif\ifpgfmathround@impl@PREPERIOD@is@negative@zero

% PRECONDITION:
%  	\ifpgfmathfloatroundhasperiod=\iftrue  holds outside of the
%  	current TeX group.
%
% POSTCONDITION:
%   \ifpgfmathfloatroundhasperiod will be set correctly AFTER the
%   current TeX group.
%   \ifpgfmathfloatroundmayneedrenormalize will be set globally
\def\pgfmathroundto@impl#1{%
	\global\pgfmathfloatroundmayneedrenormalizefalse
	\pgfmathfloat@tmptoks={}%
	\let\pgfmathround@next=\pgfutil@empty
	\let\pgfmathround@cur=\pgfutil@empty
	\let\pgfmathresult=\pgfutil@empty
	\edef\pgfmathround@input{#1}%
	\expandafter\c@pgfmathroundto@prec\pgfmathfloat@round@precision\relax
	\c@pgfmathroundto@lastzeros=0
	\c@pgfmathroundto@offsetbehindperiod=-1 % means: no period found so far
	\pgfmathround@impl@PREPERIOD@is@negative@zerotrue
	\expandafter\pgfmathroundto@impl@ITERATE@NODOT@firstcall\pgfmathround@input\pgfmathfloat@EOI
}

% \pgfmathroundto implementation in WORDS:
%
% coarse idea: 
%    1. collect all digits/sign BEFORE the first period in REVERSE order
%    2. then, collect UP TO \prec digits after the period in REVERSE order
% Steps 1. and 2. lead to the digit [sign] sequence
%    "x_{-p} x_{-p+1} ... x_{-2} x_{-1} '.' x_0 ... x_r"
% where 'r' is the total number of digits. The integer 'p' denotes the
% ACTUALLY collected number of digits behind the period.
%
% Let 'k' be the desired precision.
%
% Please note that pgfmathroundto rounds the mantisse, that means |abs(x)|.
%
% There are exactly TWO cases:
% 1. The case with p<=k and x_{-p-1} = end of input.
% 2. The case with p=k and x_{-p-1} is a further, next character.
%
% Then, for case 1.):
% 	discard any unused zeros at the tail of our number (possibly
% 	including the period)
%
% and in case 2.)
%   if NEXT DIGIT < 5:
%       do exactly the same as in case 1.) above and discard any
%       following digits.
%   else
%   	let q := -p
%   	while(x_q = 9 and q<=r )
%   		if q>=0
%   			set x_q = '0'
%   		else
%   			discard digit x_q='9'
%   		fi
%   		++q
%   		if q=0
%   			discard the period 
%   		fi
%   	end while
%   	if q = r+1
%   		insert a '1'
%   	else
%   		set x_q = x_q + 1
%   	fi
%   fi
%
% All these loops have been implemented in spaghetti-code below.
% Sorry, I fear its hard to understand. In principle, everything is
% realised using more or less finite state machines (with some number
% counting logic).
%
% Some comments:
%   - The token register \pgfmathfloat@tmptoks is used to accumulate the REVERSED input number.
%	- \pgfmathfloat@EOI always denotes 'END OF INPUT'.
%	- in the second stage, we need to reverse \pgfmathfloat@tmptoks.
%	  This is -again- done with \pgfmathfloat@tmptoks.

\def\pgfmathroundto@impl@discard@period#1.#2\pgfmathfloat@EOI{%
	\pgfmathfloatroundhasperiodfalse
	\aftergroup\pgfmathfloatroundhasperiodfalse
	\def\pgfmathresult{#1}%
}

\def\pgfmathroundto@impl@gobble@rest@and@start#1\pgfmathfloat@EOI{%
	\pgfmathroundto@impl@start
}
\def\pgfmathroundto@impl@gobble@and@start\pgfmathfloat@EOI{%
	\pgfmathroundto@impl@start
}
\def\pgfmathroundto@impl@gobble\pgfmathfloat@EOI{}%
\def\pgfmathroundto@impl@gobble@rest#1\pgfmathfloat@EOI{}%

% This method will be invoked as soon as the first step, the reverse
% collection of up to PREC digits after the period, has finished.
\def\pgfmathroundto@impl@start{%
	\ifx\pgfmathround@next\pgfutil@empty
		\ifnum\c@pgfmathroundto@offsetbehindperiod<0
			% no period found.
			\ifpgfmathfloat@fixed@digits@after@period
				\ifnum\c@pgfmathroundto@prec=0\relax
					\pgfmathfloatroundhasperiodfalse
					\aftergroup\pgfmathfloatroundhasperiodfalse
					\edef\pgfmathresult{\pgfmathround@input}%
				\else
					\pgfmathfloat@tmptoks=\expandafter{\pgfmathround@input.}%
					\c@pgfmathroundto@offsetbehindperiod=\c@pgfmathroundto@prec
					\pgfmathroundto@impl@append@zeros
					\edef\pgfmathresult{\the\pgfmathfloat@tmptoks}%
				\fi
			\else
				\pgfmathfloatroundhasperiodfalse
				\aftergroup\pgfmathfloatroundhasperiodfalse
				\edef\pgfmathresult{\pgfmathround@input}%
			\fi
		\else
			%\ifnum\c@pgfmathroundto@offsetbehindperiod>\c@pgfmathroundto@prec
			%	\pgfmath@error{Internal logic error in pgfmathroundto at [I] - should not have happened!?}%
			%\fi
			\pgfmathroundto@impl@finish@with@truncation
		\fi
	\else
		%\ifnum\c@pgfmathroundto@offsetbehindperiod=\c@pgfmathroundto@prec
		%\else
		%	\pgfmath@error{Internal logic error in pgfmathroundto at [II] - should not have happened!? I have offsetbehindperiod=\the\c@pgfmathroundto@offsetbehindperiod and prec = \the\c@pgfmathroundto@prec}%
		%\fi
		\expandafter\ifnum\pgfmathround@next<5\relax
			\pgfmathroundto@impl@finish@with@truncation
		\else
			\multiply\c@pgfmathroundto@offsetbehindperiod by-1
			\expandafter\pgfmathroundto@impl@ADD@ONE\the\pgfmathfloat@tmptoks\pgfmathfloat@EOI
		\fi
	\fi
}
			
% takes the current input and decides whether trailing zeros shall be
% discarded or more zeros need to be filled in.
\def\pgfmathroundto@impl@finish@with@truncation{%
	\ifpgfmathfloat@fixed@digits@after@period
		\expandafter\pgfmathroundto@impl@REVERSE\the\pgfmathfloat@tmptoks\pgfmathfloat@EOI
		\ifnum\c@pgfmathroundto@lastzeros=\c@pgfmathroundto@offsetbehindperiod
			\ifpgfmathround@impl@PREPERIOD@is@negative@zero
				% write '0.0000' instead of '-0.0000':
				\expandafter\pgfmathroundto@impl@discard@minus\the\pgfmathfloat@tmptoks\pgfmathfloat@EOI
			\fi
		\fi
		\ifnum\c@pgfmathroundto@prec=0\relax
			\expandafter\pgfmathroundto@impl@discard@period\the\pgfmathfloat@tmptoks\pgfmathfloat@EOI
		\else
			\advance\c@pgfmathroundto@prec by-\c@pgfmathroundto@offsetbehindperiod
			\c@pgfmathroundto@offsetbehindperiod=\c@pgfmathroundto@prec
			\pgfmathroundto@impl@append@zeros
			\edef\pgfmathresult{\the\pgfmathfloat@tmptoks}%
		\fi
	\else
		\pgfmathroundto@impl@discard@suffix@zeros
	\fi
}

\def\pgfmathroundto@impl@discard@minus-#1\pgfmathfloat@EOI{\pgfmathfloat@tmptoks={#1}}%

% appends \c@pgfmathroundto@offsetbehindperiod zeros at the end of \pgfmathfloat@tmptoks.
\def\pgfmathroundto@impl@append@zeros{%
	\ifnum\c@pgfmathroundto@offsetbehindperiod>0
		\pgfmathfloat@tmptoks=\expandafter{\the\pgfmathfloat@tmptoks0}%
		\advance\c@pgfmathroundto@offsetbehindperiod by-1
		\pgfmathroundto@impl@append@zeros
	\fi
}

\def\pgfmathroundto@impl@ADD@ONE{%
	\pgfmathfloat@tmptoks={}% no longer needed because its old value will be read from input
	\pgfmathroundto@impl@ADD@ONE@ITERATE
}
\def\pgfmathroundto@impl@ADD@ONE@ITERATE{%
	\pgfutil@ifnextchar\pgfmathfloat@EOI{%
		\global\pgfmathfloatroundmayneedrenormalizetrue
		\edef\pgfmathresult{1\the\pgfmathfloat@tmptoks}%
		\pgfmathroundto@impl@gobble
	}{%
		\pgfutil@ifnextchar.{%
			\ifnum\c@pgfmathroundto@prec=0
				% silently discard period in special case precision=0
				\def\pgfmathround@nextcmd{\pgfmathroundto@impl@ADD@ONE@ITERATE@gobble@dot}%
			\else
				\def\pgfmathround@nextcmd{\pgfmathroundto@impl@ADD@ONE@NEXT@COLLECT}%
			\fi
			\pgfmathround@nextcmd
		}{%
			\pgfutil@ifnextchar+{%
				\global\pgfmathfloatroundmayneedrenormalizetrue
				\edef\pgfmathresult{1\the\pgfmathfloat@tmptoks}%
				\pgfmathroundto@impl@gobble@rest
			}{%
				\pgfutil@ifnextchar-{%
					\global\pgfmathfloatroundmayneedrenormalizetrue
					\edef\pgfmathresult{-1\the\pgfmathfloat@tmptoks}%
					\pgfmathroundto@impl@gobble@rest
				}{%
					\pgfmathroundto@impl@ADD@ONE@NEXT
				}%
			}%
		}%
	}%
}

\def\pgfmathroundto@impl@ADD@ONE@ITERATE@gobble@dot.{%
	\pgfmathfloatroundhasperiodfalse
	\aftergroup\pgfmathfloatroundhasperiodfalse
	\pgfmathroundto@impl@ADD@ONE@ITERATE
}

\def\pgfmathroundto@impl@ADD@ONE@NEXT@COLLECT#1{%
	\pgfmathfloat@tmptoks=\expandafter{\expandafter#1\the\pgfmathfloat@tmptoks}%
	\pgfmathroundto@impl@ADD@ONE@ITERATE
}
\def\pgfmathroundto@impl@ADD@ONE@NEXT#1{%
	\ifnum#1=9
		\ifnum\c@pgfmathroundto@offsetbehindperiod<0
			\ifpgfmathfloat@fixed@digits@after@period
				\pgfmathfloat@tmptoks=\expandafter{\expandafter0\the\pgfmathfloat@tmptoks}%
			\else
				% silently DROP digit
			\fi
		\else
			\pgfmathfloat@tmptoks=\expandafter{\expandafter0\the\pgfmathfloat@tmptoks}%
		\fi
		\advance\c@pgfmathroundto@offsetbehindperiod by1
		\ifnum\c@pgfmathroundto@offsetbehindperiod=0
			\ifpgfmathfloat@fixed@digits@after@period
				\def\pgfmathround@nextcmd{\pgfmathroundto@impl@ADD@ONE@ITERATE}%
			\else
				\def\pgfmathround@nextcmd{\pgfmathroundto@impl@ADD@ONE@ITERATE@gobble@dot}%
			\fi
		\else
			\def\pgfmathround@nextcmd{\pgfmathroundto@impl@ADD@ONE@ITERATE}%
		\fi
	\else
		% re-use this counter:
		\c@pgfmathroundto@lastzeros=#1
		\advance\c@pgfmathroundto@lastzeros by1
		\edef\pgfmathresult{\the\c@pgfmathroundto@lastzeros\the\pgfmathfloat@tmptoks}%
		\pgfmathfloat@tmptoks=\expandafter{\pgfmathresult}%
		\def\pgfmathround@nextcmd{\pgfmathroundto@impl@REVERSE@ITERATE}%
	\fi
	\pgfmathround@nextcmd
}


\def\pgfmathroundto@impl@discard@suffix@zeros{%
	\ifnum\c@pgfmathroundto@lastzeros=\c@pgfmathroundto@offsetbehindperiod
		\ifpgfmathround@impl@PREPERIOD@is@negative@zero
			\pgfmathfloatroundhasperiodfalse
			\aftergroup\pgfmathfloatroundhasperiodfalse
			\def\pgfmathresult{0}% write '0' instead of '-0'
		\else
			\expandafter\pgfmathroundto@impl@discard@period\pgfmathround@input\pgfmathfloat@EOI
		\fi
	\else
		\ifnum\c@pgfmathroundto@lastzeros=0
			\expandafter\pgfmathroundto@impl@REVERSE\the\pgfmathfloat@tmptoks\pgfmathfloat@EOI
		\else
			\expandafter\pgfmathroundto@impl@discard@suffix@zeros@ITERATE\the\pgfmathfloat@tmptoks\pgfmathfloat@EOI
		\fi
	\fi
}

% PRECONDITION: 
%    \c@pgfmathroundto@lastzeros > 0
\def\pgfmathroundto@impl@discard@suffix@zeros@ITERATE#1{%
	\advance\c@pgfmathroundto@lastzeros by-1
	\ifnum\c@pgfmathroundto@lastzeros=0
		\def\pgfmathround@nextcmd{\pgfmathroundto@impl@REVERSE}%
	\else
		\def\pgfmathround@nextcmd{\pgfmathroundto@impl@discard@suffix@zeros@ITERATE}%
	\fi
	\pgfmathround@nextcmd
}

% Usage:
% \pgfmathroundto@impl@REVERSE#1\pgfmathfloat@EOI
% -> writes #1 reversed into \pgfmathfloat@tmptoks
\def\pgfmathroundto@impl@REVERSE{%
	\pgfmathfloat@tmptoks={}%
	\pgfmathroundto@impl@REVERSE@ITERATE
}

\def\pgfmathroundto@impl@REVERSE@ITERATE{%
	\pgfutil@ifnextchar\pgfmathfloat@EOI{%
		\edef\pgfmathresult{\the\pgfmathfloat@tmptoks}%
		\pgfmathroundto@impl@gobble
	}{%
		\pgfmathroundto@impl@REVERSE@NEXT
	}%
}

\def\pgfmathroundto@impl@REVERSE@NEXT#1{%
	\pgfmathfloat@tmptoks=\expandafter{\expandafter#1\the\pgfmathfloat@tmptoks}%
	\pgfmathroundto@impl@REVERSE@ITERATE
}

\def\pgfmathroundto@impl@BEGIN@DOT.{%
	\pgfmathfloat@tmptoks=\expandafter{\expandafter.\the\pgfmathfloat@tmptoks}%
	\c@pgfmathroundto@offsetbehindperiod=0
	\pgfmathroundto@impl@ITERATE@DOT
}
\def\pgfmathroundto@impl@ITERATE@DOT{%
	\pgfutil@ifnextchar\pgfmathfloat@EOI{%
		% finished.
		\pgfmathroundto@impl@gobble@and@start
	}{%
		\pgfmathroundto@impl@NEXT@DOT
	}%
}
\def\pgfmathroundto@impl@NEXT@DOT#1{%
	\ifnum\c@pgfmathroundto@offsetbehindperiod=\c@pgfmathroundto@prec
		\def\pgfmathround@next{#1}%
		\def\pgfmathround@nextcmd{\pgfmathroundto@impl@gobble@rest@and@start}%
	\else
		\advance\c@pgfmathroundto@offsetbehindperiod by1
		\ifnum#1=0
			\advance\c@pgfmathroundto@lastzeros by1
		\else
			\c@pgfmathroundto@lastzeros=0
		\fi
		\pgfmathfloat@tmptoks=\expandafter{\expandafter#1\the\pgfmathfloat@tmptoks}%
		\def\pgfmathround@nextcmd{\pgfmathroundto@impl@ITERATE@DOT}%
	\fi
	\pgfmathround@nextcmd
}%

% in contrast to pgfmathroundto@impl@ITERATE@NODOT, this method here
% checks also for signs
\def\pgfmathroundto@impl@ITERATE@NODOT@firstcall#1{%
	\def\pgfmathround@cur{#1}%
	\ifx\pgfmathround@cur\pgfmathfloat@EOI
		\pgfmathround@impl@PREPERIOD@is@negative@zerofalse
		\def\pgfmathround@nextcmd{\pgfmathroundto@impl@start}%
	\else
		\ifx\pgfmathround@cur\pgfmathfloatparsenumber@tok@PERIOD
			\pgfmathround@impl@PREPERIOD@is@negative@zerofalse
			\def\pgfmathround@nextcmd{\pgfmathroundto@impl@BEGIN@DOT.}%
		\else
			\ifx\pgfmathround@cur\pgfmathfloatparsenumber@tok@MINUS
			\else
				\pgfmathround@impl@PREPERIOD@is@negative@zerofalse
			\fi
			\pgfmathfloat@tmptoks=\expandafter{\expandafter#1\the\pgfmathfloat@tmptoks}%
			\def\pgfmathround@nextcmd{\pgfmathroundto@impl@ITERATE@NODOT}%
		\fi
	\fi
	\pgfmathround@nextcmd
}

\def\pgfmathroundto@impl@ITERATE@NODOT#1{%
	\def\pgfmathround@cur{#1}%
	\ifx\pgfmathround@cur\pgfmathfloat@EOI
		\def\pgfmathround@nextcmd{\pgfmathroundto@impl@start}%
	\else
		\ifx\pgfmathround@cur\pgfmathfloatparsenumber@tok@PERIOD
			\def\pgfmathround@nextcmd{\pgfmathroundto@impl@BEGIN@DOT.}%
		\else
			\ifx\pgfmathround@cur\pgfmathfloatparsenumber@tok@ZERO
			\else
				\pgfmathround@impl@PREPERIOD@is@negative@zerofalse
			\fi
			\pgfmathfloat@tmptoks=\expandafter{\expandafter#1\the\pgfmathfloat@tmptoks}%
			\def\pgfmathround@nextcmd{\pgfmathroundto@impl@ITERATE@NODOT}%
		\fi
	\fi
	\pgfmathround@nextcmd
}

%--------------------------------------------
% END of pgfmathroundto implementation.
%--------------------------------------------


% flags, mantisse and exponent has already been stored into
% \pgfmathfloat@a@* [using ...@Mtok]
%
% PRECONDITION:
%   \ifpgfmathfloatroundhasperiod = \iftrue outside of the current
%   group
%
% POSTCONDITION:
%   \ifpgfmathfloatroundhasperiod will be set after the current TeX
%   group.
\def\pgfmathfloatround@impl{%
	\expandafter\pgfmathroundto@impl\expandafter{\the\pgfmathfloat@a@Mtok}%
	\ifpgfmathfloatroundmayneedrenormalize
		\ifpgfmathfloatroundhasperiod
			\expandafter\pgfmathfloatround@impl@renormalize\pgfmathresult\pgfmathfloat@EOI%
		\else
			\expandafter\pgfmathfloatround@impl@renormalize\pgfmathresult.\pgfmathfloat@EOI%
		\fi
		\advance\pgfmathfloat@a@E by1
	\fi
	\edef\pgfmathresult{\the\pgfmathfloat@a@S\pgfmathresult e\the\pgfmathfloat@a@E}%
}

\def\pgfmathfloatround@impl@renormalize#1#2.#3\pgfmathfloat@EOI{%
	\pgfmathroundto@impl{#1.#2#3}%
}





% ATTENTION: this thing REQUIRES a period in the mantisse!
% collects everything into \pgfmathresult
\def\pgfmathfloattofixed@impl#1.#2\relax{%
	\ifnum\pgfmathfloat@a@E<0
		\pgfmathfloat@a@Mtok={0.}%
		\pgfutil@loop
		\ifnum\pgfmathfloat@a@E<-1
			\pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok 0}%
			\advance\pgfmathfloat@a@E by1
		\pgfutil@repeat
		\def\pgfmathfloat@loc@TMPb{#2}%
		\def\pgfmathfloat@loc@TMPc{0}%
		\ifx\pgfmathfloat@loc@TMPb\pgfmathfloat@loc@TMPc
			\edef\pgfmathresult{\the\pgfmathfloat@a@Mtok #1}%
		\else
			\edef\pgfmathresult{\the\pgfmathfloat@a@Mtok #1#2}%
		\fi
	\else
		\ifnum\pgfmathfloat@a@E=0%
			\edef\pgfmathresult{#1.#2}%
		\else
			\pgfmathfloat@a@Mtok={#1}%
			\pgfmathfloattofixed@impl@collectmantisse#2\count\pgfmathfloat@a@E
			\edef\pgfmathresult{\the\pgfmathfloat@a@Mtok}%
		\fi
	\fi
}

\def\pgfmathfloattofixed@impl@collectmantisse#1#2\count#3{%
	\pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok #1}%
	\advance\pgfmathfloat@a@E by-1%
	\def\pgfmathfloat@loc@TMPb{#2}%
	\ifx\pgfmathfloat@loc@TMPb\pgfutil@empty
		\pgfutil@loop
		\ifnum\pgfmathfloat@a@E>0%
			\pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok 0}%
			\advance\pgfmathfloat@a@E by-1%
		\pgfutil@repeat
		\pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok .0}%
	\else
		\ifnum\pgfmathfloat@a@E=0
			\pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok .#2}%
		\else
			\pgfmathfloattofixed@impl@collectmantisse#2\count#3%
		\fi
	\fi
}


% ============================================
%
%
% \pgfmathfloatparsenumber implementation
%
%
% ============================================


% accepted parser tokens:
\def\pgfmathfloatparsenumber@tok@ONE{1}
\def\pgfmathfloatparsenumber@tok@TWO{2}
\def\pgfmathfloatparsenumber@tok@THREE{3}
\def\pgfmathfloatparsenumber@tok@FOUR{4}
\def\pgfmathfloatparsenumber@tok@FIVE{5}
\def\pgfmathfloatparsenumber@tok@SIX{6}
\def\pgfmathfloatparsenumber@tok@SEVEN{7}
\def\pgfmathfloatparsenumber@tok@EIGHT{8}
\def\pgfmathfloatparsenumber@tok@NINE{9}
\def\pgfmathfloatparsenumber@tok@ZERO{0}
\def\pgfmathfloatparsenumber@tok@e{e}
\def\pgfmathfloatparsenumber@tok@E{E}
\def\pgfmathfloatparsenumber@tok@PLUS{+}
\def\pgfmathfloatparsenumber@tok@MINUS{-}
\def\pgfmathfloatparsenumber@tok@n{n}
\def\pgfmathfloatparsenumber@tok@N{N}
\def\pgfmathfloatparsenumber@tok@i{i}
\def\pgfmathfloatparsenumber@tok@I{I}
\def\pgfmathfloatparsenumber@tok@PERIOD{.}

\newif\ifpgfmathfloatparsenumberpendingperiod

% Starts a finite-start-machine parser to read a number.
%
% It assigns \pgfmathfloat@a@S, \pgfmathfloat@a@Mtok, \pgfmathfloat@a@E.
\def\pgfmathfloatparsenumber@impl#1{%
	\pgfmathfloatparsenumberpendingperiodfalse
	\pgfmathfloat@tmptoks={}% this register is used to collect PENDING ZEROS
	\pgfmathfloat@a@E=0
	% start parsing: check for sign:
	\def\pgfmathfloatparsenumber@curtok{#1}%
	\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@PLUS
		\pgfmathfloat@a@S=1\relax%
		\def\pgfmathfloatparsenumber@NEXT{\pgfmathfloatparsenumber@impl@init}%
	\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@MINUS
			\pgfmathfloat@a@S=2\relax%
			\def\pgfmathfloatparsenumber@NEXT{\pgfmathfloatparsenumber@impl@init}%
		\else
			\pgfmathfloat@a@S=1\relax%
			\def\pgfmathfloatparsenumber@NEXT{\pgfmathfloatparsenumber@impl@init#1}%
		\fi
	\fi
	\pgfmathfloatparsenumber@NEXT
}

\def\pgfmathfloatparsenumber@sanitize@digit{%
	\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@ONE
	\else
	\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@TWO
	\else
	\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@THREE
	\else
	\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@FOUR
	\else
	\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@FIVE
	\else
	\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@SIX
	\else
	\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@SEVEN
	\else
	\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@EIGHT
	\else
	\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@NINE
	\else
		\def\pgfmathfloatparsenumber@NEXT{\expandafter\pgfmathfloatparsenumber@impl@error\pgfmathfloatparsenumber@curtok}%
	\fi\fi\fi\fi\fi\fi\fi\fi\fi
}

% FROM: checksign.
%
\def\pgfmathfloatparsenumber@impl@init#1{%
	\def\pgfmathfloatparsenumber@curtok{#1}%
	\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@n
		\def\pgfmathfloatparsenumber@NEXT{\pgfmathfloatparsenumber@impl@readnan}%
	\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@i
			\def\pgfmathfloatparsenumber@NEXT{\pgfmathfloatparsenumber@impl@readinf}%
		\else
			\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@ZERO
				\def\pgfmathfloatparsenumber@NEXT{\pgfmathfloatparsenumber@impl@leadingzero}%
			\else
				\def\pgfmathfloatparsenumber@NEXT{%
					\pgfmathfloat@a@Mtok={#1}%
					\pgfmathfloatparsenumberpendingperiodtrue
					\pgfmathfloatparsenumber@impl@positiveexp}%
				\pgfmathfloatparsenumber@sanitize@digit
			\fi
		\fi
	\fi
	\pgfmathfloatparsenumber@NEXT
}

\def\pgfmathfloatparsenumber@impl@error#1\pgfmathfloat@EOI{%
	\begingroup
	\pgfmathfloat@a@Mtok={#1}%
	\pgfmath@error{Could not read input number, sorry. The unreadable part was near '\the\pgfmathfloat@a@Mtok'.}%
	\endgroup
}%

\def\pgfmathfloatparsenumber@impl@finish#1\pgfmathfloat@EOI{}

\def\pgfmathfloatparsenumber@impl@readnan an{%
	\pgfmathfloat@a@S=3\relax%
	\pgfmathfloat@a@Mtok={0.0}%
	\pgfmathfloat@a@E=0%
	\pgfmathfloatparsenumber@impl@finish
}
\def\pgfmathfloatparsenumber@impl@readinf nf{%
	\ifnum\pgfmathfloat@a@S=1
		\pgfmathfloat@a@S=4\relax%
		\pgfmathfloat@a@Mtok={0.0}%
	\else
		\pgfmathfloat@a@S=5\relax%
		\pgfmathfloat@a@Mtok={0.0}%
	\fi
	\pgfmathfloat@a@E=0%
	\pgfmathfloatparsenumber@impl@finish
}
\def\pgfmathfloatparsenumber@impl@leadingzero#1{%
	\def\pgfmathfloatparsenumber@curtok{#1}%
	\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@ZERO
		\def\pgfmathfloatparsenumber@NEXT{%
			\pgfmathfloatparsenumber@impl@leadingzero}%
	\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@PERIOD
			\def\pgfmathfloatparsenumber@NEXT{%
				\pgfmathfloat@a@E=-1
				\pgfmathfloatparsenumber@impl@leadingzero@foundperiod}%
		\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@e
			\def\pgfmathfloatparsenumber@NEXT{%
				\pgfmathfloat@a@S=0\relax%
				\pgfmathfloat@a@Mtok={0.0}%
				\pgfmathfloat@a@E=0%
				\pgfmathfloatparsenumber@impl@readexponent}%
		\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@E
			\def\pgfmathfloatparsenumber@NEXT{%
				\pgfmathfloat@a@S=0\relax%
				\pgfmathfloat@a@Mtok={0.0}%
				\pgfmathfloat@a@E=0%
				\pgfmathfloatparsenumber@impl@readexponent}%
		\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloat@EOI
			\def\pgfmathfloatparsenumber@NEXT{%
				\pgfmathfloat@a@S=0\relax%
				\pgfmathfloat@a@Mtok={0.0}%
				\pgfmathfloat@a@E=0%
				}%
		\else
		\def\pgfmathfloatparsenumber@NEXT{%
			\pgfmathfloat@a@Mtok={#1}%
			\pgfmathfloatparsenumberpendingperiodtrue
			\pgfmathfloatparsenumber@impl@positiveexp}%
		\pgfmathfloatparsenumber@sanitize@digit
		\fi\fi\fi
		\fi
	\fi
	\pgfmathfloatparsenumber@NEXT
}

\def\pgfmathfloatparsenumber@impl@leadingzero@foundperiod#1{%
	\def\pgfmathfloatparsenumber@curtok{#1}%
	\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@ZERO
		\def\pgfmathfloatparsenumber@NEXT{%
			\advance\pgfmathfloat@a@E by-1
			\pgfmathfloatparsenumber@impl@leadingzero@foundperiod}%
	\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@e
			\def\pgfmathfloatparsenumber@NEXT{%
				\pgfmathfloat@a@S=0\relax%
				\pgfmathfloat@a@Mtok={0.0}%
				\pgfmathfloat@a@E=0%
				\pgfmathfloatparsenumber@impl@readexponent}%
		\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@E
			\def\pgfmathfloatparsenumber@NEXT{%
				\pgfmathfloat@a@S=0\relax%
				\pgfmathfloat@a@Mtok={0.0}%
				\pgfmathfloat@a@E=0%
				\pgfmathfloatparsenumber@impl@readexponent}%
		\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloat@EOI
			\def\pgfmathfloatparsenumber@NEXT{%
				\pgfmathfloat@a@S=0\relax%
				\pgfmathfloat@a@Mtok={0.0}%
				\pgfmathfloat@a@E=0%
				}%
		\else
		\def\pgfmathfloatparsenumber@NEXT{%
			\pgfmathfloat@a@Mtok={#1}%
			\pgfmathfloatparsenumberpendingperiodtrue
			\pgfmathfloatparsenumber@impl@finish@number@after@period}%
		\pgfmathfloatparsenumber@sanitize@digit
		\fi\fi\fi
	\fi
	\pgfmathfloatparsenumber@NEXT
}


\def\pgfmathfloatparsenumber@impl@positiveexp#1{%
	\def\pgfmathfloatparsenumber@curtok{#1}%
	\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@ZERO
		\def\pgfmathfloatparsenumber@NEXT{%
			\advance\pgfmathfloat@a@E by1
			\pgfmathfloat@tmptoks=\expandafter{\the\pgfmathfloat@tmptoks0}%
			\pgfmathfloatparsenumber@impl@pendingzeros@positiveexp}%
	\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@PERIOD
			\def\pgfmathfloatparsenumber@NEXT{\pgfmathfloatparsenumber@impl@finish@number@after@period}%
		\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@e
			\def\pgfmathfloatparsenumber@NEXT{\pgfmathfloatparsenumber@impl@readexponent}%
		\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@E
			\def\pgfmathfloatparsenumber@NEXT{\pgfmathfloatparsenumber@impl@readexponent}%
		\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloat@EOI
			\def\pgfmathfloatparsenumber@NEXT{}%
		\else
		\def\pgfmathfloatparsenumber@NEXT{%
			\advance\pgfmathfloat@a@E by1
			\ifpgfmathfloatparsenumberpendingperiod
				\pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok.}%
				\pgfmathfloatparsenumberpendingperiodfalse
			\fi
			\pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok#1}%
			\pgfmathfloatparsenumber@impl@positiveexp}%
		\pgfmathfloatparsenumber@sanitize@digit
		\fi\fi\fi
		\fi
	\fi
	\pgfmathfloatparsenumber@NEXT
}

\def\pgfmathfloatparsenumber@impl@readexponent#1\pgfmathfloat@EOI{%
	\advance\pgfmathfloat@a@E by#1\relax
}

\def\pgfmathfloatparsenumber@impl@pendingzeros@positiveexp#1{%
	\def\pgfmathfloatparsenumber@curtok{#1}%
	\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@ZERO
		\def\pgfmathfloatparsenumber@NEXT{%
			\pgfmathfloat@tmptoks=\expandafter{\the\pgfmathfloat@tmptoks0}%
			\advance\pgfmathfloat@a@E by1
			\pgfmathfloatparsenumber@impl@pendingzeros@positiveexp}%
	\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@PERIOD
			\def\pgfmathfloatparsenumber@NEXT{\pgfmathfloatparsenumber@impl@finish@number@after@period}%
		\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@e
			\def\pgfmathfloatparsenumber@NEXT{\pgfmathfloatparsenumber@impl@readexponent}%
		\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@E
			\def\pgfmathfloatparsenumber@NEXT{\pgfmathfloatparsenumber@impl@readexponent}%
		\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloat@EOI
			\def\pgfmathfloatparsenumber@NEXT{}%
		\else
		\def\pgfmathfloatparsenumber@NEXT{%
			\advance\pgfmathfloat@a@E by1
			\ifpgfmathfloatparsenumberpendingperiod
				\pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok.}%
				\pgfmathfloatparsenumberpendingperiodfalse
			\fi
			\pgfmathfloat@a@Mtok=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfmathfloat@a@Mtok\the\pgfmathfloat@tmptoks}%
			\pgfmathfloat@tmptoks={}%
			\pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok#1}%
			\pgfmathfloatparsenumber@impl@positiveexp}%
		\pgfmathfloatparsenumber@sanitize@digit
		\fi\fi\fi
		\fi
	\fi
	\pgfmathfloatparsenumber@NEXT
}

\def\pgfmathfloatparsenumber@impl@finish@number@after@period#1{%
	\def\pgfmathfloatparsenumber@curtok{#1}%
	\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@ZERO
		\def\pgfmathfloatparsenumber@NEXT{%
			\pgfmathfloat@tmptoks=\expandafter{\the\pgfmathfloat@tmptoks0}%
			\pgfmathfloatparsenumber@impl@pendingzeros}%
	\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@e
			\def\pgfmathfloatparsenumber@NEXT{\pgfmathfloatparsenumber@impl@readexponent}%
		\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@E
			\def\pgfmathfloatparsenumber@NEXT{\pgfmathfloatparsenumber@impl@readexponent}%
		\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloat@EOI
			\def\pgfmathfloatparsenumber@NEXT{}%
		\else
		\def\pgfmathfloatparsenumber@NEXT{%
			\ifpgfmathfloatparsenumberpendingperiod
				\pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok.}%
				\pgfmathfloatparsenumberpendingperiodfalse
			\fi
			\pgfmathfloat@a@Mtok=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfmathfloat@a@Mtok\the\pgfmathfloat@tmptoks}%
			\pgfmathfloat@tmptoks={}%
			\pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok#1}%
			\pgfmathfloatparsenumber@impl@finish@number@after@period}%
		\pgfmathfloatparsenumber@sanitize@digit
		\fi\fi\fi
	\fi
	\pgfmathfloatparsenumber@NEXT
}

\def\pgfmathfloatparsenumber@impl@pendingzeros#1{%
	\def\pgfmathfloatparsenumber@curtok{#1}%
	\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@ZERO
		\def\pgfmathfloatparsenumber@NEXT{%
			\pgfmathfloat@tmptoks=\expandafter{\the\pgfmathfloat@tmptoks0}%
			\pgfmathfloatparsenumber@impl@pendingzeros}%
	\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@e
			\def\pgfmathfloatparsenumber@NEXT{\pgfmathfloatparsenumber@impl@readexponent}%
		\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloatparsenumber@tok@E
			\def\pgfmathfloatparsenumber@NEXT{\pgfmathfloatparsenumber@impl@readexponent}%
		\else
		\ifx\pgfmathfloatparsenumber@curtok\pgfmathfloat@EOI
			\def\pgfmathfloatparsenumber@NEXT{}%
		\else
		\def\pgfmathfloatparsenumber@NEXT{%
			\ifpgfmathfloatparsenumberpendingperiod
				\pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok.}%
				\pgfmathfloatparsenumberpendingperiodfalse
			\fi
			\pgfmathfloat@a@Mtok=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfmathfloat@a@Mtok\the\pgfmathfloat@tmptoks}%
			\pgfmathfloat@tmptoks={}%
			\pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok#1}%
			\pgfmathfloatparsenumber@impl@finish@number@after@period}%
		\pgfmathfloatparsenumber@sanitize@digit
		\fi\fi\fi
	\fi
	\pgfmathfloatparsenumber@NEXT
}





==> pgfplotstable.code.tex <==
%--------------------------------------------
%
% Package numtable
%
% Provides support to read and work with abstact numeric tables of the
% form
%
% COLUMN1	COLUMN2 COLUMN3
% 1 		2		3
% 4			4		552
% 1e124		0.00001	1.2345e-12
% ...
%
% Copyright 2007/2008 by Christian Feuersänger.
%
% This program is free software: you can redistribute it and/or modify
% it under the terms of the GNU General Public License as published by
% the Free Software Foundation, either version 3 of the License, or
% (at your option) any later version.
% 
% This program is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
% GNU General Public License for more details.
% 
% You should have received a copy of the GNU General Public License
% along with this program.  If not, see <http://www.gnu.org/licenses/>.
%
%--------------------------------------------

\newif\ifpgfplotstable@search@header
\newcount\c@pgfplotstable@counta
\newwrite\pgfplotstable@outfile
\newif\ifpgfplotstabletypesetdebug
\newif\ifpgfplotstableuserow

% should always be false; use only in grouped internal macros
\newif\ifpgfplots@table@options@areset
\newif\ifpgfplots@tableread@to@listener

\input pgfplotstable.coltype.code.tex

% keys which are NOT predefined:
% /pgfplots/table/alias/<col alias>/.initial={<real col>}
% /pgfplots/table/columns/<col name>/.style={}
% /pgfplots/table/display columns/<col index>/.style={}
% /pgfplots/table/create on use/<col name>/.style={create options}
\pgfkeys{%
	/pgfplots/table/header/.is if=pgfplotstable@search@header,
	/pgfplots/table/header=true,
	/pgfplots/table/x index/.store in=\pgfplots@plot@tbl@xindex,
	/pgfplots/table/x index=0,
	/pgfplots/table/x/.store in=\pgfplots@plot@tbl@x,
	/pgfplots/table/x=,
	/pgfplots/table/y index/.store in=\pgfplots@plot@tbl@yindex,
	/pgfplots/table/y index=1,
	/pgfplots/table/y/.store in=\pgfplots@plot@tbl@y,
	/pgfplots/table/y=,
	/pgfplots/table/x error index/.initial=,
	/pgfplots/table/y error index/.initial=,
	/pgfplots/table/x error/.initial=,
	/pgfplots/table/y error/.initial=,
	/pgfplots/table/row predicate/.code={},
	/pgfplots/table/skip rows between index/.style 2 args={%
		/pgfplots/table/row predicate/.append code={%
			\ifnum##1<#1\relax
			\else
				\ifnum##1<#2\relax
					\pgfplotstableuserowfalse
				\fi
			\fi}
	},
	/pgfplots/table/select equal part entry of/.style 2 args={%
		/pgfplots/table/row predicate/.code={%
			\pgfplotstableuserowtrue
			\begingroup
			% this group re-uses counters as temporary variables.
			\c@pgfplotstable@colindex=\pgfplotstablerows\relax
			\divide\c@pgfplotstable@colindex by#2\relax
			\edef\pgfplotstablepartsize{\the\c@pgfplotstable@colindex}%
			% This here should create empty cells such that
			% remaining entries are distributed equally:
			\c@pgfplotstable@rowindex=\c@pgfplotstable@colindex
			\multiply\c@pgfplotstable@rowindex by#2\relax
			\ifnum\c@pgfplotstable@rowindex<\pgfplotstablerows\relax
				\c@pgfplotstable@colindex=\pgfplotstablerows\relax
				\advance\c@pgfplotstable@colindex by-\c@pgfplotstable@rowindex
				\advance\c@pgfplotstable@colindex by\pgfplotstablepartsize				
				\edef\pgfplotstablepartsize{\the\c@pgfplotstable@colindex}%
			\fi
			%
			\multiply\c@pgfplotstable@colindex by#1\relax
			\ifnum##1<\c@pgfplotstable@colindex\relax
				\aftergroup\pgfplotstableuserowfalse
			\else
				\advance\c@pgfplotstable@colindex by\pgfplotstablepartsize\relax
				\ifnum##1<\c@pgfplotstable@colindex\relax
				\else
					\aftergroup\pgfplotstableuserowfalse
				\fi
			\fi
			\endgroup
		}%
	},
	/pgfplots/table/col sep/.is choice,
	/pgfplots/table/col sep/space/.code		= {\def\pgfplotstableread@COLSEP@CASE{0}},
	/pgfplots/table/col sep/comma/.code		= {\def\pgfplotstableread@COLSEP@CASE{1}},
	/pgfplots/table/col sep/semicolon/.code	= {\def\pgfplotstableread@COLSEP@CASE{2}},
	/pgfplots/table/col sep/colon/.code		= {\def\pgfplotstableread@COLSEP@CASE{3}},
	/pgfplots/table/col sep/braces/.code	= {\def\pgfplotstableread@COLSEP@CASE{4}},
	/pgfplots/table/col sep=space,
	% columns={name1,name2}
	% or
	% columns={[index]2,name2,name3,[index]5}
	/pgfplots/table/columns/.initial=,
	/pgfplots/table/column name/.initial=\pgfkeysnovalue,
	%
	% this thing here allows to MODIFY 'column name'.
	%
	% Argument #1 is the current column name, that means after
	% evaluating 'column name'. If this key changes anything, it
	% should write its result back into 'column name'.
	%
	% That means you can use 'column name' to assign the name as such
	% and 'assign column name' to generate final TeX code (for example
	% to insert \multicolumn{1}{c}{#1} or so).
	% default is empty which means no change.
	%/pgfplots/table/assign column name/.code={
	%	\pgfkeyssetvalue{/pgfplots/table/column name}{#1}%
	%},
	%
	%
	%
	% A style which inserts \multicolumn{1}{#1}{<column name>} for
	% each column name.
	% The column name as such can be set with the 'column name' option.
	/pgfplots/table/multicolumn names/.style={%
		/pgfplots/table/assign column name/.code={%
			\pgfkeyssetvalue{/pgfplots/table/column name}{\multicolumn{1}{#1}{##1}}%
		}%
	},
	/pgfplots/table/multicolumn names/.default=c,
	/pgfplots/table/dec sep align/.style={%
		/pgf/number format/assume math mode,
		/pgf/number format/@dec sep mark={&},
		/pgfplots/table/assign column name/.code={%
			\pgfkeyssetvalue{/pgfplots/table/column name}{\multicolumn{2}{#1}{##1}}%
		},%
		/pgfplots/table/column type={>{$}r<{$}@{}>{$}l<{$}},
		/pgfplots/table/assign cell content/.code={%
			\def\pgfmathresult{##1}%
			\ifx\pgfmathresult\pgfutil@empty
				\def\pgfmathresult{&}%
			%	\pgfutil@in@false
			\else
				\pgfmathprintnumberto{##1}\pgfmathresult%
			%	\expandafter\pgfutil@in@\expandafter&\expandafter{\pgfmathresult}%
			\fi
			%\ifpgfutil@in@
			%\else
			%	\expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult&}%
			%\fi
			\pgfkeyslet{/pgfplots/table/@cell content}\pgfmathresult
		},
	},
	/pgfplots/table/dec sep align/.default=c,
	/pgfplots/table/sci sep align/.style={%
		/pgf/number format/assume math mode,
		/pgf/number format/@sci exponent mark={&},
		/pgfplots/table/assign column name/.code={%
			\pgfkeyssetvalue{/pgfplots/table/column name}{\multicolumn{2}{#1}{##1}}%
		},%
		/pgfplots/table/column type={>{$}r<{$}@{}>{$}l<{$}},
		/pgfplots/table/assign cell content/.code={%
			\def\pgfmathresult{##1}%
			\ifx\pgfmathresult\pgfutil@empty
				\def\pgfmathresult{&}%
				\pgfutil@in@true
			\else
				\pgfmathprintnumberto{##1}\pgfmathresult%
				\expandafter\pgfutil@in@\expandafter&\expandafter{\pgfmathresult}%
			\fi
			\ifpgfutil@in@
			\else
				\expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult&}%
			\fi
			\pgfkeyslet{/pgfplots/table/@cell content}\pgfmathresult
		},
	},
	/pgfplots/table/sci sep align/.default=c,
	%
	% A style which can be used together with the 'dcolumn' package by
	% David Carlisle.
	% #1: the dcolumn type, defaults to 'D{.}{.}{2}'
	% #2: the column name type, defaults to 'c'
	/pgfplots/table/dcolumn/.style 2 args={%
		/pgf/number format/assume math mode,
		column type={#1},
		multicolumn names=#2,
	},
	/pgfplots/table/dcolumn/.default={D{.}{.}{2}}{c},
	/pgfplots/table/column type/.initial={c},
	/pgfplots/table/every table/.style={},
	/pgfplots/table/every even row/.style={},
	/pgfplots/table/every odd row/.style={},
	/pgfplots/table/every last row/.style={},
	/pgfplots/table/every first row/.style={},
	/pgfplots/table/every head row/.style={},
	/pgfplots/table/every first column/.style={},
	/pgfplots/table/every last column/.style={},
	/pgfplots/table/every even column/.style={},
	/pgfplots/table/every odd column/.style={},
	/pgfplots/table/before row/.initial=,
	/pgfplots/table/after row/.initial=,
	/pgfplots/table/begin table/.initial={\begin{tabular}},
	/pgfplots/table/end table/.initial={\end{tabular}},
	/pgfplots/table/outfile/.initial=,
	/pgfplots/table/debug/.is if=pgfplotstabletypesetdebug,
	%
	% will be redefined by |assign cell content| for every cell:
	/pgfplots/table/@cell content/.initial=,
	%
	% #1: the cells content as it has been found in the input table
	% this command key should somehow fill |cell content|.
	/pgfplots/table/assign cell content/.code={%
		\def\pgfmathresult{#1}%
		\ifx\pgfmathresult\pgfutil@empty
		\else
			\pgfmathprintnumberto{#1}\pgfmathresult%
		\fi
		\pgfkeyslet{/pgfplots/table/@cell content}\pgfmathresult
	},
	%
	% this here is the default formatting. It uses
	% \pgfmathprintnumber.
	/pgfplots/table/assign cell content as number/.code={%
		\def\pgfmathresult{#1}%
		\ifx\pgfmathresult\pgfutil@empty
		\else
			\pgfmathprintnumberto{#1}\pgfmathresult%
		\fi
		\pgfkeyslet{/pgfplots/table/@cell content}\pgfmathresult
	},
	/pgfplots/table/string type/.style={%
		/pgfplots/table/assign cell content/.style={%
			/pgfplots/table/@cell content={##1}%
		}%
	},%
	/pgfplots/table/set content/.style={%
		/pgfplots/table/postproc cell content/.style={%
			/pgfplots/table/@cell content={#1}%
		}%
	},%
	%
	/pgfplots/table/postproc cell content/.code={},
	/pgfplots/table/preproc cell content/.code={},
	%
	/pgfplots/table/multiply -1/.style={%
		/pgfplots/table/preproc cell content/.append code={%
			\pgfkeysgetvalue{/pgfplots/table/@cell content}\pgfmathresult
			\ifx\pgfmathresult\empty
			\else
				\pgfmathfloatparsenumber{\pgfmathresult}%
				\let\pgfmatharga=\pgfmathresult
				\pgfmathfloatcreate{2}{1.0}{0}%
				\let\pgfmathargb=\pgfmathresult
				\pgfmathfloatmultiply@{\pgfmatharga}{\pgfmathargb}%
				\pgfmathfloattosci@\pgfmathresult
				\pgfkeyslet{/pgfplots/table/@cell content}{\pgfmathresult}%
			\fi
		}
	},
	/pgfplots/table/empty cells with/.style={%
		/pgfplots/table/postproc cell content/.append code={%
			\ifnum\pgfplotstablepartno=0
				\pgfkeysgetvalue{/pgfplots/table/@cell content}\pgfmathresult
				\ifx\pgfmathresult\pgfutil@empty
					\pgfkeyssetvalue{/pgfplots/table/@cell content}{#1}%
				\fi
			\fi
		}%
	},
	%
	/pgfplots/table/font/.initial=,
	/pgfplots/table/.unknown/.code={%
		\pgfqkeys{/pgf/number format}{\pgfkeyscurrentname=#1}%
	},%
	/pgfplots/table/create col/assign first/.style={
		/pgfplots/table/create col/assign%
	},
	/pgfplots/table/create col/assign last/.style={
		/pgfplots/table/create col/assign%
	},
	/pgfplots/table/create col/assign/.style={
		/pgfplots/table/create col/next content={}%
	},
	/pgfplots/table/create col/next content/.initial={},
	/pgfplots/table/create col/expr/.style={%
		/pgfplots/table/create col/assign/.code={%
			\pgfmathparse{#1}%
			\pgfkeyslet{/pgfplots/table/create col/next content}\pgfmathresult%
		}%
	},%
	/pgfplots/table/create col/quotient/.style={%
		/pgfplots/table/columns={#1},
		/pgfplots/table/create col/assign first/.style={%
			/pgfplots/table/create col/next content=
		},%
		/pgfplots/table/create col/assign/.code={%
			\pgfmathfloatparsenumber{\prevrow{#1}}%
			\let\pgfmatharga=\pgfmathresult
			\pgfmathfloatparsenumber{\thisrow{#1}}%
			\let\pgfmathargb=\pgfmathresult
			\let\pgfmathaccuma=\pgfmathargb
			\pgfmathfloatdivide@{\pgfmatharga}{\pgfmathargb}%
			\expandafter\pgfmathfloattosci@\expandafter{\pgfmathresult}%
			\pgfkeyslet{/pgfplots/table/create col/next content}\pgfmathresult%
		}%
	},%
	/pgfplots/table/create col/iquotient/.style={%
		/pgfplots/table/columns={#1},
		/pgfplots/table/create col/assign first/.style={%
			/pgfplots/table/create col/next content=
		},%
		/pgfplots/table/create col/assign/.code={%
			\pgfmathfloatparsenumber{\prevrow{#1}}%
			\let\pgfmathargb=\pgfmathresult
			\pgfmathfloatparsenumber{\thisrow{#1}}%
			\let\pgfmatharga=\pgfmathresult
			\let\pgfmathaccuma=\pgfmathargb
			\pgfmathfloatdivide@{\pgfmatharga}{\pgfmathargb}%
			\expandafter\pgfmathfloattosci@\expandafter{\pgfmathresult}%
			\pgfkeyslet{/pgfplots/table/create col/next content}\pgfmathresult%
		}%
	},%
	%
	% Produces 'log2( \prevrow{#1}/\thisrow{#1} )
	%
	% Assumeing that every row contains error(h) = O(h^alpha)
	% and h_this = h_prev/2, this result in 'alpha', the convergence
	% rate.
	/pgfplots/table/create col/dyadic refinement rate/.style={%
		/pgfplots/table/columns={#1},
		/pgfplots/table/create col/assign first/.style={%
			/pgfplots/table/create col/next content=
		},%
		/pgfplots/table/create col/assign/.code={%
			\pgfmathfloatparsenumber{\prevrow{#1}}%
			\let\pgfmatharga=\pgfmathresult
			\pgfmathfloatparsenumber{\thisrow{#1}}%
			\let\pgfmathargb=\pgfmathresult
			\let\pgfmathaccuma=\pgfmathargb
			\pgfmathfloatdivide@{\pgfmatharga}{\pgfmathargb}%
			\pgfmathlog@float{\pgfmathresult}%
			\ifx\pgfmathresult\pgfutil@empty
			\else
				\pgfmathmultiply@{1.442695}{\pgfmathresult}%
			\fi
			\pgfkeyslet{/pgfplots/table/create col/next content}\pgfmathresult%
		}%
	},%
	/pgfplots/table/create col/idyadic refinement rate/.style={%
		/pgfplots/table/columns={#1},
		/pgfplots/table/create col/assign first/.style={%
			/pgfplots/table/create col/next content=
		},%
		/pgfplots/table/create col/assign/.code={%
			\pgfmathfloatparsenumber{\prevrow{#1}}%
			\let\pgfmathargb=\pgfmathresult
			\pgfmathfloatparsenumber{\thisrow{#1}}%
			\let\pgfmatharga=\pgfmathresult
			\let\pgfmathaccuma=\pgfmathargb
			\pgfmathfloatdivide@{\pgfmatharga}{\pgfmathargb}%
			\pgfmathlog@float{\pgfmathresult}%
			\ifx\pgfmathresult\pgfutil@empty
			\else
				\pgfmathmultiply@{1.442695}{\pgfmathresult}%
			\fi
			\pgfkeyslet{/pgfplots/table/create col/next content}\pgfmathresult%
		}%
	},%
	/pgfplots/table/create col/gradient/.style 2 args={%
		/pgfplots/table/columns={#1,#2},
		/pgfplots/table/create col/assign first/.code={%
			\pgfmathfloatparsenumber{\thisrow{#1}}%
			\let\pgfmathaccuma=\pgfmathresult
			\pgfmathfloatparsenumber{\thisrow{#2}}%
			\let\pgfmathaccumb=\pgfmathresult
			\def\pgfmathresult{}% leave first empty.
			\pgfkeyslet{/pgfplots/table/create col/next content}\pgfmathresult%
		},%
		/pgfplots/table/create col/assign/.code={%
			\let\pgfmathcur@x=\pgfmathaccuma
			\let\pgfmathcur@y=\pgfmathaccumb
			\pgfmathfloatparsenumber{\thisrow{#1}}%
			\let\pgfmathnext@x=\pgfmathresult
			\let\pgfmathaccuma=\pgfmathnext@x
			\pgfmathfloatparsenumber{\thisrow{#2}}%
			\let\pgfmathnext@y=\pgfmathresult
			\let\pgfmathaccumb=\pgfmathnext@y
			\pgfmathfloatsubtract@{\pgfmathnext@x}{\pgfmathcur@x}%
			\let\pgfmathdiff@x=\pgfmathresult
			\pgfmathfloatsubtract@{\pgfmathnext@y}{\pgfmathcur@y}%
			\let\pgfmathdiff@y=\pgfmathresult
			\pgfmathfloatdivide@{\pgfmathdiff@y}{\pgfmathdiff@x}%
			\expandafter\pgfmathfloattosci@\expandafter{\pgfmathresult}%
			\pgfkeyslet{/pgfplots/table/create col/next content}\pgfmathresult%
		},%
	},%
	/pgfplots/table/create col/gradient loglog/.style 2 args={%
		/pgfplots/table/columns={#1,#2},
		/pgfplots/table/create col/assign first/.code={%
			\pgfmathlog{\thisrow{#1}}%
			\let\pgfmathaccuma=\pgfmathresult
			\pgfmathlog{\thisrow{#2}}%
			\let\pgfmathaccumb=\pgfmathresult
			\def\pgfmathresult{}% leave first empty.
			\pgfkeyslet{/pgfplots/table/create col/next content}\pgfmathresult%
		},%
		/pgfplots/table/create col/assign/.code={%
			\let\pgfmathcur@x=\pgfmathaccuma
			\let\pgfmathcur@y=\pgfmathaccumb
			\pgfmathlog{\thisrow{#1}}%
			\let\pgfmathnext@x=\pgfmathresult
			\let\pgfmathaccuma=\pgfmathresult
			\pgfmathlog{\thisrow{#2}}%
			\let\pgfmathnext@y=\pgfmathresult
			\let\pgfmathaccumb=\pgfmathresult
			\pgfplots@loop@CONTINUEtrue
			\ifx\pgfmathcur@x\pgfutil@empty		\pgfplots@loop@CONTINUEfalse\fi
			\ifx\pgfmathcur@y\pgfutil@empty		\pgfplots@loop@CONTINUEfalse\fi
			\ifx\pgfmathnext@x\pgfutil@empty	\pgfplots@loop@CONTINUEfalse\fi
			\ifx\pgfmathnext@y\pgfutil@empty	\pgfplots@loop@CONTINUEfalse\fi
			\ifpgfplots@loop@CONTINUE
				\pgfmathsubtract@{\pgfmathnext@x}{\pgfmathcur@x}%
				\let\pgfmathdiff@x=\pgfmathresult
				\pgfmathsubtract@{\pgfmathnext@y}{\pgfmathcur@y}%
				\let\pgfmathdiff@y=\pgfmathresult
				\pgfmathdivide@{\pgfmathdiff@y}{\pgfmathdiff@x}%
			\else
				\pgfmathfloatcreate{3}{0.0}{0}%
				\pgfmathfloattosci@\pgfmathresult
			\fi
			\pgfkeyslet{/pgfplots/table/create col/next content}\pgfmathresult%
		},%
	},%
	/pgfplots/table/create col/gradient semilogx/.style 2 args={%
		/pgfplots/table/columns={#1,#2},
		/pgfplots/table/create col/assign first/.code={%
			\pgfmathlog{\thisrow{#1}}%
			\ifx\pgfmathresult\pgfutil@empty
				\pgfmathfloatcreate{3}{0.0}{0}%
			\else
				\expandafter\pgfmathfloatqparsenumber\expandafter{\pgfmathresult}%
			\fi
			\let\pgfmathaccuma=\pgfmathresult
			\pgfmathfloatparsenumber{\thisrow{#2}}%
			\let\pgfmathaccumb=\pgfmathresult
			\def\pgfmathresult{}% leave first empty.
			\pgfkeyslet{/pgfplots/table/create col/next content}\pgfmathresult%
		},%
		/pgfplots/table/create col/assign/.code={%
			\let\pgfmathcur@x=\pgfmathaccuma
			\let\pgfmathcur@y=\pgfmathaccumb
			\pgfmathlog{\thisrow{#1}}%
			\ifx\pgfmathresult\pgfutil@empty
				\pgfmathfloatcreate{3}{0.0}{0}%
			\else
				\expandafter\pgfmathfloatqparsenumber\expandafter{\pgfmathresult}%
			\fi
			\let\pgfmathnext@x=\pgfmathresult
			\let\pgfmathaccuma=\pgfmathresult
			%
			\pgfmathfloatparsenumber{\thisrow{#2}}%
			\let\pgfmathnext@y=\pgfmathresult
			\let\pgfmathaccumb=\pgfmathresult
			\pgfmathfloatsubtract@{\pgfmathnext@x}{\pgfmathcur@x}%
			\let\pgfmathdiff@x=\pgfmathresult
			\pgfmathfloatsubtract@{\pgfmathnext@y}{\pgfmathcur@y}%
			\let\pgfmathdiff@y=\pgfmathresult
			\pgfmathfloatdivide@{\pgfmathdiff@y}{\pgfmathdiff@x}%
			\expandafter\pgfmathfloattosci@\expandafter{\pgfmathresult}%
			\pgfkeyslet{/pgfplots/table/create col/next content}\pgfmathresult%
		},%
	},%
	/pgfplots/table/create col/gradient semilogy/.style 2 args={%
		/pgfplots/table/columns={#1,#2},
		/pgfplots/table/create col/assign first/.code={%
			\pgfmathfloatparsenumber{\thisrow{#1}}%
			\let\pgfmathaccuma=\pgfmathresult
			\pgfmathlog{\thisrow{#2}}%
			\ifx\pgfmathresult\pgfutil@empty
				\pgfmathfloatcreate{3}{0.0}{0}%
			\else
				\expandafter\pgfmathfloatqparsenumber\expandafter{\pgfmathresult}%
			\fi
			\let\pgfmathaccumb=\pgfmathresult
			\def\pgfmathresult{}% leave first empty.
			\pgfkeyslet{/pgfplots/table/create col/next content}\pgfmathresult%
		},%
		/pgfplots/table/create col/assign/.code={%
			\let\pgfmathcur@x=\pgfmathaccuma
			\let\pgfmathcur@y=\pgfmathaccumb
			\pgfmathlog{\thisrow{#2}}%
			\ifx\pgfmathresult\pgfutil@empty
				\pgfmathfloatcreate{3}{0.0}{0}%
			\else
				\expandafter\pgfmathfloatparsenumber\expandafter{\pgfmathresult}%
			\fi
			\let\pgfmathnext@y=\pgfmathresult
			\let\pgfmathaccumb=\pgfmathresult
			%
			\pgfmathfloatparsenumber{\thisrow{#1}}%
			\let\pgfmathnext@x=\pgfmathresult
			\let\pgfmathaccuma=\pgfmathresult
			\pgfmathfloatsubtract@{\pgfmathnext@x}{\pgfmathcur@x}%
			\let\pgfmathdiff@x=\pgfmathresult
			\pgfmathfloatsubtract@{\pgfmathnext@y}{\pgfmathcur@y}%
			\let\pgfmathdiff@y=\pgfmathresult
			\pgfmathfloatdivide@{\pgfmathdiff@y}{\pgfmathdiff@x}%
			\expandafter\pgfmathfloattosci@\expandafter{\pgfmathresult}%
			\pgfkeyslet{/pgfplots/table/create col/next content}\pgfmathresult%
		},%
	},%
}
\pgfkeysgetvalue{/pgfplots/table/postproc cell content/.@cmd}\pgfplotstable@postproccellcontent@EMPTY

% \pgfplotstableread[OPTIONS] {FILE} to \name
%
% This method reads a table from FILE to macro \name.
%
% FILE is something like
% G	Basis	dof	L2	A	Lmax	cgiter	maxlevel	eps
% 5	5	5	8.31160034e-02	0.00000000e+00	1.80007647e-01	2	2	-1
% 17	17	17	2.54685628e-02	0.00000000e+00	3.75580565e-02	5	3	-1
% ...
%
% A number format line is also understood:
% G	Basis	dof	L2	A	Lmax	cgiter	maxlevel	eps
% $flags int	int	int	sci:8	sci:8	sci:8	int	int	std:8
% 5	5	5	8.31160034e-02	0.00000000e+00	1.80007647e-01	2	2	-1
%
% or a three-column-gnuplot file with 2 comment headers like
% #Curve 0, 20 points
% #x y type
% 0.00000 0.00000 i
% 0.52632 0.50235 i
%
% The table data is stored columnwise in lists and can be accessed
% with the other methods of this package.
%
% \pgfplotstableread[<options>]{<file>}{<\macro>}
% \pgfplotstableread[<options>]{<file>} to listener{<\macro>}
%
% The 'to listener' variant does NOT assemble a table data structure.
% Instead, it processes the input table row-wise and invokes <\macro>
% after each complete row. During the evaluation of <\macro>, the
% following methods can be used to query values:
%   \pgfplotstablereadgetcolindex{<index>}{<\macro>}
%   \pgfplotstablereadgetcolname{<name>}{<\macro>}
% Attention: 'to listener' is scoped by TeX groups, so any assignments
% need to be done globally (or with aftergroup magic).
\def\pgfplotstableread{%
	\pgfutil@ifnextchar[{%
		\pgfplotstableread@impl
	}{%
		\pgfplotstableread@impl[]%
	}%
}

% BACKWARDS COMPATIBILITY
\let\pgfnumtableread=\pgfplotstableread

\def\pgfplotstablegetcolumnlist#1\to#2{%
	\let#2=#1
}

% Returns a column vector in form of \pgfplotslist
% into #3.
%
% #1: the column name (not a macro)
% #2: the table structure
% #3: the output macro name.
\def\pgfplotstablegetcolumnbyname#1\of#2\to#3{%
	\pgfutil@ifundefined{\string#2@#1}{%
		% Oh, there is no column '#1' in table '#2'!
		%
		% Ok, then check for the 'create on use' and the 'alias'
		% features...
		% 1. create on use:
		%
		% WARNING : this code has been REPLICATED in
		% *** \pgfplotstablereadgetptrtocolname ***
		% *** \pgfplotstablegetcolumnbyname ***
		% *** \pgfplotstableresolvecolname ***
		\def\pgfplotstable@loc@TMPa{/pgfplots/table/create on use/#1}%
		\pgfkeysifdefined{\pgfplotstable@loc@TMPa/.@cmd}{%	
			% aah - a 'create on use' style exists. Apply it!
			\expandafter\pgfplotstablecreatecol\expandafter[\pgfplotstable@loc@TMPa]{#1}{#2}%
			% and return the newly generated col:
			\expandafter\let\expandafter#3\csname\string#2@#1\endcsname
		}{%
			% ok, then it is either an alias or it is simply not
			% existant.
			\def\pgfplotstable@loc@TMPa{/pgfplots/table/alias/#1}%
			\pgfkeysifdefined{\pgfplotstable@loc@TMPa}{%
				\pgfkeysgetvalue{\pgfplotstable@loc@TMPa}{\pgfplotstable@loc@TMPb}%
				\let\pgfplotstable@loc@TMPa=\pgfplotstable@loc@TMPb
				\pgfutil@ifundefined{\string#2@\pgfplotstable@loc@TMPa}{%
					\pgfplots@error{Sorry, could not retrieve aliased column '\pgfplotstable@loc@TMPa' from table '\pgfplotstablenameof{#2}'. The original request was for '#1', which does not exist either.}%
					\pgfplotslistnewempty#3
				}{%
					\expandafter\let\expandafter#3\csname\string#2@\pgfplotstable@loc@TMPa\endcsname
				}%
			}{%
				\pgfplots@error{Sorry, could not retrieve column '#1' from table '\pgfplotstablenameof{#2}'. Please check spelling (or introduce name aliases).}%
				\pgfplotslistnewempty#3
			}%
		}%
	}{%
		\expandafter\let\expandafter#3\csname\string#2@#1\endcsname
	}%
}

% Retrieves the column *NAME* '#1' of table #2 and writes it into
% '#3'.
%
% If there is no such column, column aliases will be checked. Finally
% if there are no aliases, the command fails with an error.
%
% The 'create on use' statements can't be used in this context.
% @see \pgfplotstablegetcolumnbyname
%
% #1: a column name (not a macro)
% #2: the table structure
% #3: a macro name which will be filled with the (probably modified)
% column name into #2.
\def\pgfplotstableresolvecolname#1\of#2\to#3{%
	\pgfutil@ifundefined{\string#2@#1}{%
		% Oh, there is no column '#1' in table '#2'!
		%
		% Ok, then check for the 'alias' feature ...
		%
		% WARNING : this code has been REPLICATED in
		% *** \pgfplotstablereadgetptrtocolname ***
		% *** \pgfplotstablegetcolumnbyname ***
		% *** \pgfplotstableresolvecolname ***
		\def\pgfplotstable@loc@TMPa{/pgfplots/table/alias/#1}%
		\pgfkeysifdefined{\pgfplotstable@loc@TMPa}{%
			\pgfkeysgetvalue{\pgfplotstable@loc@TMPa}{\pgfplotstable@loc@TMPb}%
			\let\pgfplotstable@loc@TMPa=\pgfplotstable@loc@TMPb
			\pgfutil@ifundefined{\string#2@\pgfplotstable@loc@TMPa}{%
				\def\pgfplotstable@loc@TMPb{/pgfplots/table/create on use/#1}%
				\pgfkeysifdefined{\pgfplotstable@loc@TMPb/.@cmd}{%
					\pgfplots@error{Sorry, '\pgfplotstable@loc@TMPb' from table '\pgfplotstableread@filename' can't be evaluated in this context. Please prepare the table before using it here.}%
				}{%
					\pgfplots@error{Sorry, could not retrieve aliased column '\pgfplotstable@loc@TMPa' from table '\pgfplotstablenameof{#2}'. The original request was for '#1', which does not exist either.}%
				}%
				\let#3=\pgfutil@empty
			}{%
				\let#3=\pgfplotstable@loc@TMPa
			}%
		}{%
			\pgfplots@error{Sorry, could not retrieve column '#1' from table '\pgfplotstablenameof{#2}'. Please check spelling (or introduce name aliases).}%
			\let#3=\pgfutil@empty
		}%
	}{%
		\def#3{#1}%
	}%
}

% Invokes either \pgfplotstablegetcolumnbyindex or
% \pgfplotstablegetcolumnbyname.
\def\pgfplotstablegetcolumn#1\of#2\to#3{%
	\pgfplotstable@is@colname{#1}%
	\ifpgfplotstableread@foundcolnames
	\else
		\pgfplotstablegetcolumnnamebyindex{#1}\of{#2}\to{#3}
	\fi
	\pgfplotstablegetcolumnbyname{#1}\of#2\to{#3}%
}%

\def\pgfplotstablegetcolumnnamebyindex#1\of#2\to#3{%
	\pgfplotslistselect#1\of#2\to#3\relax
}%
\def\pgfplotstablegetcolumnbyindex#1\of#2\to#3{%
	\pgfplotslistselect#1\of#2\to#3\relax
	\expandafter\pgfplotstablegetcolumnbyname#3\of#2\to{#3}%
}

\def\pgfplotstablecopy#1\to#2{%
	\let#2=#1%
	\pgfplotstablegetname#2\pgfplotstable@loc@TMPa
	\expandafter\let\csname\string#1@@table@name\endcsname=\pgfplotstable@loc@TMPa
	\pgfplotslistforeachungrouped#1\as\pgfplotstable@loc@TMPa{%
		\def\pgfplotstable@loc@TMPb{%
			\expandafter\let\csname\string#2@\pgfplotstable@loc@TMPa\endcsname}%
		\expandafter\pgfplotstable@loc@TMPb\csname\string#1@\pgfplotstable@loc@TMPa\endcsname
	}%
}

% Returns the file name of table '#1' into macro #2.
\def\pgfplotstablegetname#1#2{%
	\expandafter\let\expandafter#2\csname\string#1@@table@name\endcsname
}
	
% expands to the table file name of table '#1'
\def\pgfplotstablenameof#1{%
	\csname\string#1@@table@name\endcsname
}

% Creates a new column named #1 and appends it to table #2.
%
% The column entries will be created using the command keys
% 'create col/assign' 
% 'create col/assign last'
%
% The key 'create col/assign' will be invoked for every row of table #2.
% It is supposed to assign the key 'create col/next content'.
% During evaluation of 'create col/assign', the macro '\thisrow{<col name>}' 
% expands to the current row's value of the column named by <col name>.
% Furthermore, '\nextrow{<col name>}' expands to the \emph{next} row's
% value of the designated column.
%
% Since the "next row" is not available if we are currently processing
% the last row, 'create col/assign last' is used in for the last row's
% value.
%
% You can use
% - \thisrow{<col name>}, 
% - \getthisrow{<col name>}{\macro}
% - \nextrow{<col name>}, 
% - \getnextrow{<col name>}{\macro}
\def\pgfplotstablecreatecol{%
	\pgfutil@ifnextchar[{%
		\pgfplotstablecreatecol@opt
	}{%
		\pgfplotstablecreatecol@opt[]%
	}%
}%


% Typesets a table.
%
% \pgfplotstabletypeset[<options>]<\tablestructure>
%
% If you do not select any columns, the complete table is drawn.
%
% There are several options and styles which are available in
% <options>, see the declaration above.
%
% ATTENTION: the default implementation employs
% \begin{tabular}...\end{tabular} and is therefor only usable with
% LaTeX!
%
% You will need to reconfigure the tables.
%
% Inside of \pgfplotstabletypeset, the macros \pgfplotstablecol and
% \pgfplotstablerow will expand to the current column index and row
% index.
\def\pgfplotstabletypeset{%
	\pgfutil@ifnextchar[{%	
		\pgfplotstabletypeset@opt
	}{%
		\pgfplotstabletypeset@opt[]%
	}%
}

% Like \pgfplotstabletypeset, but the first argument is a file name.
\def\pgfplotstabletypesetfile{%
	\pgfutil@ifnextchar[{%	
		\pgfplotstabletypesetfile@opt
	}{%
		\pgfplotstabletypesetfile@opt[]%
	}%
}
\def\pgfplotstabletypesetfile@opt[#1]#2{%
	\begingroup
	\ifpgfplots@table@options@areset
	\else
		\pgfplots@table@options@aresettrue
		\pgfplotstableset{/pgfplots/table/every table={#2},#1}%
	\fi
	\pgfplotstableread{#2}\pgfplotstabletypesetfile@opt@@
	\pgfplotstabletypeset\pgfplotstabletypesetfile@opt@@
	\endgroup
}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% IMPLEMENTATION
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\ifpgfplotstableread@curline@contains@colnames
\newif\ifpgfplotstableread@foundcolnames
\newif\ifpgfplotstableread@skipline

% Accept one of
% \pgfplotstableread[#1]{<file>}{<\macro>}
% \pgfplotstableread[#1]{<file>} to listener{<\macro>}
% or
% \pgfplotstableread[#1]{<file>} to {<\macro>} (DEPRECATED)
\def\pgfplotstableread@impl[#1]#2{%
	\pgfutil@ifnextchar t{%
		\pgfplotstableread@impl@@{#1}{#2}%
	}{%
		\pgfplotstableread@impl@{#1}{#2}%
	}%
}%

% I don't know why; but I started with 
% >> \pgfplotstableread[]{file} to \macro
% That ' to ' is really ugly. This here is for backwards
% compatibility:
\def\pgfplotstableread@impl@@#1#2to {%
	\pgfutil@ifnextchar l{%
		\pgfplotstableread@impl@@listener{#1}{#2}%
	}{%
		\pgfplotstableread@impl@{#1}{#2}%
	}%
}%
\def\pgfplotstableread@impl@@listener#1#2listener#3{%
	\pgfplots@tableread@to@listenertrue
	\pgfplotstableread@impl@{#1}{#2}{#3}%
	\pgfplots@tableread@to@listenerfalse
}%

\def\pgfplotstableread@impl@#1#2#3{%
	\begingroup
	\ifpgfplots@table@options@areset
	\else
		\pgfplotstableset{/pgfplots/table/every table={#2},#1}%
	\fi
%\pgfplots@message{ATTEMPTING TO READ #2}%
	\openin1=#2.tex
	\ifeof1
		\openin1=#2\relax
	\else
		\pgfplots@warning{%
			You requested to open table '#2', but there is also a '#2.tex'. 
			TeX will automatically append the suffix '.tex', so I will now open '#2.tex'.
			Please make sure you don't accidentally load TeX files - this may produce unrecoverable errors.}%
		\closein1
		\openin1=#2\relax
	\fi
	\def\pgfplotstableread@filename{#2}%
	\let\pgfplotstableread@lineno=\c@pgf@counta
	\let\pgfplotstableread@numcols=\c@pgf@countb
	\let\pgfplotstableread@curcol=\c@pgf@countc
	\let\pgfplotstableread@usablelineno=\c@pgf@countd
	\pgfplotstableread@lineno=0
	\pgfplotstableread@usablelineno=0
	\pgfplotstableread@numcols=0
	\global\pgfplotslistnewempty\pgfplotstable@colnames
	\ifeof1
		\pgfplotstable@error{Could not read table file '#2'.}%
		\global\pgfplotslistnewempty\pgfplotstable@colnames
	\else
		\ifpgfplots@tableread@to@listener
			\let\pgfplotstable@listener=#3%
			\let\pgfplotstableread@impl@nextrow@NEXT=\pgfplotstableread@impl@nextrow@NEXT@listener
			\let\pgfplotstablereadgetcolindex=\pgfplotstablereadgetcolindex@
			\let\pgfplotstablereadgetcolname=\pgfplotstablereadgetcolname@
			\let\pgfplotstablereadgetptrtocolname=\pgfplotstablereadgetptrtocolname@
			\let\pgfplotstablereadgetptrtocolindex=\pgfplotstablereadgetptrtocolindex@
			\let\pgfplotstablereadevalptr=\pgfplotstablereadevalptr@
		\fi
		%
		\pgfplotstableread@loop@over@lines
		\closein1
		%
		\pgfplotstableread@finish
	\fi
	\endgroup
	\ifpgfplots@tableread@to@listener
		% there are no data structures in this case.
	\else
		% Now, we can access the global variables!
		% copy them to #3.
		\let#3=\pgfplotstable@colnames
		\expandafter\def\csname\string#3@@table@name\endcsname{#2}%
		\c@pgfplotstable@counta=0\relax%
		\pgfplotslistforeachungrouped\pgfplotstable@colnames\as\pgfplotstable@loc@TMPa{%
			\def\pgfplotstable@loc@TMPb{%
				\expandafter\let\csname\string#3@\pgfplotstable@loc@TMPa\endcsname}%
			\expandafter\pgfplotstable@loc@TMPb\csname pgfp@numtable@glob@col@\the\c@pgfplotstable@counta\endcsname
	%\message{Column '\pgfplotstable@loc@TMPa' has entries: \expandafter\meaning\csname pgfp@numtable@glob@col@\the\c@pgfplotstable@counta\endcsname}%
			\expandafter\global\expandafter\let\csname pgfp@numtable@glob@col@\the\c@pgfplotstable@counta\endcsname=\pgfutil@empty
			\advance\c@pgfplotstable@counta by1\relax
		}%
	\fi
	\global\let\pgfplotstable@colnames=\pgfutil@empty
}

\def\pgfplotstableread@finish{%
	\ifpgfplots@tableread@to@listener
	\else
		\ifpgfplotstableread@foundcolnames
		\else
			\pgfplotstableread@create@column@names@with@numbers
		\fi
		\pgfplotstableread@curcol=0\relax%
		\pgfutil@loop
		\ifnum\pgfplotstableread@curcol<\pgfplotstableread@numcols
			\expandafter\pgfplotsapplistXflushbuffers\csname pgfp@numtable@glob@col@\the\pgfplotstableread@curcol\endcsname
			\advance\pgfplotstableread@curcol by1
		\pgfutil@repeat
	\fi
}

\def\pgfplotstableread@loop@over@lines{%
	\ifeof1
%\pgfplots@message{EOF}%
	\else
		\read1 to\pgfplotstable@LINE
		\ifeof1
		\else
		\expandafter\pgfplotstableread@checkspecial@line\pgfplotstable@LINE\pgfplotstable@EOI
		\ifpgfplotstableread@skipline
		\else
			%--------------------------------------------------
			% \ifnum\pgfplotstableread@lineno=0
			% 	\let\pgfplotstable@firstline=\pgfplotstable@LINE
			% \fi
			%-------------------------------------------------- 
%\pgfplots@message{READING LINE \the\pgfplotstableread@lineno: '\meaning\pgfplotstable@LINE'.}%
			\pgfplotstableread@curline@contains@colnamesfalse
			\ifnum\pgfplotstableread@numcols=0\relax
				\pgfplotstableread@curcol=0\relax
				\pgfplotstableread@impl@DO\pgfplotstableread@impl@countcols@and@identifynames@NEXT\pgfplotstable@LINE
				%\expandafter\pgfplotstableread@impl@countcols@and@identifynames@ITERATE\pgfplotstable@LINE\pgfplotstable@EOI
				\pgfplotstableread@numcols=\pgfplotstableread@curcol
				\pgfplotstableread@curcol=0\relax
				% Create empty column lists:
				\pgfplotstableread@create@column@lists
				%
				\ifnum\pgfplotstableread@usablelineno=0\relax
				\ifnum\pgfplotstableread@lineno=2\relax
				\ifnum\pgfplotstableread@numcols=3\relax
					% The file started with
					% #...
					% #...
					% X Y i
					% -> thats a gnuplot file!
					\pgfplotstableread@curline@contains@colnamesfalse
				\fi
				\fi
				\fi
				% Now, read the first line.
				% It contains either
				% - column names,
				% - numerical data,
				% - nothing (comments).
				\ifpgfplotstableread@curline@contains@colnames
					\pgfplotstableread@foundcolnamestrue
					\pgfplotstableread@curcol=0\relax
					\pgfplotstableread@impl@DO\pgfplotstableread@impl@collectcolnames@NEXT\pgfplotstable@LINE
					%\expandafter\pgfplotstableread@impl@collectcolnames@ITERATE\pgfplotstable@LINE\pgfplotstable@EOI
				\else
					\pgfplotstableread@foundcolnamesfalse
					\pgfplotstableread@curcol=0\relax
					% Leave column name lists empty...
					\pgfplotstableread@impl@DO\pgfplotstableread@impl@nextrow@NEXT\pgfplotstable@LINE
					%\expandafter\pgfplotstableread@impl@nextrow@ITERATE\pgfplotstable@LINE\pgfplotstable@EOI
				\fi
%\pgfplots@message{After reading first row: found '\the\pgfplotstableread@numcols' columns; column name list='\meaning\pgfplotstable@colnames'}%
			\else
				\pgfplotstableread@curcol=0\relax
				\pgfplotstableread@impl@DO\pgfplotstableread@impl@nextrow@NEXT\pgfplotstable@LINE
				%\expandafter\pgfplotstableread@impl@nextrow@ITERATE\pgfplotstable@LINE\pgfplotstable@EOI
			\fi
			\ifnum\pgfplotstableread@curcol=\pgfplotstableread@numcols
			\else
				\pgfplotstable@error{ERROR: the input table has an unexpected number of columns in row '\the\pgfplotstableread@lineno'. Expected: '\the\pgfplotstableread@numcols'; got '\the\pgfplotstableread@curcol. Maybe the input table is corrupted?}%
			\fi
			\ifpgfplots@tableread@to@listener
				\ifpgfplotstableread@curline@contains@colnames
				\else
					% report row!
					\pgfplotstable@listener
				\fi
			\fi
			\advance\pgfplotstableread@usablelineno by1\relax
		\fi
		\fi
		\advance\pgfplotstableread@lineno by1\relax
		\expandafter\pgfplotstableread@loop@over@lines
	\fi
}

% WARNING: this routine is also use in pgfplots.code.tex ...
\def\pgfplotstableread@checkspecial@line{%
	\pgfutil@ifnextchar##{%
		\pgfplotstableread@skiplinetrue
		\pgfplotstableread@impl@gobble
	}{%
		\pgfutil@ifnextchar${%
			\pgfplotstableread@process@flags@line
		}{%
			\pgfutil@ifnextchar\pgfplotstable@EOI{%
				\pgfplotstableread@skiplinetrue
				\pgfplotstableread@impl@gobble
			}{%
				\pgfutil@ifnextchar\par{%
					\pgfplotstableread@skiplinetrue
					\pgfplotstableread@impl@gobble
				}{%
					\pgfplotstableread@skiplinefalse
					\pgfplotstableread@impl@gobble
				}%
			}%
		}%
	}%
}

\long\def\pgfplotstableread@process@flags@line$flags {%
%\pgfplots@message{Ignoring flags line ...}%
	\pgfplotstableread@skiplinetrue
	\pgfplotstableread@impl@gobble
}

\def\pgfplotstableread@create@column@lists{%
	\pgfutil@loop
	\ifnum\pgfplotstableread@curcol<\pgfplotstableread@numcols
		\def\pgfplots@loc@TMPa{\pgfplotsapplistXnewempty[to global]}%
		\expandafter\pgfplots@loc@TMPa\csname pgfp@numtable@glob@col@\the\pgfplotstableread@curcol\endcsname
		\advance\pgfplotstableread@curcol by1\relax
	\pgfutil@repeat
}

\def\pgfplotstableread@create@column@names@with@numbers{%
	\pgfplotstableread@curcol=0\relax
	\pgfutil@loop
	\ifnum\pgfplotstableread@curcol<\pgfplotstableread@numcols
		\expandafter\pgfplotslistpushbackglobal\the\pgfplotstableread@curcol\to\pgfplotstable@colnames
		\advance\pgfplotstableread@curcol by1\relax
	\pgfutil@repeat
}

\long\def\pgfplotstableread@impl@gobble#1\pgfplotstable@EOI{}%

\def\pgfplotstable@EOI{\pgfplotstable@EOI}%

%%%%%%%%%%%%%%%

% A loop command which processes every single entry in a raw data row #2 
% and invokes the macro #1{<arg>}  for each found column entry.
%
% Columns are separated by the /pgfplots/table/col sep character.
%
% #1: a command which takes precisely one argument. It will be called
% for each found column entry
%
% #2: a macro containing a raw data line with <col sep> separated
% entries.
\def\pgfplotstableread@impl@DO#1#2{%
	\let\pgfplotstableread@impl@ITERATE@NEXT@=#1\relax
	\ifcase\pgfplotstableread@COLSEP@CASE\relax
		% SPACE:
		\expandafter\pgfplotstableread@impl@ITERATE#2\pgfplotstable@EOI
	\or
		% COMMA:
		\let\pgfplotstableread@impl@ITERATE@NEXT=\pgfplotstableread@impl@ITERATE@NEXT@COMMA
		\expandafter\pgfplotstableread@impl@ITERATE#2,\pgfplotstable@EOI
	\or
		% SEMICOLON:
		\let\pgfplotstableread@impl@ITERATE@NEXT=\pgfplotstableread@impl@ITERATE@NEXT@SEMICOLON
		\expandafter\pgfplotstableread@impl@ITERATE#2;\pgfplotstable@EOI
	\or
		% COLON:
		\let\pgfplotstableread@impl@ITERATE@NEXT=\pgfplotstableread@impl@ITERATE@NEXT@COLON
		\expandafter\pgfplotstableread@impl@ITERATE#2:\pgfplotstable@EOI
	\or
		% BRACE:
		\let\pgfplotstableread@impl@ITERATE@NEXT=\pgfplotstableread@impl@ITERATE@NEXT@BRACE
		\expandafter\pgfplotstableread@impl@ITERATE#2\pgfplotstable@EOI
	\fi
}%
\def\pgfplotstableread@impl@ITERATE{%
	\pgfutil@ifnextchar\pgfplotstable@EOI{%
		\pgfplotstableread@impl@gobble
	}{%
		\pgfplotstableread@impl@ITERATE@NEXT
	}%
}%
\def\pgfplotstableread@impl@ITERATE@NEXT#1 {%
	\pgfplotstableread@impl@ITERATE@NEXT@{#1}%
	\pgfplotstableread@impl@ITERATE
}%
\def\pgfplotstableread@impl@ITERATE@NEXT@COMMA#1,{%
	\pgfplotstableread@impl@ITERATE@NEXT@{#1}%
	\pgfplotstableread@impl@ITERATE
}%
\def\pgfplotstableread@impl@ITERATE@NEXT@SEMICOLON#1;{%
	\pgfplotstableread@impl@ITERATE@NEXT@{#1}%
	\pgfplotstableread@impl@ITERATE
}%
\def\pgfplotstableread@impl@ITERATE@NEXT@COLON#1:{%
	\pgfplotstableread@impl@ITERATE@NEXT@{#1}%
	\pgfplotstableread@impl@ITERATE
}%
\def\pgfplotstableread@impl@ITERATE@NEXT@BRACE#1{%
	\pgfplotstableread@impl@ITERATE@NEXT@{#1}%
	\pgfplotstableread@impl@ITERATE
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% these values are only usable for a read-listener, that means:
% when using
%
% \pgfplotstableread{<file>} to listener<\macro>
%
% -> <\macro> can than use the methods
%
% \pgfplotstablereadgetcolindex{<index>}{<\content>}
% performs \let\content=<content of column no <index> >
\def\pgfplotstablereadgetcolindex@#1#2{%
	\pgfutil@ifundefined{pgfplotstblread@colcontent@no#1}{%
		\pgfplots@error{Sorry, the requested column number '#1' in table '\pgfplotstableread@filename' does not exist!? Please verify you used the correct index 0 <= i < N.}%
		\let#2=\pgfutil@empty
	}{%
		\expandafter\let\expandafter#2\csname pgfplotstblread@colcontent@no#1\endcsname
	}%
}%

% \pgfplotstablereadgetcolname{<index>}{<name>}
% performs \let\content=<content of column named <name> >
\def\pgfplotstablereadgetcolname@#1#2{%
	\pgfplotstablereadgetptrtocolname{#1}{\pgfplots@loc@TMPa}%
	\pgfplotstablereadevalptr\pgfplots@loc@TMPa{#2}%
}%

% \pgfplotstablereadgetptrtocolname{<name>}{\ptr}
% Creates some sort of "pointer" to the column named <name>. This
% pointer can than be used every time a new line has been reported to
% the listener. IT works like this:
%
% \let\ptr=\pgfutil@empty
% \def\macro{%
% 	\ifx\ptr\empty
% 		\pgfplotstablereadgetptrtocolname{<my col>}{\ptr}%
% 	\fi
% 	\pgfplotstablereadevalptr{\ptr}{\content}%
% 	-> do something with \content!
% }
% 	
% \pgfplotstableread{<file>} to listener<\macro>
%
% -> will evaluate \macro foreach row.
\def\pgfplotstablereadgetptrtocolname@#1#2{%
	% Implementation note: it is necessary to replicate code becuase
	% in this context, the table structure is NOT available.
	\pgfutil@ifundefined{pgfplotstblread@colindex@for@name#1}{%
		% Oh, there is no column '#1'!
		%
		% Check for the 'alias' feature!
		%
		% WARNING : this code has been REPLICATED in
		% *** \pgfplotstablereadgetptrtocolname ***
		% *** \pgfplotstablegetcolumnbyname ***
		% *** \pgfplotstableresolvecolname ***
		%
		\def\pgfplotstable@loc@TMPa{/pgfplots/table/alias/#1}%
		\pgfkeysifdefined{\pgfplotstable@loc@TMPa}{%
			\pgfkeysgetvalue{\pgfplotstable@loc@TMPa}{\pgfplotstable@loc@TMPb}%
			\let\pgfplotstable@loc@TMPa=\pgfplotstable@loc@TMPb
			\pgfutil@ifundefined{pgfplotstblread@colindex@for@name\pgfplotstable@loc@TMPa}{%
				\pgfplots@error{Sorry, could not retrieve aliased column '\pgfplotstable@loc@TMPa' from table '\pgfplotstableread@filename'. The original request was for '#1', which does not exist either.}%
				\def#2{0}%
			}{%
				\edef#2{\csname pgfplotstblread@colindex@for@name\pgfplotstable@loc@TMPa\endcsname}%
			}%
		}{%
			\def\pgfplotstable@loc@TMPa{/pgfplots/table/create on use/#1}%
			\pgfkeysifdefined{\pgfplotstable@loc@TMPa/.@cmd}{%
				\pgfplots@error{Sorry, '\pgfplotstable@loc@TMPa' from table '\pgfplotstableread@filename' can't be evaluated in this context. Please prepare the table before using it here.}%
			}{%
				\pgfplots@error{Sorry, could not retrieve column '#1' from table '\pgfplotstableread@filename'. Please check spelling (or introduce name aliases).}%
			}%
			\def#2{0}%
		}%
	}{%
		\edef#2{\csname pgfplotstblread@colindex@for@name#1\endcsname}%
	}%
}%

% As \pgfplotstablereadgetptrtocolname, but this here access columns
% by index.
\def\pgfplotstablereadgetptrtocolindex@#1#2{\def#2{#1}}%

% \pgfplotstablereadevalptr{<\ptr>}{<\content}
% writes the current value of <\ptr> to <\content>. The pointer <\ptr>
% must be initialised with \pgfplotstablereadgetptrtocolname
\let\pgfplotstablereadevalptr@=\pgfplotstablereadgetcolindex@
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\long\def\pgfplotstableread@impl@nextrow@NEXT@listener#1{%
	\expandafter\def\csname pgfplotstblread@colcontent@no\the\pgfplotstableread@curcol\endcsname{#1}%
	\advance\pgfplotstableread@curcol by1\relax
}

\long\def\pgfplotstableread@impl@nextrow@NEXT#1{%
%\pgfplots@message{Inserting '#1' at (\the\pgfplotstableread@lineno, \the\pgfplotstableread@curcol).}%
	\pgfplotslist@assembleentry{#1}\into\t@pgfplots@tokc
	\def\pgfplotstableread@TMP{\expandafter\pgfplotsapplistXpushback\expandafter{\the\t@pgfplots@tokc}\to}%
	\expandafter\pgfplotstableread@TMP\csname pgfp@numtable@glob@col@\the\pgfplotstableread@curcol\endcsname
	\advance\pgfplotstableread@curcol by1\relax
}



\long\def\pgfplotstableread@impl@collectcolnames@NEXT#1{%
%\pgfplots@message{Got column name no \the\pgfplotstableread@curcol\ as '#1'}%
	\pgfutil@ifundefined{pgfplotstableread@impl@COLNAME@#1}{%
		\def\pgfplotstable@loc@TMPa{#1}%
	}{% generate unique column names
		\pgfplots@warning{Table '\pgfplotstableread@filename' has non-unique column name '#1'. Only the first occurence can be accessed via column names.}%
		\edef\pgfplotstable@loc@TMPa{#1--index\the\pgfplotstableread@curcol}%
	}%
	\expandafter\def\csname pgfplotstableread@impl@COLNAME@#1\endcsname{foo}% remember this name.
	\expandafter\pgfplotslistpushbackglobal\expandafter{\pgfplotstable@loc@TMPa}\to\pgfplotstable@colnames
	\ifpgfplots@tableread@to@listener
		% create an associative container colindex -> colname
		% for use in a listener.
		\def\pgfplots@loc@TMPb{%
			\expandafter\def\csname pgfplotstblread@colindex@for@name#1\endcsname}%
		\expandafter\pgfplots@loc@TMPb\expandafter{\the\pgfplotstableread@curcol}%
	\fi
	\advance\pgfplotstableread@curcol by1\relax
}




\long\def\pgfplotstableread@impl@countcols@and@identifynames@NEXT#1{%
	\advance\pgfplotstableread@curcol by1\relax
	\ifpgfplotstable@search@header
		\ifpgfplotstableread@curline@contains@colnames
		\else
			\pgfplotstableread@isnumber@ITERATE#1\pgfplotstable@EOI
%\ifpgfplotstableread@curline@contains@colnames\pgfplots@message{'#1' is a column name!}\else\pgfplots@message{'#1' is NO column name!}\fi
		\fi
	\fi
}
\def\pgfplotstableread@isnumber@plus{+}
\def\pgfplotstableread@isnumber@minus{-}
\def\pgfplotstableread@isnumber@zero{0}
\def\pgfplotstableread@isnumber@one{1}
\def\pgfplotstableread@isnumber@two{2}
\def\pgfplotstableread@isnumber@three{3}
\def\pgfplotstableread@isnumber@four{4}
\def\pgfplotstableread@isnumber@five{5}
\def\pgfplotstableread@isnumber@six{6}
\def\pgfplotstableread@isnumber@seven{7}
\def\pgfplotstableread@isnumber@eight{8}
\def\pgfplotstableread@isnumber@nine{9}
\def\pgfplotstableread@isnumber@e{e}
\def\pgfplotstableread@isnumber@E{E}
\def\pgfplotstableread@isnumber@period{.}

\def\pgfplotstableread@isnumber@ITERATE#1{%
	\def\pgfplotstableread@CURTOK{#1}%
	\ifx\pgfplotstableread@CURTOK\pgfplotstable@EOI
		\def\pgfplotstableread@NEXT{}%
	\else
		\def\pgfplotstableread@NEXT{\pgfplotstableread@isnumber@ITERATE}%
		\ifx\pgfplotstableread@CURTOK\pgfplotstableread@isnumber@plus
		\else
		\ifx\pgfplotstableread@CURTOK\pgfplotstableread@isnumber@minus
		\else
		\ifx\pgfplotstableread@CURTOK\pgfplotstableread@isnumber@zero
		\else
		\ifx\pgfplotstableread@CURTOK\pgfplotstableread@isnumber@one
		\else
		\ifx\pgfplotstableread@CURTOK\pgfplotstableread@isnumber@two
		\else
		\ifx\pgfplotstableread@CURTOK\pgfplotstableread@isnumber@three
		\else
		\ifx\pgfplotstableread@CURTOK\pgfplotstableread@isnumber@four
		\else
		\ifx\pgfplotstableread@CURTOK\pgfplotstableread@isnumber@five
		\else
		\ifx\pgfplotstableread@CURTOK\pgfplotstableread@isnumber@six
		\else
		\ifx\pgfplotstableread@CURTOK\pgfplotstableread@isnumber@seven
		\else
		\ifx\pgfplotstableread@CURTOK\pgfplotstableread@isnumber@eight
		\else
		\ifx\pgfplotstableread@CURTOK\pgfplotstableread@isnumber@nine
		\else
		\ifx\pgfplotstableread@CURTOK\pgfplotstableread@isnumber@e
		\else
		\ifx\pgfplotstableread@CURTOK\pgfplotstableread@isnumber@E
		\else
		\ifx\pgfplotstableread@CURTOK\pgfplotstableread@isnumber@period
		\else
%\message{NO ITS NOT!  Token: '\meaning\pgfplotstableread@CURTOK'}%
			% it's no number, so it is a column name.
			\pgfplotstableread@curline@contains@colnamestrue
			\def\pgfplotstableread@NEXT{\pgfplotstableread@impl@gobble}%
		\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
	\fi
	\pgfplotstableread@NEXT
}

\def\pgfplotstable@error#1{\pgfplots@error{#1}}%


\def\pgfplotstableset{%
	\pgfqkeys{/pgfplots/table}%
}%

% Accepts a macro #1 which contains an argument denoting a column
% name.
%
% It checks whether #1 starts with '#', indicating that it is actually
% a column INDEX. If that is the case,
% \ifpgfplotstableread@foundcolnames is set to false and the index is
% returned into #1.
%
% Otherwise, \ifpgfplotstableread@foundcolnames is set to true.
\def\pgfplotstable@is@colname#1{%
	\expandafter\pgfplotstabletypeset@is@colname@#1\pgfplotstable@EOI
	\ifpgfplotstableread@foundcolnames
	\else
		\let#1=\pgfplotstable@loc@TMPa
	\fi
}%
\def\pgfplotstabletypeset@is@colname@{%
	\pgfutil@ifnextchar[{%
		\pgfplotstabletypeset@is@colname@index
	}{%
		\pgfplotstableread@foundcolnamestrue
		\pgfplotstabletypeset@is@colname@name
	}%
}
\def\pgfplotstabletypeset@is@colname@index@@{index}%
\def\pgfplotstabletypeset@is@colname@index[#1]#2\pgfplotstable@EOI{%
	\def\pgfplotstable@loc@TMPa{#1}%
	\ifx\pgfplotstable@loc@TMPa\pgfplotstabletypeset@is@colname@index@@
		\pgfplotstableread@foundcolnamesfalse
		\def\pgfplotstable@loc@TMPa{#2}%
	\else
		\pgfplotstableread@foundcolnamestrue
	\fi
}%
\def\pgfplotstabletypeset@is@colname@name#1\pgfplotstable@EOI{}%

\def\pgfplotstabletypeset@getfinalentry#1#2{%
	\begingroup
	\def\pgfplotstablepartno{0}%
	\pgfkeyssetvalue{/pgfplots/table/@cell content}{#1}%
	\pgfkeysvalueof{/pgfplots/table/preproc cell content/.@cmd}#1\pgfeov
	\pgfkeysgetvalue{/pgfplots/table/@cell content}\pgfmathresult%
	%
	\pgfkeysgetvalue{/pgfplots/table/assign cell content/.@cmd}\pgfplotstable@assigncell
	\expandafter\pgfplotstable@assigncell\pgfmathresult\pgfeov
	%
	\pgfkeysgetvalue{/pgfplots/table/postproc cell content/.@cmd}\pgfplotstable@postproccellcontent
	\ifx\pgfplotstable@postproccellcontent\pgfplotstable@postproccellcontent@EMPTY
	\else
		% apply postprocessing to final cell content.
		% This is complicated if there is an '&' in '@cell content',
		% so handle that specially!
		%
		% FIXME also support more than one '&' ?
		\def\pgfplotstabletypeset@rawinput{#1}%
		\pgfkeysgetvalue{/pgfplots/table/@cell content}\pgfmathresult%
		\expandafter\pgfutil@in@\expandafter&\expandafter{\pgfmathresult}%
		\ifpgfutil@in@
			\expandafter\pgfplotstabletypeset@postproc@separately\pgfmathresult\pgfplotstable@EOI
		\else
			\pgfplotstable@postproccellcontent#1\pgfeov
		\fi
	\fi
	\pgfkeysgetvalue{/pgfplots/table/@cell content}\pgfmathresult%
	\pgfmath@smuggleone\pgfmathresult
	\endgroup
	\let#2=\pgfmathresult
}%

% This routine invokes 'postproc cell content' for columns which
% contain the column separate '&'.
%
% #1&#2 is the formatted number, the result of 'dec sep align
% #3 is the (unformatted) input number.
\def\pgfplotstabletypeset@postproc@separately#1&#2\pgfplotstable@EOI{%
	\def\pgfmathresult{#1}%
	\pgfkeyslet{/pgfplots/table/@cell content}\pgfmathresult
	\expandafter\pgfplotstable@postproccellcontent\pgfplotstabletypeset@rawinput\pgfeov
	\pgfkeysgetvalue{/pgfplots/table/@cell content}\pgfplotstable@entry@a
	%
	\def\pgfplotstablepartno{1}%
	\def\pgfmathresult{#2}%
	\pgfkeyslet{/pgfplots/table/@cell content}\pgfmathresult
	\expandafter\pgfplotstable@postproccellcontent\pgfplotstabletypeset@rawinput\pgfeov
	\pgfkeysgetvalue{/pgfplots/table/@cell content}\pgfmathresult
	\t@pgfplots@toka=\expandafter{\pgfplotstable@entry@a}%
	\t@pgfplots@tokb=\expandafter{\pgfmathresult}%
	\edef\pgfmathresult{\the\t@pgfplots@toka&\the\t@pgfplots@tokb}%
	\pgfkeyslet{/pgfplots/table/@cell content}\pgfmathresult
}

% processes the option 'assign column name'
\def\pgfplotstabletypeset@assign@final@colname#1#2{%
	\pgfkeysifdefined{/pgfplots/table/assign column name/.@cmd}{%
		\pgfkeysvalueof{/pgfplots/table/assign column name/.@cmd}#1\pgfeov
		\pgfkeysgetvalue{/pgfplots/table/column name}{#2}%
	}{}%
}
\def\pgfplotstabletypeset@nocolname{\pgfkeysnovalue}

% checks if #1 contains invalid chars for pgfkeys and sets
% \ifpgfutil@in@ to true if that is the case.
\def\pgfplotstable@checkspecialchars@pgfkeys#1\pgfplotstable@EOI{%
	\pgfutil@in@/{#1}%
	\ifpgfutil@in@
	\else
		\pgfutil@in@={#1}%
		\ifpgfutil@in@
		\else
			\pgfutil@in@,{#1}%
		\fi
	\fi

}%

\def\pgfplotstable@insertemptycells@forbalance{%
	\pgfutil@loop
	\ifnum\c@pgfplotstable@counta<\pgfplotstable@firstnumrows\relax
		% let's hope @getfinalentry handles empty strings!
		\pgfplotstabletypeset@getfinalentry{}{\pgfplotstable@entry}%
		\expandafter\pgfplotslistpushback\pgfplotstable@entry\to\pgfplotstable@col@processed
		\pgfplotslistpushback\to\pgfplotstable@col@processed
		\advance\c@pgfplotstable@counta by1\relax
	\pgfutil@repeat
}

% TODO
% - replace grouped list foreach by popfront-loop and use arrays
%   directly -> group only the pgfkeys eval
\def\pgfplotstabletypeset@opt[#1]#2{%
	\begingroup
	%--------------------------------------------------
	% \pgfutil@ifundefined{#2}{%
	% 	\pgfplots@error{There is no such table '\string#2' loaded into memory. Maybe you meant to use '\string\pgfplotstabletypesetfile{\string#2}' instead of '\string\pgfplotstabletypeset{\string#2}'?}%
	% 	\pgfplotslistnewempty#2
	% }{}%
	%-------------------------------------------------- 
	\def\pgfplotstablecol{\the\c@pgfplotstable@colindex}%
	\def\pgfplotstablerow{\the\c@pgfplotstable@rowindex}%
	\def\pgfplotstablecols{\the\c@pgfplotstable@numcols}%
	\def\pgfplotstablerows{\the\c@pgfplotstable@numrows}%
	\ifpgfplots@table@options@areset
	\else
		\pgfplotstablegetname{#2}\pgfplotstable@loc@TMPa
		\t@pgfplots@toka=\expandafter{\pgfplotstable@loc@TMPa}%
		\edef\pgfplotstable@loc@TMPa{/pgfplots/table/every table={\the\t@pgfplots@toka}}%
		\expandafter\pgfplotstableset\expandafter{\pgfplotstable@loc@TMPa,#1}%
	\fi
	\pgfkeysgetvalue{/pgfplots/table/columns}{\pgfplotstable@colnames}%
	\ifx\pgfplotstable@colnames\pgfutil@empty
		\pgfplotstablegetcolumnlist#2\to\pgfplotstable@colnames
	\else
		\expandafter\pgfplotslistnew\expandafter\pgfplotstable@colnames\expandafter{\pgfplotstable@colnames}%
	\fi
	\global\pgfplotslistnewempty\pgfplotstabletypeset@final@colnames
	\global\pgfplotslistnewempty\pgfplotstabletypeset@final@coltypes
	\global\pgfplotslistnewempty\pgfplotstabletypeset@final@cols
	\let\c@pgfplotstable@numcols=\c@pgf@counta
	\let\c@pgfplotstable@numrows=\c@pgf@countd
	\let\c@pgfplotstable@rowindex=\c@pgf@countc
	\let\c@pgfplotstable@colindex=\c@pgf@countb
	\pgfplotslistsize\pgfplotstable@colnames\to\c@pgfplotstable@numcols
	\def\pgfplotstable@firstnumrows{-1}%
	\c@pgfplotstable@numrows=-1\relax
	\c@pgfplotstable@colindex=0\relax
	\pgfplotslistforeach\pgfplotstable@colnames\as\pgfplotstable@colname{%
		\c@pgfplotstable@rowindex=0\relax
		\pgfplotstable@is@colname\pgfplotstable@colname
		\ifpgfplotstableread@foundcolnames
		\else
			\pgfplotstablegetcolumnnamebyindex\pgfplotstable@colname\of#2\to\pgfplotstable@colname
		\fi
		\pgfplotstablegetcolumnbyname\pgfplotstable@colname\of#2\to\pgfplotstable@col
		%
		% Init number of *input* rows here. This may not be the same
		% as the number of *output* rows (see the row predicate
		% below).
		%
		% Accessable with \pgfplotstablerows in style keys.
		\ifnum\c@pgfplotstable@numrows=-1\relax
			\pgfplotslistsize\pgfplotstable@col\to\c@pgfplotstable@numrows
			\global\c@pgfplotstable@numrows=\c@pgfplotstable@numrows
		\fi
		%
		% Set keys for columns!
		\ifodd\c@pgfplotstable@colindex
			\t@pgfplots@toka={every odd column}%
		\else
			\t@pgfplots@toka={every even column}%
		\fi
		\ifnum\c@pgfplotstable@colindex=0\relax
			\t@pgfplots@toka=\expandafter{\the\t@pgfplots@toka,every first column}%
		\fi
		% save this now before we increment '\c@pgfplotstable@colindex':
		\edef\pgfplotstable@displaycolkey{display columns/\the\c@pgfplotstable@colindex/.try}%
		%
		\global\advance\c@pgfplotstable@colindex by1\relax
		\ifnum\c@pgfplotstable@colindex=\c@pgfplotstable@numcols
			\t@pgfplots@toka=\expandafter{\the\t@pgfplots@toka,every last column}%
		\fi
		\t@pgfplots@tokb=\expandafter{\pgfplotstable@colname}%
		\expandafter\pgfplotstable@checkspecialchars@pgfkeys\the\t@pgfplots@tokb\pgfplotstable@EOI
		\ifpgfutil@in@
			\edef\pgfplotstable@loc@TMPa{\the\t@pgfplots@toka,columns/{\the\t@pgfplots@tokb}/.try}%
		\else
			\edef\pgfplotstable@loc@TMPa{\the\t@pgfplots@toka,columns/\the\t@pgfplots@tokb/.try}%
		\fi
		\t@pgfplots@toka=\expandafter{\pgfplotstable@loc@TMPa}%
		\t@pgfplots@tokb=\expandafter{\pgfplotstable@displaycolkey}%
		\edef\pgfplotstable@loc@TMPa{\the\t@pgfplots@toka,\the\t@pgfplots@tokb}%
		\expandafter\pgfplotstableset\expandafter{\pgfplotstable@loc@TMPa}%
		%
		\pgfkeysgetvalue{/pgfplots/table/column name}{\pgfplotstable@colname@out}%
		\ifx\pgfplotstable@colname@out\pgfplotstabletypeset@nocolname
			\let\pgfplotstable@colname@out=\pgfplotstable@colname
		\fi
		\expandafter\pgfplotstabletypeset@assign@final@colname\expandafter{\pgfplotstable@colname@out}\pgfplotstable@colname@out
		{\globaldefs=1
		\expandafter\pgfplotslistpushback\pgfplotstable@colname@out\to\pgfplotstabletypeset@final@colnames
		}%
		\pgfkeysgetvalue{/pgfplots/table/column type}{\pgfplotstable@coltype}%
		{\globaldefs=1
		\expandafter\pgfplotslistpushback\pgfplotstable@coltype\to\pgfplotstabletypeset@final@coltypes
		}%
		%
		\pgfplotslistnewempty\pgfplotstable@col@processed
		\c@pgfplotstable@counta=0 
		\pgfplotslistforeachungrouped\pgfplotstable@col\as\pgfplotstable@entry{%
			\pgfplotstableuserowtrue
			\edef\pgfplotstable@loc@TMPa{\noexpand\pgfkeysvalueof{/pgfplots/table/row predicate/.@cmd}\the\c@pgfplotstable@rowindex}%
			\pgfplotstable@loc@TMPa\pgfeov
			\ifpgfplotstableuserow
				\ifnum\pgfplotstable@firstnumrows=-1\relax
				\else
					\ifnum\c@pgfplotstable@counta=\pgfplotstable@firstnumrows
						\t@pgfplots@toka=\expandafter{\pgfplotstable@entry}%
						\t@pgfplots@tokb=\expandafter{\pgfplotstable@colname@out}%
						\pgfplots@warning{Unbalanced cell with content '\the\t@pgfplots@toka' of column '\the\t@pgfplots@tokb' has been skipped: row count \the\c@pgfplotstable@counta+1 > \pgfplotstable@firstnumrows (which is the number of rows in the first column)}%
						\pgfplotstableuserowfalse
					\fi
				\fi
				\ifpgfplotstableuserow
					\expandafter\pgfplotstabletypeset@getfinalentry\expandafter{\pgfplotstable@entry}{\pgfplotstable@entry}%
					\expandafter\pgfplotslistpushback\pgfplotstable@entry\to\pgfplotstable@col@processed
					\advance\c@pgfplotstable@counta by1\relax
				\fi
			\fi
			\advance\c@pgfplotstable@rowindex by1\relax
		}%
		\ifnum\pgfplotstable@firstnumrows=-1\relax
			\xdef\pgfplotstable@firstnumrows{\the\c@pgfplotstable@counta}%
		\else
			% balance columns:
			\pgfplotstable@insertemptycells@forbalance
		\fi
		{\globaldefs=1
		\expandafter\pgfplotslistpushback\expandafter{\pgfplotstable@col@processed}\to\pgfplotstabletypeset@final@cols
		}%
	}%
	%
	% Ok, I have now everything which will come into the final table.
	%
	% But I have it column-oriented; I need to transpose the storage.
	%
	% The following code assembles a
	% \begin{tabular}{}
	% ...
	% \end{tabular}
	% statement piece after piece.
	%
%\message{I have now \meaning\pgfplotstabletypeset@final@colnames, and \meaning\pgfplotstabletypeset@final@cols.}%
	% Step 1: column names.
	\c@pgfplotstable@colindex=0\relax
	% STEP 1.1: collect column types:
	\def\pgfplotstable@resulttypes{}%
	\pgfplotslistforeachungrouped\pgfplotstabletypeset@final@coltypes\as\pgfplotstable@coltype{%
		\t@pgfplots@toka=\expandafter{\pgfplotstable@resulttypes}%
		\t@pgfplots@tokb=\expandafter{\pgfplotstable@coltype}%
		\edef\pgfplotstable@resulttypes{\the\t@pgfplots@toka\the\t@pgfplots@tokb}%
	}%
	\pgfkeysgetvalue{/pgfplots/table/begin table}{\pgfplotstable@entry}%
	\t@pgfplots@toka=\expandafter{\pgfplotstable@entry}%
	\ifx\pgfplotstable@resulttypes\pgfutil@empty
		\edef\pgfplotstable@result{\the\t@pgfplots@toka}%
	\else
		\t@pgfplots@tokb=\expandafter{\pgfplotstable@resulttypes}%
		\edef\pgfplotstable@result{\the\t@pgfplots@toka{\the\t@pgfplots@tokb}}%
	\fi
	%
	\pgfkeysgetvalue{/pgfplots/table/font}{\pgfplotstable@font}%
	\ifx\pgfplotstable@font\pgfutil@empty
	\else
		\t@pgfplots@toka=\expandafter{\pgfplotstable@font}%
		\t@pgfplots@tokb=\expandafter{\pgfplotstable@result}%
		\edef\pgfplotstable@result{\noexpand\begingroup\the\t@pgfplots@toka\the\t@pgfplots@tokb}%
	\fi
	%

	% Step 1.2: Collect FIRST ROW (column names)
	\begingroup
	\pgfplotstableset{every head row}%
	\pgfkeysgetvalue{/pgfplots/table/before row}{\pgfplotstable@before}%
	\pgfkeysgetvalue{/pgfplots/table/after row}{\pgfplotstable@after}%
	\t@pgfplots@toka=\expandafter{\pgfplotstable@before}%
	\t@pgfplots@tokb=\expandafter{\pgfplotstable@after}%
	\xdef\pgfplots@glob@TMPc{%
		\noexpand\def\noexpand\pgfplotstable@before{\the\t@pgfplots@toka}%
		\noexpand\def\noexpand\pgfplotstable@after{\the\t@pgfplots@tokb}%
	}%
	\endgroup
	\pgfplots@glob@TMPc
	% insert 'before row' here:
	\t@pgfplots@toka=\expandafter{\pgfplotstable@before}%
	\t@pgfplots@tokb=\expandafter{\pgfplotstable@result}%
	\edef\pgfplotstable@result{\the\t@pgfplots@tokb\the\t@pgfplots@toka}%
	%
	\pgfplotslistforeachungrouped\pgfplotstabletypeset@final@colnames\as\pgfplotstable@colname@out{%
		\advance\c@pgfplotstable@colindex by1\relax
		\t@pgfplots@toka=\expandafter{\pgfplotstable@result}%
		\ifnum\c@pgfplotstable@colindex=\c@pgfplotstable@numcols\relax
			\t@pgfplots@tokb=\expandafter{\pgfplotstable@colname@out \\}%
		\else
			\t@pgfplots@tokb=\expandafter{\pgfplotstable@colname@out &}%
		\fi
		\edef\pgfplotstable@result{\the\t@pgfplots@toka\the\t@pgfplots@tokb}%
	}%
	% insert 'after row' here:
	\t@pgfplots@toka=\expandafter{\pgfplotstable@result}%
	\t@pgfplots@tokb=\expandafter{\pgfplotstable@after}%
	\edef\pgfplotstable@result{\the\t@pgfplots@toka\the\t@pgfplots@tokb}%
	%
%\message{I have now \meaning\pgfplotstable@result.}%
	% Step 2: column contents.
	% I will first convert \pgfplotstabletypeset@final@cols into an array.
	\c@pgfplotstable@colindex=0\relax
	\pgfplotsarraynewempty\pgfplotstabletypeset@final@cols@array
	\pgfplotslistforeachungrouped\pgfplotstabletypeset@final@cols\as\pgfplotstable@col@processed{%
		\expandafter\pgfplotsarraypushback\expandafter{\pgfplotstable@col@processed}\to\pgfplotstabletypeset@final@cols@array
	}%
	% init numrows:
	\pgfplotsarrayselect\c@pgfplotstable@colindex\of\pgfplotstabletypeset@final@cols@array\to\pgfplotstable@col@processed
	\pgfplotslistsize\pgfplotstable@col@processed\to\c@pgfplotstable@numrows
	%
	% Now, we loop over every column as long as there are still rows
	% left. We assemble rows while we go.
	%
	\c@pgfplotstable@rowindex=0\relax
	\ifnum\c@pgfplotstable@colindex<\c@pgfplotstable@numcols
		\pgfplots@loop@CONTINUEtrue
	\else
		\pgfplots@loop@CONTINUEfalse
	\fi
	\pgfutil@loop
	\ifpgfplots@loop@CONTINUE
		\pgfplotsarrayselect\c@pgfplotstable@colindex\of\pgfplotstabletypeset@final@cols@array\to\pgfplotstable@col@processed
		\pgfplotslistcheckempty\pgfplotstable@col@processed
		\ifpgfplotslistempty
			% assume that each column has the same number of entries
			% (normalised tables):
			\pgfplots@loop@CONTINUEfalse
		\else
			\ifnum\c@pgfplotstable@colindex=0\relax
				% Install styles for the next row.
				\begingroup
				\ifodd\c@pgfplotstable@rowindex
					\t@pgfplots@toka={every odd row}%
				\else
					\t@pgfplots@toka={every even row}%
				\fi
				\ifnum\c@pgfplotstable@rowindex=0\relax
					\t@pgfplots@toka=\expandafter{\the\t@pgfplots@toka,every first row}%
				\fi
				% misuse as temporary variable:
				\c@pgfplotstable@colindex=\c@pgfplotstable@rowindex
				\advance\c@pgfplotstable@colindex by1\relax
				\ifnum\c@pgfplotstable@colindex=\c@pgfplotstable@numrows
					\edef\pgfplotstable@loc@TMPa{\the\t@pgfplots@toka,every row no \the\c@pgfplotstable@rowindex/.try,every last row}%
				\else
					\edef\pgfplotstable@loc@TMPa{\the\t@pgfplots@toka,every row no \the\c@pgfplotstable@rowindex/.try}%
				\fi
				\expandafter\pgfplotstableset\expandafter{\pgfplotstable@loc@TMPa}%
				\pgfkeysgetvalue{/pgfplots/table/before row}{\pgfplotstable@before}%
				\pgfkeysgetvalue{/pgfplots/table/after row}{\pgfplotstable@after}%
				\t@pgfplots@toka=\expandafter{\pgfplotstable@before}%
				\t@pgfplots@tokb=\expandafter{\pgfplotstable@after}%
				\xdef\pgfplots@glob@TMPc{%
					\noexpand\def\noexpand\pgfplotstable@before{\the\t@pgfplots@toka}%
					\noexpand\def\noexpand\pgfplotstable@after{\the\t@pgfplots@tokb}%
				}%
				\endgroup
				\pgfplots@glob@TMPc
				% insert 'before row' here:
				\t@pgfplots@toka=\expandafter{\pgfplotstable@before}%
				\t@pgfplots@tokb=\expandafter{\pgfplotstable@result}%
				\edef\pgfplotstable@result{\the\t@pgfplots@tokb\the\t@pgfplots@toka}%
			\fi
			%
			%
			\pgfplotslistpopfront\pgfplotstable@col@processed\to\pgfplotstable@entry
			\pgfplotsarrayletentry\c@pgfplotstable@colindex\of\pgfplotstabletypeset@final@cols@array=\pgfplotstable@col@processed
			\advance\c@pgfplotstable@colindex by1\relax
			\t@pgfplots@toka=\expandafter{\pgfplotstable@result}%
			\ifnum\c@pgfplotstable@colindex=\c@pgfplotstable@numcols\relax
				\t@pgfplots@tokb=\expandafter{\pgfplotstable@entry \\}%
			\else
				\t@pgfplots@tokb=\expandafter{\pgfplotstable@entry &}%
			\fi
			\edef\pgfplotstable@result{\the\t@pgfplots@toka\the\t@pgfplots@tokb}%
			\ifnum\c@pgfplotstable@colindex=\c@pgfplotstable@numcols\relax
				\c@pgfplotstable@colindex=0\relax
				% insert 'after row' here:
				\t@pgfplots@toka=\expandafter{\pgfplotstable@result}%
				\t@pgfplots@tokb=\expandafter{\pgfplotstable@after}%
				\edef\pgfplotstable@result{\the\t@pgfplots@toka\the\t@pgfplots@tokb}%
				\advance\c@pgfplotstable@rowindex by1\relax
			\fi
%\message{I have now \meaning\pgfplotstable@result.}%
		\fi
	\pgfutil@repeat
	\t@pgfplots@toka=\expandafter{\pgfplotstable@result}%
	\pgfkeysgetvalue{/pgfplots/table/end table}{\pgfplotstable@entry}%
	\t@pgfplots@tokb=\expandafter{\pgfplotstable@entry}%
	\edef\pgfplotstable@result{\the\t@pgfplots@toka\the\t@pgfplots@tokb}%
	\ifx\pgfplotstable@font\pgfutil@empty
	\else
		\t@pgfplots@toka=\expandafter{\pgfplotstable@result\endgroup}%
		\edef\pgfplotstable@result{\the\t@pgfplots@toka}%
	\fi
	\ifpgfplotstabletypesetdebug
		\t@pgfplots@toka=\expandafter{\pgfplotstable@result}%
		\immediate\write16{------- PGFPLOTSTABLE DEBUG MODE: --------}%
		\immediate\write16{{\the\t@pgfplots@toka}}%
	\fi
	\pgfkeysgetvalue{/pgfplots/table/outfile}{\pgfplotstable@entry}%
	\ifx\pgfplotstable@entry\pgfutil@empty
	\else
		\begingroup
		\immediate\openout\pgfplotstable@outfile=\pgfplotstable@entry\relax
		\t@pgfplots@toka=\expandafter{\pgfplotstable@result}%
		\immediate\write\pgfplotstable@outfile{\the\t@pgfplots@toka}%
		\immediate\closeout\pgfplotstable@outfile
		\endgroup
	\fi
	\pgfplotstable@result
	\endgroup
}%

\newif\ifpgfplotstable@isfirstrow
\newif\ifpgfplotstable@islastrow
\newif\ifpgfplotstablecreatecol@isreallynew

\def\pgfplotstablecreatecol@opt[#1]#2#3{%
	\begingroup
	\pgfplotstableset{columns=,#1}%
	\pgfkeysgetvalue{/pgfplots/table/columns}{\pgfplotstable@colnames}%
	\ifx\pgfplotstable@colnames\pgfutil@empty
		\pgfplotstablegetcolumnlist#3\to\pgfplotstable@colnames
	\else
		\expandafter\pgfplotslistnew\expandafter\pgfplotstable@colnames\expandafter{\pgfplotstable@colnames}%
	\fi
	\pgfplotslistnewempty\pgfplotstable@colnames@real
	\t@pgfplots@toka=\expandafter{#2}% this should handle macro names in '#2'.
	\edef\pgfplotstable@newcolname{\the\t@pgfplots@toka}%
	\global\pgfplotstablecreatecol@isreallynewtrue
	\pgfplotslistforeachungrouped\pgfplotstable@colnames\as\pgfplotstable@colname{%
		\pgfplotstable@is@colname\pgfplotstable@colname
		\ifpgfplotstableread@foundcolnames
			\expandafter\pgfplotslistpushback\expandafter{\pgfplotstable@colname}\to\pgfplotstable@colnames@real
		\else
			\pgfplotstablegetcolumnnamebyindex\pgfplotstable@colname\of#2\to\pgfplotstable@colname
			\expandafter\pgfplotslistpushback\expandafter{\pgfplotstable@colname}\to\pgfplotstable@colnames@real
		\fi
		\ifx\pgfplotstable@colname\pgfplotstable@newcolname
			\global\pgfplotstablecreatecol@isreallynewfalse
		\fi
	}%
	\pgfplotstable@isfirstrowtrue
	\pgfplotstable@islastrowfalse
	\pgfplotslistnewempty\pgfplotstable@newcol
	%
	\let\c@pgfplotstable@numrows=\c@pgf@countd
	\let\c@pgfplotstable@rowindex=\c@pgf@countc
	\c@pgfplotstable@numrows=-1\relax
	\c@pgfplotstable@rowindex=0\relax
	\def\pgfplotstablerow{\the\c@pgfplotstable@rowindex}%
	\def\pgfplotstablerows{\the\c@pgfplotstable@numrows}%
	%
	\def\prevrow##1{\csname pgfplotstablecreate@prev@##1\endcsname}%
	\def\thisrow##1{\csname pgfplotstablecreate@cur@##1\endcsname}%
	\def\nextrow##1{\csname pgfplotstablecreate@next@##1\endcsname}%
	\def\getprevrow##1##2{\expandafter\let\expandafter##2\csname pgfplotstablecreate@prev@##1\endcsname}%
	\def\getthisrow##1##2{\expandafter\let\expandafter##2\csname pgfplotstablecreate@cur@##1\endcsname}%
	\def\getnextrow##1##2{\expandafter\let\expandafter##2\csname pgfplotstablecreate@next@##1\endcsname}%
	%
	\pgfplots@loop@CONTINUEtrue
	% allow this here to accumulate something.
	\let\pgfmathaccuma=\pgfutil@empty
	\let\pgfmathaccumb=\pgfutil@empty
	\pgfutil@loop% loop over each row until there are no more rows.
	\ifpgfplots@loop@CONTINUE
		\ifnum\c@pgfplotstable@numrows=-1\relax
			\pgfplotslistfront\pgfplotstable@colnames\to\pgfplotstable@colname
			\expandafter\pgfplotslistsize\csname\string#3@\pgfplotstable@colname\endcsname\to\c@pgfplotstable@numrows
		\fi
		\pgfplotslistforeachungrouped\pgfplotstable@colnames\as\pgfplotstable@colname{%
			\expandafter\pgfplotstableresolvecolname\expandafter{\pgfplotstable@colname}\of#3\to\pgfplotstable@real@colname
			\ifpgfplotstable@isfirstrow
				\expandafter\pgfplotslistcheckempty\csname\string#3@\pgfplotstable@real@colname\endcsname
				\ifpgfplotslistempty
					% the table is completely empty. break.
					\pgfplots@loop@CONTINUEfalse
				\else
					\expandafter\let\csname pgfplotstablecreate@prev@\pgfplotstable@colname\endcsname=\pgfutil@empty
					\expandafter\pgfplotslistpopfront\csname\string#3@\pgfplotstable@real@colname\endcsname\to\pgfplotstable@entry
					\expandafter\let\csname pgfplotstablecreate@cur@\pgfplotstable@colname\endcsname=\pgfplotstable@entry
				\fi
			\else
				\expandafter\let\expandafter\pgfplotstable@prev\csname pgfplotstablecreate@cur@\pgfplotstable@colname\endcsname
				\expandafter\let\csname pgfplotstablecreate@prev@\pgfplotstable@colname\endcsname=\pgfplotstable@prev
				%
				\expandafter\let\expandafter\pgfplotstable@next\csname pgfplotstablecreate@next@\pgfplotstable@colname\endcsname
				\expandafter\let\csname pgfplotstablecreate@cur@\pgfplotstable@colname\endcsname=\pgfplotstable@next
			\fi
			\expandafter\pgfplotslistcheckempty\csname\string#3@\pgfplotstable@real@colname\endcsname
			\ifpgfplotslistempty
				\expandafter\let\csname pgfplotstablecreate@next@\pgfplotstable@colname\endcsname=\pgfutil@empty
				\pgfplotstable@islastrowtrue
			\else
				\expandafter\pgfplotslistpopfront\csname\string#3@\pgfplotstable@real@colname\endcsname\to\pgfplotstable@entry
				\expandafter\let\csname pgfplotstablecreate@next@\pgfplotstable@colname\endcsname=\pgfplotstable@entry
			\fi
		}%
		\ifpgfplots@loop@CONTINUE
			% Compute content:
			%
			\begingroup
			\ifpgfplotstable@isfirstrow
				\pgfkeysvalueof{/pgfplots/table/create col/assign first/.@cmd}\pgfeov
			\else
				\ifpgfplotstable@islastrow
					\pgfkeysvalueof{/pgfplots/table/create col/assign last/.@cmd}\pgfeov
				\else
					\pgfkeysvalueof{/pgfplots/table/create col/assign/.@cmd}\pgfeov
				\fi
			\fi
			\pgfkeysgetvalue{/pgfplots/table/create col/next content}{\pgfplotstable@entry}%
			\t@pgfplots@toka=\expandafter{\pgfplotstable@entry}%
			\t@pgfplots@tokb=\expandafter{\pgfmathaccuma}%
			\xdef\pgfplots@glob@TMPc{%
				\noexpand\def\noexpand\pgfplotstable@entry{\the\t@pgfplots@toka}%
				\noexpand\def\noexpand\pgfmathaccuma{\the\t@pgfplots@tokb}%
			}%
			\pgfmath@smuggleone\pgfmathaccumb
			\endgroup
			\pgfplots@glob@TMPc
			\expandafter\pgfplotslistpushback\expandafter{\pgfplotstable@entry}\to\pgfplotstable@newcol
			%
			\ifpgfplotstable@islastrow
				\pgfplots@loop@CONTINUEfalse
			\fi
		\fi
		\pgfplotstable@isfirstrowfalse
		\advance\c@pgfplotstable@rowindex by1\relax
	\pgfutil@repeat
	\global\let\pgfplots@glob@TMPc=\pgfplotstable@newcol
	\global\let\pgfplots@glob@TMPb=\pgfplotstable@newcolname
	\endgroup
	\ifpgfplotstablecreatecol@isreallynew
		\expandafter\pgfplotslistpushback\expandafter{\pgfplots@glob@TMPb}\to#3
	\fi
	\expandafter\let\csname\string#3@\pgfplots@glob@TMPb\endcsname=\pgfplots@glob@TMPc
}%

\endinput


==> pgfplotstable.coltype.code.tex <==
%--------------------------------------------
%
% Package numtable.
%
% This file provides support for column types in LaTeX tabular
% environments, i.e.
%
%\begin{tabular}{>{\pgfplotstablecoltype}c<{\endpgfplotstablecoltype}}
%	1 \\
%	2 \\
%	3 \\
%\end{tabular}
%
%
%
% Copyright 2007/2008 by Christian Feuersänger.
%
% This program is free software: you can redistribute it and/or modify
% it under the terms of the GNU General Public License as published by
% the Free Software Foundation, either version 3 of the License, or
% (at your option) any later version.
% 
% This program is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
% GNU General Public License for more details.
% 
% You should have received a copy of the GNU General Public License
% along with this program.  If not, see <http://www.gnu.org/licenses/>.
%
%--------------------------------------------



% If I did not get it wrong, the tabular package, initialised with a
% column type like
% >{\pgfplotstablecoltype}c<{\endpgfplotstablecoltype}
% yields
%
% \pgfplotstablecoltype \ignorespaces <content> \unskip \endpgfplotstablecoltype
% OR
% \pgfplotstablecoltype \ignorespaces <content> \\ \endpgfplotstablecoltype
%
% So, I define \pgfplotstablecoltype to skip \ignorespaces and \unskip and simply
% get <content>.
\def\pgfplotstablecoltype{%
	\begingroup
	\let\pgfplotstablecoltype@content=\empty
	\pgfutil@ifnextchar[{%
		\pgfplotstablecoltype@
	}{%
		\pgfplotstablecoltype@until@end@start
	}%
}%
\def\pgfplotstablecoltype@[#1]{%
	\pgfqkeys{/pgf/number format}{#1}%
	\pgfplotstablecoltype@until@end@start
}%

\def\pgfplotstablecoltype@until@end@start\ignorespaces{%
	\pgfplotstablecoltype@until@end
}%
\def\pgfplotstablecoltype@until@end{%
	\pgfutil@ifnextchar\\{%
		\pgfplotstablecoltype@finish%
	}{%
		\pgfutil@ifnextchar{\unskip}{%
			\pgfplotstablecoltype@finish%
		}{%
			\pgfplotstablecoltype@next
		}%
	}%
}
\def\pgfplotstablecoltype@next#1{%
	\expandafter\def\expandafter\pgfplotstablecoltype@content\expandafter{\pgfplotstablecoltype@content#1}%
	\pgfplotstablecoltype@until@end
}
\def\pgfplotstablecoltype@finish{%
%\message{COLLECTED \meaning\pgfplotstablecoltype@content}%
	\pgfmathprintnumber{\pgfplotstablecoltype@content}%
	\endgroup
}%

%\def\pgfplotstablecoltype{\message{COLLECT}}%
\def\endpgfplotstablecoltype{}%


==> pgfplotsutil.code.tex <==
%--------------------------------------------
%
% Package pgfplots
%
% Provides a user-friendly interface to create function plots (normal
% plots, semi-logplots and double-logplots).
% 
% It is based on Till Tantau's PGF package.
%
% Copyright 2007/2008 by Christian Feuersänger.
%
% This program is free software: you can redistribute it and/or modify
% it under the terms of the GNU General Public License as published by
% the Free Software Foundation, either version 3 of the License, or
% (at your option) any later version.
% 
% This program is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
% GNU General Public License for more details.
% 
% You should have received a copy of the GNU General Public License
% along with this program.  If not, see <http://www.gnu.org/licenses/>.
%
%--------------------------------------------

\def\pgfplots@EOI{\pgfplots@EOI}%

\newtoks\t@pgfplots@toka
\newtoks\t@pgfplots@tokb
\newtoks\t@pgfplots@tokc
\newdimen\pgfplots@tmpa

% use these macros for GLOBAL temporary assignments.
% you can NEVER rely on their values unless you know exactly what you are doing.
\gdef\pgfplots@glob@TMPa{}%
\gdef\pgfplots@glob@TMPb{}%
\gdef\pgfplots@glob@TMPc{}%

% use these macros for LOCAL temporary assigments.
% you can NEVER rely on their values unless you know exactly what you are doing.
\def\pgfplots@loc@TMPa{}%
\def\pgfplots@loc@TMPb{}%
\def\pgfplots@loc@TMPc{}%

\input pgfplotsliststructure.code.tex
\input pgfplotsliststructureext.code.tex
\input pgfplotsarray.code.tex
\input pgfplotstable.code.tex

% Produces an \aftergroup statement for each single token in #1.
%
% ATTENTION: you *can't* use braces inside of '#1'!
\def\pgfplotsqaftergroupeach#1{%
	\pgfplotsqaftergroupeach@#1\pgfplots@EOI
}
\def\pgfplotsqaftergroupeach@#1{%
	\gdef\pgfplots@TMP{#1}%
	\ifx\pgfplots@TMP\pgfplots@EOI
	\else
		\aftergroup#1%
		\expandafter\pgfplotsqaftergroupeach@
	\fi
}

\def\pgfplotsaftergroupcollectinto#1#2\pgfplots@EOI{%
	\def#1{#2}%
}%

% Assigns list contents #2 to a list macro #1.
%
% The list contents may be provided in one of two formats:
% a) in the (deprecated) list format 'first\\second\\thirst\\'
% or
% b) in the PGF foreach list format 'first,second,third'.
\def\pgfplots@assign@list#1#2{%
	\def\pgfplots@TMP{#2}%
	\ifx\pgfplots@TMP\pgfutil@empty
		\pgfplotslistnewempty#1%
	\else
		\pgfplots@check@backwards@compatible@list@format #2\\\pgfplots@EOI
		\ifpgfplots@is@old@list@format
			\pgfplotslistnew#1{#2}%
		\else
			\pgfplots@foreach@to@list{#2}\to#1
		\fi
	\fi
}%

% Sets the boolean \ifpgfplots@is@old@list@format  to true if and only
% if the input is a list in the format '{first\\second\\}'.
%
% This format is deprecated, but is still provided for backwards
% compatibility.
%
% Usage:
% \pgfplots@check@backwards@compatible@list@format <argument>'\\'\pgfplots@EOI
% you NEED to append '\\\pgfplots@EOI' at the end.
\def\pgfplots@check@backwards@compatible@list@format#1\\#2\pgfplots@EOI{%
	\def\pgfplots@TMP{#2}%
	\ifx\pgfplots@TMP\pgfutil@empty
		\pgfplots@is@old@list@formatfalse
	\else
		\pgfplots@is@old@list@formattrue
	\fi
}%

\def\pgfplots@error#1{\PackageError{pgfplots}{#1}{}}%
\def\pgfplots@warning#1{\pgfplots@message{! Package pgfplots Warning: #1}}%
\def\pgfplots@message#1{%
	\immediate\write16{#1}%
}%
\def\pgfplots@assert@tikzinternal@exists#1{%
	\pgfutil@ifundefined{#1}{%
		\pgfplots@error{Sorry, pgfplots relies on the existance of the tikz internal macro '#1'.
		 Unfortunately, this does no longer exist ... you will need to get an updated version of pgfplots to fix this problem.}%
		\expandafter\let\csname #1\endcsname=\pgfutil@empty
	}{}%
}%


% A future-version compatibility method which checks whether the
% macro '#2' exists.
%
% We assume that '#2' usually contains the value of the tikz key '#1'.
% Example:
% /tikz/variable is usually stored into '\tikz@plot@var'.
%
% However, this may change in future versions.
%
% So, we do the following:
% 1. check whether '#2' exists, if yet: ok.
% 2. if not, check whether the value is stored directly into '/tikz/#1'.
% 3. if not, check whether the value is stored directly into '/pgf/#1'.
% 4. If everything fails, provide an error message.
%
% #1: a tikz key without key prefix (/tikz/ and /pgf/ will be prepended).
% #2: a macro name WITHOUT backslash.
% #3: the default value if everything fails.
\def\pgfplots@gettikzinternal@keyval#1#2#3{%
	\pgfutil@ifundefined{#2}{%
		\pgfkeysifdefined{/tikz/#1}{%
			\pgfkeysgetvalue{/tikz/#1}\pgfplots@TMP
			\expandafter\let\csname #1\endcsname=\pgfplots@TMP
		}{%
			\pgfkeysifdefined{/pgf/#1}{%
				\pgfkeysgetvalue{/pgf/#1}\pgfplots@TMP
				\expandafter\let\csname #1\endcsname=\pgfplots@TMP
			}{%
				\expandafter\def\csname #1\endcsname{#3}%
				{\t@pgfplots@tokc={#3}%
				\pgfplots@warning{Sorry, could not find value of '/tikz/#1'. Assuming '\the\t@pgfplots@tokc'.}%
				}%
			}%
		}%
	}{}%
}%

\def\pgfplots@getcurrent@plothandler#1{%
	\pgfutil@ifundefined{tikz@plot@handler}{%
		\pgfplots@error{Sorry, can't get the current plot handler. It appears that tikz and pgfplots is no longer compatible!? You will need to get a newer version of pgfplots.}%
		\let#1=\pgfplothandlerlineto
	}{%
		\let#1=\tikz@plot@handler
	}%
}%


% Converts an arbitrary command to a string in which all characters
% have category 12.
%
% #1: a macro name (which takes no arguments)
% #2: a macro name which will be assigned to '#1' converted to string.
%
% This uses '\meaning#1' hackery.
\def\pgfplots@command@to@string#1#2{%
	\expandafter\pgfplots@command@to@string@@\meaning#1\pgfplots@EOI{#2}%
}%
{
\let\CATCODE=\catcode
\CATCODE`\:=12
\CATCODE`\-=12
\CATCODE`\>=12
\CATCODE`\m=12
\CATCODE`\a=12
\CATCODE`\c=12
\CATCODE`\r=12
\CATCODE`\o=12
\xdef\pgfplts@glb@TMP{macro:->}%
}
\expandafter\def\expandafter\pgfplots@command@to@string@@\pgfplts@glb@TMP#1\pgfplots@EOI#2{%
	\def#2{#1}%
}%

% Usage:
% \pgfplots@if{pgfplots@scaled@ticks}{true-code}{false-code}
%
% it is to be used if the tex boolean is only known as string, not as
% macro.
\def\pgfplots@if#1#2#3{%
	\csname if#1\endcsname
		#2%
	\else
		#3%
	\fi
}%


==> summary.tex <==
{
%\ssp
%\smallssp
Chapter~1 gives a brief history of the field of holography along with an overview of this thesis.  A more detailed description of holography is provided in Chapter~2 along with a discussion of digital holography.  Chapter~3 examines the design of a one-step monochromatic hologram printer capable producing white-light viewable transmission holograms created with the aid of an LCOS display system and printed in a dot-matrix sequence. The lens system employed includes a microlens array and an afocal relay telescope which are both quantitatively examined in order to maximise the contrast, diffraction efficiency and depth of view of the final hologram image. A brief overview of speckle reduction techniques and their applicability to pulsed digital holography is presented along with experimental results of the use of a microlens array to reduce speckle effects. Chapter~4 presents an analysis of the unwanted side effects of the angular intensity distribution of a hologram pixel, using a case study for analysis. Chapter~5 examines methods for increasing both the printing speed and resolution of the hologram printer.  Chapter~6 describes the analysis and design of a temperature-energy feedback system to correct for pulsed laser instabilities arising from mode beating due to temperature variations. Chapter~7 provides a conclusion to the work and discusses possible future developments.
}

==> t-pgfplotstable.tex <==
%--------------------------------------------
%
% Package pgfplotstable
%
% It is based on Till Tantau's PGF package.
%
% Copyright 2007/2008 by Christian Feuersänger.
%
% This program is free software: you can redistribute it and/or modify
% it under the terms of the GNU General Public License as published by
% the Free Software Foundation, either version 3 of the License, or
% (at your option) any later version.
% 
% This program is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
% GNU General Public License for more details.
% 
% You should have received a copy of the GNU General Public License
% along with this program.  If not, see <http://www.gnu.org/licenses/>.
%
%--------------------------------------------

\usemodule[pgfplots]

\endinput

